Worst-Case Complexity of an SQP Method for Nonlinear Equality Constrained Stochastic Optimization

A worst-case complexity bound is proved for a sequential quadratic optimization (commonly known as SQP) algorithm that has been designed for solving optimization problems involving a stochastic objective function and deterministic nonlinear equality constraints. Barring additional terms that arise due to the adaptivity of the monotonically nonincreasing merit parameter sequence, the proved complexity bound is comparable to that known for the stochastic gradient algorithm for unconstrained nonconvex optimization. The overall complexity bound, which accounts for the adaptivity of the merit parameter sequence, shows that a result comparable to the unconstrained setting (with additional logarithmic factors) holds with high probability.

==> archived_versions/2021-08-06/abstract.tex <==
We prove a complexity result for the deterministic Sequential Quadratic Programming (SQP) methods developed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

==> archived_versions/2021-08-06/body.tex <==
%******************************************
% Paper-dependent macros here
%******************************************
\newcommand{\flow}{f_{\text{\rm low}}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\kappadec}{\kappa_{\text{\rm dec}}}
\newcommand{\bK}{\bar{K}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\btau}{\bar{\tau}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bg}{\bar{g}}
\newcommand{\bxi}{\bar{\xi}}

\newcommand{\xiktri}{\xi_k^{\rm trial}}
\newcommand{\ktaudec}{\kappa_{\tau_{\rm dec}}}
\newcommand{\kmax}{k_{\max}}
\newcommand{\smax}{s_{\max}}

\newcommand{\dktrue}{d_k^{\text{\rm true}}}
\newcommand{\uktrue}{u_k^{\text{\rm true}}}
\newcommand{\wktrue}{w_k^{\text{\rm true}}}
\newcommand{\yktrue}{y_k^{\text{\rm true}}}
\newcommand{\tktritrue}{\tau_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Dktrue}{D_k^{\text{\rm true}}}

\newcommand{\strue}{s^{\text{\rm true}}}

\newcommand{\Lbad}{\Lcal_{\text{\rm bad}}}
\newcommand{\Lgood}{\Lcal_{\text{\rm good}}}
\newcommand{\Ebad}{E_{\text{\rm bad}}}
\newcommand{\Cdec}{C_{\text{\rm dec}}}
\newcommand{\Idec}{\Ical_{\text{\rm dec}}}


\def\Ek#1{E_{k,#1}}
\def\tred#1{\textcolor{red}{#1}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%*********
% Section
%*********

%\newtheorem{assumption}{Assumption}

%\def\proof{\par{\it Proof}. \ignorespaces}
%\def\endproof{{\ \vbox{\hrule\hbox{%
% \vrule height1.3ex\hskip0.8ex\vrule}\hrule
%}}\par}
%\def\noprint#1{}

\section{Introduction} \label{sec:intro}

We consider the design and analysis of algorithms for minimizing smooth, nonlinear functions which are subject to equality constraints. Problems of this form arise in various important applications throughout science and engineering, including optimal control, PDE-constrained optimization and resource allocation \cite{DPBertsekas_1998,JTBetts_2010,FSKupfer_EWSachs_1992,TRees_HSDollar_AJWathen_2010}. Unlike the vast majority of the literature on equality constrained optimization, we assume that our objective functions is stochastic, in the sense that the objective is the expected value of a function defined with respect to a random variable with an unknown distribution. We assume that the computation of the objective function and its gradient is intractable, but we have access to (unbiased) stochastic gradient estimates.

Recently, a number of algorithms have been proposed for this class of problems. These approaches fall essentially into two regimes: penalty based methods \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018} and sequential quadratic programming (SQP) methods \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}. Penalty methods attempt to solve this problem by adding an additional term to the objective function, weighted by a penalty parameter, which penalizes constraint violation. Unconstrained optimization techniques are then applied to approximately solve a sequence of penalized subproblems. Methods of this type can perform poorly due to ill-conditioning or nonsmoothness of the penalized subproblems, depending on the type of penalty function used. This methodology also often suffers due to sensitivity to the scheme used for updating the penalty parameter. In addition to these practical issues, little theoretical guarantees are known for the stochastic penalty methods proposed in \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018}.

In practice, penalty methods are frequently outperformed by SQP based methods. It is commonly accepted in deterministic optimization that one of the state-of-the-art algorithms is an SQP method that chooses stepsizes based on a line search applied to a merit function. In addition, for deterministic optimization with equality constraints, these algorithms are intimately connected to applying Newton's method to the stationarity conditions of the problem \cite{RBWilson_1963}.  In this work, we develop an algorithm based off of the SQP method proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Our algorithm employs a dynamic step-size rule, single or small stochastic gradient batches, and an adaptive merit function. We prove that, with high-probability, the number of iterations, $k$, until our SQP method generates a point at which approximate optimality conditions hold in expectation is $\mathcal{O}(k^{-4})$. This is the first known worst-case complexity result for a stochastic method with an adaptive merit function for equality constrained optimization. Our result effectively matches the worst-case complexity of stochastic gradient methods with projections for simple constraints \cite{DDavis_DDrusvyatskiy_2019}. Prior to this work, the only known complexity results for stochastic constrained optimization were for problems with simple constraints that enable projection based methods \cite{DDavis_DDrusvyatskiy_2019,SGhadimi_GLan_HZhang_2016} and Frank-Wolfe type methods to be tractable \cite{EHazan_HLuo_2016} \footnote{MO: Technically, one of Mihai's algorithms has a complexity result, but it requires a-priori knowledge of the merit parameter (aka non-adaptive, set and forget). Should I change this sentence or just mention this later?}. Unfortunately, these approaches do not apply to equality constrained optimization.

Formally, we study the optimization problem
\bequation \label{eq:fdef}
    \underset{x \in \R{n}}{\min} f(x) \; \mbox{s.t.} \; c(x) = 0, \; \; \mbox{with} \; \; f(x) = \E[F(x,\omega)],
\eequation
where $f : \R{n} \rightarrow \R{}$, $c : \R{n} \rightarrow \R{m}$, $\omega$ is a random variable with associated probability space $(\Omega,\mathcal{F}, P)$, $F : \R{n} \times \Omega \rightarrow \R{}$, and $\E$ represents the expectation taken with respect to $P$. We presume that one has access to values of the constraint function and its derivatives, but it is intractable to evaluate the objective and/or its derivatives.

The major technical hurdle in proving a complexity result for stochastic SQP methods arises from their use of an adaptive merit function. Merit functions are a commonly used tools in deterministic constrained optimization, as they provide a way to assess the quality of a step in terms of two (often competing) goals: minimizing the objective function $f$ and reducing the constraint violation in $c$. In our algorithm, we use the $\ell$-1 norm penalty  function $\phi : \R{n} \times \R{}_{>0}$ defined by,
\bequation \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1.
\eequation
Here, $\tau \in \R{}_{>0}$ is the merit parameter which, in our algorithm, is a positive non-increasing sequence $\{\tau_k\}$ that is adaptively chosen at each iteration $k$. The updating behavior of $\tau$ is the core difficulty in providing a complexity result, as the function being optimized at each iteration is modified based on stochastic information. Given that our algorithm uses only a single stochastic gradient at each iteration, the updates to $\tau$ may be based on very poor approximations to the true gradient, causing erratic behavior. We note that even when the sequence $\{\tau_k\}$ is deterministically lower bounded, such as when the noise is deterministically bounded, the complexity analysis is non-trivial as the number of iterations until the sequence $\{\tau_k\}$ settles near its lower bound is itself a random process. The behavior of $\tau$ is difficult to characterize, so previous analyses rely on ``fast-forwarding" to an iterate at which the merit parameter remains constant, greatly simplifying the theoretical challenges \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}. This strategy is not possible when a complexity result is desired however, as the behavior of the full iterate sequence must be analyzed instead.

We wish to stress here that while our techniques are developed for an SQP method which uses the merit function in \eqref{eq:phidef}, they may be applicable to a wide variety of algorithmic frameworks for stochastic optimization with deterministic constraints. The approaches used can be modified to apply to methods which adaptively update critical parameters at each iteration, such as adaptive penalty methods \cite{RHByrd_GLopez-Calva_JNocedal_2012,RHByrd_JNocedal_RAWaltz,MMongeau_ASartenaer_1995}, adaptive augmented Lagrangian \cite{FECurtis_HJiang_DPRobinson_2015}, adaptive barrier methods \cite{JNocedal_AWachter_RAWaltz_2009}, and penalty-interior point methods \cite{FECurtis_2012}. In addition, many constrained algorithms generate repeated (often unconstrained) subproblems defined by an auxilliary parameter sequence which is updated dynamically based off of the solution to the previous subproblem. Algorithms of this type include penalty methods, augmented Lagrangian methods, and interior point methods \cite{JNocedal_SJWright_2006}. In the case where the objective is stochastic, this auxilliary sequence would also be a random variable, the behavior of which would be paramount to proving a complexity result for this type of method. Thus, we believe that the techniques we derive for our SQP method are broadly applicable and foundational for performing a  complexity analysis of deterministically constrained stochastic optimization methods.

We note here that other stochastic SQP methods have been proposed in the literature \cite{SNa_MAnitescu_KMladen_2021}. These methods are either non-adaptive, in the sense that the merit parameter must be fixed a-priori, or require high-accuracy gradient estimates at each iteration. Due to this, we focus on the algorithmic framework developed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

\subsection{Outline of Complexity Result} \label{subsec:complexitypreview}

In this section, we provide a sketch of our complexity result and describe how it compares to other results in the literature. Our result is proved under relatively common smoothness conditions on $f$ and $c$ as well as the linear independence constraint qualification (LICQ). We assume that, conditioned on some event $E$, the stochastic gradients are unbiased estimators of $\nabla f(x)$ with variance bounded by $M$, as is standard in the literature. Additionally, we assume that the stochastic gradients exhibit a bounded measure of asymmetry, the merit parameter sequence $\{\tau_k\}$ is lower bounded by some $\tau_{\min} > 0$, and the number of iterations at which $\tau_k$ is decreased is bounded by a positive integer $s_{\max}$ (this last condition is gauranteed by the definition of our algorithm under the rest of the assumptions). These last three assumptions are required to ensure that the merit function is well behaved with high probability, even though it is being updated based on stochastic gradient information. Exact definitions of these assumptions can be found in Section \ref{subsec:assumptions}.

Under the conditions listed above, after performing $k_{\max}+1$ iterations, our algorithm generates a point $x_{k^*}$ which satisfies, with probability at least $1-\delta$,
\bequation \label{eq:bigOcomplexity}
    \begin{split}
   \E[\|\nabla f(x_{k^*}) &+ J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c(x_{k^*})\| |
    E] \\
   &= \mathcal{O}\left(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c(x_0)\|_1 + M + (\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\right),
   \end{split}
\eequation
where $J_{k^*}$ is the Jacobian of the constraints at the point $x_{k^*}$, $y_{k^*}^{true}$ is the Lagrange multiplier at $x_{k^*}$, and $f_{\min}$ is a lower bound on $f(x)$.

The form of this result is commonly referred to as a convergence rate, however it can be easily manipulated into a worst-case complexity result. In terms of finding a point, $x_{k^*}$, such that $\E[\| \nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\| |E] \leq \varepsilon$ and $\E[\sqrt{\|c(x_{k^*})\|}|E] \leq \varepsilon$, by Jensen's inequality, our algorithm requires at most $\Ocal(\varepsilon^{-4})$ iterations.
As such, we use the terms complexity and convergence rate interchangably throughout.

The first three quantities in this result are essentially the same as those for the stochastic gradient method, representing the initial function gap as well as the variance. This is to be expected, given our mild assumptions on the matrices used in the quadratic subproblem at each iteration as well as the use of a single stochastic gradient at each iteration.

The final two terms are unique to our setting and arise due to the having a potentially poor initial estimate of $\tau_{\min}$. Given oracle knowledge of $\tau_{\min}$, these last two terms could be removed by choosing $\tau_{-1} \leq \tau_{\min}$ (as is done in the non-adaptive algorithm of \cite{SNa_MAnitescu_KMladen_2021}). However, this quantity is unknown so careful attention must be paid to the behaivor of the $\{\tau_k\}$ sequence to obtain a complexity result. The result holds in high probability due to the possibility of having an excessive number of iterations at which the computed $\tau_k$ is significantly larger than the value that the merit parameter would take if the step direction and merit parameter update were computed using the full gradient. On these types of iterations, the requirement for a bounded measure of asymmetry in the distribution of the stochastic gradients guarantees that there is always some nonzero probability of decreasing $\tau$. However, there still may exist realizations (which are guaranteed to occur with probability no more than $\delta$), where $\tau$ is ``too large" for enough iterations that the above complexity result does not hold.

We note that in terms of an overall complexity result with respect to the gradient of the Lagrangian, with probability at least $1-\delta$, we obtain a result which is the same order as the complexity result derived in \cite{DDavis_DDrusvyatskiy_2019}, whenever $s_{\max}$ satisfies a reasonable bound. Due to the definition of our algorithm, $s_{\max} = \mathcal{O}(\log(\tau_{\min}))$ for all sufficiently large $k_{\max}$. Thus, it follows that this complexity result gives an informative bound whenever $\tau_{\min}$ does not grow exponentially in $k_{\max}$. We prove that this is the case for sub-Gaussian distributions in Section \ref{subsec:subgauss}, where we show that, with probability at least $1-\delta$, $\tau_{\min} = \mathcal{O}(\log(\frac{k_{\max}}{\delta}))$ and
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O}\left(\frac{\log \log \frac{k_{\max}}{\delta}}{\sqrt{k_{\max}+1}}\right).
\eequationNN

\subsection{Notation}

Our algorithm is iterative, generating a sequence of iterates $\{x_k\}$. We also append the iteration number to other quantities corresponding to each iteration, e.g., $f_k := f(x_k)$. We denote the Jacobian of $c$ by $J_k := \nabla c(x_k)^\top$.

We adopt the notation that $\|\cdot\|$ is the $\ell$-2 norm for vectors and is the induced $\ell$-2 norm for matrices. We denote by $\mathbb{S}^{n}$ the set of $n \times n$ dimensional symmetric matrices. The set of natural numbers is denoted as $\N{} := \{0,1,2,\dots,\}$.

When discussing stochastic quantities, we use capital letters to denote the random variable and lower case letters to denote a realization of that random variable. For example, for the stochastic gradients at iteration $k$, $G_k$ denotes the random variable while $g_k$ is a realization of this random variable.

\subsection{Outline}

In the following section, we give an overview of the sequential quadratic programming framework and describe our algorithm. In Section \ref{sec:complexity}, we describe our assumptions on the stochastic gradients and prove our complexity result. We also provide examples of distributions under which our assumptions hold with high-probability. Finally, we provide some concluding thoughts and future directions in Section \ref{sec:conclusion}.

\section{Algorithm}

We make the following assumption about the optimization problem \eqref{eq:fdef} and the algorithm that we analyze, which generates a sequence of iterates $\{x_k\} \subset \R{n}$.

\begin{assumption} \label{assum:fcsmooth}
    There exists a convex set $\mathcal{X} \subseteq \R{n}$ that contains the iterates $\{x_k\}$ for any realization of Algorithm \ref{alg:ssqp}. The objective function $f : \R{n} \rightarrow \R{}$ is continuously differentiable and bounded below over $\mathcal{X}$, and its gradient $\nabla f: \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $L$ and is bounded over $\mathcal{X}$. The constraint function $c : \R{n} \rightarrow \R{m}$ (where $m \leq n$) and its Jacobian $\nabla c^\top : \R{n} \rightarrow \R{m\times n}$ are bounded over $\mathcal{X}$, each gradient $\nabla c_i : \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $\gamma_i$ over $\mathcal{X}$ for all $i=\{1,\dots,m\}$, and the singular values of $\nabla c^\top$ are bounded away from zero over $\mathcal{X}$.
\end{assumption}

This assumption is largely standard smoothness requirements. However, requiring that the iterates remain in a convex set over which the gradient of $f$ and Jacobian of $c$ are bounded is a stronger assumption than those commonly made for unconstrained stochastic gradient methods. Indeed, even if $f$ has bounded level sets, there is no guarantee that the iterates will remain in any specific level set, as stochastic gradient methods are not descent methods. However, we believe that this is a more reasonable assumption due to the inclusion of constraints, which drive the iterates towards the {\it deterministic} constrained region. Finally, we note that the requirement on the Jacobian of $c$ to have singular values which are bounded away from zero holds for any constraint set that satisfies LICQ.

Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) := f(x) + c(x)^\top y$, first-order stationarity conditions for \eqref{eq:fdef}, which are necessary due to LICQ, are given by
\bequation \label{eq:optconds}
    0 =
    \left[ \begin{matrix}
        \nabla_x \ell(x,y) \\
        \nabla_y \ell(x,y)
    \end{matrix} \right]
    =
    \left[ \begin{matrix}
        \nabla f(x) + \nabla c(x) y \\
        c(x)
    \end{matrix} \right].
\eequation
As seen in \eqref{eq:bigOcomplexity}, our goal in this work is to prove a bound on the number of iterations required to find an approximate solution in terms of the gradient of the Lagrangian and the constraint violation.

\subsection{Merit Function}

In Section \ref{sec:intro}, we introduced our $\ell$-1 penalty merit function in \eqref{eq:phidef}. The merit parameter $\tau$ is adaptively updated at each iteration and is used to define our line search procedure. We use a local model of the merit function $q : \R{n} \times \R{}_{>0} \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A key quantity in our algorithm is the reduction in the model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\Delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation} \label{eq:deltadef}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}
The reduction in the model of the merit function is a critical component of our complexity analysis. We will show that this can be used to give an upper bound on the merit function decrease at each iteration and thus it plays a similar role to the norm of the gradient squared in the analysis of stochastic gradient methods.

\subsection{Algorithm Preliminaries}

The algorithm that we develop for solving \eqref{eq:fdef} is based on a stochastic SQP paradigm. Specifically, at iteration $k$, a stochastic gradient estimate, $g_k$, is obtained (assumptions on the properties of $g_k$ can be found in Section \ref{subsec:assumptions}). Then, a search direction is computed by solving a quadratic optimization subproblem based on a stochastic local quadratic model of $f$ and a local affine model of $c$ about $x_k$. Letting $f_k := f(x_k)$, $c_k = c(x_k)$, and $J_k := \nabla c(x_k)^\top$ and given a sequence $\{H_k\}$ satisfying Assumption \ref{assum:Hk} below (a standard type of sufficiency condition for equality constrained optimization), this subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}

The optimal solution, $d_k$, of this subproblem, and an associated Lagrange multiplier, $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}


\begin{assumption} \label{assum:Hk}
    The sequence $\{H_k\}$ is bounded in norm by $\kappa_H \in \R{}_{>0}$. In addition, there exists a constant $\zeta \in \R{}_{>0}$ such that, for all $k = \{0,\dots,k_{\max}\}$, the matrix $H_k$ has the property $u^\top H_k u \geq \zeta \|u\|_2^2$ for all $u \in \R{n}$ such that $J_k u = 0$.
\end{assumption}

We stress that our algorithm and analysis does {\it not} assume that $H_k$ is a stochastic approximation of the Hessian of the Lagriangian at $x_k$ for some multiplier $y_k$. We merely assume that the sequence $\{H_k\}$ satisfies Assumption \ref{assum:Hk}.

Under Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk}, the following result is well known in the literature.

\blemma
    The linear system \eqref{eq:sqpsystem} has a unique solution.
\elemma

\subsection{Algorithm}

\begin{algorithm}[ht]
  \caption{Stochastic SQP Algorithm}
  \label{alg:ssqp}
  \begin{algorithmic}[1]
    \Require $x_0 \in \R{n}$; $\tau_{-1} \in \R{}_{>0}$; $\epsilon \in (0,1)$; $\sigma \in (0,1)$; $\xi_{-1} \in \R{}_{>0}$; $\kmax \in \N{}$; $\{\beta_k\} \subset (0,1]$; $\theta \in \R{}_{\geq0}$; $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$
    \For{\textbf{all} $k \in \{0,1,\dotsc,\kmax\}$}
	  \State Compute $(d_k,y_k)$ as the solution of \eqref{eq:sqpsystem}
	  \If{$d_k = 0$}
	    \State Set $\tau_k^{trial} \gets \infty$, $\tau_k \gets \tau_{k-1}$, $\xi_k^{trial} \gets \infty$, and $\xi_k \gets \xi_{k-1}$
	    \State Set $\widehat\alpha_{k,\text{init}} \gets 1$, $\widetilde\alpha_{k,\text{init}} \gets 1$, and $\alpha_k \leftarrow 1$
	  \Else\ (if $d_k \neq 0$)
	    \State Set $\tau_k^{trial}$ by \eqref{eq:tautrial} and $\tau_k$ by \eqref{eq:taudef} %\label{step.tau_stochastic}
	    \State Set $\xi_k^{trial}$  and $\xi_k$ by \eqref{eq:xidef} %\label{step.xi}
        \State Set
        \bequationNN
          \widehat\alpha_{k,\text{init}} \gets \tfrac{\beta_k\Delta q(x_k,\tau_k,g_k,H_k,d_k)}{(\tau_k L_k + \Gamma_k)\|d_k\|_2^2}\ \ \text{and}\ \  \widetilde\alpha_{k,\text{init}} \gets \widehat\alpha_{k,\text{init}} - \tfrac{4\|c_k\|_1}{(\tau_k L_k +  \Gamma_k)\|d_k\|_2^2}
        \eequationNN
        \State Set $\widehat\alpha_k \gets \proj_k(\widehat\alpha_{k,\text{init}})$ and $\widetilde\alpha_k \gets \proj_k(\widetilde\alpha_{k,\text{init}})$, then \label{step.alpha_projection_stochastic} \label{step.alpha_stochastic}
        \bequationNN
          \alpha_k \gets
		    \bcases
		      \widehat\alpha_k & \text{if $\widehat\alpha_k < 1$} \\
		      1 & \text{if $\widetilde\alpha_k \leq 1 \leq \widehat\alpha_k$} \\
		      \widetilde\alpha_k & \text{if $\widetilde\alpha_k > 1$}
		    \ecases
        \eequationNN
      \EndIf
      \State Set $x_{k+1} \gets x_k + \alpha_k d_k$
    \EndFor
    \State Sample $k^* \in \{0, \dotsc, \kmax\}$ according to the probability distribution
    \bequationNN
        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
    \eequationNN
    \Return $x_{k^*}$
  \end{algorithmic}
\end{algorithm}

After the search direction $d_k$ is computed, the merit parameter $\tau_k$ is updated. This is done by first setting, for some $\sigma \in (0,1)$, a trial value $\tau_k^{trial} \in \R{}_{>0} \cup  \{\infty\}$ by 
\bequation \label{eq:tautrial}
    \tau_k^{trial}\gets
    \begin{cases}
        \infty & \mbox{if $g_k^\top d_k + \max\{d_k^\top H_k d_k, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{g_k^\top d_k + \max\{d_k^\top H_k d_k,0\}} & \mbox{otherwise,}
    \end{cases}
\eequation
(If $c_k = 0$, then it follows from \eqref{eq:sqpsystem} and Assumption \ref{assum:Hk} that $d_k^\top H_k d_k \geq 0$ and $g_k^\top d_k + d_k^\top H_k d_k = 0$, meaning $\tau_k^{trial} \gets \infty$. Hence, $\tau_k^{trial} < \infty$ requires $\|c_k\|_1 > 0$, in which case $\tau_k^{trial} > 0$.) Then, the merit parameter is set, for some $\epsilon \in (0,1)$, by
\bequation \label{eq:taudef}
    \tau_k \gets \bcases
        \tau_{k-1} & \mbox{if $\tau_{k-1} \leq \tau_k^{trial}$} \\
        (1-\epsilon)\tau_k^{trial} & \mbox{otherwise,}
    \ecases
\eequation
which ensures that $\tau_k \leq \tau_k^{trial}$ and,
\bequation \label{eq:qquadlb}
    \Delta q(x_k,\tau,g_k,H_k,d_k) \geq \frac12 \tau \max\{d_k^\top H_k d_k, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
for any $\tau \leq \tau_k$.

Our algorithm adaptively estimates a lower bound for the ratio between the reduction in the model of the merit function and the merit parameter times the squared norm of the search direction. This is used to determine an interval into which the stepsize will be projected; control of this parameter is paramount to ensure convergence in expectation. We set
\bequation \label{eq:xidef}
    \xiktri \gets \frac{\Delta q(x_k, \tau_k, g_k, H_k, d_k)}{\tau_k \|d_k\|^2}
    \; \mbox{ then } \;
    \xi_k \gets \bcases
        \xi_{k-1} & \mbox{if }\xi_{k-1} \leq \xiktri \\
        (1-\epsilon)\xiktri & \mbox{otherwise,}
    \ecases
\eequation
which ensures $\xi_k \leq \xiktri$ for all $kb$. In previous work, it was show that $\{\xi_k\}$ is bounded away from zero {\it deterministically} \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

For generality, Algorithm \ref{alg:ssqp} is stated with Lipschitz constant estimates $\{L_k\}$ and $\{\Gamma_k\}$ given as inputs (with the idea that $\Gamma_k := \sum_{i \in 1,\dots,m} \gamma_{k,i}$ for all $k$). Our analysis in the next section presumes that Lipschitz constants are known, although in practice these can be estimated using standard techniques (see, e.g., \cite{FECurtis_DPRobinson_2019}) in an attempt to ensure that the same convergence results hold for the case where the constants are known. The sequence $\{\beta_k\}$ is introduced to control the setpsizes. Throughout most of the analysis, the sequence $\{\beta_k\}$ can be chosen arbitrarily. However, our final complexity result is established for a fixed step size of $\beta_k = \mathcal{O}(1/\sqrt{k_{\max}+1})$ for all $k\in\{0,\dots,k_{\max}\}$. We define
\bequationNN
    \mbox{Proj}_k(\cdot) := \mbox{Proj}\left(\cdot \; \Bigg| \left[\frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k}, \frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k} + \theta \beta_k^2 \right]\right),
\eequationNN
where $\mbox{Proj}(\cdot \; | \; \mathcal{I})$ represents the projection operator onto the interval $\mathcal{I} \subset \R{}$.

We remark that the only substational changes from Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} are the fixed iteration count, $k_{\max}$, and the inclusion of a return value, $x_{k^*}$. Our method of sampling $k^*$ is consistent with the literature \cite{DDavis_DDrusvyatskiy_2019} and amounts to uniform sampling when a fixed step size sequence is employed.

%\balgorithm
%\caption{A Stochastic SQP Algorithm}
%\label{alg:ssqp}
%    \balgorithmic[1ht!]
%        \Require $x_0 \in \R{n};$ $\bar{\tau}_{-1} \in \R{}_{>0}$; $\epsilon \in (0, 1)$; $\sigma \in (0, 1);$ $\bar{\xi}_{-1} \in \R{}_{>0}$; $\{\beta_k\} \subset \R{}_{>0}$; $\theta \in \R{}_{>0};$ $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$; $K \in \N{}$
%        \State Run Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for $k = 0, \dotsc, K$
%        \State Sample $k^* \in \{0, \dotsc, K\}$ according to the probability distribution
%        \bequationNN
%        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
%        \eequationNN
%        \Return $x_{k^*}$
%    \ealgorithmic
%\ealgorithm

\section{Complexity Analysis} \label{sec:complexity}

In this section, we will prove our complexity result. We begin by describing our algorithm as a random process as well as the assumptions that we make on our stochastic gradient estimates (Section \ref{subsec:assumptions}). Then, we repeat (and sometimes slightly modify) a number of key lemmas from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} about Algorithm \ref{alg:ssqp} (Section \ref{subsec:algprops}). Afterwards, we present our complexity analysis and prove the result previewed in Section \ref{subsec:complexitypreview} (Section \ref{subsec:complexity}). We conclude this section by discussing distributions for which our assumptions are satisfied with high-probability (Section \ref{subsec:subgauss}) and outline a complexity result which relaxes one of our assumptions slightly (Section \ref{subsec:ratioparam}).

Our analysis relies on the orthogonal decomposition of the search directions given by $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$. We note here that conditioned on the algorithm having reached $x_k$ at iteration $k$, the normal component, $v_k$, is {\it deterministic}, depending only on the constraint value $c_k$ and the Jacobian $J_k$.

In addition to the quantities $d_k$, $y_k$, and $\tau_k^{trial}$ which are computed at each iteration using the stochastic gradient $g_k$, the following analysis relies on the quantities $\dktrue$, $\yktrue$, and $\tktritrue$ which are computed using the true gradient, $\nabla f(x_k)$. Specifically, let
\bequation \label{eq:sqpsystemdet}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    \dktrue \\ \yktrue
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    \nabla f(x_k) \\ c_k
    \end{matrix}
    \right]
\eequation
and
\bequationNN
    \tktritrue \gets
    \begin{cases}
        \infty & \mbox{if $\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}} & \mbox{otherwise}.
    \end{cases}
\eequationNN
Finally, we let $\dktrue = \uktrue + v_k$, where $\uktrue \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.

The definition of $\tktritrue$ guarantees that
\bequation \label{eq:qquadlbtrue}
    \Delta q(x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \frac12 \tau \max\{(\dktrue)^\top H_k \dktrue, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
holds for any $\tau \leq \tktritrue$.

\subsection{Algorithm \ref{alg:ssqp} as a Stochastic Process and Assumptions} \label{subsec:assumptions}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(X_k,G_k,D_k,\Tcal_k,S_k,\Xi_k,R_k,\Acal_k)\},
\eequationNN
where
\bitemize
  \item $X_k$ is the algorithm iterate in iteration $k$,
  \item $G_k$ is the stochastic gradient in iteration $k$,
  \item $D_k$ is the search direction in iteration $k$,
  \item $\Tcal_k$ is the merit parameter in iteration $k$,
  \item $S_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\Xi_k$ is the ratio parameter in iteration $k$,
  \item $R_k$ is the number of ratio parameter decreases up to the end of iteration $k$, and
  \item $\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(X_k,G_k,D_k,\Tcal_k, S_k,\Xi_k,R_k,\Acal_k)$ is denoted as
\bequationNN
  (x_k,g_k,d_k,\tau_k,s_k,\xi_k,r_k,\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{G_0,\dots,G_{k-1}\}$, the realization of which (along with $X_0 = x_0$) determines the realization of
\bequationNN
  \{X_j\}_{j=1}^k\ \ \text{and}\ \ \{(D_j,\Tcal_j,S_j,\Xi_j,R_j,\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

We consider a conditional model under the following assumption.

\bassumption\label{assum:eventE}
  Conditioned on the event $E := E(\kmax,s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    %\item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\xi_k = \xi_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E, \Fcal_k] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E, \Fcal_k, \nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \leq \ktaudec.
    \ealigned
  \eequationNN
\eassumption


The requirements on $G_k$ to be an unbiased estimator of $\nabla f(x_k)$ with bounded variance are standard for stochastic gradient methods. However, unlike the unconstrained setting, additional assumptions are required. The assumption on the existence of a $\tau_{\min} > 0$ is similar to Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, under which a global convergence result was proven. In Lemma 2.16 of the same work, it was proven that $\tktritrue$ has a deterministic lower bound. Based on this result, without loss of generality, we assume that $\tktritrue \geq \tau_{\min}$ holds for all $k$. In Proposition 3.18 of the same paper, the authors show that $\tau_{\min}$ exists with probability 1 whenever $G_k$ is a bounded random variable. We extend this result to show that $\tau_{\min}$ exists with high probability when $G_k$ follows a sub-Gaussian distribution in Section \ref{subsec:subgauss}.

By the definition of Algorithm \ref{alg:ssqp}, it should be clear that $s_{\max}$ in Assumption \ref{assum:eventE} must exist. Under the condition that $\tau_{\min} > 0$ exists, it follows that
\bequation \label{eq:smaxbound}
    s_{\max} \leq \min\left\{\kmax+1, \left\lceil\frac{\log(\tau_{\min}/\tau_{-1})}{\log(1-\epsilon)}\right\rceil\right\}.
\eequation
For the purposes of our analysis and results, we keep $s_{\max}$ decoupled from the above inequality as it is a fundamentally necessary component in order to guarantee that our results holds with high probability.

For convenience in the analysis, we make the assumption that the ratio parameter sequence $\{\xi_k\}$ is fixed. This sequence has a deterministic lower bound, as proven in Lemma 3.5 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, unlike the merit parameter sequence. In addition, this sequence is unique to our algorithm (and the algorithm in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}), while merit functions are a commonly used tool in constrained optimization. For this reason, we focus our attention on the properties of the merit parameter sequence instead. The approaches we develop for the merit parameter sequence can be applied to ratio parameter sequence as well. We outline a complexity result where both parameters are adaptively updated in Section \ref{subsec:ratioparam}.

Our final assumption requires that the stochastic gradient estimate is bounded in absolute value when conditioned on the event that $\tau_k < \tau_{k-1}$ and $\nabla f(x_k)^\top (d_k - \dktrue) < 0$ hold simultaneously. This event is fundamental in the analysis, as it arises naturally using $\Delta q(\cdot)$ as a measure of decrease in $\phi$ (see Lemma \ref{lem:phidecrease}). 
We remark that this inequality holds with high-probability whenever $G_k$ follows a sub-Guassian distribution with $\ktaudec = \Ocal(\log (k_{\max}))$. We prove this result in Section \ref{subsec:subgauss}.

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tktritrue$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tktritrue$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tktritrue$ occurs, we introduce the following assumption.

\begin{assumption} \label{assum:ptau}
At every iteration $k \in \{0,\dots,k_{\max}\}$,
\bequation
    \begin{split}
        \Prob[G_k^\top D_k &+ \max\{D_k^\top H_k D_k,0\} \\
        &\geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | E, \mathcal{F}_k] \geq p_{\tau},
    \end{split}
\eequation
for some $p_{\tau} \in (0,1]$.
\end{assumption}
This assumption boils down to the distribution of $G_k$ having a bounded measure of asymmetry and is unique to our setting. It guarantees that there is always at least $p_{\tau}$ probability that $\tau_k$ decreases at any iteration for which $\tau_k$ would decrease if the step (and $\tau$ update) were computed using the full gradient, $\nabla f(x_k)$, as opposed to the stochastic gradient, $g_k$. This property ensures that, with high probability, $\tau_k$ is not larger than it ``should" be on too many iterations.

In \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, it was shown that this assumption is satisfied with $p_{\tau} = \frac12$ when $G_k$ is drawn from a Gaussian distribution. We show that this result can be extended to all distributions that obey a mild form of symmetry in Section \ref{subsec:subgauss}.

\subsection{Properties of Algorithm \ref{alg:ssqp}} \label{subsec:algprops}

Here we repeat a number of key results from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} that will be integral to our complexity analysis.

By Lemma 2.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for all $k = \{0,\dots,k_{\max}\}$, there exists $\kappa_{uv} \in \R{}_{>0}$ such that, if $\|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2$, then $\frac12 (\dktrue)^\top H_k \dktrue \geq \frac14 \zeta \|\uktrue\|^2$, where $\zeta$ is defined in Assumption \ref{assum:Hk}. Then, let
\bequationNN
    \Psi_k := \begin{cases}
        \|\uktrue\|^2 + \|c_k\| & \mbox{if } \|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2 \\
        \|c_k\| & \mbox{otherwise.}
    \end{cases}
\eequationNN
Now we can state a few lemmas which are relevant to our final complexity result.
\begin{lemma} \label{lem:kappapsi}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_{\Psi} \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$, the search true direction and constraint violation satisfy $\|\dktrue\|^2 + \|c_k\| \leq (\kappa_{\Psi} + 1) \Psi_k$.
\end{lemma}

\begin{proof}
    The result follows directly from Lemma 2.11 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

\begin{lemma} \label{lem:kappaq}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_q \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$ and any $\tau \leq \tktritrue$, the reduction in the model of the merit function satisfies $\Delta q (x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \kappa_q \tau \Psi_k$.
\end{lemma}

\begin{proof}
    The proof follows from \eqref{eq:qquadlbtrue} combined with the proof of Lemma 2.12 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and the filtration $\mathcal{F}_k$.

Now, we can state a lemma about the expected values of a number of random variables in our algorithm.

\blemma \label{lem:dexpectation}
Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. For all $k = \{0,\dots,k_{\max}\}$, $\E_k[D_k] = \dktrue$, $\E_k[U_k] = \uktrue$, and $\E_k[Y_k] = \yktrue$.  Moreover, there exists $\kappa_d \in \R{}_{>0}$, independent of $k$, such that,
\bequationNN
\left\|\left[\begin{matrix}
H_k & J_k^\top \\
J_k & 0
\end{matrix}\right]\right\| \leq \kappa_d.
\eequationNN
In addition, $\E_k[\|D_k - \dktrue\|] \leq \kappa_d \sqrt{M}$, and $\E_k[\|D_k - \dktrue\| | E, \mathcal{F}_k, \nabla f(x_k)^\top (D_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \leq \kappa_d \ktaudec$.
\elemma

\bproof
    Except for the final inequality, the result is proven in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. To see the final inequality, we note that by the same argument as in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for any realization of $G_k$ and $D_k$,
    \bequationNN
        \|d_k - \dktrue\| \leq \kappa_d \|g_k - \nabla f(x_k)\|.
    \eequationNN
    Therefore,
    \begin{align*}
        &\E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \E_k[\|G_k - \nabla f(x_k)\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \ktaudec.
    \end{align*}
\eproof

Next, we provide some bounds on the expectation of a few key quantities.

\blemma\label{lem:product_bounds}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequationNN 
    \begin{split}
        \nabla f(x_k)^\top \dktrue &\geq \E_k[G_k^\top D_k] \geq \nabla f(x_k)^\top \dktrue - \zeta^{-1}M\ \ \text{and} \\ \E_k[D_k^\top H_k D_k] &\geq (\dktrue)^\top H_k \dktrue.
    \end{split}
  \eequationNN
\elemma

\bproof
    The result is proven in Lemma \cite[Lemma 3.9]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

We conclude this section with a lemma that will allow us to characterize descent in $\phi$ in terms of $\Delta q(\cdot)$.

\blemma\label{lem:phidecrease}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Suppose that $\{\beta_k\}$ is chosen such that $\beta_k \xi_k \tau_k/(\tau_k L + \Gamma) \in (0,1]$ for all $k \in \{0,\dots,k_{\max}\}$.  Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequation \label{eq:phidecrease}
    \baligned
      \phi(x_k + \alpha_k d_k, \tau_k) - \phi(x_k, \tau_k)
      &\leq -\alpha_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue) \\
      &\quad + \thalf \alpha_k \beta_k  \Delta q(x_k,\tau_k,g_k,H_k,d_k) \\
      &\quad + \alpha_k \tau_k \nabla f(x_k)^\top (d_k - \dktrue),
    \ealigned
  \eequation
  where $d_k$ and $\dktrue$ are respectively defined by \eqref{eq:sqpsystem} and \eqref{eq:sqpsystemdet}.
\elemma

\bproof
    The result follows directly from Lemma 3.7 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

\subsection{Complexity Result} \label{subsec:complexity}

In this section, we present our complexity result under the condition that Assumption \ref{assum:eventE} occurs. We derive our result in largely the same way as the global convergence result in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, with two major changes, which stem from the need to characterize the behavior of the algorithm with respect to the merit parameter updating. At a high-level, the two modifications are as follows:
\begin{enumerate}
    \item We derive a new upper bound for the last term in \eqref{eq:phidecrease}. This inequality allows us to characterize decrease in the merit function and is central to the overall analysis. A new upper bound is needed in our setting, as this final term is the product of three random variables while $\tau$ is still being adaptively updated and has not settled at a lower bound. To handle this, we show that this term is bounded, under Assumption \ref{assum:eventE}, in terms of the probability that the event $\Ek3$ (defined formally below) occurs at iteration $k$. This event only occurs on iterations $k$ where $\tau_k < \tau_{k-1}$ which, when combined with a maximum of $s_{\max}$ decreases of $\tau$ due to Assumption \ref{assum:eventE}, allows us to obtain a bound on this quantity that holds with high-probability. The new upper bound is derived in Lemma \ref{lem:innerprod} while our high-probability bound on the summation (over $k=0,\dots,k_{\max}$) of the probabilities of $\Ek3$ occuring is presented in Lemma \ref{lem:Eksumlsmax}.
    \item We characterize iterations at which $\tktritrue < \tau_k$ occurs. These iterations are problematic for the analysis due to the inclusion of $\tau_k$ in $\Delta q(x_k,\tau_k,\nabla f(x_k), H_k, \dktrue)$, which is used during the analysis to measure progress in the algorithm. One particular concern arises in the final complexity result; if $k^*$ occurs at an iterate such that $\tau_{k^*}^{trial,\text{true}} < \tau_{k^*}$, then $\Delta q(x_{k^*},\tau_{k^*},\nabla f(x_{k^*}), H_{k^*}, d^{\text{true}}_{k^*})$ cannot be related to our optimality conditions \eqref{eq:optconds}. To solve this issue, we introduce a theoretical sequence, $\hat{\tau}_k$, which, for all $k$, is the minimum of $\tau_k$ and $\tktritrue$, and analyze the algorithm's progress with respect to this sequence. Due to Assumption \ref{assum:ptau}, whenever the event $\tktritrue < \tau_k$ occurs, there is at least $p_{\tau}$ probability of decreasing $\tau$. Taken in combination with $s_{\max}$ from Assumption \ref{assum:eventE}, this enables us to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ occurs. We introduce Lemma \ref{lem:dqbound} and Lemma \ref{lem:hattaudiff} to handle iterations such that $\tktritrue < \tau_k$. Additionally, we derive Lemma \ref{lem:Ktaulsmax} to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ can occur.
\end{enumerate}

Now, we analyze the first modification mentioned above. As in the previous section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k \in \{0,\dotsc,\kmax\}$, let $\Ek1$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) \geq 0$, let $\Ek2$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} = \tau_{k-1}$, and let $\Ek3$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue)$ and $\Tcal_{k} < \tau_{k-1}$.

Now, we derive a bound on the final term in \eqref{eq:phidecrease}.

\begin{lemma} \label{lem:innerprod}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$, the existence of which follows under Assumption \ref{assum:fcsmooth}. Let
\bequationNN
\alpha_{\min,k} := \frac{\beta_k \xi_{\min} \tau_{\min}}{\tau_{\min}L_k + \Gamma_k} \mbox{ and } \alpha_{\max,k} := \frac{\beta_k \xi_{\min} \tau_{k-1}}{\tau_{k-1}L_k + \Gamma_k},
\eequationNN
where $\tau_{\min}$ and $\xi_{\min}$ are defined as in Assumption \ref{assum:eventE}.

Then, with $\kappa_d \in \R{}_{>0}$ defined by Lemma \ref{lem:dexpectation},
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq  (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek1], \\
\E_{k,2} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek2], \\
\E_{k,3} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\tau_{\min}$, $\alpha_{\min,k}$, and $\alpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &= \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek1] \Prob_k[\Ek1] + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By the Law of Total Expectation and Lemma \ref{lem:dexpectation}, this means that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, we have
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} \alpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} \alpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{\min} \alpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{\min} \alpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}
Summing these three inequalities,
\begin{align}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \nonumber \\
    &\leq \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+\frac13(\tau_{k-1} (\alpha_{\max,k} - \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+\frac13(2 \tau_{\min} \alpha_{\min,k} - \tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \nonumber \\
    &= \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -\theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-\frac13(\tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2) - 2 \tau_{\min} \alpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]. \label{eq:innerprodproof1}
\end{align}
Now, by Lemma \ref{lem:dexpectation},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|\nabla f(x_k)\| \E_k[\|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[\nabla f(x_k)^\top(D_k - \dktrue)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek2] \Prob_k [\Ek2] \\
    &= \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \\
    &\leq \kappa_g \E_k[\|D_k - \dktrue\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma \ref{lem:dexpectation}. Using these three inequalities with
\eqref{eq:innerprodproof1}, yields
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
which proves the result.
\end{proof}

Now, we turn our attention to the second modification mentioned in the outline of this section. Our complexity result is derived through the use of \eqref{eq:phidecrease}, which relates decrease in our merit function to $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$. On any iteration for which $\tau_k \leq \tktritrue$ holds, $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$ can be directly related to the optimality conditions defined in \eqref{eq:optconds}. Unfortunately, the same is not true for $k$ such that $\tau_k > \tktritrue$. Thus, in order to provide an informative bound on such iterations, we introduce the following sequence:
\bequation \label{eq:hattaudef}
    \hat{\Tcal}_k := \min\{\Tcal_k, \tktritrue\},
\eequation
which we will use throughout the rest of the analysis.

Now, we derive a bound on the conditional expectation of $\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)$ using the definition of $\hat{\Tcal}_k$.

\begin{lemma} \label{lem:dqbound}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$ and let $\kappa_d$ be defined as in Lemma \ref{lem:dexpectation}. Let $\hat{\Tcal}_k$ be defined in \eqref{eq:hattaudef}. Then,
\begin{align*}
    \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)]
    &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
    +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
    &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
    &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)).
\end{align*}
\end{lemma}

\begin{proof}
    To begin, by the definition of \eqref{eq:deltadef},
    \begin{align}
        &\E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \nonumber \\ &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k, 0\}) + \|c_k\|_1] \nonumber \\
        &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k - \nabla f(x_k)^\top \dktrue  + \frac12 \max\{D_k^\top H_k D_k, 0\} \nonumber \\
        &\quad- \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] \nonumber \\ &\quad+ \E_k[-\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] + \|c_k\|_1 \nonumber \\
        &= \E_k[\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} \nonumber \\
        &\quad- \frac12 \max\{D_k^\top H_k D_k, 0\})] + \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]. \label{eq:dqbound1}
    \end{align}
    Now, for simplicity of notation, let \tred{TODO: Figure out if there's a better name than $Z_k$.}
    \bequationNN
        Z_k =  \nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12 \max\{D_k^\top H_k D_k, 0\}.
    \eequationNN
    Let $E_Z$ denote the event that $Z_k \geq 0$ occurs and let $E_Z^c$ denote the event that $Z_k < 0$ occurs. Then, by the Law of Total Expectation,
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k] &= \E_k[\hat{\Tcal}_k Z_k | E_Z] \Prob_k[E_Z] + \E_k[\hat{\Tcal}_k Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Therefore, by the Law of Total Probability, Lemma \ref{lem:product_bounds}, Jensen's inequality, and convexity of $\max\{\cdot,0\}$, it follows that
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{k-1} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} \E_k[Z_k] + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} (\nabla f(x_k)^\top \dktrue - \E_k[G_k^\top D_k] \\
        &\quad+ \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12\E_k[\max\{D_k^\top H_k D_k, 0\}]) \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \zeta^{-1} M + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Similarly, we have
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{\min} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &= \tau_{\min} \E_k[Z_k] + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &\leq \tau_{\min} \zeta^{-1} M + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z].
    \end{align*}
    Summing these two inequalities yields
    \begin{align}
        \E_k[\hat{\Tcal}_k Z_k] &\leq \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M + \frac12 (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \nonumber \\
        &\quad+ \frac12(\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \label{eq:dqbound2}.
    \end{align}
    Next, we note that by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, Jensen's inequality, and the concavity of the square root,
    \begin{align*}
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] &\leq 
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top \dktrue|] +\E_k[|G_k^\top \dktrue - G_k^\top D_k|] \\
        &\leq \|\dktrue\| \E_k [\|\nabla f(x_k) - G_k\|] + \E_k[\|G_k\|\|\dktrue - D_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]} \\ &\quad+ \kappa_d \E_k[(\|G_k - \nabla f(x_k)\| + \|\nabla f(x_k)\|) \|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d \E_k[\|\nabla f(x_k) - G_k\|^2] \\
        &\quad+ \kappa_d \|\nabla f(x_k)\| \E_k[\|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d (M + \kappa_g \sqrt{M}) = \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}).
    \end{align*}
    In addition, by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
        &\leq \|H_k\|\|\dktrue\|^2 + \|H_k\|\E_k[\|D_k\|^2] \\
        &\leq \kappa_H \kappa_d^2 \kappa_g^2 + 2\kappa_H \kappa_d^2 (\E_k [\|G_k - \nabla f(x_k)\|^2] + \kappa_g^2) \\
        &\leq \kappa_H \kappa_d^2 (3\kappa_g^2 + 2 M).
    \end{align*}
    Now, by the Law of Total Expectation and the above two inequalities,
    \begin{align*}
         \E_k[Z_k | E_z] \Prob_k[E_Z] &= \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    By the same argument,
    \begin{align*}
         -\E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] &\leq \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    Thus, combining this with \eqref{eq:dqbound1} and \eqref{eq:dqbound2},
    \begin{align*}
        \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
        +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
        &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)),
    \end{align*}
    proving the result.
\end{proof}

Next, we introduce a lemma which controls the difference in $\Delta q(\cdot)$ on iterations where $\tktritrue < \Tcal_k$.
\begin{lemma} \label{lem:hattaudiff}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d),
    \end{align*}
    and
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k, \Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d (M + \kappa_g^2) (2 + \kappa_H \kappa_d),
    \end{align*}
    where $\alpha_{\min,k}$ and $\alpha_{\max,k}$ are defined in Lemma \ref{lem:innerprod}.
\end{lemma}

\begin{proof}
    By the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &= \E_k[\Acal_k (\Tcal_k - \hat{\Tcal}_k) (\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) |\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\}| \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \kappa_g^2 + \thalf\kappa_H \kappa_d^2 \kappa_g^2).
    \end{align*}
    Next, by the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &= \E_k[\Acal_k (\hat{\Tcal}_k - \Tcal_k) (G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \E_k[|G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\}|] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \E_k[\|G_k\|^2] + \thalf \kappa_d^2 \kappa_H \E_k[\|G_k\|^2]) \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (2\kappa_d (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2) \\
        &\quad+ \kappa_d^2 \kappa_H (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2)) \\
        &\leq (\alpha_{\max,k} \tau_k - \alpha_{\min,k} \hat{\tau}_k) (2\kappa_d (M + \kappa_g^2) + \kappa_d^2 \kappa_H (M + \kappa_g^2)).
    \end{align*}
\end{proof}

Next, we present the statements of two lemmas, which provide upper bounds, in high probability, on key components of the complexity result. The proofs of these lemmas are relegated to Appendix \ref{app:simple} for presentation purposes. Both of these lemmas use the following function in their statement. For any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, let
\bequation \label{eq:lsd}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\eequation

Now we can state the first lemma, which gives a high-probability bound on the sum of the probabilities from applying Lemma \ref{lem:innerprod} at each iteration.

\begin{lemma} \label{lem:Eksumlsmax}
    Let Assumption \ref{assum:eventE} hold. Then,
    \bequation \label{eq:Ek3lsmax}
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob [E_{k,3} | E, \mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\Bigg | E \right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Before stating the next lemma, recall the definition of $\hat{\Tcal}_k$ in \eqref{eq:hattaudef} and let $\mathcal{K}_{\tau}$ denote the index set
\bequation \label{eq:Ktau}
    \mathcal{K}_{\tau} := \{k : \tktritrue < \tau_{k-1}\}.
\eequation
By the definitions of $\tau_k$, $\tktritrue$, and $\hat{\Tcal}_k$, this set of iterations is a superset of the iterations at which $\hat{\Tcal}_k < \Tcal_k$ occurs and can therefore be used to characterize the number of iterations at which this event occurs. In addition, the event $\tktritrue < \tau_{k-1}$ does {\it not} depend on $G_k$, which makes it more convenient to work with analytically. In particular, this means that $G_k$ is conditionally independent of the event $\tktritrue < \tau_{k-1}$ given $\Fcal_k$ and $E$.

In the following lemma, we bound the cardinality of $\Kcal_{\tau}$ with high probability.

\begin{lemma} \label{lem:Ktaulsmax}
    Let Assumptions \ref{assum:eventE} and \ref{assum:ptau} hold. Let $\mathcal{K}_{\tau} = \{k : \tktritrue < \tau_{k-1}\}$. Then,
    \bequation \label{eq:Ktaulsmax}
        \Prob\left[|\mathcal{K}_{\tau}| \leq \left\lceil \frac{\ell(s_{\max},\delta)+1}{p_{\tau}}\right\rceil \Bigg| E\right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Now we are prepared to state our complexity result in terms of $\Delta q(\cdot)$.

\begin{theorem} \label{thm:complexity}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold. 
Let the sequence $\{\hat{\Tcal}_k\}$ be defined in \eqref{eq:hattaudef}.

Define 
\bequationNN
A_{\min} := \frac{\xi_{\min} \tau_{\min}}{\tau_{\min}L + \gamma} \mbox{ and }
A_{\max} := \frac{\xi_{-1} \tau_{-1}}{\tau_{-1}L + \gamma}
\eequationNN
as well as
\begin{align*}
\hat{M} &:= \frac12 A_{\max} (\tau_{-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M})
+ \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M))\\ 
&\quad \ + \frac{\tau_{-1} + \tau_{\min}}{4} A_{\max} \zeta^{-1} M + \theta \tau_{-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
and
\begin{align*}
    \kappa_{\Delta q} &:= \beta (A_{\max} \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d (2M + 3\kappa_g^2) (1 + \frac12 \kappa_H \kappa_d), \\
    \kappa_{E_3} &:= \beta (\tau_{-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec.
\end{align*}
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{k_{\max}+1}} \quad \mbox{ for some } \quad \gamma \leq \frac{A_{\min}}{A_{\max} + \theta}.
\eequationNN
Then,
\begin{align}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \nonumber \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \nonumber \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil. \label{eq:complexity}
\end{align}
\end{theorem}

\begin{proof}
By Lemma \ref{lem:phidecrease} and Lemma \ref{lem:innerprod},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) \\
    &\quad + \Acal_k \Tcal_k \nabla f(x_k)^\top (D_k - \dktrue)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}

First, we focus on iterations where $k \in \mathcal{K}_{\tau}^c$ so that $\tktritrue \geq \tau_{k-1}$ and thus, $\tau_k \leq \tktritrue$. We mention once again that $G_k$ is conditionally independent of the event $\tktritrue \geq \tau_{k-1}$ given $E$ and $\Fcal_k$. Therefore, by \eqref{eq:qquadlb}, \eqref{eq:qquadlbtrue}, and Lemma \ref{lem:dqbound},
\begin{align*}
    &\E_k [\phi(x_k + \alpha_k D_k, \Tcal_k) | k \in \mathcal{K}_{\tau}^c] - \E_k [\phi(x_k, \Tcal_k) | k \in \mathcal{K}_{\tau}^c] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in \mathcal{K}_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &=\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in \mathcal{K}_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &\leq -\beta (A_{\min} - \frac12 (A_{\max}+\theta) \beta) \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}^c] + \frac{\tau_{k-1} + \tau_{\min}}{4} \beta^2 A_{\max} \zeta^{-1} M \\
    &\quad+ \frac12 \beta^2 A_{\max} (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)) \\
    &\quad+ \beta (\tau_{k-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in \mathcal{K}_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}^c] + \kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}^c] + \beta^2 \hat{M}.
\end{align*}

Now, we condition on $k \in \mathcal{K}_{\tau}$. Once again, $G_k$ is conditionally independent of this event given $\Fcal_k$ and $E$. By (\ref{eq:qquadlb}), (\ref{eq:qquadlbtrue}), Lemma \ref{lem:dqbound}, and Lemma \ref{lem:hattaudiff},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) | k \in \mathcal{K}_{\tau}] - \E_k [\phi(x_k, \Tcal_k) | k \in \mathcal{K}_{\tau}] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad+\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad-\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad+ \kappa_{E_3} \Prob_k[\Ek3 | k \in \mathcal{K}_{\tau}] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}] + \kappa_{\Delta q} \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}] + \beta^2 \hat{M}.
\end{align*}

Now by the law of total probability and the law of total expectation,
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &=\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &\quad+ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] + \beta^2 \hat{M} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] + \beta^2 \hat{M} \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &=-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3}] + \beta^2 \hat{M} + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}]
\end{align*}

Summing this inequality for all $k \in \{0,\dots,k_{\max}\}$, by Lemma \ref{lem:Eksumlsmax} it follows that, with probability at least $1-\delta/2$,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \sum_{k=0}^{k_{\max}} (-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{E_3} \Prob_k[E_{k,3}] + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}]) \\
    &\quad+ (k_{\max}+1) \beta^2 \hat{M}, \\
    &\leq -\sum_{k=0}^{k_{\max}} \frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{\Delta q} \sum_{k=0}^{k_{\max}} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M}.
\end{align*}

Now, let $g : = \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that are measurable with respect to the filtration $\mathcal{F}_{k_{\max}}$. Note that $\Prob_k[k \in \Kcal_{\tau}] \in \{0,1\}$ since the event $k \in \Kcal_{\tau}$ does not depend on $G_k$ when conditioned on $\Fcal_k$ and $E$. Therefore, by total expectation, the definition of our filtration, Lemma \ref{lem:Ktaulsmax}, and the union bound, with probability at least $1-\delta$,
\begin{align}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k)| E] - \E[\phi(X_k,\Tcal_k) | E] \nonumber \\
    &= \int_{g \in \mathcal{F}_{k_{\max}}} \sum_{k=0}^{k_{\max}} \E [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k,\Tcal_k) | E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] f_{G}(g) dg \nonumber \\
    &\leq \int_{g \in \mathcal{F}_{k_{\max}}} \Bigg(-\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)|E,G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \nonumber \\
    &\quad+ \kappa_{\Delta q} \sum_{k=0}^{k_{\max}} \Prob[k \in \mathcal{K}_{\tau}|E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}]\Bigg) f_{G}(g) dg \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &= -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] + \kappa_{\Delta q} \E\big[|\mathcal{K}_{\tau}|\big|E\big] \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &\leq -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] + \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M}, \label{eq:complexityproof1}
\end{align}
where $f_{G}(g)$ is the probability density function of the random variable $G$. Working with left side of this inequality,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E] - \E[\phi(X_k,\Tcal_k) | E] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k f(X_k + \Acal_k D_k) + \|c(X_k + \Acal_k D_k)\|_1 | E] - \E[\Tcal_k f(X_k) + \|c(X_k)\|_1 | E] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k (f(X_k + \Acal_k D_k) - f_{\min}) + \|c(X_k + \Acal_k D_k)\|_1 | E] - \E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E].
\end{align*}
It follows by the monotonicity of the $\Tcal_k$ sequence that
\bequationNN
-\E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E] \geq - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E].
\eequationNN
Thus,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E] - \E[\phi(X_k,\Tcal_k) | E] \\
    &\geq \E [\Tcal_{k_{\max}} (f(X_{k_{\max}+1}) - f_{\min}) + \|c(X_{k_{\max}+1})\|_1 | E] - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1.
\end{align*}
Combining this with \eqref{eq:complexityproof1},
\begin{align*}
    &\beta \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min}} \\
    &\quad+ \frac{2 (k_{\max}+1) \beta^2 \hat{M}}{A_{\min}} + \frac{2}{A_{\min}} \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
Dividing both sides of this inequality by the summation of $\beta$,
\begin{align*}
    &\frac{1}{\sum_{k=0}^{k_{\max}} \beta} \sum_{k=0}^{k_{\max}} \beta \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 (k_{\max}+1) \beta^2 \hat{M} + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil,
\end{align*}
so that by the definitions of $K^*$ and $\beta$,
\begin{align*}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
\end{proof}

Now we convert this into a result in terms of our optimality conditions \eqref{eq:optconds}.

\begin{corollary} \label{coro:complexity}
    Let the assumptions of Theorem \ref{thm:complexity} hold. Then, with probability at least $1-\delta$,
    \begin{align}
        &\E\left[\frac{\|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\|^2}{\kappa_H^2} + \|c(X_{K^*})\| \Bigg| E\right] \nonumber \\
        &\leq \frac{(\kappa_{\Psi} + 1)(2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1))}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \label{eq:coro} \\
        &\quad+ \frac{2 (\kappa_{\Psi} + 1) \kappa_{\Delta q}}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil \nonumber. 
    \end{align}
\end{corollary}

\begin{proof}
    The result follows by Lemma \ref{lem:kappapsi}, Lemma \ref{lem:kappaq}, and Theorem \ref{thm:complexity} combined with \eqref{eq:sqpsystemdet}, which implies that
    \bequationNN
        \|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\| = \|H_{k^*} D^{true}_{K^*}\| \leq \kappa_H \|D^{true}_{K^*}\|.
    \eequationNN
\end{proof}

We remark again that this result, in terms of the norm of the gradient of the Lagrangian, matches the worst-case complexity of the projected stochastic gradient method \cite{DDavis_DDrusvyatskiy_2019}.

\subsection{Complexity Result for Symmetric Sub-Gaussian Distributions} \label{subsec:subgauss}

In this section, we show that Assumptions \ref{assum:eventE} and \ref{assum:ptau} occur with high probability when the stochastic gradient $G_k$ follows a symmetric, sub-Gaussian distribution.

Throughout this section, we work with the following assumption.

\begin{assumption} \label{assum:symmsubgauss}
    At every iteration $k = \{0,\dots,k_{\max}\}$, the stochastic gradient $G_k$ satisfies
    \bequation
        \E[G_k | \mathcal{F}_k] = \nabla f(x_k),
    \eequation
    \bequation \label{eq:subgauss}
        \E[\exp(\|\nabla f(x_k)-G_k\|^2/M) | \mathcal{F}_k] \leq \exp(1),
    \eequation
    and the quantities $G_k - \nabla f(x_k)$ and $\nabla f(x_k) - G_k$ are equivalent in distribution. Finally, for all $k = \{0,\dots,k_{\max}\}$, the ratio parameter $\xi_k$ satisfies $\xi_k = \xi_{\min}$.
\end{assumption}

The above assumption has a number of important implications. The first is that Assumption \ref{assum:ptau} occurs (without conditioning on event $E$) with $p_{\tau} = \frac12$, as we show in the following lemma.

\blemma \label{lem:subgptau}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then,
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | \mathcal{F}_k] \geq \frac12.
    \eequationNN
\elemma

\bproof
    Let $Z_k$ be a basis for the null space of $J_k$, which under Assumption \ref{assum:fcsmooth} is a matrix in $\R{n\times(n-m)}$. Then, let $W_k$ be such that $U_k = Z_k W_k$ and $\wktrue$ be such that $\uktrue = Z_k \wktrue$. It follows from the first block in \eqref{eq:sqpsystem} that 
    \bequationNN
        H_k (Z_k W_k + v_k) + J_k^\top Y_k = -G_k \Longleftrightarrow Z_k W_k = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (G_k + H_k v_k).
    \eequationNN
    Using this equality and simplifying,
    \bequationNN
        G_k^\top D_k + D_k^\top H_k D_k = v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} G_k + H_k^{1/2} v_k).
    \eequationNN
    In a similar fashion, by \eqref{eq:sqpsystemdet},
    \bequationNN
        Z_k \wktrue = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (\nabla f(x_k) + H_k v_k)
    \eequationNN
    so that
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + (\dktrue)^\top H_k \dktrue \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} \nabla f(x_k) + H_k^{1/2} v_k).
    \end{align*}

    Then,
    \begin{align*}
        &G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (G_k -\nabla f(x_k))),
    \end{align*}
    and,
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (\nabla f(x_k) - G_k)),
    \end{align*}
    are equivalent in distribution by Assumption \ref{assum:symmsubgauss}. Therefore,
    \begin{align*}
        &\Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \\
        &=\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | \mathcal{F}_k].
    \end{align*}
    In addition, we have
    \begin{align*}
        1 &= \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \\
        &+\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | \mathcal{F}_k] \\
        &-\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} = 0 | \mathcal{F}_k].
    \end{align*}
    Taking these two together, it follows that
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \geq \frac12,
    \eequationNN
    proving the claim.
\eproof

Next, we repeat a well known property of sub-Gaussian random variables.
\blemma \label{lem:subgboundedrv}
    Suppose Assumption \ref{assum:symmsubgauss} holds. Then, for any $\delta \in (0,1)$,
    \bequation \label{eq:subgboundedrv}
        \Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)}\right] \geq 1 - \delta.
    \eequation
\elemma

\bproof
    By Markov's inequality and Assumption \ref{assum:symmsubgauss},
    \begin{align*}
        &\Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2 > M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)\right] \\
        &= \Prob\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) > \exp\left(1 + \log \frac{k_{\max}+1}{\delta}\right)\right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &= \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\sum_{k=0}^{k_{\max}} \E\left[\exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &\leq \exp(-1) \frac{\delta}{k_{\max}+1} (k_{\max}+1)\exp(1) = \delta.
    \end{align*}
\eproof

We conclude this section by showing that under Assumption \ref{assum:symmsubgauss}, event $E$ as defined in Assumption \ref{assum:eventE} occurs with high probability.

\blemma \label{lem:subgeventE}
    Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then, there exists a constant $\kappa_{\tau_{\min}}$ such that, with probability at least $1-\delta$, event $E$ of Assumption \ref{assum:eventE} occurs with
    \bequationNN
        \ktaudec = \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)}.
    \eequationNN
    and
    \bequation \label{eq:sgtaumin}
        \tau_{\min} = \frac{(1-\sigma)(1-\epsilon)}{\kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \kappa_{\tau_{\min}}}, \quad  s_{\max} = \left\lceil\frac{\log \frac{(1-\sigma)(1-\epsilon)}{\tau_{-1} \kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \tau_{-1}\kappa_{\tau_{\min}}}}{\log 1-\epsilon }\right\rceil.
    \eequation
\elemma

\bproof
    We begin the proof by noting that by Jensen's inequality and the convexity of $\exp(\cdot)$,
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2| \mathcal{F}_k] \leq M.
    \eequationNN
    The bound on $\ktaudec$ follows directly from Lemma \ref{lem:subgboundedrv}. Finally, the bound on $\tau_{\min}$ follows from \cite[Lemma 2.16]{ABerahas_FECurtis_DPRobinson_BZhou_2020} combined with \ref{lem:subgboundedrv} and the bound on $s_{\max}$ follows from combining the bound on $\tau_{\min}$ with \eqref{eq:smaxbound}.
\eproof

\iffalse
\tred{Update 4/20 that I don't know where to put right now.}

We can also get a similar (though looser bound) for the case where we just have bounded variance!

\blemma \label{lem:boundeddiffvariance}
    For all $k \in \{0,\dots,k_{\max}\}$, let
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2 | \mathcal{F}_k] \leq M.
    \eequationNN
   Then,
    \bequationNN
        \Prob\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{\frac{(k_{\max}+1)M}{\delta}}\right] \geq 1-\delta.
    \eequationNN
\elemma

\bproof
    Let $g := \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that is measurable with respect to the filtration $\mathcal{F}_{k_{\max}}$. Then, by Markov's inequality, concavity of the square root, Jensen's inequality, and the law of total expectation,
    \begin{align*}
        &\Prob\Bigg[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2 > \frac{(k_{\max}+1)M}{\delta}\Bigg] \\
        &\leq \E\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &\leq \sum_{k=0}^{k_{\max}} \E\left[\|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &= \frac{\delta}{(k_{\max}+1)M} \sum_{k=0}^{k_{\max}} \int_{g \in \mathcal{F}_{k_{\max}}} \E\left[\|G_{k} - \nabla f(x_k)\|^2 | G_{0} = g_{0}, \dots, G_{k-1} = g_{k-1}\right] f_{G} dg \\
        &\leq \frac{\delta}{(k_{\max}+1)M} (k_{\max} + 1) M \int_{g \in \mathcal{F}_{k_{\max}}} f_{G}(g) dg = \delta,
    \end{align*}
    where $f_G(g)$ is the probability density function of the random variable $G$.
\eproof

What does this mean for our results? We can repeat the proof of Lemma \ref{lem:subgeventE} so that with probability at least $1-\delta$,
\bequationNN
    \tau_{\min} = \mathcal{O}\left(\sqrt{\frac{\delta}{k_{\max}+1}}\right)
\eequationNN
and, for sufficiently large $k_{\max}$,
\bequationNN
    s_{\max} = \mathcal{O}\left(\log \sqrt{\frac{k_{\max}+1}{\delta}}\right). 
\eequationNN
Thus,
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O} \left(\frac{\log \sqrt{\frac{k_{\max}+1}{\delta}}}{\sqrt{k_{\max}+1}} \right),
\eequationNN
which means we can always get a useful complexity result, so long as $k_{\max}$ is sufficently large.

Unfortunately, because the bound from Lemma \ref{lem:boundeddiffvariance} is $\mathcal{O}(\sqrt{k_{\max}+1})$, we cannot use this approach to directly bound $\ktaudec$ and obtain a meaningful complexity result. Thus, additional assumptions are still needed in this case.
\fi

\subsection{Complexity Result with Decreasing Ratio Parameter} \label{subsec:ratioparam}

In this section, we relax Assumption \ref{assum:eventE} with respect to the random variable $\{\Xi_k\}$ and allow it to be adaptive over the course of the algorithm. Due to the definition of $\{\Xi_k\}$, it satisfies a deterministic lower-bound, $\xi_{\min}$, such that $\xi_k \geq \xi_{\min} > 0$ holds for all $k$ \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Therefore, it follows that there exists a maximum number of decreases of $\xi$, which we denote by $r_{\max}$, that satisfies
\bequationNN
    r_{\max} \leq \min\left\{k_{\max}+1, \left\lceil \frac{\log(\xi_{\min}/\xi_{-1})}{\log(1-\epsilon)} \right\rceil\right\}.
\eequationNN

Now, we can state our new assumption.

\bassumption\label{assum:eventExi}
  Conditioned on the event $E_{\xi} := E(\kmax,s_{\max},\tau_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E_{\xi}, \Fcal_k] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E_{\xi}, \Fcal_k] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k = \xi_{k-1}] \leq \kappa_1, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k = \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_2, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_3.
    \ealigned
  \eequationNN
\eassumption

This assumption is largely the same as Assumption \ref{assum:eventE}. The major new requirement due to the adaptive $\{\Xi_k\}$ sequence is the addition of two more events under which the norm difference of $\nabla f(x_k)$ and $G_k$ is bounded.

We remark that this assumption holds with high-probability under Assumption \ref{assum:symmsubgauss} (without the condition that $\xi_k = \xi_{\min}$), a result which can easily be derived by simple modification of the techniques used in Section \ref{subsec:subgauss}. We leave this derivation as an exercise for the reader.

The complexity analysis for this case follows by essentially the same arguments as those used to derive a complexity result under Assumption \ref{assum:eventE}. A slight modification of Lemma \ref{lem:innerprod} is needed to include the three events related to $\nabla f(x_k)^T(d_k-\dktrue)$ that appear in Assumption \ref{assum:eventExi} (as opposed to the one in Assumption \ref{assum:eventE}), which yields a result in terms of the probabilities of these three events. Then, a slightly modified Lemma \ref{lem:Eksumlsmax} and the union bound can be applied two additional times to derive a complexity result. Since the analysis is a relatively straightforward extension of the results in Section \ref{subsec:complexity}, we simply state our complexity result here.
\begin{theorem}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:ptau}, and \ref{assum:eventExi} hold. Then, with probability at least $1-\delta$,
    \begin{align*}
        &\E[\|\nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c_{k^*}\| |
        E_{\xi}] \\
        &= \mathcal{O}\Bigg(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c_0\|_1 + M}{\sqrt{k_{\max}+1}} \\
        &\quad+ \frac{(\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta)) + (\xi_{-1} - \xi_{\min})(r_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\Bigg).
    \end{align*}
\end{theorem}

\bproof
    We leave the proof as an exercise for the reader.
\eproof

\section{Conclusion} \label{sec:conclusion}

In this work, we derived the first worst-case complexity result for an adaptive stochastic algorithm for equality constrained optimization. We developed a stochastic SQP algorithm with an adaptive $\ell$-1 merit function, based on the framework proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}. While key to a practical algorithm, the adaptivity in the merit function introduced a number of theoretical challenges to overcome. Under mostly standard assumptions, we prove that, with high probability, the expected value of the norm of the gradient of the Lagrangian decays at a rate of $k^{-4}$, matching the worst-case complexity of the projected stochastic gradient method. We believe the theoretical tools developed within may be applicable to a broad class of constrained stochastic optimization methods that utilize an adaptive merit function. 

\iffalse
OLD STUFF BELOW:
\subsection{Quick Complexity Highlight}
Quick highlight of the main complexity result for meeting on 3/9/2021:

Let $\mathcal{I} \subseteq \{0,1,\dots,\kmax\}$ denote the index set of ``good" iterations. Overall analysis will lead to a result of the form (with $\beta_k := \beta = \gamma/\sqrt{\kmax+1}$:
\begin{align*}
    &\sum_{k \in \mathcal{I}} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\quad\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &\quad+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau}.
\end{align*}
To get the expectation that we want, we need to add and subtract:
\begin{align*}
    &\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + \sum_{k \in \mathcal{I}^c} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)].
\end{align*}
Then, because the number of ``bad" iterations is bounded by $\ell(s_{\max},\delta)/p_{\tau}$,
\begin{align*}
    &\frac{\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)]}{\sum_{k=0}^{\kmax} \beta} \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\sum_{k=0}^{\kmax} \beta} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sum_{k=0}^{\kmax} \beta}.
\end{align*}
So that,
\begin{align*}
    &\E [\Delta q(x^*, \tau^*, \nabla f(x^*), H^*, d^{*,true})] \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\sqrt{\kmax + 1}} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sqrt{\kmax+1}}.
\end{align*}

Algorithm \ref{alg:ssqp} generates a random process $\{\bar{G}_k,X_k,\bar{D}_k,\bar{\mathcal{T}}_k,\bar{\Xi}_k,\bar{\mathcal{A}}_k\}$. We will denote all random quantities by capital letters and their realizations by small letters. The random gradient estimate is denoted by $\bar{G}_k$ and its realizations by $\bar{g}_k = \bar{G}_k(\omega)$. Similarly, let the random quantities $x_k = X_k(\omega)$ (iterates), $\bar{d}_k = \bar{D}_k(\omega)$ (search directions), $\btau_k = \bar{\mathcal{T}}_k(\omega)$ (merit parameter), $\bxi_k = \bar{\Xi}_k(\omega)$ (reduction ratio), and $\bar{\alpha}_k = \bar{\mathcal{A}}_k(\omega)$ (step sizes) denote their respective realizations. We will assume that the estimates $\bar{G}_k$ obey some standard properties, conditioned on the past.

To formalize conditioning on the past, let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by the random variables $\bar{G}_0, \dotsc \bar{G}_{k-1}$. For completness, we set $\mathcal{F}_{-1} = \sigma(x_0)$. As a result, we have that $\mathcal{F}_{k}$ for $k \geq -1$ is a filtration.

Let $E_{\tau,low}$ denote the event that the merit parameter sequence eventually remains constant at a sufficiently small positive value.
We will derive our complexity result under the assumption that this event occurs.

\begin{assumption} \label{assum:taulow}
Event $E_{\tau,low}$ occurs in the sense that there exists an iteration
number $\bar{k}_{\tau,\xi} \in \mathbb{N}$ and a merit parameter value
$\btau_{\min} \in \R{}_{>0}$ such that
\begin{equation} \label{eq:taumin}
    \btau_k = \btau_{\min} \leq \btau_k^{trial} \quad and \quad
    \xi_k = \xi_{\min} \quad for \; all \quad k \geq \bar{k}_{\tau,\xi}.
\end{equation}
In addition, the sequence of random gradients $\bar{G}_k$ generated by Algorithm \ref{alg:ssqp} satisfies
\begin{equation*}
    \E_{k,\tau,small}[\bar{G}_k] = g_k \quad and \quad \E_{k,\tau,small}[\|\bar{G}_k - g_k\|^2] \leq M
\end{equation*}
where $\E_{k,\tau,small}$ denotes expectation with respect to the distribution of $\omega$ conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_{k}$.
\end{assumption}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k$, let $\Ek1$ be the event that $g_k^\top(\bd_k - d_k) \geq 0$, let $\Ek2$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} = \btau_{k-1}$, and let $\Ek3$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} < \btau_{k-1}$.

We require an additonal assumption to obtain our complexity result:
\begin{assumption} \label{assum:boundedrv}
There exists $\kappa_{\Ek3} > 0$ such that
\begin{equation} \label{eq:boundedrv}
    \E_k [\|\bar{g}_k-g_k\||\Ek3] \leq \kappa_{E_3}.
\end{equation}
\end{assumption}
The above assumption holds under a number of conditions, including when
$\bar{g}_k$ is a bounded random vector.

%NEW
\textcolor{red}{TODO:} Ignoring $\xi_k$ for now. Will probably need additional cases in the proof eventually...

\begin{lemma} \label{lem:innerprodold}
Suppose that Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|g_k\|_2\}$, the existence of which follows under \cite[Assumption 1]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\bxi_k = \bxi_{\min}$ and define
\bequationNN
\balpha_{\min,k} := \frac{\beta_k \bxi_{\min} \btau_{\min}}{\btau_{\min}L_k + \Gamma_k} \mbox{ and } \balpha_{\max,k} := \frac{\beta_k \bxi_{\min} \btau_{k-1}}{\btau_{k-1}L_k + \Gamma_k}.
\eequationNN

Then, with $\kappa_d \in \R{}_{>0}$ from Lemma 3.6 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} which satisfies
$\|\bar{d}_k-d_k\| \leq \kappa_d \|\bar{g}_k-g_k\|$,
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq  (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek1] \\
\E_{k,2} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek2] \\
\E_{k,3} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\btau_{\min}$, $\balpha_{\min,k}$, and $\balpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &= \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek1] \Prob_k[\Ek1] + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By Lemma 3.6, this means that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, by Lemma 3.6, we have
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} \balpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} \balpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{\min} \balpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{\min} \balpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}

Summing these three inequalities yields

\begin{align}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \nonumber \\
    &\leq \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+(\btau_{k-1} (\balpha_{\max,k} - \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+(2 \btau_{\min} \balpha_{\min,k} - \btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3]) \nonumber \\
    &= \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -3 \theta \beta_k^2 \btau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-(\btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2) - 2 \btau_{\min} \balpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]). \label{eq:innerprodproof1old}
\end{align}
Now, by Assumption \ref{assum:boundedrv},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|g_k\| \E_k[\|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \E_k[\|\bar{g}_k - g_k\| | \Ek3] \Prob_k[\Ek3]  \\
    &\leq \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[g_k^\top(\bd_k - d_k)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek2] \\
    &= \E_k[\|g_k\| \|\bar{d}_k - d_k\|] - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \E_k[\|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma 3.6. Using these three inequalities with
\eqref{eq:innerprodproof1old}, yields
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
which proves the result.
\end{proof}

The above result provides an upper bound in terms of the probability that the event $\Ek3$ occurs. Due to the assumed lower bound on $\btau_k$, this event can only occur a finite number of times. To obtain our final result, we need an upper bound on the summation of the probability that $\Ek3$ occurs. The first component of this upper bound comes from the Chernoff bound.

\begin{lemma} \label{lem:chernoff}
Let $Z_0, \dotsc, Z_{k}$ be independent Bernoulli random variables and let $s \in \mathbb{N}_{>0}$.
%Let
%\begin{equation} \label{eq:lsd}
%    \ell(s,\delta) := S + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 S \log(1/\delta)}.
%\end{equation}
Then, for any $\delta \in (0, 1)$,%\todo{FEC: I suggest ``Let ... random variables for any $k \in \mathbb{N}_{\geq0}$.  Then, for any $s \in \mathbb{N}_{\geq0}$ and $\delta \in (0,1)$, ....}
\begin{equation}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s\right] \leq \delta,
\end{equation}
whenever
\begin{equation} \label{eq:lsdold}
    \sum_{i=0}^{k} \Prob[Z_i = 1] \geq \ell(s,\delta) \quad where \quad \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\end{equation}
\end{lemma}

\begin{proof}
Denote $\mu = \sum_{i=0}^{k} \Prob[Z_i = 1]$.%\todo{FEC: In the general form, the definition of $\mu$ is in terms of expected value.  Maybe for clarity we should write $\mu = \sum_{i=0}^k E[Z_i] = \sum_{i=0}^k \Prob[Z_i = 1]$, where the latter is true only because we have Bernoulli random variables.} Then by Chernoff's bound, for any $\rho \in (0,1)$,
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq (1-\rho) \mu \right]
    \leq e^{-\mu \rho^2/2}.
\end{equation*}
Now, setting $\rho = 1 - s/\mu$ (which is in $(0,1)$ by (\ref{eq:lsd})), we have
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s \right]
    \leq e^{-\mu (1-s/\mu)^2/2}.
\end{equation*}
To prove the result, we need to show that%\todo{FEC: In the proof, you start with what we need, then work backwards to show what we want.  I'd prefer if we start with what we have (assumed in the statement) and prove that it gives what we want.  Does that make sense?}
\begin{equation*}
    e^{-\mu (1-s/\mu)^2/2} \leq \delta
\end{equation*}
holds. Therefore, we need
\begin{equation*}
    -\mu(1-s/\mu)^2/2 \leq \log(\delta)
\end{equation*}
to be satisfied. Rearranging this inequality, and using $\log(\delta) = -\log(1/\delta)$,%\todo{FEC: I don't see where the last equation comes from.  Did you scale it by $2\mu$?  I'm not seeing it.}
\begin{equation*}
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta) = \mu^2 - 2\mu (s+\log(1/\delta)) + s^2. 
\end{equation*}
Therefore, using the quadratic equation and taking the positive root,
\begin{align*}
    \mu &\geq s + \log(1/\delta) + \frac12\sqrt{4(s+\log(1/\delta))^2 - 4 s^2} \\
    &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)},
\end{align*}
which proves the result.
\end{proof}

Unfortunately, the events $\Ek3$ are not independent of each other so we can not directly apply Chernoff's bound. However, we can use this result in combination with an observation about the limited nature of the dependency between these events to prove the following result.

%IDEA: Rewrite lemma to prove that $K_stop <= k_{S,\delta}$ w.h.p. when $k_{s,\delta}$ exists. Gets rid of this whole J_i,stop nonsense

%This rewrite sucks, should just do it instance-wise.

%Essential components:
%   Independence when the leave one out sum is less than s.
%   Conclusion: w.h.p K_stop <= k_s,delta (or something similar).

%Crappy parts:
%   Conditioning on k_s,delta being well defined. Any better way to handle it? Yes if we do it instance wise. But then that notation is a bit frustrating
%   Top part is fine, gets rough as soon as we introduce E_s,delta.

\begin{lemma} \label{lem:depbernoulli}
For any $k \in \mathbb{N}_{\geq 0}$, let $Z_0, \dotsc, Z_{k}$ be Bernoulli random variables. Let $s \in \mathbb{N}_{>0}$.%\todo{FEC: Is it right to say that $Z_i$ is Bernoulli upfront?  Or should we be saying that, conditioned on ${\cal F}_i$, the random variable $Z_i$ is Bernoulli?  I guess technically it's Bernoulli in any case, since it's 0--1, but maybe we should say the condition since we always talk about conditional probabilities?}
For any $\hat{k} \in \{0,\dotsc,k\}$ and $i \in \{0,\dotsc,\hat{k}\}$, let $E_{\hat{k},i}$ be the event that $\sum_{j\leq \hat{k},j\neq i} Z_j < s$. We assume the following about the random variable $Z_i$ for each $i \in \{0,\dotsc,k\}$:
\begin{enumerate}
    \item $\Prob[Z_i = 1 | \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\hat{k}}]$.
    \item $\Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}^c] = 0.$
\end{enumerate}
%Let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_{k}$. %and let $\bar{G}_{i}$ be measurable with respect to $\mathcal{F}_i$ for all $i \in \{-1,\dotsc,\hat{k}-1\}$.
Let $\delta \in (0,1)$ and let $\ell(s,\delta)$ be defined as in (\ref{eq:lsd}). Let $K_{s,\delta}$ be the random variable such that, for any realization of $\bar{G}_0,\dotsc,\bar{G}_{k-1}$ that is measurable with respect to $\mathcal{F}_k$,
\bequationNN
    k_{s,\delta} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta) \right\},
\eequationNN
($k_{s,\delta} = \infty$ for any realization such that $\sum_{i=0}^k \Prob[Z_i=1|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta)$ does not occur).
In addition, let $K_{stop}$ be the random variable
\bequationNN
K_{stop} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} Z_i = s\right\},
\eequationNN
($k_{stop} = \infty$ for any realization of $Z$ such that $\sum_{i=0}^{k} z_i < s$).

We define two events:%\todo{FEC: How do these events depend on $k$?  Should we take it that $k$ is ``fixed'' in some sense, but we are considering the events for any $s$?  But shouldn't we be proving the result ``for any $k$'' as well, in which case the events should depend on $k$, too?}
\begin{enumerate}
    \item Let $E_{k,s,\delta}$ be the event that 
    $\sum_{i=0}^k \Prob[Z_i=1|\mathcal{F}_i] \geq \ell(s,\delta)$.
    \item Let $E_{k,s,\delta,stop}$ be the event that $K_{stop} > K_{s,\delta}$.
\end{enumerate}
Then,
\begin{equation*}
    \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
\end{equation*}
%We assume the following:
%\begin{enumerate}
%    \item For any $i \in \{0,\dotsc,\hat{k}\}$, let $J_{i,stop}$ be the event that $i > K_{stop}$ and  
%    \bequationNN
%    \Prob[(Z_i = 1) \cap J_{i,stop} | \mathcal{F}_i] = 0.
%    \eequationNN
%    (high level idea: once a realization of $Z$ has $s$ successes, the probability of $Z_i = 1$ is $0$.)
    %and thus $\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] = \sum_{i=0}^{K_{stop}} \Prob[Z_i = 1 | \mathcal{F}_i]$.
%the minimum integer such that $\sum_{i=0}^{k_{stop}} Z_i = s$ (set $k_{stop} = \infty$ if $\sum_{i=0}^{\hat{k}} Z_i < s$). Let $Y_i = 0$ for all $i > k_{stop}$.
%    \item For any $\bar{k} \in \{0,\dotsc,\hat{k}\}$, let $J_{\bar{k},i}$ be the event that $\sum_{j\leq \bar{k},j\neq i} Z_j < s$. Then, $\Prob[Z_i = 1| \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, J_{\bar{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\bar{k}}]$. (high level idea: if the summation leaving out $Z_i$ does not equal $s$, then $Z_i$ is independent of all other $Z_j$.)
%\end{enumerate}

%$\Prob[Z_i = 1|\nu_i] = \Prob[Z_i = 1|\nu_i, Z_0, %\dotsc, Z_{i-1}$.
%let $\Prob[Z_i=1|\nu_i] = \Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}]$ hold unless $\sum_{j=0}^{\bar{k}} Z_j = s$ in which case $\Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}] = 0$ holds for any $i$ such that $\sum_{j\leq \bar{k}, j\neq i} Z_j = s$.
%Then, for any $\delta \in (0,1)$,
%\begin{equation}
%    \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \geq 1 - \delta,
%\end{equation}
%where $\ell(s,\delta)$ is defined in (\ref{eq:lsd}).
\end{lemma}

\begin{proof}
    %We work with any fixed sequence $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ satisfying these conditions.
    %Note that by the definition of our filtration, it should be clear that $\Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{k-1}] = \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]$ for any $i \in \{0,\dotsc,k\}$.
    
    %We begin the proof by showing that
    %\begin{equation*}
    %    \Prob\left[ \right] \geq 1 - \delta,
    %\end{equation*}
    %holds for any fixed $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$. To prove this, we assume that $\sum_{i=0}^{\hat{k}} \Prob[Z_i| \bar{g_0}, \dotsc, \bar{g}_{i-1}] \geq \ell(s,\delta)$ (as the result is trivial otherwise).
    
    Let $E_{k,s,\delta}$ and $E_{k,s,\delta,stop}$ both occur. Then, since $E_{k,s,\delta}$ occurs, $k_{s,\delta}$ is finite. In addition, because $E_{k,s,\delta,stop}$ occurs,
    we have that
    \bequationNN
        \sum_{i=0}^{k_{s,\delta}} z_i < s.
    \eequationNN
    Therefore, for all $i \in \{0,\dotsc,k_{s,\delta}\}$, $E_{k_{s,\delta},i}$ occurs. Thus, for all $i,j \in \{0,\dotsc,k_{s,\delta}\}$, $Z_i$ and $Z_j$ were mutually independent.
    
    Due to the independence $Z$ in this case, by Lemma \ref{lem:chernoff},
    \bequationNN
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s\right] \leq \delta,
    \eequationNN
    and thus,
    \bequationNN
        \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
    \eequationNN
    
    Now, let $\hat{Z}_0, \dotsc, \hat{Z}_{k}$ be independent Bernoulli random variables such that $\Prob[\hat{Z}_i = 1] = \Prob[Z_i = 1|\mathcal{F}_i]$ for all $i=0,\dotsc,k$. Let $E$ be the event that $\sum_{i=0}^{k_{s,\delta}} Z_i < s$ and let $E_{k,s,\delta}$ occur. Now, for each $i=0,\dotsc,k_{s,\delta}$, it follows that if event $E$ occurs, $E_{k_{s,\delta},i}$ must occur as well, so $Z_i$ is independent of $Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{k_{s,\delta}}$ conditioned on the event $E$. Thus, whenever $E$ occurs, $Z_0,\dotsc,Z_{k_{s,\delta}}$ are identical in distribution to $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s,\delta}}$. Therefore, by Lemma \ref{lem:chernoff},
    \begin{equation}
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = \Prob\left[\sum_{i=0}^{k_{s,\delta}} \hat{Z}_i < s\right] \leq
        \delta.
    \end{equation}
    It follows that
    \begin{equation*}
           \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i \geq s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = 1 -    \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] \geq 1 - \delta,
    \end{equation*}
    and thus
    \begin{equation*}
        \Prob[k_{stop} \leq k_{S,\delta}] \geq 1 - \delta.
    \end{equation*}
    In addition, by the definition of $k_{stop}$ and $J_{i,stop}$, with probability at least $1-\delta$,
    \begin{align*}
        \sum_{i=0}^{\hat{k}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}]
        &= \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq \sum_{i=0}^{k_{S,\delta}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq 1 + \ell(s,\delta),
    \end{align*}
    and thus,
    \begin{equation*}
        \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1|\bar{g}_0, \dotsc, \bar{g}_{i-1}] \leq 1 + \ell(s,\delta) \right] \geq 1 - \delta.
    \end{equation*}
    Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_{\hat{k}}} \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{\hat{k}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\hat{k}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\hat{k}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
\end{proof}

This setup applies to $\Ek3$ under Assumption \ref{assum:taulow} due to the definitions of $\btau$ and $\btau_{\min}$. In particular, at each iteration where $\Ek3$ occurs, $\btau_{k} \leq (1-\varepsilon)\btau_{k-1}$ holds. Therefore, if we perform this process $s$ times, until
\begin{equation*}
    \btau_{\min} \geq (1-\varepsilon)^s \btau_{-1},
\end{equation*}
it follows that $\Ek3$ cannot occur again by Assumption \ref{assum:taulow}. Thus, solving this inequality for $s$, we have
\bequation \label{eq:Stmin}
    s_{\btau_{\min}} := \left\lceil\frac{\log(\btau_{\min}/\tau_{-1})}{\log(1-\varepsilon)}\right\rceil
\eequation
which is the maximum number of times $\Ek3$ can occur.

Now we can show how to apply the above lemma to $\Ek3$.

\begin{lemma}
    Let Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\beta_j = \beta$, $L_j = L$, and $\Gamma_j = \Gamma$ for all $j=0,\dotsc, k$. Let 
    \bequationNN
        \balpha_{\min} := \frac{\beta \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max} := \frac{\beta \bxi_{\min} \btau_{-1}}{\btau_{-1}L + \Gamma}.
    \eequationNN
    Let $\delta \in (0,1)$. Then, with probability at least $1-\delta$,
    \begin{align}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top (\bar{d}_j-d_j)]
        &\leq (\btau_{-1} (\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3}(1 + \ell(s_{\btau_{\min}},\delta))\\
    &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}, \nonumber
    \end{align}
    where
    \bequationNN
        \ell(s_{\btau_{\min}},\delta) := s_{\btau_{\min}} + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s_{\btau_{\min}} \log(1/\delta)}.
    \eequationNN
\end{lemma}

\begin{proof}
    By Lemma \ref{lem:innerprod},
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq \sum_{j=0}^k (\btau_{j-1}(\balpha_{\max,j} + \theta \beta_j^2) - \btau_{\min} \balpha_{\min,j}) \kappa_g \kappa_d \kappa_{E_3} \Prob_j[E_{j,3}]\\
        &\quad+ \theta \beta_j^2 \btau_{j-1} \kappa_g \kappa_d \sqrt{M}.
    \end{align*}
    Using our assumption on $\beta$, $L$, and $\Gamma$, we can upper bound this inequality as
    \begin{align} \label{eq:ipproof1}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} \sum_{j=0}^k \Prob_j[E_{j,3}]\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}. \nonumber
    \end{align}
   
    To show the final result, we need to apply Lemma \ref{lem:depbernoulli}. To do this, let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_k$ and for all $i=0,\dotsc,k$, let $Z_i = 1$ if $E_{i,3}$ occurs and let $Z_i = 0$ otherwise. Recall that $\Prob_i[\cdot]$ is conditioned on the event $E_{\tau,low}$ occurring as well as the filtration $\mathcal{F}_i$.
    
    Now, let $s = s_{\btau_{\min}}$, so that $s$ is the maximum number of iterations in which $\Ek3$ can occur by Assumption \ref{assum:taulow}. Then, it is easy to verify that by the definition of our filtration, the probability that $\Ek3$ occurs is independent of the $E_{i,3}$ for all other $i$, whenever $\Ek3$ can occur without contradicting Assumption \ref{assum:taulow}. This holds whenever $E_{\hat{k},i}$ occurs, so that the first property of $Z_i$ in Lemma \ref{lem:depbernoulli} holds. On the other hand, when $E_{\hat{k},i}^c$ occurs it is clear that if $\Ek3$ occurs as well that Assumption \ref{assum:taulow} must be contradicted. Thus, second property of $Z_i$ in Lemma \ref{lem:depbernoulli} is satisfied as well.
    
    Now, presume that $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s_{\btau_{\min}},\delta)$. Then, by Lemma \ref{lem:depbernoulli},
    \bequationNN
        \Prob[K_{stop} \leq k_{s_{\btau_{\min}},\delta}] \geq 1 - \delta.
    \eequationNN
    In addition, by the definition of $s_{\btau_{\min}}$ and $K_{stop}$, it follows that whenever $K_{stop}$ is finite,
    \bequationNN
        \sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] =
        \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}].
    \eequationNN
    Thus, with probability at least $1 - \delta$,
     \bequationNN
        \sum_{i=0}^{k} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq \sum_{i=0}^{k_{s_{\btau_{\min}}}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]
        \leq 1 + \ell(s_{\btau_{\min}},\delta).
    \eequationNN
    
    On the other hand, if $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] < \ell(s_{\btau_{\min}},\delta)$, it is clear that $\sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq 1 + \ell(s_{\btau_{\min}},\delta)$. Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_k} \Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_k} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
    
    Combining this with (\ref{eq:ipproof1}),
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} (1 + \ell(s_{\btau_{\min}},\delta))\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M},
    \end{align*}
    holds with probability at least $1-\delta$.
\end{proof}

\begin{theorem}
Suppose that Assumption 4 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} holds. Define 
\bequationNN
\bar{A}_{\min} := \frac{\bar{\xi}_{\min} \bar{\tau}_{\min}}{\tau_{-1}L + \gamma} \mbox{ and }
\bar{A}_{\max} := \frac{\xi_{-1} \tau_{-1}}{\bar{\tau}_{\min}L + \gamma}
\eequationNN
as well as
\bequationNN
\bar{M} := \tau_{-1} \left(\frac12 (\bar{A}_{\max} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{K+1}}
\eequationNN
for some
\bequationNN
\gamma \leq \min\left\{\frac{\bar{A}_{\min}}{\bar{A}_{\max} + \theta},
\frac{1}{\bar{A}_{\min}}\right\}.
\eequationNN
Then,
\begin{equation}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + c_0 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation}
\end{theorem}

\begin{proof}
Let
\bequationNN
\bar{A}_k = \frac{\bar{\xi}_{k} \bar{\tau}_{k}}{\bar{\tau_{k}}L + \gamma} \mbox{ and }
\bar{M}_k = \bar{\tau}_{k} \left(\frac12 (\bar{A}_{k} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
It follows that $\bar{A}_k \beta \leq \bar{\alpha}_k \leq (\bar{A}_k + \theta)\beta$. Using  Lemmas 3.2(d), 3.5, 3.8, and 3.9 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} (with the replacement of $\bar{\tau}_{\min}$ by $\bar{\tau}_k$), we have
\begin{align*}
    &\E_k[\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\leq \E_k [-\bar{\alpha}_k \Delta q(x_k, \bar{\tau_k}, g_k, H_k, d_k) + \frac12 \bar{\alpha}_k \beta \Delta q(x_k, \bar{\tau_k}, \bar{g}_k, H_k, \bar{d}_k) + \bar{\alpha}_k \bar{\tau}_k g_k^\top (\bar{d}_k - d_k)] \\
    &\leq -\beta(\bar{A}_k - \frac12(\bar{A}_k + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}_k \\
    &\leq -\beta(\bar{A}_{\min} - \frac12(\bar{A}_{\max} + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M} \\
    &\leq -\frac12 \beta \bar{A}_{\min} \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}
\end{align*}
Summing this inequality from $0$ to $K$,
\begin{align}
&\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \nonumber \\ 
&\leq -\frac12 \bar{A}_{\min} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)] + (K+1) \beta^2 \bar{M}. \label{eq:stochasticproof1old}
\end{align}
Now, we work with the left hand side of this inequality,
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k f(x_k + \bar{\alpha}_k \bar{d}_k) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k f_k + c_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k (f(x_k + \bar{\alpha}_k \bar{d}_k) - f_{\min}) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k].
\end{align*}
Now, conditioned on the algorithm reaching $x_k$, it follows by the monotonicity of $\tau$
that
\bequationNN
-\E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k] \geq - \E_k[\bar{\tau}_{k-1} (f_k - f_{\min}) + c_k].
\eequationNN
Therefore, summing this inequality yields
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\geq \E_K [\bar{\tau}_K (f_{K+1} - f_{\min}) + \|c_K\|_1] - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1.
\end{align*}
Using this lower bound with \eqref{eq:stochasticproof1old}
\begin{equation*}
    \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min}}.
\end{equation*}
Dividing both sides by the summation of $\beta$,
\begin{equation*}
    \frac{1}{\sum_{k=0}^K \beta} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Now, by the definition of $x_{k^*}$, the left hand side is simply
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Using the definition of $\beta$, this becomes
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation*}
\end{proof}

\newpage
\appendix

\section{FEC Notes}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)\},
\eequationNN
where
\bitemize
  \item $\Xbar_k$ is the algorithm iterate in iteration $k$,
  \item $\Gbar_k$ is the stochastic gradient in iteration $k$,
  \item $\Dbar_k$ is the search direction in iteration $k$,
  \item $\overline\Tcal_k$ is the merit parameter in iteration $k$,
  \item $\Sbar_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\overline\Xi_k$ is the ratio parameter in iteration $k$, and
  \item $\overline\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)$ is denoted as
\bequationNN
  (\xbar_k,\gbar_k,\dbar_k,\bar\tau_k,\sbar_k,\bar\xi_k,\bar\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{\Gbar_0,\dots,\Gbar_{k-1}\}$, the realization of which (along with $\Xbar_0 = x_0$) determines the realization of
\bequationNN
  \{\Xbar_j\}_{j=1}^k\ \ \text{and}\ \ \{(\Dbar_j,\overline\Tcal_j,\Sbar_j,\overline\Xi_j,\overline\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

Let us consider a conditional model under the following assumption.
We introduce the following assumption.

\newpage

\bassumption\label{ass:FEC}
  Conditioned on the event $E := E(k_{\max},s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(k_{\max}+1)$th iterate is determined,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\bar\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$, and
    \item in every realization we have $\bar\xi_k = \bar\xi_{-1} = \bar\xi_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$,
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,k_{\max}\}$:
  \bequationNN
    \baligned
      \E[\Gbar_k &| E, \Fcal_k] = \nabla f(\xbar_k), \\
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ \text{and}\ \ 
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2 &| E, \Fcal_k, \nabla f(\xbar_k)^T(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0, \bar\tau_k < \bar\tau_{k-1}] \leq \kappa,
    \ealigned
  \eequationNN
  where $d(\xbar_k,\nabla f(\xbar_k))$ is the step that would be computed at an iterate $\xbar_k$ if the true gradient $\nabla f(\xbar_k)$ were used in the search direction computation.
\eassumption

Going forward, let us define the binary random variable
\bequation %\label{eq:zkdef}
  Z_k = \bcases 1 & \text{if $\nabla f(\xbar_k)^T(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0$ and $\bar\tau_k < \bar\tau_{k-1}$} \\ 0 & \text{otherwise.} \ecases
\eequation
Due to the definition of the event $E$, direct consequences of Assumption~\ref{ass:FEC} are
\bequation\label{eq:probz0}
  \baligned
    \P[Z_k = 1 &| E, \Fcal_k, \Sbar_{k-1} = s_{\max}] = 0 \\ \text{and}\ \ 
    \P[Z_k = 1 &| E, \Fcal_k, \Tbar_{k-1}(1 - \epsilon) < \tau_{\min}] = 0.
  \ealigned
\eequation

\bequationNN
  \P[Z_j = 1 | E, \Fcal_k, \Sbar_{k-1} < s_{\max}, \Tbar_{k-1}(1 - \epsilon) \geq \tau_{\min}]\ \ \text{for $j \in \{k,\dots,k_{\max}\}$}
\eequationNN

Our overall goal is to prove an upper bound (in high probability) on
\bequationNN
  \sum_{k=0}^{k_{\max}} p_k,\ \ \text{where}\ \ p_k := \P[Z_k = 1 | E, \Fcal_k].
\eequationNN
%From total probability and \eqref{temp}:
%\bequationNN
%  \baligned
%    \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k]
%    &= \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} < s_{\max}] \cdot \P[\Sbar_{k_{\max}} < s_{\max} | E, \Fcal_k] \\
%    &+ \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} = s_{\max}] \cdot \P[\Sbar_{k_{\max}} = s_{\max} | E, \Fcal_k]
%  \ealigned
%\eequationNN

As a first step, we prove the following.

\blemma\label{lem:chernoff_new}
  For any $k \in \N{}$, let $\{Y_0,\dots,Y_k\}$ be independent Bernoulli random variables.  Then, for any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, it follows that
  \bequationNN
    \mu := \sum_{j=0}^k \P[Y_j = 1] \geq \ell(s,\delta)\ \ \implies\ \ \P\left[\sum_{j=0}^k Y_j \leq s\right] \leq \delta,
  \eequationNN
  where
  \bequation\label{eq:lsd_new}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
  \eequation
\elemma
\bproof
  By the multiplicative form of Chernoff's bound, it follows for $\rho := 1 - s/\mu$ (which is in the interval $(0,1)$ by (\ref{eq:lsd_new})) that
  \bequationNN
    \P\left[\sum_{j=0}^{k} Y_j \leq s \right] \leq e^{-\frac{\mu \rho^2}{2}} = e^{-\frac{\mu (1-s/\mu)^2}{2}}.
  \eequationNN
  Hence, to prove the result, all that remains is to show that $e^{-\frac{\mu (1-s/\mu)^2}{2}} \leq \delta$, i.e.,
  \bequationNN
    -\frac{\mu(1-s/\mu)^2}{2} \leq \log(\delta)
  \eequationNN
  Using $\log(\delta) = -\log(1/\delta)$, this inequality is equivalent to
  \bequationNN
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta),
  \eequationNN
  which holds if and only if $\mu^2 - 2\mu (s+\log(1/\delta)) + s^2 \geq 0$.  Viewing the left-hand side of this inequality as a convex quadratic function in $\mu$, one finds that the inequality holds as long as $\mu$ is greater than or equal to the positive root of the quadratic, i.e.,
  \bequationNN
    \baligned
      \mu
        &\geq s + \log(1/\delta) + \sqrt{(s+\log(1/\delta))^2 - s^2} \\
        &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2s\log(1/\delta)}.
    \ealigned
  \eequationNN
  Since this holds under assumption in the lemma, the result is proved.
\eproof

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tau_k^{trial}$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ and $\xi_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tau_k^{trial}$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tau_k^{trial}$ occurs, we introduce the following assumption.

\begin{assumption} %\label{assum:ptau}
At every iteration $k$,
\bequation
    \Prob[\bar{g}_k^\top \bar{d}_k + \max\{\bar{d}_k^\top H_k \bar{d}_k,0\} \geq g_k^\top d_k + \max\{d_k^\top H_k d_k,0\} | E, \mathcal{F}_k] \geq p_{\tau}.
\eequation
\end{assumption}
This assumption is satisfied with $p_{\tau}$ when $\bar{g}_k$ is drawn from a Gaussian distrbution \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

This assumption is leads to the following lemma.

\blemma \label{lem:Etautrial_old}
    Let Assumptions \ref{ass:FEC} and \ref{assum:ptau} hold. Let $E_{\tau_k^{trial}}$ be the event that $\tau_k^{trial} < \bar{\tau}_{k-1}$. Then,
    \bequation
        \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, E_{\tau_k^{trial}}] \geq p_{\tau}.
    \eequation
\elemma

\bproof
    TODO: Copy proof from my notes.
\eproof

Due to the above lemma and Assumption \ref{ass:FEC}, it follows that
\bequationNN
    \Prob[E_{\tau_k^{trial}} | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN
In addition, by the definition of $\bar{\tau}_k$,
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, E_{\tau_{k}^{trial}}^c] = 0,
\eequationNN
so 
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN

Now, by Lemma \ref{lem:Etautrial} and the fact that $E_{\tau_{k}^{trial}}$ is not dependent on $\bar{g}_k$, it follows that
\bequation \label{eq:Etrialtaudec_old}
    \Prob[E_{\tau_{k}^{trial}} | \mathcal{F}_k, E, \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E] < p_{\tau}] = 0.
\eequation

Idea from here: Let $\bar{P}_k = \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, \bar{S}_{k-1} < s_{\max}]$ and let $Z_k$ be the indicator of the event that $\bar{\tau}_k < \bar{\tau}_{k-1}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}

Then, by \eqref{eq:Etrialtaudec}, with probability $1-\delta$, the number of occurrences of $E_{\tau_{k}^{trial}}$ is bounded by
\bequationNN
    |E_{\tau_{k}^{trial}}| \leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil.
\eequationNN
Thus, by the definition of $\bar{\tau}_k$, it follows that
\bequationNN
    |\tau_k^{trial} < \bar{\tau}_k|\leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil. 
\eequationNN

\newpage

\section{Mike's Simpler Problem} \label{app:simple}

Let $Y_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:simple1}
  \baligned
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \geq s_{\max}\right] &= 0
  \ealigned
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in [0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:simple2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Y_k = s_{\max} \right].
\eequation

The following lemma proves \eqref{eq:simple2}.
\begin{lemma} \label{lem:simple1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
    \bequationNN
      \baligned
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] &= 0,
      \ealigned
    \eequationNN
    for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in (0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k = s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} p_k + \sum_{k=j}^{k_{\max}} 0 = \sum_{k=0}^{j-1} p_k.
    \end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
    \end{align*}
    which completes the proof.
\end{proof}

The left side of this equation is similar to our goal for the actual problem, while the right is potentially easier to work with. 
A good starting point would be to try to prove a bound on
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right]
\eequationNN
for any $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$.

It clearly follows that
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right] = 1 -  \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right].
\eequationNN
We can find a lower bound on the right hand side of this equation using the following lemma.
\begin{lemma} \label{lem:simple2}
    Let $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$ and let $\hat{Y}_0,\dotsc,\hat{Y}_{\ell}$ be independent \\Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then,
    \bequationNN
        \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    For all $k \in \{0,\dotsc,\ell\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,\ell\}$, let
    \bequationNN 
        \bar{y}_k := \bcases
        1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
        0 & \textrm{otherwise},
        \ecases
    \eequationNN
    and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    \begin{align*}
        \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ are equivalent in distribution to $Y_0, \dotsc, Y_{\ell}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} Y_k < s_{\max}\right],
    \eequationNN
    where the last equality holds because 
    $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ and $Y_0, \dotsc, Y_{\ell}$ are equivalent in distribution.
\end{proof}

We can use these lemmas as well as Lemma \ref{lem:chernoff_new} to get our desired bound in high probability.

\begin{lemma} \label{lem:simple3}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Y_k$ be Bernoulli random variables which satisfy \eqref{eq:simple1}, where $p_k \in (0,1]$. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $\sum_{k=0}^{k_{\max}} p_k \leq \ell(s_{\max},\delta) + 1$. Then, by the definition of $Y_k$, it is clear that
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1
    \eequationNN
    holds deterministically, so the result is trivial in this case. Thus, for the remainder of the proof, we assume that $\sum_{k=0}^{k_{\max}} p_k > \ell(s_{\max},\delta) + 1$.
    
    Now, let $k_{s_{\max},\delta}$ be the minimum integer such that
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} p_k \geq \ell(s_{\max},\delta).
    \eequationNN
    Let $\hat{Y}_0,\dotsc,\hat{Y}_{k_{s_{\max},\delta}}$ be independent Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then, by Lemma \ref{lem:simple2} and Lemma \ref{lem:chernoff_new},
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &\geq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}

%Since the $\hat{Y}_k$ variables are independent, we can use this lemma and the CDF of the binomial distribution to get an exact description of the summation of interest. Alternatively, we can derive a bound for it by using a tail bound, such as Hoeffding's inequality or Chernoff's bound. The second option is likely to be more relevant in the more general setting of our actual algorithm.

What I'd hope a final result to look like:
\bequationNN
    \Prob\left[\sum_{k=0}^{k_{\max}} \Prob\Big[Z_k = 1 \Big| \mathcal{F}_{k}\Big] \leq \ell(s_{\max},\delta)\right] \geq 1 -\delta.
\eequationNN

Update: 2/8/2021

Let $\bar{P}_k = \Prob[Z_k=1| E, \mathcal{F}_k, \bar{S}_{k-1} < s_{\max}]$ and let $\bar{p}_k \in [0,1]$ for all \\$k \in \{0,\dotsc,k_{\max}\}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$ such that $\Prob\left[\left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\right] \neq 0$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}


Old idea:

If
\bequation \label{eq:simple3}
    \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | E, \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] \geq 1-\delta
\eequation
holds for any $\bar{g}_0,\dotsc,\bar{g}_{k_{\max}}$, then we are done because:
\begin{align*}
    &\Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i = 1| \mathcal{F}_i] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{g} \in \mathcal{F}_{k_{\max}}} \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
    &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{k_{\max}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta).
\end{align*}
Unfortunately, when conditioning on a realization from the filtration, we fix both the probabilities as well as whether the events occurred. Thus, the probabilities on the left side of \eqref{eq:simple3} is always 0 or 1.

\section{A Different Problem}
Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:different1}
  \begin{split}
    &\Prob\Bigg[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0,\dotsc,Z_{k-1}\Bigg] \in [0,1] \\ \text{and}\ \
    &\Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] = 0
  \end{split}
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:different2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
\eequation
We prove this inequality in the following lemma.

\begin{lemma} \label{lem:different1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy \eqref{eq:different1}, for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k \geq s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] + \sum_{k=j}^{k_{\max}} 0 \\
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right].
    \end{align*}
    
    %Now, letting $E_j^c$ denote the complement of $E_j$, the definition of $Z_k$ yields
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c \right] = \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \textrm{ for all $k \leq j$.}
    %\eequationNN
    %Thus,
    %\begin{align*}
    %    \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right]
    %    &\geq \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right] \\
    %    &= \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right].
    %\end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
\end{align*}
which completes the proof.
\end{proof}

Next, we would like to derive an analog to Lemma \ref{lem:simple2}.
\begin{lemma} \label{lem:different2}
    Let $p \in \{s_{\max}-1,\dotsc,k_{\max}\}$. Then, there exist independent Bernoulli random variables $\hat{Z}_0, \dotsc, \hat{Z}_p$ which satisfy
    \begin{align*}
        &\Prob\left[\sum_{k=0}^{p} Z_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{p} \hat{Z}_k < s_{\max} \right] \\
        \textrm{and } &\sum_{k=0}^p \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \sum_{k=0}^p \Prob\left[ \hat{Z}_k = 1\right].
    \end{align*}
\end{lemma}

\begin{proof}
    General idea: For any sequence of $\Prob\left[Z_k = 1 \Big| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right]$, there exists a fixed sequence of independent random variables that could generate this sequence in the same way that $\bar{Y}_k$ was generated in Lemma \ref{lem:simple2}. If we can get to that point, believe we can verbatim copy the rest of the proof.
    
    %To begin, note that for all $Z_0,\dotsc,Z_{k_{\max}}$ satisfying \eqref{eq:different1}, there exists a set of independent Bernoulli random variables 
    %$\hat{Z}_0, \dotsc, \hat{Z}_p$ such that
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right].
    %\eequationNN

    %For all $k \in \{0,\dotsc,p\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,p\}$, let
    %\bequationNN 
    %    \bar{y}_k := \bcases
    %    1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
    %    0 & \textrm{otherwise},
    %    \ecases
    %\eequationNN
    %and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    %and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    %\begin{align*}
    %    \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
    %    \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    %\end{align*}
    
    %Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{p}$ are equivalent in distribution to $Y_0, \dotsc, Y_{p}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{p} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{p} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    %\bequationNN
    %    \Prob\left[ \sum_{k=0}^{p} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} Y_k < s_{\max}\right],
    %\eequationNN
    %where the last equality holds because 
    %$\bar{Y}_0, \dotsc, \bar{Y}_{p}$ and $Y_0, \dotsc, Y_{p}$ are equivalent in distribution.
\end{proof}

\begin{lemma}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Z_k$ be Bernoulli random variables which satisfy \eqref{eq:different1}. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1} \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $E$ be the event that 
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}\right] > \ell(s_{\max},\delta).
    \eequationNN
    
    Then, let $K_{s_{\max},\delta}$ be the random variable whose realization $k_{s_{\max},\delta}$ is the minimum integer that satisfies
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}, E\right] \geq \ell(s_{\max},\delta).
    \eequationNN

    Now, for any $Z_0,\dotsc, Z_p$ which satisfies \eqref{eq:different1} and $E$, there exist independent Bernoulli random variables $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s_{\max}},\delta}$ such that
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, E, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right] \textrm{ for all } k \in \{0,\dotsc,k_{s_{\max},\delta}\}.
    \eequationNN

    Then, let $\bar{Z}_0,\dotsc,\bar{Z}_{k_{s_{\max},\delta}}$ be Bernoulli random variables such that
    \begin{align*}
        \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &= \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}


%DETERMINISTIC ANALYSIS BELOW
Given an objective function $f : \R{n} \rightarrow \R{}$ and a
constraint function $c : \R{n} \rightarrow \R{m}$, consider the optimization problem
\begin{equation} \label{eq:fdef}
    \underset{x \in \R{n}}{\min} \enspace f(x) \; \mbox{ s.t. } c(x)=0.
\end{equation}
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) = f(x) + c(x)^\top y$, the first-order stationarity conditions
for \eqref{eq:fdef} are given by
\begin{equation} \label{eq:1on}
    0 = \left[
    \begin{matrix}
    \nabla_x \ell(x,y) \\ \nabla_y \ell(x,y)
    \end{matrix}
    \right]
    = \left[
    \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\ c(x)
    \end{matrix}
    \right].
\end{equation}
Letting $f_k := f(x_k)$, $g_k := \nabla f(x_k)$, $c_k := c(x_k)$, and $J_k := \nabla c(x_k)^\top$ for all $k \in \mathbb{N}$ and given a sequence $\{H_k\}$ satisfying a standard type of sufficiency condition for equality constrained optimization, the SQP subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}
The optimal solution $d_k$ of this subproblem, and an associated Lagrange multiplier $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}
At each iteration, the algorithm uses a merit function with the $\ell_1$-norm penalty function $\phi : \R{n} \times \R{}_+ \rightarrow \R{}$ defined by
\begin{equation} \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1
\end{equation}
where $\tau \in \R{}_+$ is a merit parameter that is updated at each iteration of the algorithm. We use a local model of the merit function $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A useful quantity is the reduction in is model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}

For the purposes of this note, we will declare $x_k$ an approximate solution of (\ref{eq:fdef}) when
\begin{equation} \label{eq:eps1on}
    \|g_k + J_k^\top y_k\| \leq \epsilon  \quad \mbox{ and } \quad \|c_k\| \leq \epsilon,
\end{equation}
both hold for some $k \in \mathbb{N}$. We will derive a worst-case complexity result
in terms of the maximum number of iterations required to find a point statisfying \eqref{eq:eps1on}. We refer the reader to \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the
full definition of the algorithms. To prove our complexity result, we will use the following results which were proven in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}:
\begin{itemize}
    \item The merit parameter $\tau_k$ has an upper and lower bound given by $\tau_{-1} \geq \tau_k \geq \tau_{\min}$ (Lemma 2.14).
    \item The stepsize $\alpha_k$ is lower bounded by $\alpha_{\min}$ (Lemma 2.15).
    \item Let $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$ for all $k \in \mathbb{N}$. Then, by Lemma 2.7,
    \begin{equation} \label{eq:vltc}
        \max\left\{\|v_k\|,\|v_k\|^2\right\} \leq \kappa_v \|c_k\|,
    \end{equation}
    for some $\kappa_v > 0$.
    \item Let $\kappa_{uv}$ and $\zeta$ be strictly positive scalars. Then, by Lemma 2.8,
    \begin{equation} \label{eq:dposcurve}
        \|u_k\|^2 \geq \kappa_{uv} \|v_k\|^2 \implies d_k^\top H_k d_k \geq \frac14 \zeta \|u_k\|^2.
    \end{equation}
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:deltabound}
        \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \frac12 \tau_k \max\{d_k^\top H_k d_k, 0\} + \sigma\|c_k\|_1,
    \end{equation}
    (equation 2.9 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:meritdecrease}
        \phi(x_k + \alpha_k d_k, \tau_k) \leq \phi(x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k),
    \end{equation}
    (Lemma 2.12).
\end{itemize}

Armed with these results, we will prove the following lemma about sufficient decrease in the merit function whenever \eqref{eq:eps1on} does not hold.
\begin{lemma} \label{lem:suffdecrease}
Define
\begin{equation} \label{eq:kappahat}
    \hat{\kappa} := \frac{1}{\sqrt{1+\kappa_{uv}}\max\{\kappa_J,\kappa_H\}\kappa_v}
\end{equation}
and
\begin{equation} \label{eq:kappadec}
    \kappadec := \min\left\{\sigma \hat{\kappa},
    \frac18 \tau_{\min}\zeta\kappa_{uv}\kappa_v^2 \hat{\kappa}^2\right\}.
\end{equation}
Let $\epsilon < 1$ and let at least one of $\|g_k + J_k^\top y_k\| > \epsilon$ and/or $\|c_k\| > \epsilon$ hold. Then,
\begin{equation} \label{eq:suffdecrease}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\end{equation}
\end{lemma}

\begin{proof}
To begin, assume for contradiction that
\bequationNN
\|d_k\| \leq \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\eequationNN
Then, by the definitions of $d_k$ and $y_k$ as well as $\|H_k\| \leq \kappa_H$,
\bequationNN
\|g_k + J_k^\top y_k\| = \|H_k d_k\| \leq \kappa_H \|d_k\| \leq \frac{\epsilon \kappa_H}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
In addition, by the definition of $d_k$ and $\|J_k\| \leq \kappa_J$,
\bequationNN
\|c_k\| = \|J_k d_k\| \leq \kappa_J \|d_k\| \leq \frac{\epsilon \kappa_J}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
Therefore, \eqref{eq:eps1on} holds at $k$, which is a contradiction and we must
have
\begin{equation} \label{eq:dlength}
\|d_k\| > \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\end{equation}

We consider two cases in the rest of the proof. First, let $\|c_k\| \leq \hat{\kappa} \epsilon$. Then, by \eqref{eq:vltc} and $\|c_k\| \leq \hat{\kappa} \epsilon$,
\bequationNN
\|v_k\|^2 \leq \kappa_v^2 \|c_k\|^2 \leq \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
On the other hand, by \eqref{eq:dlength},
\begin{align*}
    \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} &< \|d_k\|^2 \\
    &= \|u_k\|^2 + \|v_k\|^2 \\
    &\leq \|u_k\|^2 + \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies
\begin{align*} \label{eq:ulb}
    \|u_k\|^2 &\geq \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &= \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \frac{ \epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \frac{\kappa_{uv}\epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &\geq \kappa_{uv} \|v_k\|^2.
\end{align*}
Thus, by \eqref{eq:dposcurve}, we have
\bequationNN
d_k^\top H_k d_k \geq \frac14 \zeta\|u_k\|^2 \geq \frac14 \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
Therefore,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} \\
    &\geq \frac18 \tau_{\min} \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies \eqref{eq:suffdecrease} in this case.

Now, presume that $\|c_k\| > \hat{\kappa} \epsilon$ holds. Then, by \eqref{eq:deltabound} and $\epsilon < 1$,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \sigma \|c_k\|_1 \\
    &\geq \sigma \hat{\kappa} \epsilon^2.
\end{align*}
Thus, (\ref{eq:suffdecrease}) holds in this case as well.
\end{proof}

We can use this lemma to prove the following complexity result.

\begin{theorem}
Let
\begin{equation} \label{eq:kbar}
    \bK := \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec} \epsilon^{-2},
\end{equation}
where $\kappadec$ is defined in \eqref{eq:kappadec}.
Presume Assumptions 1 and 2 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} hold.
Then, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in no more than $\bK$ iterations (a similar result holds for Algorithm 2.2 with a revised definition of $\alpha_{\min}$).
\end{theorem}

\begin{proof}
Assume for contradiction that for all iterations $k = 0,1, \dotsc, \bK$, \eqref{eq:eps1on}
does not hold. Then, by Lemma \ref{lem:suffdecrease}, we have
\bequationNN
\Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\eequationNN
Then, at each iteration, by \eqref{eq:meritdecrease},
\begin{align*}
    \phi (x_k + \alpha_k d_k, \tau_k) &\leq \phi (x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k) \\
    &\leq \phi(x_k, \tau_k) - \eta \alpha_{\min} \kappadec \epsilon^2.
\end{align*}
Using the definition of $\phi$ in \eqref{eq:phidef} as well as $x_{k+1} = x_k + \alpha_k d_k$, the above inequality becomes,
\bequationNN
\tau_k f_{k+1} + \|c_{k+1}\|_1 \leq \tau_k f_k + \|c_k\|_1 - \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Summing this inequality for all iterations $k = 0,1, \dotsc, \bK$, we have
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \sum_{k=0}^{\bK} \tau_k (f_{k+1}-f_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Now, by removing the first and last term of the summation, this inequality can be rewritten
as
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \tau_{\bK}f_{\bK+1} - \tau_0 f_0
+ \sum_{k=1}^{\bK} f_k (\tau_{k-1} - \tau_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
By definition, $\tau_k$ is a decreasing sequence. Therefore, we have $\tau_{k-1} - \tau_k \geq 0$
for all $k$. Then, since $\|c_{\bK+1}\|_1 \geq 0$ and $f_k \geq \flow$ holds for all $k$, we have
\bequationNN
- \|c_0\|_1 + \tau_{\bK}\flow - \tau_0 f_0
+ \flow (\tau_{0} - \tau_{\bK}) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Rearranging this inequality, we have
\bequationNN
\bK+1 \leq \frac{\tau_0 (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
\leq \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
= \bK,
\eequationNN
which is a contradiction. Therefore, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in
at most $\bK$ iterations.
\end{proof}
\fi



==> archived_versions/2021-09-10/abstract.tex <==
A worst-case complexity bound is proved for a sequential quadratic optimization (commonly known as SQP) algorithm that has been designed for solving optimization problems involving a stochastic objective function and deterministic nonlinear equality constraints.  Barring additional terms that arise due to the adaptivity of the merit parameter sequence, the proved complexity bound is comparable to that known for the stochastic gradient algorithm for unconstrained nonconvex optimization.  The overall complexity bound, which accounts for the adaptivity of the monotonically nonincreasing merit parameter sequence, shows that a result comparable to the unconstrained setting (ignoring log factors) holds with high probability.

==> archived_versions/2021-09-10/body.tex <==
%******************************************
% Paper-dependent macros here
%******************************************
\newcommand{\flow}{f_{\text{\rm low}}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\kappadec}{\kappa_{\text{\rm dec}}}
\newcommand{\bK}{\bar{K}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\btau}{\bar{\tau}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bg}{\bar{g}}
\newcommand{\bxi}{\bar{\xi}}

\newcommand{\xiktri}{\xi_k^{\rm trial}}
\newcommand{\ktaudec}{\kappa_{\tau_{\rm dec}}}
\newcommand{\kmax}{k_{\max}}
\newcommand{\smax}{s_{\max}}

\newcommand{\dktrue}{d_k^{\text{\rm true}}}
\newcommand{\uktrue}{u_k^{\text{\rm true}}}
\newcommand{\wktrue}{w_k^{\text{\rm true}}}
\newcommand{\yktrue}{y_k^{\text{\rm true}}}
\newcommand{\tktritrue}{\tau_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Dktrue}{D_k^{\text{\rm true}}}

\newcommand{\strue}{s^{\text{\rm true}}}

\newcommand{\Lbad}{\Lcal_{\text{\rm bad}}}
\newcommand{\Lgood}{\Lcal_{\text{\rm good}}}
\newcommand{\Ebad}{E_{\text{\rm bad}}}
\newcommand{\Cdec}{C_{\text{\rm dec}}}
\newcommand{\Idec}{\Ical_{\text{\rm dec}}}
\newcommand{\ktau}{k_{\tau}}
\newcommand{\tcalktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}



\def\Ek#1{E_{k,#1}}
\def\tred#1{\textcolor{red}{#1}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%*********
% Section
%*********

%\newtheorem{assumption}{Assumption}

%\def\proof{\par{\it Proof}. \ignorespaces}
%\def\endproof{{\ \vbox{\hrule\hbox{%
% \vrule height1.3ex\hskip0.8ex\vrule}\hrule
%}}\par}
%\def\noprint#1{}

\section{Introduction} \label{sec:intro}

We consider the analysis of an algorithm for minimizing a smooth, nonlinear function subject to nonlinear equality constraints.  Problems of this form arise in various important applications throughout science and engineering, including optimal control, PDE-constrained optimization, and resource allocation \cite{DPBertsekas_1998,JTBetts_2010,FSKupfer_EWSachs_1992,TRees_HSDollar_AJWathen_2010}.  Unlike the vast majority of the literature on equality constrained optimization, we consider problems in which the objective function is stochastic, in the sense that it is the expected value of a function defined with respect to a random variable.  The algorithm that we consider assumes that evaluations of the objective function and its gradient are intractable to obtain, but that it has access to (unbiased) stochastic gradient estimates.

A few algorithms have been proposed recently for solving problems of this type.  These approaches fall into two categories: penalty based methods \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018} and sequential quadratic optimization (commonly known as SQP) methods \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}.  Penalty methods aim to solve the constrained optimization problem by adding a term to the objective function, weighted by a penalty parameter, that penalizes constraint violation.  Unconstrained optimization techniques are then applied to minimize the resulting penalty function, after which the penalty parameter may be modified, and the minimization performed again, until a solution is obtained that (approximately) satisfies the original constraints.  Methods of this type can be employed successfully, but often perform poorly due to ill-conditioning and/or nonsmoothness of the penalty subproblems. This methodology also often suffers due to sensitivity of the scheme used for updating the penalty parameter.% In addition to these practical issues, little theoretical guarantees are known for the stochastic penalty methods proposed in \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018}.

In practice in both deterministic and stochastic optimization contexts, penalty methods are frequently outperformed by SQP-based methods.  It is commonly accepted in deterministic optimization that one of the state-of-the-art algorithms is an SQP method that chooses stepsizes based on a line search applied to a merit function.  In addition, for deterministic optimization with equality constraints, these algorithms are intimately connected to applying Newton's method to the stationarity conditions of the problem~\cite{RBWilson_1963}.

In this paper, we analyze the worst-case complexity properties of the SQP method proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.  In particular, we prove that, with high-probability, the number of iterations $k$ until the method generates a point at which approximate optimality conditions hold in expectation is $\mathcal{O}(k^{-4})$. This is the first known worst-case complexity result for a method with an adaptive merit function for equality constrained stochastic optimization.  Our result effectively matches the worst-case complexity of stochastic gradient methods with projections for simple constraints \cite{DDavis_DDrusvyatskiy_2019}. Prior to this work, the only known complexity results for stochastic constrained optimization were for problems with simple constraints that enable projection-based methods \cite{DDavis_DDrusvyatskiy_2019,SGhadimi_GLan_HZhang_2016} and Frank-Wolfe type methods to be tractable \cite{EHazan_HLuo_2016} \footnote{MO: Technically, one of Mihai's algorithms has a complexity result, but it requires a-priori knowledge of the merit parameter (aka non-adaptive, set and forget). Should I change this sentence or just mention this later?}. Unfortunately, these approaches do not apply to equality constrained optimization.

Formally, we study the optimization problem
\bequation \label{eq:fdef}
    \underset{x \in \R{n}}{\min} f(x) \; \mbox{s.t.} \; c(x) = 0, \; \; \mbox{with} \; \; f(x) = \E[F(x,\omega)],
\eequation
where $f : \R{n} \rightarrow \R{}$, $c : \R{n} \rightarrow \R{m}$, $\omega$ is a random variable with associated probability space $(\Omega,\mathcal{F}, P)$, $F : \R{n} \times \Omega \rightarrow \R{}$, and $\E$ represents the expectation taken with respect to $P$. We presume that one has access to values of the constraint function and its derivatives, but it is intractable to evaluate the objective and/or its derivatives.

The major technical hurdle in proving a complexity result for stochastic SQP methods arises from their use of an adaptive merit function. Merit functions are a commonly used tools in deterministic constrained optimization, as they provide a way to assess the quality of a step in terms of two (often competing) goals: minimizing the objective function $f$ and reducing the constraint violation in $c$. In our algorithm, we use the $\ell$-1 norm penalty  function $\phi : \R{n} \times \R{}_{>0}$ defined by,
\bequation \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1.
\eequation
Here, $\tau \in \R{}_{>0}$ is the merit parameter which, in our algorithm, is a positive non-increasing sequence $\{\tau_k\}$ that is adaptively chosen at each iteration $k$. The updating behavior of $\tau$ is the core difficulty in providing a complexity result, as the function being optimized at each iteration is modified based on stochastic information. Given that our algorithm uses only a single stochastic gradient at each iteration, the updates to $\tau$ may be based on very poor approximations to the true gradient, causing erratic behavior. We note that even when the sequence $\{\tau_k\}$ is deterministically lower bounded, such as when the noise is deterministically bounded, the complexity analysis is non-trivial as the number of iterations until the sequence $\{\tau_k\}$ settles near its lower bound is itself a random process. The behavior of $\tau$ is difficult to characterize, so previous analyses rely on ``fast-forwarding" to an iterate at which the merit parameter remains constant, greatly simplifying the theoretical challenges \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}. This strategy is not possible when a complexity result is desired however, as the behavior of the full iterate sequence must be analyzed instead.

We wish to stress here that while our techniques are developed for an SQP method which uses the merit function in \eqref{eq:phidef}, they may be applicable to a wide variety of algorithmic frameworks for stochastic optimization with deterministic constraints. The approaches used can be modified to apply to methods which adaptively update critical parameters at each iteration, such as adaptive penalty methods \cite{RHByrd_GLopez-Calva_JNocedal_2012,RHByrd_JNocedal_RAWaltz,MMongeau_ASartenaer_1995}, adaptive augmented Lagrangian \cite{FECurtis_HJiang_DPRobinson_2015}, adaptive barrier methods \cite{JNocedal_AWachter_RAWaltz_2009}, and penalty-interior point methods \cite{FECurtis_2012}. In addition, many constrained algorithms generate repeated (often unconstrained) subproblems defined by an auxilliary parameter sequence which is updated dynamically based off of the solution to the previous subproblem. Algorithms of this type include penalty methods, augmented Lagrangian methods, and interior point methods \cite{JNocedal_SJWright_2006}. In the case where the objective is stochastic, this auxilliary sequence would also be a random variable, the behavior of which would be paramount to proving a complexity result for this type of method. Thus, we believe that the techniques we derive for our SQP method are broadly applicable and foundational for performing a  complexity analysis of deterministically constrained stochastic optimization methods.

We note here that other stochastic SQP methods have been proposed in the literature \cite{SNa_MAnitescu_KMladen_2021}. These methods are either non-adaptive, in the sense that the merit parameter must be fixed a-priori, or require high-accuracy gradient estimates at each iteration. Due to this, we focus on the algorithmic framework developed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

\subsection{Outline of Complexity Result} \label{subsec:complexitypreview}

In this section, we provide a sketch of our complexity result and describe how it compares to other results in the literature. Our result is proved under relatively common smoothness conditions on $f$ and $c$ as well as the linear independence constraint qualification (LICQ). We assume that, conditioned on some event $E$, the stochastic gradients are unbiased estimators of $\nabla f(x)$ with variance bounded by $M$, as is standard in the literature. Additionally, we assume that the stochastic gradients exhibit a bounded measure of asymmetry, the merit parameter sequence $\{\tau_k\}$ is lower bounded by some $\tau_{\min} > 0$, and the number of iterations at which $\tau_k$ is decreased is bounded by a positive integer $s_{\max}$ (this last condition is gauranteed by the definition of our algorithm under the rest of the assumptions). These last three assumptions are required to ensure that the merit function is well behaved with high probability, even though it is being updated based on stochastic gradient information. Exact definitions of these assumptions can be found in Section \ref{subsec:assumptions}.

Under the conditions listed above, after performing $k_{\max}+1$ iterations, our algorithm generates a point $x_{k^*}$ which satisfies, with probability at least $1-\delta$,
\bequation \label{eq:bigOcomplexity}
    \begin{split}
   \E[\|\nabla f(x_{k^*}) &+ J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c(x_{k^*})\| |
    E] \\
   &= \mathcal{O}\left(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c(x_0)\|_1 + M + (\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\right),
   \end{split}
\eequation
where $J_{k^*}$ is the Jacobian of the constraints at the point $x_{k^*}$, $y_{k^*}^{true}$ is the Lagrange multiplier at $x_{k^*}$, and $f_{\min}$ is a lower bound on $f(x)$.

The form of this result is commonly referred to as a convergence rate, however it can be easily manipulated into a worst-case complexity result. In terms of finding a point, $x_{k^*}$, such that $\E[\| \nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\| |E] \leq \varepsilon$ and $\E[\sqrt{\|c(x_{k^*})\|}|E] \leq \varepsilon$, by Jensen's inequality, our algorithm requires at most $\Ocal(\varepsilon^{-4})$ iterations.
As such, we use the terms complexity and convergence rate interchangably throughout.

The first three quantities in this result are essentially the same as those for the stochastic gradient method, representing the initial function gap as well as the variance. This is to be expected, given our mild assumptions on the matrices used in the quadratic subproblem at each iteration as well as the use of a single stochastic gradient at each iteration.

The final two terms are unique to our setting and arise due to the having a potentially poor initial estimate of $\tau_{\min}$. Given oracle knowledge of $\tau_{\min}$, these last two terms could be removed by choosing $\tau_{-1} \leq \tau_{\min}$ (as is done in the non-adaptive algorithm of \cite{SNa_MAnitescu_KMladen_2021}). However, this quantity is unknown so careful attention must be paid to the behaivor of the $\{\tau_k\}$ sequence to obtain a complexity result. The result holds in high probability due to the possibility of having an excessive number of iterations at which the computed $\tau_k$ is significantly larger than the value that the merit parameter would take if the step direction and merit parameter update were computed using the full gradient. On these types of iterations, the requirement for a bounded measure of asymmetry in the distribution of the stochastic gradients guarantees that there is always some nonzero probability of decreasing $\tau$. However, there still may exist realizations (which are guaranteed to occur with probability no more than $\delta$), where $\tau$ is ``too large" for enough iterations that the above complexity result does not hold.

We note that in terms of an overall complexity result with respect to the gradient of the Lagrangian, with probability at least $1-\delta$, we obtain a result which is the same order as the complexity result derived in \cite{DDavis_DDrusvyatskiy_2019}, whenever $s_{\max}$ satisfies a reasonable bound. Due to the definition of our algorithm, $s_{\max} = \mathcal{O}(\log(\tau_{\min}))$ for all sufficiently large $k_{\max}$. Thus, it follows that this complexity result gives an informative bound whenever $\tau_{\min}$ does not grow exponentially in $k_{\max}$. We prove that this is the case for sub-Gaussian distributions in Section \ref{subsec:subgauss}, where we show that, with probability at least $1-\delta$, $\tau_{\min} = \mathcal{O}(\log(\frac{k_{\max}}{\delta}))$ and
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O}\left(\frac{\log \log \frac{k_{\max}}{\delta}}{\sqrt{k_{\max}+1}}\right).
\eequationNN

\subsection{Notation}

Our algorithm is iterative, generating a sequence of iterates $\{x_k\}$. We also append the iteration number to other quantities corresponding to each iteration, e.g., $f_k := f(x_k)$. We denote the Jacobian of $c$ by $J_k := \nabla c(x_k)^\top$.

We adopt the notation that $\|\cdot\|$ is the $\ell$-2 norm for vectors and is the induced $\ell$-2 norm for matrices. We denote by $\mathbb{S}^{n}$ the set of $n \times n$ dimensional symmetric matrices. The set of natural numbers is denoted as $\N{} := \{0,1,2,\dots,\}$. For an integer $k \in \N{}_{>0}$, we use the notation $[k]$ to define the set $[k] := \{0,\dots,k\}$. We denote a set of vectors $v_{[k]} := \{v_0,\dots,v_k\}$.

When discussing stochastic quantities, we use capital letters to denote the random variable and lower case letters to denote a realization of that random variable. For example, for the stochastic gradients at iteration $k$, $G_k$ denotes the random variable while $g_k$ is a realization of this random variable.

\subsection{Outline}

In the following section, we give an overview of the sequential quadratic programming framework and describe our algorithm. In Section \ref{sec:complexity}, we describe our assumptions on the stochastic gradients and prove our complexity result. We also provide examples of distributions under which our assumptions hold with high-probability. Finally, we provide some concluding thoughts and future directions in Section \ref{sec:conclusion}.

\section{Algorithm}

We make the following assumption about the optimization problem \eqref{eq:fdef} and the algorithm that we analyze, which generates a sequence of iterates $\{x_k\} \subset \R{n}$.

\begin{assumption} \label{assum:fcsmooth}
    There exists a convex set $\mathcal{X} \subseteq \R{n}$ that contains the iterates $\{x_k\}$ for any realization of Algorithm \ref{alg:ssqp}. The objective function $f : \R{n} \rightarrow \R{}$ is continuously differentiable and bounded below over $\mathcal{X}$, and its gradient $\nabla f: \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $L$ and is bounded over $\mathcal{X}$. The constraint function $c : \R{n} \rightarrow \R{m}$ (where $m \leq n$) and its Jacobian $\nabla c^\top : \R{n} \rightarrow \R{m\times n}$ are bounded over $\mathcal{X}$, each gradient $\nabla c_i : \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $\gamma_i$ over $\mathcal{X}$ for all $i=\{1,\dots,m\}$, and the singular values of $\nabla c^\top$ are bounded away from zero over $\mathcal{X}$.
\end{assumption}

This assumption is largely standard smoothness requirements. However, requiring that the iterates remain in a convex set over which the gradient of $f$ and Jacobian of $c$ are bounded is a stronger assumption than those commonly made for unconstrained stochastic gradient methods. Indeed, even if $f$ has bounded level sets, there is no guarantee that the iterates will remain in any specific level set, as stochastic gradient methods are not descent methods. However, we believe that this is a more reasonable assumption due to the inclusion of constraints, which drive the iterates towards the {\it deterministic} constrained region. Finally, we note that the requirement on the Jacobian of $c$ to have singular values which are bounded away from zero holds for any constraint set that satisfies LICQ.

Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) := f(x) + c(x)^\top y$, first-order stationarity conditions for \eqref{eq:fdef}, which are necessary due to LICQ, are given by
\bequation \label{eq:optconds}
    0 =
    \left[ \begin{matrix}
        \nabla_x \ell(x,y) \\
        \nabla_y \ell(x,y)
    \end{matrix} \right]
    =
    \left[ \begin{matrix}
        \nabla f(x) + \nabla c(x) y \\
        c(x)
    \end{matrix} \right].
\eequation
As seen in \eqref{eq:bigOcomplexity}, our goal in this work is to prove a bound on the number of iterations required to find an approximate solution in terms of the gradient of the Lagrangian and the constraint violation.

\subsection{Merit Function}

In Section \ref{sec:intro}, we introduced our $\ell$-1 penalty merit function in \eqref{eq:phidef}. The merit parameter $\tau$ is adaptively updated at each iteration and is used to define our line search procedure. We use a local model of the merit function $q : \R{n} \times \R{}_{>0} \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A key quantity in our algorithm is the reduction in the model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\Delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation} \label{eq:deltadef}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}
The reduction in the model of the merit function is a critical component of our complexity analysis. We will show that this can be used to give an upper bound on the merit function decrease at each iteration and thus it plays a similar role to the norm of the gradient squared in the analysis of stochastic gradient methods.

\subsection{Algorithm Preliminaries}

The algorithm that we develop for solving \eqref{eq:fdef} is based on a stochastic SQP paradigm. Specifically, at iteration $k$, a stochastic gradient estimate, $g_k$, is obtained (assumptions on the properties of $g_k$ can be found in Section \ref{subsec:assumptions}). Then, a search direction is computed by solving a quadratic optimization subproblem based on a stochastic local quadratic model of $f$ and a local affine model of $c$ about $x_k$. Letting $f_k := f(x_k)$, $c_k = c(x_k)$, and $J_k := \nabla c(x_k)^\top$ and given a sequence $\{H_k\}$ satisfying Assumption \ref{assum:Hk} below (a standard type of sufficiency condition for equality constrained optimization), this subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}

The optimal solution, $d_k$, of this subproblem, and an associated Lagrange multiplier, $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}


\begin{assumption} \label{assum:Hk}
    The sequence $\{H_k\}$ is bounded in norm by $\kappa_H \in \R{}_{>0}$. In addition, there exists a constant $\zeta \in \R{}_{>0}$ such that, for all $k = \{0,\dots,k_{\max}\}$, the matrix $H_k$ has the property $u^\top H_k u \geq \zeta \|u\|_2^2$ for all $u \in \R{n}$ such that $J_k u = 0$.
\end{assumption}

We stress that our algorithm and analysis does {\it not} assume that $H_k$ is a stochastic approximation of the Hessian of the Lagriangian at $x_k$ for some multiplier $y_k$. We merely assume that the sequence $\{H_k\}$ satisfies Assumption \ref{assum:Hk}.

Under Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk}, the following result is well known in the literature.

\blemma
    The linear system \eqref{eq:sqpsystem} has a unique solution.
\elemma

\subsection{Algorithm}

\begin{algorithm}[ht]
  \caption{Stochastic SQP Algorithm}
  \label{alg:ssqp}
  \begin{algorithmic}[1]
    \Require $x_0 \in \R{n}$; $\tau_{-1} \in \R{}_{>0}$; $\epsilon \in (0,1)$; $\sigma \in (0,1)$; $\xi_{-1} \in \R{}_{>0}$; $\kmax \in \N{}$; $\{\beta_k\} \subset (0,1]$; $\theta \in \R{}_{\geq0}$; $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$
    \For{\textbf{all} $k \in \{0,1,\dotsc,\kmax\}$}
	  \State Compute $(d_k,y_k)$ as the solution of \eqref{eq:sqpsystem}
	  \If{$d_k = 0$}
	    \State Set $\tau_k^{trial} \gets \infty$, $\tau_k \gets \tau_{k-1}$, $\xi_k^{trial} \gets \infty$, and $\xi_k \gets \xi_{k-1}$
	    \State Set $\widehat\alpha_{k,\text{init}} \gets 1$, $\widetilde\alpha_{k,\text{init}} \gets 1$, and $\alpha_k \leftarrow 1$
	  \Else\ (if $d_k \neq 0$)
	    \State Set $\tau_k^{trial}$ by \eqref{eq:tautrial} and $\tau_k$ by \eqref{eq:taudef} %\label{step.tau_stochastic}
	    \State Set $\xi_k^{trial}$  and $\xi_k$ by \eqref{eq:xidef} %\label{step.xi}
        \State Set
        \bequationNN
          \widehat\alpha_{k,\text{init}} \gets \tfrac{\beta_k\Delta q(x_k,\tau_k,g_k,H_k,d_k)}{(\tau_k L_k + \Gamma_k)\|d_k\|_2^2}\ \ \text{and}\ \  \widetilde\alpha_{k,\text{init}} \gets \widehat\alpha_{k,\text{init}} - \tfrac{4\|c_k\|_1}{(\tau_k L_k +  \Gamma_k)\|d_k\|_2^2}
        \eequationNN
        \State Set $\widehat\alpha_k \gets \proj_k(\widehat\alpha_{k,\text{init}})$ and $\widetilde\alpha_k \gets \proj_k(\widetilde\alpha_{k,\text{init}})$, then \label{step.alpha_projection_stochastic} \label{step.alpha_stochastic}
        \bequationNN
          \alpha_k \gets
		    \bcases
		      \widehat\alpha_k & \text{if $\widehat\alpha_k < 1$} \\
		      1 & \text{if $\widetilde\alpha_k \leq 1 \leq \widehat\alpha_k$} \\
		      \widetilde\alpha_k & \text{if $\widetilde\alpha_k > 1$}
		    \ecases
        \eequationNN
      \EndIf
      \State Set $x_{k+1} \gets x_k + \alpha_k d_k$
    \EndFor
    \State Sample $k^* \in \{0, \dotsc, \kmax\}$ according to the probability distribution
    \bequationNN
        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
    \eequationNN
    \Return $x_{k^*}$
  \end{algorithmic}
\end{algorithm}

After the search direction $d_k$ is computed, the merit parameter $\tau_k$ is updated. This is done by first setting, for some $\sigma \in (0,1)$, a trial value $\tau_k^{trial} \in \R{}_{>0} \cup  \{\infty\}$ by 
\bequation \label{eq:tautrial}
    \tau_k^{trial}\gets
    \begin{cases}
        \infty & \mbox{if $g_k^\top d_k + \max\{d_k^\top H_k d_k, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{g_k^\top d_k + \max\{d_k^\top H_k d_k,0\}} & \mbox{otherwise,}
    \end{cases}
\eequation
(If $c_k = 0$, then it follows from \eqref{eq:sqpsystem} and Assumption \ref{assum:Hk} that $d_k^\top H_k d_k \geq 0$ and $g_k^\top d_k + d_k^\top H_k d_k = 0$, meaning $\tau_k^{trial} \gets \infty$. Hence, $\tau_k^{trial} < \infty$ requires $\|c_k\|_1 > 0$, in which case $\tau_k^{trial} > 0$.) Then, the merit parameter is set, for some $\epsilon \in (0,1)$, by
\bequation \label{eq:taudef}
    \tau_k \gets \bcases
        \tau_{k-1} & \mbox{if $\tau_{k-1} \leq \tau_k^{trial}$} \\
        (1-\epsilon)\tau_k^{trial} & \mbox{otherwise,}
    \ecases
\eequation
which ensures that $\tau_k \leq \tau_k^{trial}$ and,
\bequation \label{eq:qquadlb}
    \Delta q(x_k,\tau,g_k,H_k,d_k) \geq \frac12 \tau \max\{d_k^\top H_k d_k, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
for any $\tau \leq \tau_k$.

Our algorithm adaptively estimates a lower bound for the ratio between the reduction in the model of the merit function and the merit parameter times the squared norm of the search direction. This is used to determine an interval into which the stepsize will be projected; control of this parameter is paramount to ensure convergence in expectation. We set
\bequation \label{eq:xidef}
    \xiktri \gets \frac{\Delta q(x_k, \tau_k, g_k, H_k, d_k)}{\tau_k \|d_k\|^2}
    \; \mbox{ then } \;
    \xi_k \gets \bcases
        \xi_{k-1} & \mbox{if }\xi_{k-1} \leq \xiktri \\
        (1-\epsilon)\xiktri & \mbox{otherwise,}
    \ecases
\eequation
which ensures $\xi_k \leq \xiktri$ for all $kb$. In previous work, it was show that $\{\xi_k\}$ is bounded away from zero {\it deterministically} \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

For generality, Algorithm \ref{alg:ssqp} is stated with Lipschitz constant estimates $\{L_k\}$ and $\{\Gamma_k\}$ given as inputs (with the idea that $\Gamma_k := \sum_{i \in 1,\dots,m} \gamma_{k,i}$ for all $k$). Our analysis in the next section presumes that Lipschitz constants are known, although in practice these can be estimated using standard techniques (see, e.g., \cite{FECurtis_DPRobinson_2019}) in an attempt to ensure that the same convergence results hold for the case where the constants are known. The sequence $\{\beta_k\}$ is introduced to control the setpsizes. Throughout most of the analysis, the sequence $\{\beta_k\}$ can be chosen arbitrarily. However, our final complexity result is established for a fixed step size of $\beta_k = \mathcal{O}(1/\sqrt{k_{\max}+1})$ for all $k\in\{0,\dots,k_{\max}\}$. We define
\bequationNN
    \mbox{Proj}_k(\cdot) := \mbox{Proj}\left(\cdot \; \Bigg| \left[\frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k}, \frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k} + \theta \beta_k^2 \right]\right),
\eequationNN
where $\mbox{Proj}(\cdot \; | \; \mathcal{I})$ represents the projection operator onto the interval $\mathcal{I} \subset \R{}$.

We remark that the only substational changes from Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} are the fixed iteration count, $k_{\max}$, and the inclusion of a return value, $x_{k^*}$. Our method of sampling $k^*$ is consistent with the literature \cite{DDavis_DDrusvyatskiy_2019} and amounts to uniform sampling when a fixed step size sequence is employed.

%\balgorithm
%\caption{A Stochastic SQP Algorithm}
%\label{alg:ssqp}
%    \balgorithmic[1ht!]
%        \Require $x_0 \in \R{n};$ $\bar{\tau}_{-1} \in \R{}_{>0}$; $\epsilon \in (0, 1)$; $\sigma \in (0, 1);$ $\bar{\xi}_{-1} \in \R{}_{>0}$; $\{\beta_k\} \subset \R{}_{>0}$; $\theta \in \R{}_{>0};$ $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$; $K \in \N{}$
%        \State Run Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for $k = 0, \dotsc, K$
%        \State Sample $k^* \in \{0, \dotsc, K\}$ according to the probability distribution
%        \bequationNN
%        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
%        \eequationNN
%        \Return $x_{k^*}$
%    \ealgorithmic
%\ealgorithm

\section{Complexity Analysis} \label{sec:complexity}

In this section, we will prove our complexity result. We begin by describing our algorithm as a random process as well as the assumptions that we make on our stochastic gradient estimates (Section \ref{subsec:assumptions}). Then, we repeat (and sometimes slightly modify) a number of key lemmas from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} about Algorithm \ref{alg:ssqp} (Section \ref{subsec:algprops}). Afterwards, we present our complexity analysis and prove the result previewed in Section \ref{subsec:complexitypreview} (Section \ref{subsec:complexity}). We conclude this section by discussing distributions for which our assumptions are satisfied with high-probability (Section \ref{subsec:subgauss}) and outline a complexity result which relaxes one of our assumptions slightly (Section \ref{subsec:ratioparam}).

Our analysis relies on the orthogonal decomposition of the search directions given by $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$. We note here that conditioned on the algorithm having reached $x_k$ at iteration $k$, the normal component, $v_k$, is {\it deterministic}, depending only on the constraint value $c_k$ and the Jacobian $J_k$.

In addition to the quantities $d_k$, $y_k$, and $\tau_k^{trial}$ which are computed at each iteration using the stochastic gradient $g_k$, the following analysis relies on the quantities $\dktrue$, $\yktrue$, and $\tktritrue$ which are computed using the true gradient, $\nabla f(x_k)$. Specifically, let
\bequation \label{eq:sqpsystemdet}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    \dktrue \\ \yktrue
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    \nabla f(x_k) \\ c_k
    \end{matrix}
    \right]
\eequation
and
\bequationNN
    \tktritrue \gets
    \begin{cases}
        \infty & \mbox{if $\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}} & \mbox{otherwise}.
    \end{cases}
\eequationNN
Finally, we let $\dktrue = \uktrue + v_k$, where $\uktrue \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.

The definition of $\tktritrue$ guarantees that
\bequation \label{eq:qquadlbtrue}
    \Delta q(x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \frac12 \tau \max\{(\dktrue)^\top H_k \dktrue, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
holds for any $\tau \leq \tktritrue$.

\subsection{Algorithm \ref{alg:ssqp} as a Stochastic Process and Assumptions} \label{subsec:assumptions}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(X_k,G_k,D_k,\Tcal_k,S_k,\Xi_k,R_k,\Acal_k)\},
\eequationNN
where
\bitemize
  \item $X_k$ is the algorithm iterate in iteration $k$,
  \item $G_k$ is the stochastic gradient in iteration $k$,
  \item $D_k$ is the search direction in iteration $k$,
  \item $\Tcal_k$ is the merit parameter in iteration $k$,
  \item $S_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\Xi_k$ is the ratio parameter in iteration $k$,
  \item $R_k$ is the number of ratio parameter decreases up to the end of iteration $k$, and
  \item $\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(X_k,G_k,D_k,\Tcal_k, S_k,\Xi_k,R_k,\Acal_k)$ is denoted as
\bequationNN
  (x_k,g_k,d_k,\tau_k,s_k,\xi_k,r_k,\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{G_0,\dots,G_{k-1}\}$, the realization of which (along with $X_0 = x_0$) determines the realization of
\bequationNN
  \{X_j\}_{j=1}^k\ \ \text{and}\ \ \{(D_j,\Tcal_j,S_j,\Xi_j,R_j,\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration. We condition on a specific realization of Algorithm \ref{alg:ssqp} up to iteration $k$, using the notation $g_{[k-1]}$, while we condition on $\Fcal_{k}$ to denote conditioning on all realizations of $G_{[k-1]}$ that are measurable with respect to the filtration $\Fcal_{k}$.

We consider a conditional model under the following assumption.

\bassumption\label{assum:eventE}
  Conditioned on the event $E := E(\kmax,s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    %\item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\xi_k = \xi_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E, g_{[k-1]}] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E, g_{[k-1]}] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E, g_{[k-1]}, \nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \leq \ktaudec.
    \ealigned
  \eequationNN
\eassumption


The requirements on $G_k$ to be an unbiased estimator of $\nabla f(x_k)$ with bounded variance are standard for stochastic gradient methods. However, unlike the unconstrained setting, additional assumptions are required. The assumption on the existence of a $\tau_{\min} > 0$ is similar to Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, under which a global convergence result was proven. In Lemma 2.16 of the same work, it was proven that $\tktritrue$ has a deterministic lower bound. Based on this result, without loss of generality, we assume that $\tktritrue \geq \tau_{\min}$ holds for all $k$. In Proposition 3.18 of the same paper, the authors show that $\tau_{\min}$ exists with probability 1 whenever $G_k$ is a bounded random variable. We extend this result to show that $\tau_{\min}$ exists with high probability when $G_k$ follows a sub-Gaussian distribution in Section \ref{subsec:subgauss}.

By the definition of Algorithm \ref{alg:ssqp}, it should be clear that $s_{\max}$ in Assumption \ref{assum:eventE} must exist. Under the condition that $\tau_{\min} > 0$ exists, it follows that
\bequation \label{eq:smaxbound}
    s_{\max} \leq \min\left\{\kmax+1, \left\lceil\frac{\log(\tau_{\min}/\tau_{-1})}{\log(1-\epsilon)}\right\rceil\right\}.
\eequation
For the purposes of our analysis and results, we keep $s_{\max}$ decoupled from the above inequality as it is a fundamentally necessary component in order to guarantee that our results holds with high probability.

For convenience in the analysis, we make the assumption that the ratio parameter sequence $\{\xi_k\}$ is fixed. This sequence has a deterministic lower bound, as proven in Lemma 3.5 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, unlike the merit parameter sequence. In addition, this sequence is unique to our algorithm (and the algorithm in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}), while merit functions are a commonly used tool in constrained optimization. For this reason, we focus our attention on the properties of the merit parameter sequence instead. The approaches we develop for the merit parameter sequence can be applied to ratio parameter sequence as well. We outline a complexity result where both parameters are adaptively updated in Section \ref{subsec:ratioparam}.

Our final assumption requires that the stochastic gradient estimate is bounded in absolute value when conditioned on the event that $\tau_k < \tau_{k-1}$ and $\nabla f(x_k)^\top (d_k - \dktrue) < 0$ hold simultaneously. This event is fundamental in the analysis, as it arises naturally using $\Delta q(\cdot)$ as a measure of decrease in $\phi$ (see Lemma \ref{lem:phidecrease}). 
We remark that this inequality holds with high-probability whenever $G_k$ follows a sub-Guassian distribution with $\ktaudec = \Ocal(\log (k_{\max}))$. We prove this result in Section \ref{subsec:subgauss}.

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tktritrue$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tktritrue$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tktritrue$ occurs, we introduce the following assumption.

\begin{assumption} \label{assum:ptau}
At every iteration $k \in \{0,\dots,k_{\max}\}$,
\bequation
    \begin{split}
        \Prob[G_k^\top D_k &+ \max\{D_k^\top H_k D_k,0\} \\
        &\geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | E, g_{[k-1]}] \geq p_{\tau},
    \end{split}
\eequation
for some $p_{\tau} \in (0,1]$.
\end{assumption}
This assumption boils down to the distribution of $G_k$ having a bounded measure of asymmetry and is unique to our setting. It guarantees that there is always at least $p_{\tau}$ probability that $\tau_k$ decreases at any iteration for which $\tau_k$ would decrease if the step (and $\tau$ update) were computed using the full gradient, $\nabla f(x_k)$, as opposed to the stochastic gradient, $g_k$. This property ensures that, with high probability, $\tau_k$ is not larger than it ``should" be on too many iterations.

In \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, it was shown that this assumption is satisfied with $p_{\tau} = \frac12$ when $G_k$ is drawn from a Gaussian distribution. We show that this result can be extended to all distributions that obey a mild form of symmetry in Section \ref{subsec:subgauss}.

\subsection{Properties of Algorithm \ref{alg:ssqp}} \label{subsec:algprops}

Here we repeat a number of key results from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} that will be integral to our complexity analysis.

By Lemma 2.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for all $k = \{0,\dots,k_{\max}\}$, there exists $\kappa_{uv} \in \R{}_{>0}$ such that, if $\|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2$, then $\frac12 (\dktrue)^\top H_k \dktrue \geq \frac14 \zeta \|\uktrue\|^2$, where $\zeta$ is defined in Assumption \ref{assum:Hk}. Then, let
\bequationNN
    \Psi_k := \begin{cases}
        \|\uktrue\|^2 + \|c_k\| & \mbox{if } \|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2 \\
        \|c_k\| & \mbox{otherwise.}
    \end{cases}
\eequationNN
Now we can state a few lemmas which are relevant to our final complexity result.
\begin{lemma} \label{lem:kappapsi}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_{\Psi} \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$, the search true direction and constraint violation satisfy $\|\dktrue\|^2 + \|c_k\| \leq (\kappa_{\Psi} + 1) \Psi_k$.
\end{lemma}

\begin{proof}
    The result follows directly from Lemma 2.11 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

\begin{lemma} \label{lem:kappaq}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_q \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$ and any $\tau \leq \tktritrue$, the reduction in the model of the merit function satisfies $\Delta q (x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \kappa_q \tau \Psi_k$.
\end{lemma}

\begin{proof}
    The proof follows from \eqref{eq:qquadlbtrue} combined with the proof of Lemma 2.12 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and the a specific realization $g_{[k-1]}$.

Now, we can state a lemma about the expected values of a number of random variables in our algorithm.

\blemma \label{lem:dexpectation}
Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. For all $k = \{0,\dots,k_{\max}\}$, $\E_k[D_k] = \dktrue$, $\E_k[U_k] = \uktrue$, and $\E_k[Y_k] = \yktrue$.  Moreover, there exists $\kappa_d \in \R{}_{>0}$, independent of $k$, such that,
\bequationNN
\left\|\left[\begin{matrix}
H_k & J_k^\top \\
J_k & 0
\end{matrix}\right]\right\| \leq \kappa_d.
\eequationNN
In addition, $\E_k[\|D_k - \dktrue\|] \leq \kappa_d \sqrt{M}$, and $\E_k[\|D_k - \dktrue\| | E, \mathcal{F}_k, \nabla f(x_k)^\top (D_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \leq \kappa_d \ktaudec$.
\elemma

\bproof
    Except for the final inequality, the result is proven in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. To see the final inequality, we note that by the same argument as in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for any realization of $G_k$ and $D_k$,
    \bequationNN
        \|d_k - \dktrue\| \leq \kappa_d \|g_k - \nabla f(x_k)\|.
    \eequationNN
    Therefore,
    \begin{align*}
        &\E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \E_k[\|G_k - \nabla f(x_k)\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \ktaudec.
    \end{align*}
\eproof

Next, we provide some bounds on the expectation of a few key quantities.

\blemma\label{lem:product_bounds}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequationNN 
    \begin{split}
        \nabla f(x_k)^\top \dktrue &\geq \E_k[G_k^\top D_k] \geq \nabla f(x_k)^\top \dktrue - \zeta^{-1}M\ \ \text{and} \\ \E_k[D_k^\top H_k D_k] &\geq (\dktrue)^\top H_k \dktrue.
    \end{split}
  \eequationNN
\elemma

\bproof
    The result is proven in Lemma \cite[Lemma 3.9]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

We conclude this section with a lemma that will allow us to characterize descent in $\phi$ in terms of $\Delta q(\cdot)$.

\blemma\label{lem:phidecrease}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Suppose that $\{\beta_k\}$ is chosen such that $\beta_k \xi_k \tau_k/(\tau_k L + \Gamma) \in (0,1]$ for all $k \in \{0,\dots,k_{\max}\}$.  Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequation \label{eq:phidecrease}
    \baligned
      \phi(x_k + \alpha_k d_k, \tau_k) - \phi(x_k, \tau_k)
      &\leq -\alpha_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue) \\
      &\quad + \thalf \alpha_k \beta_k  \Delta q(x_k,\tau_k,g_k,H_k,d_k) \\
      &\quad + \alpha_k \tau_k \nabla f(x_k)^\top (d_k - \dktrue),
    \ealigned
  \eequation
  where $d_k$ and $\dktrue$ are respectively defined by \eqref{eq:sqpsystem} and \eqref{eq:sqpsystemdet}.
\elemma

\bproof
    The result follows directly from Lemma 3.7 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

\subsection{Complexity Result} \label{subsec:complexity}

In this section, we present our complexity result under the condition that Assumption \ref{assum:eventE} occurs. We derive our result in largely the same way as the global convergence result in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, with two major changes, which stem from the need to characterize the behavior of the algorithm with respect to the merit parameter updating. At a high-level, the two modifications are as follows:
\begin{enumerate}
    \item We derive a new upper bound for the last term in \eqref{eq:phidecrease}. This inequality allows us to characterize decrease in the merit function and is central to the overall analysis. A new upper bound is needed in our setting, as this final term is the product of three random variables while $\tau$ is still being adaptively updated and has not settled at a lower bound. To handle this, we show that this term is bounded, under Assumption \ref{assum:eventE}, in terms of the probability that the event $\Ek3$ (defined formally below) occurs at iteration $k$. This event only occurs on iterations $k$ where $\tau_k < \tau_{k-1}$ which, when combined with a maximum of $s_{\max}$ decreases of $\tau$ due to Assumption \ref{assum:eventE}, allows us to obtain a bound on this quantity that holds with high-probability. The new upper bound is derived in Lemma \ref{lem:innerprod} while our high-probability bound on the summation (over $k=0,\dots,k_{\max}$) of the probabilities of $\Ek3$ occuring is presented in Lemma \ref{lem:Eksumlsmax}.
    \item We characterize iterations at which $\tktritrue < \tau_k$ occurs. These iterations are problematic for the analysis due to the inclusion of $\tau_k$ in $\Delta q(x_k,\tau_k,\nabla f(x_k), H_k, \dktrue)$, which is used during the analysis to measure progress in the algorithm. One particular concern arises in the final complexity result; if $k^*$ occurs at an iterate such that $\tau_{k^*}^{trial,\text{true}} < \tau_{k^*}$, then $\Delta q(x_{k^*},\tau_{k^*},\nabla f(x_{k^*}), H_{k^*}, d^{\text{true}}_{k^*})$ cannot be related to our optimality conditions \eqref{eq:optconds}. To solve this issue, we introduce a theoretical sequence, $\hat{\tau}_k$, which, for all $k$, is the minimum of $\tau_k$ and $\tktritrue$, and analyze the algorithm's progress with respect to this sequence. Due to Assumption \ref{assum:ptau}, whenever the event $\tktritrue < \tau_k$ occurs, there is at least $p_{\tau}$ probability of decreasing $\tau$. Taken in combination with $s_{\max}$ from Assumption \ref{assum:eventE}, this enables us to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ occurs. We introduce Lemma \ref{lem:dqbound} and Lemma \ref{lem:hattaudiff} to handle iterations such that $\tktritrue < \tau_k$. Additionally, we derive Lemma \ref{lem:Ktaulsmax} to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ can occur.
\end{enumerate}

Now, we analyze the first modification mentioned above. As in the previous section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and the a specific realization $g_{[k-1]}$.

Our analysis relies on the following three events. For all $k \in \{0,\dotsc,\kmax\}$, let $\Ek1$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) \geq 0$, let $\Ek2$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} = \tau_{k-1}$, and let $\Ek3$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue)$ and $\Tcal_{k} < \tau_{k-1}$.

Now, we derive a bound on the final term in \eqref{eq:phidecrease}.

\begin{lemma} \label{lem:innerprod}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$, the existence of which follows under Assumption \ref{assum:fcsmooth}. Let
\bequationNN
\alpha_{\min,k} := \frac{\beta_k \xi_{\min} \tau_{\min}}{\tau_{\min}L_k + \Gamma_k} \mbox{ and } \alpha_{\max,k} := \frac{\beta_k \xi_{\min} \tau_{k-1}}{\tau_{k-1}L_k + \Gamma_k},
\eequationNN
where $\tau_{\min}$ and $\xi_{\min}$ are defined as in Assumption \ref{assum:eventE}.

Then, with $\kappa_d \in \R{}_{>0}$ defined by Lemma \ref{lem:dexpectation},
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq  (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek1], \\
\E_{k,2} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek2], \\
\E_{k,3} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\tau_{\min}$, $\alpha_{\min,k}$, and $\alpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &= \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek1] \Prob_k[\Ek1] + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By the Law of Total Expectation and Lemma \ref{lem:dexpectation}, this means that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, we have
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} \alpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} \alpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{\min} \alpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{\min} \alpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}
Summing these three inequalities,
\begin{align}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \nonumber \\
    &\leq \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+\frac13(\tau_{k-1} (\alpha_{\max,k} - \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+\frac13(2 \tau_{\min} \alpha_{\min,k} - \tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \nonumber \\
    &= \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -\theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-\frac13(\tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2) - 2 \tau_{\min} \alpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]. \label{eq:innerprodproof1}
\end{align}
Now, by Lemma \ref{lem:dexpectation},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|\nabla f(x_k)\| \E_k[\|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[\nabla f(x_k)^\top(D_k - \dktrue)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek2] \Prob_k [\Ek2] \\
    &= \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \\
    &\leq \kappa_g \E_k[\|D_k - \dktrue\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma \ref{lem:dexpectation}. Using these three inequalities with
\eqref{eq:innerprodproof1}, yields
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
which proves the result.
\end{proof}

Now, we turn our attention to the second modification mentioned in the outline of this section. Our complexity result is derived through the use of \eqref{eq:phidecrease}, which relates decrease in our merit function to $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$. On any iteration for which $\tau_k \leq \tktritrue$ holds, $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$ can be directly related to the optimality conditions defined in \eqref{eq:optconds}. Unfortunately, the same is not true for $k$ such that $\tau_k > \tktritrue$. Thus, in order to provide an informative bound on such iterations, we introduce the following sequence:
\bequation \label{eq:hattaudef}
    \hat{\Tcal}_k := \min\{\Tcal_k, \tktritrue\},
\eequation
which we will use throughout the rest of the analysis (note that because we are conditioned on the history up to the start of iteration $k$, $\Tcal_k$ is a random variable, while $\tktritrue$ is not).

Now, we derive a bound on the conditional expectation of $\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)$ using the definition of $\hat{\Tcal}_k$.

\begin{lemma} \label{lem:dqbound}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$ and let $\kappa_d$ be defined as in Lemma \ref{lem:dexpectation}. Let $\hat{\Tcal}_k$ be defined in \eqref{eq:hattaudef}. Then,
\begin{align*}
    \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)]
    &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
    +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
    &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
    &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)).
\end{align*}
\end{lemma}

\begin{proof}
    To begin, by the definition of \eqref{eq:deltadef},
    \begin{align}
        &\E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \nonumber \\ &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k, 0\}) + \|c_k\|_1] \nonumber \\
        &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k - \nabla f(x_k)^\top \dktrue  + \frac12 \max\{D_k^\top H_k D_k, 0\} \nonumber \\
        &\quad- \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] \nonumber \\ &\quad+ \E_k[-\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] + \|c_k\|_1 \nonumber \\
        &= \E_k[\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} \nonumber \\
        &\quad- \frac12 \max\{D_k^\top H_k D_k, 0\})] + \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]. \label{eq:dqbound1}
    \end{align}
    Now, for simplicity of notation, let \tred{TODO: Figure out if there's a better name than $Z_k$.}
    \bequationNN
        Z_k =  \nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12 \max\{D_k^\top H_k D_k, 0\}.
    \eequationNN
    Let $E_Z$ denote the event that $Z_k \geq 0$ occurs and let $E_Z^c$ denote the event that $Z_k < 0$ occurs. Then, by the Law of Total Expectation,
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k] &= \E_k[\hat{\Tcal}_k Z_k | E_Z] \Prob_k[E_Z] + \E_k[\hat{\Tcal}_k Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Therefore, by the Law of Total Probability, Lemma \ref{lem:product_bounds}, Jensen's inequality, and convexity of $\max\{\cdot,0\}$, it follows that
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{k-1} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} \E_k[Z_k] + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} (\nabla f(x_k)^\top \dktrue - \E_k[G_k^\top D_k] \\
        &\quad+ \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12\E_k[\max\{D_k^\top H_k D_k, 0\}]) \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \zeta^{-1} M + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Similarly, we have
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{\min} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &= \tau_{\min} \E_k[Z_k] + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &\leq \tau_{\min} \zeta^{-1} M + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z].
    \end{align*}
    Summing these two inequalities yields
    \begin{align}
        \E_k[\hat{\Tcal}_k Z_k] &\leq \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M + \frac12 (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \nonumber \\
        &\quad+ \frac12(\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \label{eq:dqbound2}.
    \end{align}
    Next, we note that by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, Jensen's inequality, and the concavity of the square root,
    \begin{align*}
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] &\leq 
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top \dktrue|] +\E_k[|G_k^\top \dktrue - G_k^\top D_k|] \\
        &\leq \|\dktrue\| \E_k [\|\nabla f(x_k) - G_k\|] + \E_k[\|G_k\|\|\dktrue - D_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]} \\ &\quad+ \kappa_d \E_k[(\|G_k - \nabla f(x_k)\| + \|\nabla f(x_k)\|) \|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d \E_k[\|\nabla f(x_k) - G_k\|^2] \\
        &\quad+ \kappa_d \|\nabla f(x_k)\| \E_k[\|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d (M + \kappa_g \sqrt{M}) = \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}).
    \end{align*}
    In addition, by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
        &\leq \|H_k\|\|\dktrue\|^2 + \|H_k\|\E_k[\|D_k\|^2] \\
        &\leq \kappa_H \kappa_d^2 \kappa_g^2 + 2\kappa_H \kappa_d^2 (\E_k [\|G_k - \nabla f(x_k)\|^2] + \kappa_g^2) \\
        &\leq \kappa_H \kappa_d^2 (3\kappa_g^2 + 2 M).
    \end{align*}
    Now, by the Law of Total Expectation and the above two inequalities,
    \begin{align*}
         \E_k[Z_k | E_z] \Prob_k[E_Z] &= \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    By the same argument,
    \begin{align*}
         -\E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] &\leq \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    Thus, combining this with \eqref{eq:dqbound1} and \eqref{eq:dqbound2},
    \begin{align*}
        \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
        +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
        &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)),
    \end{align*}
    proving the result.
\end{proof}

Next, we introduce a lemma which controls the difference in $\Delta q(\cdot)$ on iterations where $\tktritrue < \Tcal_k$.
\begin{lemma} \label{lem:hattaudiff}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d),
    \end{align*}
    and
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k, \Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d (M + \kappa_g^2) (2 + \kappa_H \kappa_d),
    \end{align*}
    where $\alpha_{\min,k}$ and $\alpha_{\max,k}$ are defined in Lemma \ref{lem:innerprod}.
\end{lemma}

\begin{proof}
    By the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &= \E_k[\Acal_k (\Tcal_k - \hat{\Tcal}_k) (\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) |\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\}| \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \kappa_g^2 + \thalf\kappa_H \kappa_d^2 \kappa_g^2).
    \end{align*}
    Next, by the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &= \E_k[\Acal_k (\hat{\Tcal}_k - \Tcal_k) (G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \E_k[|G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\}|] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \E_k[\|G_k\|^2] + \thalf \kappa_d^2 \kappa_H \E_k[\|G_k\|^2]) \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (2\kappa_d (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2) \\
        &\quad+ \kappa_d^2 \kappa_H (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2)) \\
        &\leq (\alpha_{\max,k} \tau_k - \alpha_{\min,k} \hat{\tau}_k) (2\kappa_d (M + \kappa_g^2) + \kappa_d^2 \kappa_H (M + \kappa_g^2)).
    \end{align*}
\end{proof}

Next, we present the statements of two lemmas, which provide upper bounds, in high probability, on key components of the complexity result. The proofs of these lemmas are relegated to Appendix \ref{app:simple} for presentation purposes. Both of these lemmas use the following function in their statement. For any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, let
\bequation \label{eq:lsd}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\eequation

Now we can state the first lemma, which gives a high-probability bound on the sum of the probabilities from applying Lemma \ref{lem:innerprod} at each iteration.

\begin{lemma} \label{lem:Eksumlsmax}
    Let Assumption \ref{assum:eventE} hold. Then,
    \bequation \label{eq:Ek3lsmax}
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob [E_{k,3} | E, \mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\Bigg | E \right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Before stating the next lemma, recall the definition of $\hat{\Tcal}_k$ in \eqref{eq:hattaudef} and let
$k_{\tau}$ denote the index set
\bequation \label{eq:smallktau}
    k_{\tau} := \{k : \tktritrue < \tau_{k-1}\}.
\eequation
In addition, we let
$\mathcal{K}_{\tau}$ denote the associated random index set
\bequation \label{eq:Ktau}
    \mathcal{K}_{\tau} := \{k : \tcalktritrue < \Tcal_{k-1}\}.
\eequation
By the definitions of $\Tcal_k$, $\tcalktritrue$, and $\hat{\Tcal}_k$, this set of iterations is a superset of the iterations at which $\hat{\Tcal}_k < \Tcal_k$ occurs and can therefore be used to characterize the number of iterations at which this event occurs. In addition, the event $\tktritrue < \tau_{k-1}$ does {\it not} depend on $G_k$, which makes it more convenient to work with analytically. In particular, this means that $G_k$ is conditionally independent of the event $\tktritrue < \tau_{k-1}$ given $g_{[k-1]}$ and $E$.

In the following lemma, we bound the cardinality of $\Kcal_{\tau}$ with high probability.

\begin{lemma} \label{lem:Ktaulsmax}
    Let Assumptions \ref{assum:eventE} and \ref{assum:ptau} hold. Let $\mathcal{K}_{\tau} = \{k : \tcalktritrue < \Tcal_{k-1}\}$. Then,
    \bequation \label{eq:Ktaulsmax}
        \Prob\left[|\mathcal{K}_{\tau}| \leq \left\lceil \frac{\ell(s_{\max},\delta)+1}{p_{\tau}}\right\rceil \Bigg| E\right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Now we are prepared to state our complexity result in terms of $\Delta q(\cdot)$.

\begin{theorem} \label{thm:complexity}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold. 
Let the sequence $\{\hat{\Tcal}_k\}$ be defined in \eqref{eq:hattaudef}.

Define 
\bequationNN
A_{\min} := \frac{\xi_{\min} \tau_{\min}}{\tau_{\min}L + \gamma} \mbox{ and }
A_{\max} := \frac{\xi_{-1} \tau_{-1}}{\tau_{-1}L + \gamma}
\eequationNN
as well as
\begin{align*}
\hat{M} &:= \frac12 A_{\max} (\tau_{-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M})
+ \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M))\\ 
&\quad \ + \frac{\tau_{-1} + \tau_{\min}}{4} A_{\max} \zeta^{-1} M + \theta \tau_{-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
and
\begin{align*}
    \kappa_{\Delta q} &:= \beta (A_{\max} \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d (2M + 3\kappa_g^2) (1 + \frac12 \kappa_H \kappa_d), \\
    \kappa_{E_3} &:= \beta (\tau_{-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec.
\end{align*}
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{k_{\max}+1}} \quad \mbox{ for some } \quad \gamma \leq \frac{A_{\min}}{A_{\max} + \theta}.
\eequationNN
Then,
\begin{align}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \nonumber \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \nonumber \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil. \label{eq:complexity}
\end{align}
\end{theorem}

\begin{proof}
By Lemma \ref{lem:phidecrease} and Lemma \ref{lem:innerprod},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) \\
    &\quad + \Acal_k \Tcal_k \nabla f(x_k)^\top (D_k - \dktrue)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}

First, we focus on iterations where $k \in k_{\tau}^c$ so that $\tktritrue \geq \tau_{k-1}$ and thus, $\tau_k \leq \tktritrue$. We mention once again that $G_k$ is conditionally independent of the event $\tktritrue \geq \tau_{k-1}$ given $E$ and $g_{[k-1]}$. Therefore, by \eqref{eq:qquadlb}, \eqref{eq:qquadlbtrue}, and Lemma \ref{lem:dqbound},
\begin{align*}
    &\E_k [\phi(x_k + \alpha_k D_k, \Tcal_k) | k \in k_{\tau}^c] - \E_k [\phi(x_k, \Tcal_k) | k \in k_{\tau}^c] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in k_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &=\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in k_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &\leq -\beta (A_{\min} - \frac12 (A_{\max}+\theta) \beta) \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] + \frac{\tau_{k-1} + \tau_{\min}}{4} \beta^2 A_{\max} \zeta^{-1} M \\
    &\quad+ \frac12 \beta^2 A_{\max} (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)) \\
    &\quad+ \beta (\tau_{k-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3| k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] + \kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}^c] + \beta^2 \hat{M}.
\end{align*}

Now, we condition on $k \in \mathcal{K}_{\tau}$. Once again, $G_k$ is conditionally independent of this event given $\Fcal_k$ and $E$. By (\ref{eq:qquadlb}), (\ref{eq:qquadlbtrue}), Lemma \ref{lem:dqbound}, and Lemma \ref{lem:hattaudiff},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) | k \in \mathcal{K}_{\tau}] - \E_k [\phi(x_k, \Tcal_k) | k \in \mathcal{K}_{\tau}] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad+\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad-\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in \mathcal{K}_{\tau}] \\
    &\quad+ \kappa_{E_3} \Prob_k[\Ek3 | k \in \mathcal{K}_{\tau}] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}] + \kappa_{\Delta q} \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}] + \beta^2 \hat{M}.
\end{align*}

Now by the law of total probability and the law of total expectation,
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &=\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &\quad+ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}] \Prob_k[k \in \mathcal{K}_{\tau}] + \beta^2 \hat{M} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in \mathcal{K}_{\tau}^c] \Prob_k[k \in \mathcal{K}_{\tau}^c] + \beta^2 \hat{M} \Prob_k[k \in \mathcal{K}_{\tau}^c] \\
    &=-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3}] + \beta^2 \hat{M} + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}]
\end{align*}

Summing this inequality for all $k \in \{0,\dots,k_{\max}\}$, by Lemma \ref{lem:Eksumlsmax} it follows that, with probability at least $1-\delta/2$,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \sum_{k=0}^{k_{\max}} (-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{E_3} \Prob_k[E_{k,3}] + \kappa_{\Delta q} \Prob_k[k \in \mathcal{K}_{\tau}]) \\
    &\quad+ (k_{\max}+1) \beta^2 \hat{M}, \\
    &\leq -\sum_{k=0}^{k_{\max}} \frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{\Delta q} \sum_{k=0}^{k_{\max}} \Prob_k[k \in \mathcal{K}_{\tau}] \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M}.
\end{align*}

Now, let $g : = \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that are measurable with respect to the filtration $\mathcal{F}_{k_{\max}}$. Note that $\Prob_k[k \in \Kcal_{\tau}] \in \{0,1\}$ since the event $k \in \Kcal_{\tau}$ does not depend on $G_k$ when conditioned on $\Fcal_k$ and $E$. Therefore, by total expectation, the definition of our filtration, Lemma \ref{lem:Ktaulsmax}, and the union bound, with probability at least $1-\delta$,
\begin{align}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k)| E] - \E[\phi(X_k,\Tcal_k) | E] \nonumber \\
    &= \int_{g \in \mathcal{F}_{k_{\max}}} \sum_{k=0}^{k_{\max}} \E [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k,\Tcal_k) | E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] f_{G}(g) dg \nonumber \\
    &\leq \int_{g \in \mathcal{F}_{k_{\max}}} \Bigg(-\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)|E,G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \nonumber \\
    &\quad+ \kappa_{\Delta q} \sum_{k=0}^{k_{\max}} \Prob[k \in \mathcal{K}_{\tau}|E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}]\Bigg) f_{G}(g) dg \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &= -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] + \kappa_{\Delta q} \E\big[|\mathcal{K}_{\tau}|\big|E\big] \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &\leq -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] + \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\delta/2)+1) +(k_{\max}+1) \beta^2 \hat{M}, \label{eq:complexityproof1}
\end{align}
where $f_{G}(g)$ is the probability density function of the random variable $G$. Working with left side of this inequality,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E] - \E[\phi(X_k,\Tcal_k) | E] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k f(X_k + \Acal_k D_k) + \|c(X_k + \Acal_k D_k)\|_1 | E] - \E[\Tcal_k f(X_k) + \|c(X_k)\|_1 | E] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k (f(X_k + \Acal_k D_k) - f_{\min}) + \|c(X_k + \Acal_k D_k)\|_1 | E] - \E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E].
\end{align*}
It follows by the monotonicity of the $\Tcal_k$ sequence that
\bequationNN
-\E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E] \geq - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E].
\eequationNN
Thus,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E] - \E[\phi(X_k,\Tcal_k) | E] \\
    &\geq \E [\Tcal_{k_{\max}} (f(X_{k_{\max}+1}) - f_{\min}) + \|c(X_{k_{\max}+1})\|_1 | E] - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1.
\end{align*}
Combining this with \eqref{eq:complexityproof1},
\begin{align*}
    &\beta \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min}} \\
    &\quad+ \frac{2 (k_{\max}+1) \beta^2 \hat{M}}{A_{\min}} + \frac{2}{A_{\min}} \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
Dividing both sides of this inequality by the summation of $\beta$,
\begin{align*}
    &\frac{1}{\sum_{k=0}^{k_{\max}} \beta} \sum_{k=0}^{k_{\max}} \beta \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 (k_{\max}+1) \beta^2 \hat{M} + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil,
\end{align*}
so that by the definitions of $K^*$ and $\beta$,
\begin{align*}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
\end{proof}

Now we convert this into a result in terms of our optimality conditions \eqref{eq:optconds}.

\begin{corollary} \label{coro:complexity}
    Let the assumptions of Theorem \ref{thm:complexity} hold. Then, with probability at least $1-\delta$,
    \begin{align}
        &\E\left[\frac{\|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\|^2}{\kappa_H^2} + \|c(X_{K^*})\| \Bigg| E\right] \nonumber \\
        &\leq \frac{(\kappa_{\Psi} + 1)(2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1))}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \label{eq:coro} \\
        &\quad+ \frac{2 (\kappa_{\Psi} + 1) \kappa_{\Delta q}}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil \nonumber. 
    \end{align}
\end{corollary}

\begin{proof}
    The result follows by Lemma \ref{lem:kappapsi}, Lemma \ref{lem:kappaq}, and Theorem \ref{thm:complexity} combined with \eqref{eq:sqpsystemdet}, which implies that
    \bequationNN
        \|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\| = \|H_{k^*} D^{true}_{K^*}\| \leq \kappa_H \|D^{true}_{K^*}\|.
    \eequationNN
\end{proof}

We remark again that this result, in terms of the norm of the gradient of the Lagrangian, matches the worst-case complexity of the projected stochastic gradient method \cite{DDavis_DDrusvyatskiy_2019}.

\subsection{Complexity Result for Symmetric Sub-Gaussian Distributions} \label{subsec:subgauss}

In this section, we show that Assumptions \ref{assum:eventE} and \ref{assum:ptau} occur with high probability when the stochastic gradient $G_k$ follows a symmetric, sub-Gaussian distribution.

Throughout this section, we work with the following assumption.

\begin{assumption} \label{assum:symmsubgauss}
    At every iteration $k = \{0,\dots,k_{\max}\}$, the stochastic gradient $G_k$ satisfies
    \bequation
        \E[G_k | \mathcal{F}_k] = \nabla f(x_k),
    \eequation
    \bequation \label{eq:subgauss}
        \E[\exp(\|\nabla f(x_k)-G_k\|^2/M) | \mathcal{F}_k] \leq \exp(1),
    \eequation
    and the quantities $G_k - \nabla f(x_k)$ and $\nabla f(x_k) - G_k$ are equivalent in distribution. Finally, for all $k = \{0,\dots,k_{\max}\}$, the ratio parameter $\xi_k$ satisfies $\xi_k = \xi_{\min}$.
\end{assumption}

The above assumption has a number of important implications. The first is that Assumption \ref{assum:ptau} occurs (without conditioning on event $E$) with $p_{\tau} = \frac12$, as we show in the following lemma.

\blemma \label{lem:subgptau}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then,
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | \mathcal{F}_k] \geq \frac12.
    \eequationNN
\elemma

\bproof
    Let $Z_k$ be a basis for the null space of $J_k$, which under Assumption \ref{assum:fcsmooth} is a matrix in $\R{n\times(n-m)}$. Then, let $W_k$ be such that $U_k = Z_k W_k$ and $\wktrue$ be such that $\uktrue = Z_k \wktrue$. It follows from the first block in \eqref{eq:sqpsystem} that 
    \bequationNN
        H_k (Z_k W_k + v_k) + J_k^\top Y_k = -G_k \Longleftrightarrow Z_k W_k = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (G_k + H_k v_k).
    \eequationNN
    Using this equality and simplifying,
    \bequationNN
        G_k^\top D_k + D_k^\top H_k D_k = v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} G_k + H_k^{1/2} v_k).
    \eequationNN
    In a similar fashion, by \eqref{eq:sqpsystemdet},
    \bequationNN
        Z_k \wktrue = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (\nabla f(x_k) + H_k v_k)
    \eequationNN
    so that
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + (\dktrue)^\top H_k \dktrue \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} \nabla f(x_k) + H_k^{1/2} v_k).
    \end{align*}

    Then,
    \begin{align*}
        &G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (G_k -\nabla f(x_k))),
    \end{align*}
    and,
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (\nabla f(x_k) - G_k)),
    \end{align*}
    are equivalent in distribution by Assumption \ref{assum:symmsubgauss}. Therefore,
    \begin{align*}
        &\Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \\
        &=\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | \mathcal{F}_k].
    \end{align*}
    In addition, we have
    \begin{align*}
        1 &= \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \\
        &+\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | \mathcal{F}_k] \\
        &-\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} = 0 | \mathcal{F}_k].
    \end{align*}
    Taking these two together, it follows that
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | \mathcal{F}_k] \geq \frac12,
    \eequationNN
    proving the claim.
\eproof

Next, we repeat a well known property of sub-Gaussian random variables.
\blemma \label{lem:subgboundedrv}
    Suppose Assumption \ref{assum:symmsubgauss} holds. Then, for any $\delta \in (0,1)$,
    \bequation \label{eq:subgboundedrv}
        \Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)}\right] \geq 1 - \delta.
    \eequation
\elemma

\bproof
    By Markov's inequality and Assumption \ref{assum:symmsubgauss},
    \begin{align*}
        &\Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2 > M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)\right] \\
        &= \Prob\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) > \exp\left(1 + \log \frac{k_{\max}+1}{\delta}\right)\right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &= \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\sum_{k=0}^{k_{\max}} \E\left[\exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \right] \\
        &\leq \exp(-1) \frac{\delta}{k_{\max}+1} (k_{\max}+1)\exp(1) = \delta.
    \end{align*}
\eproof

We conclude this section by showing that under Assumption \ref{assum:symmsubgauss}, event $E$ as defined in Assumption \ref{assum:eventE} occurs with high probability.

\blemma \label{lem:subgeventE}
    Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then, there exists a constant $\kappa_{\tau_{\min}}$ such that, with probability at least $1-\delta$, event $E$ of Assumption \ref{assum:eventE} occurs with
    \bequationNN
        \ktaudec = \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)}.
    \eequationNN
    and
    \bequation \label{eq:sgtaumin}
        \tau_{\min} = \frac{(1-\sigma)(1-\epsilon)}{\kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \kappa_{\tau_{\min}}}, \quad  s_{\max} = \left\lceil\frac{\log \frac{(1-\sigma)(1-\epsilon)}{\tau_{-1} \kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \tau_{-1}\kappa_{\tau_{\min}}}}{\log 1-\epsilon }\right\rceil.
    \eequation
\elemma

\bproof
    We begin the proof by noting that by Jensen's inequality and the convexity of $\exp(\cdot)$,
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2| \mathcal{F}_k] \leq M.
    \eequationNN
    The bound on $\ktaudec$ follows directly from Lemma \ref{lem:subgboundedrv}. Finally, the bound on $\tau_{\min}$ follows from \cite[Lemma 2.16]{ABerahas_FECurtis_DPRobinson_BZhou_2020} combined with \ref{lem:subgboundedrv} and the bound on $s_{\max}$ follows from combining the bound on $\tau_{\min}$ with \eqref{eq:smaxbound}.
\eproof

\iffalse
\tred{Update 4/20 that I don't know where to put right now.}

We can also get a similar (though looser bound) for the case where we just have bounded variance!

\blemma \label{lem:boundeddiffvariance}
    For all $k \in \{0,\dots,k_{\max}\}$, let
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2 | \mathcal{F}_k] \leq M.
    \eequationNN
   Then,
    \bequationNN
        \Prob\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{\frac{(k_{\max}+1)M}{\delta}}\right] \geq 1-\delta.
    \eequationNN
\elemma

\bproof
    Let $g := \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that is measurable with respect to the filtration $\mathcal{F}_{k_{\max}}$. Then, by Markov's inequality, concavity of the square root, Jensen's inequality, and the law of total expectation,
    \begin{align*}
        &\Prob\Bigg[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2 > \frac{(k_{\max}+1)M}{\delta}\Bigg] \\
        &\leq \E\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &\leq \sum_{k=0}^{k_{\max}} \E\left[\|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &= \frac{\delta}{(k_{\max}+1)M} \sum_{k=0}^{k_{\max}} \int_{g \in \mathcal{F}_{k_{\max}}} \E\left[\|G_{k} - \nabla f(x_k)\|^2 | G_{0} = g_{0}, \dots, G_{k-1} = g_{k-1}\right] f_{G} dg \\
        &\leq \frac{\delta}{(k_{\max}+1)M} (k_{\max} + 1) M \int_{g \in \mathcal{F}_{k_{\max}}} f_{G}(g) dg = \delta,
    \end{align*}
    where $f_G(g)$ is the probability density function of the random variable $G$.
\eproof

What does this mean for our results? We can repeat the proof of Lemma \ref{lem:subgeventE} so that with probability at least $1-\delta$,
\bequationNN
    \tau_{\min} = \mathcal{O}\left(\sqrt{\frac{\delta}{k_{\max}+1}}\right)
\eequationNN
and, for sufficiently large $k_{\max}$,
\bequationNN
    s_{\max} = \mathcal{O}\left(\log \sqrt{\frac{k_{\max}+1}{\delta}}\right). 
\eequationNN
Thus,
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O} \left(\frac{\log \sqrt{\frac{k_{\max}+1}{\delta}}}{\sqrt{k_{\max}+1}} \right),
\eequationNN
which means we can always get a useful complexity result, so long as $k_{\max}$ is sufficently large.

Unfortunately, because the bound from Lemma \ref{lem:boundeddiffvariance} is $\mathcal{O}(\sqrt{k_{\max}+1})$, we cannot use this approach to directly bound $\ktaudec$ and obtain a meaningful complexity result. Thus, additional assumptions are still needed in this case.
\fi

\subsection{Complexity Result with Decreasing Ratio Parameter} \label{subsec:ratioparam}

In this section, we relax Assumption \ref{assum:eventE} with respect to the random variable $\{\Xi_k\}$ and allow it to be adaptive over the course of the algorithm. Due to the definition of $\{\Xi_k\}$, it satisfies a deterministic lower-bound, $\xi_{\min}$, such that $\xi_k \geq \xi_{\min} > 0$ holds for all $k$ \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Therefore, it follows that there exists a maximum number of decreases of $\xi$, which we denote by $r_{\max}$, that satisfies
\bequationNN
    r_{\max} \leq \min\left\{k_{\max}+1, \left\lceil \frac{\log(\xi_{\min}/\xi_{-1})}{\log(1-\epsilon)} \right\rceil\right\}.
\eequationNN

Now, we can state our new assumption.

\bassumption\label{assum:eventExi}
  Conditioned on the event $E_{\xi} := E(\kmax,s_{\max},\tau_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E_{\xi}, \Fcal_k] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E_{\xi}, \Fcal_k] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k = \xi_{k-1}] \leq \kappa_1, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k = \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_2, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^T(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_3.
    \ealigned
  \eequationNN
\eassumption

This assumption is largely the same as Assumption \ref{assum:eventE}. The major new requirement due to the adaptive $\{\Xi_k\}$ sequence is the addition of two more events under which the norm difference of $\nabla f(x_k)$ and $G_k$ is bounded.

We remark that this assumption holds with high-probability under Assumption \ref{assum:symmsubgauss} (without the condition that $\xi_k = \xi_{\min}$), a result which can easily be derived by simple modification of the techniques used in Section \ref{subsec:subgauss}. We leave this derivation as an exercise for the reader.

The complexity analysis for this case follows by essentially the same arguments as those used to derive a complexity result under Assumption \ref{assum:eventE}. A slight modification of Lemma \ref{lem:innerprod} is needed to include the three events related to $\nabla f(x_k)^T(d_k-\dktrue)$ that appear in Assumption \ref{assum:eventExi} (as opposed to the one in Assumption \ref{assum:eventE}), which yields a result in terms of the probabilities of these three events. Then, a slightly modified Lemma \ref{lem:Eksumlsmax} and the union bound can be applied two additional times to derive a complexity result. Since the analysis is a relatively straightforward extension of the results in Section \ref{subsec:complexity}, we simply state our complexity result here.
\begin{theorem}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:ptau}, and \ref{assum:eventExi} hold. Then, with probability at least $1-\delta$,
    \begin{align*}
        &\E[\|\nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c_{k^*}\| |
        E_{\xi}] \\
        &= \mathcal{O}\Bigg(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c_0\|_1 + M}{\sqrt{k_{\max}+1}} \\
        &\quad+ \frac{(\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta)) + (\xi_{-1} - \xi_{\min})(r_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\Bigg).
    \end{align*}
\end{theorem}

\bproof
    We leave the proof as an exercise for the reader.
\eproof

\section{Conclusion} \label{sec:conclusion}

In this work, we derived the first worst-case complexity result for an adaptive stochastic algorithm for equality constrained optimization. We developed a stochastic SQP algorithm with an adaptive $\ell$-1 merit function, based on the framework proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}. While key to a practical algorithm, the adaptivity in the merit function introduced a number of theoretical challenges to overcome. Under mostly standard assumptions, we prove that, with high probability, the expected value of the norm of the gradient of the Lagrangian decays at a rate of $k^{-4}$, matching the worst-case complexity of the projected stochastic gradient method. We believe the theoretical tools developed within may be applicable to a broad class of constrained stochastic optimization methods that utilize an adaptive merit function. 

\iffalse
OLD STUFF BELOW:
\subsection{Quick Complexity Highlight}
Quick highlight of the main complexity result for meeting on 3/9/2021:

Let $\mathcal{I} \subseteq \{0,1,\dots,\kmax\}$ denote the index set of ``good" iterations. Overall analysis will lead to a result of the form (with $\beta_k := \beta = \gamma/\sqrt{\kmax+1}$:
\begin{align*}
    &\sum_{k \in \mathcal{I}} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\quad\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &\quad+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau}.
\end{align*}
To get the expectation that we want, we need to add and subtract:
\begin{align*}
    &\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + \sum_{k \in \mathcal{I}^c} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)].
\end{align*}
Then, because the number of ``bad" iterations is bounded by $\ell(s_{\max},\delta)/p_{\tau}$,
\begin{align*}
    &\frac{\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)]}{\sum_{k=0}^{\kmax} \beta} \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\sum_{k=0}^{\kmax} \beta} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sum_{k=0}^{\kmax} \beta}.
\end{align*}
So that,
\begin{align*}
    &\E [\Delta q(x^*, \tau^*, \nabla f(x^*), H^*, d^{*,true})] \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\sqrt{\kmax + 1}} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sqrt{\kmax+1}}.
\end{align*}

Algorithm \ref{alg:ssqp} generates a random process $\{\bar{G}_k,X_k,\bar{D}_k,\bar{\mathcal{T}}_k,\bar{\Xi}_k,\bar{\mathcal{A}}_k\}$. We will denote all random quantities by capital letters and their realizations by small letters. The random gradient estimate is denoted by $\bar{G}_k$ and its realizations by $\bar{g}_k = \bar{G}_k(\omega)$. Similarly, let the random quantities $x_k = X_k(\omega)$ (iterates), $\bar{d}_k = \bar{D}_k(\omega)$ (search directions), $\btau_k = \bar{\mathcal{T}}_k(\omega)$ (merit parameter), $\bxi_k = \bar{\Xi}_k(\omega)$ (reduction ratio), and $\bar{\alpha}_k = \bar{\mathcal{A}}_k(\omega)$ (step sizes) denote their respective realizations. We will assume that the estimates $\bar{G}_k$ obey some standard properties, conditioned on the past.

To formalize conditioning on the past, let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by the random variables $\bar{G}_0, \dotsc \bar{G}_{k-1}$. For completness, we set $\mathcal{F}_{-1} = \sigma(x_0)$. As a result, we have that $\mathcal{F}_{k}$ for $k \geq -1$ is a filtration.

Let $E_{\tau,low}$ denote the event that the merit parameter sequence eventually remains constant at a sufficiently small positive value.
We will derive our complexity result under the assumption that this event occurs.

\begin{assumption} \label{assum:taulow}
Event $E_{\tau,low}$ occurs in the sense that there exists an iteration
number $\bar{k}_{\tau,\xi} \in \mathbb{N}$ and a merit parameter value
$\btau_{\min} \in \R{}_{>0}$ such that
\begin{equation} \label{eq:taumin}
    \btau_k = \btau_{\min} \leq \btau_k^{trial} \quad and \quad
    \xi_k = \xi_{\min} \quad for \; all \quad k \geq \bar{k}_{\tau,\xi}.
\end{equation}
In addition, the sequence of random gradients $\bar{G}_k$ generated by Algorithm \ref{alg:ssqp} satisfies
\begin{equation*}
    \E_{k,\tau,small}[\bar{G}_k] = g_k \quad and \quad \E_{k,\tau,small}[\|\bar{G}_k - g_k\|^2] \leq M
\end{equation*}
where $\E_{k,\tau,small}$ denotes expectation with respect to the distribution of $\omega$ conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_{k}$.
\end{assumption}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k$, let $\Ek1$ be the event that $g_k^\top(\bd_k - d_k) \geq 0$, let $\Ek2$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} = \btau_{k-1}$, and let $\Ek3$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} < \btau_{k-1}$.

We require an additonal assumption to obtain our complexity result:
\begin{assumption} \label{assum:boundedrv}
There exists $\kappa_{\Ek3} > 0$ such that
\begin{equation} \label{eq:boundedrv}
    \E_k [\|\bar{g}_k-g_k\||\Ek3] \leq \kappa_{E_3}.
\end{equation}
\end{assumption}
The above assumption holds under a number of conditions, including when
$\bar{g}_k$ is a bounded random vector.

%NEW
\textcolor{red}{TODO:} Ignoring $\xi_k$ for now. Will probably need additional cases in the proof eventually...

\begin{lemma} \label{lem:innerprodold}
Suppose that Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|g_k\|_2\}$, the existence of which follows under \cite[Assumption 1]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\bxi_k = \bxi_{\min}$ and define
\bequationNN
\balpha_{\min,k} := \frac{\beta_k \bxi_{\min} \btau_{\min}}{\btau_{\min}L_k + \Gamma_k} \mbox{ and } \balpha_{\max,k} := \frac{\beta_k \bxi_{\min} \btau_{k-1}}{\btau_{k-1}L_k + \Gamma_k}.
\eequationNN

Then, with $\kappa_d \in \R{}_{>0}$ from Lemma 3.6 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} which satisfies
$\|\bar{d}_k-d_k\| \leq \kappa_d \|\bar{g}_k-g_k\|$,
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq  (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek1] \\
\E_{k,2} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek2] \\
\E_{k,3} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\btau_{\min}$, $\balpha_{\min,k}$, and $\balpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &= \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek1] \Prob_k[\Ek1] + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By Lemma 3.6, this means that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, by Lemma 3.6, we have
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} \balpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} \balpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{\min} \balpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{\min} \balpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}

Summing these three inequalities yields

\begin{align}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \nonumber \\
    &\leq \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+(\btau_{k-1} (\balpha_{\max,k} - \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+(2 \btau_{\min} \balpha_{\min,k} - \btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3]) \nonumber \\
    &= \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -3 \theta \beta_k^2 \btau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-(\btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2) - 2 \btau_{\min} \balpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]). \label{eq:innerprodproof1old}
\end{align}
Now, by Assumption \ref{assum:boundedrv},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|g_k\| \E_k[\|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \E_k[\|\bar{g}_k - g_k\| | \Ek3] \Prob_k[\Ek3]  \\
    &\leq \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[g_k^\top(\bd_k - d_k)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek2] \\
    &= \E_k[\|g_k\| \|\bar{d}_k - d_k\|] - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \E_k[\|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma 3.6. Using these three inequalities with
\eqref{eq:innerprodproof1old}, yields
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
which proves the result.
\end{proof}

The above result provides an upper bound in terms of the probability that the event $\Ek3$ occurs. Due to the assumed lower bound on $\btau_k$, this event can only occur a finite number of times. To obtain our final result, we need an upper bound on the summation of the probability that $\Ek3$ occurs. The first component of this upper bound comes from the Chernoff bound.

\begin{lemma} \label{lem:chernoff}
Let $Z_0, \dotsc, Z_{k}$ be independent Bernoulli random variables and let $s \in \mathbb{N}_{>0}$.
%Let
%\begin{equation} \label{eq:lsd}
%    \ell(s,\delta) := S + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 S \log(1/\delta)}.
%\end{equation}
Then, for any $\delta \in (0, 1)$,%\todo{FEC: I suggest ``Let ... random variables for any $k \in \mathbb{N}_{\geq0}$.  Then, for any $s \in \mathbb{N}_{\geq0}$ and $\delta \in (0,1)$, ....}
\begin{equation}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s\right] \leq \delta,
\end{equation}
whenever
\begin{equation} \label{eq:lsdold}
    \sum_{i=0}^{k} \Prob[Z_i = 1] \geq \ell(s,\delta) \quad where \quad \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\end{equation}
\end{lemma}

\begin{proof}
Denote $\mu = \sum_{i=0}^{k} \Prob[Z_i = 1]$.%\todo{FEC: In the general form, the definition of $\mu$ is in terms of expected value.  Maybe for clarity we should write $\mu = \sum_{i=0}^k E[Z_i] = \sum_{i=0}^k \Prob[Z_i = 1]$, where the latter is true only because we have Bernoulli random variables.} Then by Chernoff's bound, for any $\rho \in (0,1)$,
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq (1-\rho) \mu \right]
    \leq e^{-\mu \rho^2/2}.
\end{equation*}
Now, setting $\rho = 1 - s/\mu$ (which is in $(0,1)$ by (\ref{eq:lsd})), we have
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s \right]
    \leq e^{-\mu (1-s/\mu)^2/2}.
\end{equation*}
To prove the result, we need to show that%\todo{FEC: In the proof, you start with what we need, then work backwards to show what we want.  I'd prefer if we start with what we have (assumed in the statement) and prove that it gives what we want.  Does that make sense?}
\begin{equation*}
    e^{-\mu (1-s/\mu)^2/2} \leq \delta
\end{equation*}
holds. Therefore, we need
\begin{equation*}
    -\mu(1-s/\mu)^2/2 \leq \log(\delta)
\end{equation*}
to be satisfied. Rearranging this inequality, and using $\log(\delta) = -\log(1/\delta)$,%\todo{FEC: I don't see where the last equation comes from.  Did you scale it by $2\mu$?  I'm not seeing it.}
\begin{equation*}
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta) = \mu^2 - 2\mu (s+\log(1/\delta)) + s^2. 
\end{equation*}
Therefore, using the quadratic equation and taking the positive root,
\begin{align*}
    \mu &\geq s + \log(1/\delta) + \frac12\sqrt{4(s+\log(1/\delta))^2 - 4 s^2} \\
    &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)},
\end{align*}
which proves the result.
\end{proof}

Unfortunately, the events $\Ek3$ are not independent of each other so we can not directly apply Chernoff's bound. However, we can use this result in combination with an observation about the limited nature of the dependency between these events to prove the following result.

%IDEA: Rewrite lemma to prove that $K_stop <= k_{S,\delta}$ w.h.p. when $k_{s,\delta}$ exists. Gets rid of this whole J_i,stop nonsense

%This rewrite sucks, should just do it instance-wise.

%Essential components:
%   Independence when the leave one out sum is less than s.
%   Conclusion: w.h.p K_stop <= k_s,delta (or something similar).

%Crappy parts:
%   Conditioning on k_s,delta being well defined. Any better way to handle it? Yes if we do it instance wise. But then that notation is a bit frustrating
%   Top part is fine, gets rough as soon as we introduce E_s,delta.

\begin{lemma} \label{lem:depbernoulli}
For any $k \in \mathbb{N}_{\geq 0}$, let $Z_0, \dotsc, Z_{k}$ be Bernoulli random variables. Let $s \in \mathbb{N}_{>0}$.%\todo{FEC: Is it right to say that $Z_i$ is Bernoulli upfront?  Or should we be saying that, conditioned on ${\cal F}_i$, the random variable $Z_i$ is Bernoulli?  I guess technically it's Bernoulli in any case, since it's 0--1, but maybe we should say the condition since we always talk about conditional probabilities?}
For any $\hat{k} \in \{0,\dotsc,k\}$ and $i \in \{0,\dotsc,\hat{k}\}$, let $E_{\hat{k},i}$ be the event that $\sum_{j\leq \hat{k},j\neq i} Z_j < s$. We assume the following about the random variable $Z_i$ for each $i \in \{0,\dotsc,k\}$:
\begin{enumerate}
    \item $\Prob[Z_i = 1 | \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\hat{k}}]$.
    \item $\Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}^c] = 0.$
\end{enumerate}
%Let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_{k}$. %and let $\bar{G}_{i}$ be measurable with respect to $\mathcal{F}_i$ for all $i \in \{-1,\dotsc,\hat{k}-1\}$.
Let $\delta \in (0,1)$ and let $\ell(s,\delta)$ be defined as in (\ref{eq:lsd}). Let $K_{s,\delta}$ be the random variable such that, for any realization of $\bar{G}_0,\dotsc,\bar{G}_{k-1}$ that is measurable with respect to $\mathcal{F}_k$,
\bequationNN
    k_{s,\delta} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta) \right\},
\eequationNN
($k_{s,\delta} = \infty$ for any realization such that $\sum_{i=0}^k \Prob[Z_i=1|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta)$ does not occur).
In addition, let $K_{stop}$ be the random variable
\bequationNN
K_{stop} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} Z_i = s\right\},
\eequationNN
($k_{stop} = \infty$ for any realization of $Z$ such that $\sum_{i=0}^{k} z_i < s$).

We define two events:%\todo{FEC: How do these events depend on $k$?  Should we take it that $k$ is ``fixed'' in some sense, but we are considering the events for any $s$?  But shouldn't we be proving the result ``for any $k$'' as well, in which case the events should depend on $k$, too?}
\begin{enumerate}
    \item Let $E_{k,s,\delta}$ be the event that 
    $\sum_{i=0}^k \Prob[Z_i=1|\mathcal{F}_i] \geq \ell(s,\delta)$.
    \item Let $E_{k,s,\delta,stop}$ be the event that $K_{stop} > K_{s,\delta}$.
\end{enumerate}
Then,
\begin{equation*}
    \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
\end{equation*}
%We assume the following:
%\begin{enumerate}
%    \item For any $i \in \{0,\dotsc,\hat{k}\}$, let $J_{i,stop}$ be the event that $i > K_{stop}$ and  
%    \bequationNN
%    \Prob[(Z_i = 1) \cap J_{i,stop} | \mathcal{F}_i] = 0.
%    \eequationNN
%    (high level idea: once a realization of $Z$ has $s$ successes, the probability of $Z_i = 1$ is $0$.)
    %and thus $\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] = \sum_{i=0}^{K_{stop}} \Prob[Z_i = 1 | \mathcal{F}_i]$.
%the minimum integer such that $\sum_{i=0}^{k_{stop}} Z_i = s$ (set $k_{stop} = \infty$ if $\sum_{i=0}^{\hat{k}} Z_i < s$). Let $Y_i = 0$ for all $i > k_{stop}$.
%    \item For any $\bar{k} \in \{0,\dotsc,\hat{k}\}$, let $J_{\bar{k},i}$ be the event that $\sum_{j\leq \bar{k},j\neq i} Z_j < s$. Then, $\Prob[Z_i = 1| \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, J_{\bar{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\bar{k}}]$. (high level idea: if the summation leaving out $Z_i$ does not equal $s$, then $Z_i$ is independent of all other $Z_j$.)
%\end{enumerate}

%$\Prob[Z_i = 1|\nu_i] = \Prob[Z_i = 1|\nu_i, Z_0, %\dotsc, Z_{i-1}$.
%let $\Prob[Z_i=1|\nu_i] = \Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}]$ hold unless $\sum_{j=0}^{\bar{k}} Z_j = s$ in which case $\Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}] = 0$ holds for any $i$ such that $\sum_{j\leq \bar{k}, j\neq i} Z_j = s$.
%Then, for any $\delta \in (0,1)$,
%\begin{equation}
%    \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \geq 1 - \delta,
%\end{equation}
%where $\ell(s,\delta)$ is defined in (\ref{eq:lsd}).
\end{lemma}

\begin{proof}
    %We work with any fixed sequence $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ satisfying these conditions.
    %Note that by the definition of our filtration, it should be clear that $\Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{k-1}] = \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]$ for any $i \in \{0,\dotsc,k\}$.
    
    %We begin the proof by showing that
    %\begin{equation*}
    %    \Prob\left[ \right] \geq 1 - \delta,
    %\end{equation*}
    %holds for any fixed $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$. To prove this, we assume that $\sum_{i=0}^{\hat{k}} \Prob[Z_i| \bar{g_0}, \dotsc, \bar{g}_{i-1}] \geq \ell(s,\delta)$ (as the result is trivial otherwise).
    
    Let $E_{k,s,\delta}$ and $E_{k,s,\delta,stop}$ both occur. Then, since $E_{k,s,\delta}$ occurs, $k_{s,\delta}$ is finite. In addition, because $E_{k,s,\delta,stop}$ occurs,
    we have that
    \bequationNN
        \sum_{i=0}^{k_{s,\delta}} z_i < s.
    \eequationNN
    Therefore, for all $i \in \{0,\dotsc,k_{s,\delta}\}$, $E_{k_{s,\delta},i}$ occurs. Thus, for all $i,j \in \{0,\dotsc,k_{s,\delta}\}$, $Z_i$ and $Z_j$ were mutually independent.
    
    Due to the independence $Z$ in this case, by Lemma \ref{lem:chernoff},
    \bequationNN
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s\right] \leq \delta,
    \eequationNN
    and thus,
    \bequationNN
        \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
    \eequationNN
    
    Now, let $\hat{Z}_0, \dotsc, \hat{Z}_{k}$ be independent Bernoulli random variables such that $\Prob[\hat{Z}_i = 1] = \Prob[Z_i = 1|\mathcal{F}_i]$ for all $i=0,\dotsc,k$. Let $E$ be the event that $\sum_{i=0}^{k_{s,\delta}} Z_i < s$ and let $E_{k,s,\delta}$ occur. Now, for each $i=0,\dotsc,k_{s,\delta}$, it follows that if event $E$ occurs, $E_{k_{s,\delta},i}$ must occur as well, so $Z_i$ is independent of $Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{k_{s,\delta}}$ conditioned on the event $E$. Thus, whenever $E$ occurs, $Z_0,\dotsc,Z_{k_{s,\delta}}$ are identical in distribution to $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s,\delta}}$. Therefore, by Lemma \ref{lem:chernoff},
    \begin{equation}
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = \Prob\left[\sum_{i=0}^{k_{s,\delta}} \hat{Z}_i < s\right] \leq
        \delta.
    \end{equation}
    It follows that
    \begin{equation*}
           \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i \geq s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = 1 -    \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] \geq 1 - \delta,
    \end{equation*}
    and thus
    \begin{equation*}
        \Prob[k_{stop} \leq k_{S,\delta}] \geq 1 - \delta.
    \end{equation*}
    In addition, by the definition of $k_{stop}$ and $J_{i,stop}$, with probability at least $1-\delta$,
    \begin{align*}
        \sum_{i=0}^{\hat{k}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}]
        &= \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq \sum_{i=0}^{k_{S,\delta}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq 1 + \ell(s,\delta),
    \end{align*}
    and thus,
    \begin{equation*}
        \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1|\bar{g}_0, \dotsc, \bar{g}_{i-1}] \leq 1 + \ell(s,\delta) \right] \geq 1 - \delta.
    \end{equation*}
    Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_{\hat{k}}} \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{\hat{k}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\hat{k}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\hat{k}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
\end{proof}

This setup applies to $\Ek3$ under Assumption \ref{assum:taulow} due to the definitions of $\btau$ and $\btau_{\min}$. In particular, at each iteration where $\Ek3$ occurs, $\btau_{k} \leq (1-\varepsilon)\btau_{k-1}$ holds. Therefore, if we perform this process $s$ times, until
\begin{equation*}
    \btau_{\min} \geq (1-\varepsilon)^s \btau_{-1},
\end{equation*}
it follows that $\Ek3$ cannot occur again by Assumption \ref{assum:taulow}. Thus, solving this inequality for $s$, we have
\bequation \label{eq:Stmin}
    s_{\btau_{\min}} := \left\lceil\frac{\log(\btau_{\min}/\tau_{-1})}{\log(1-\varepsilon)}\right\rceil
\eequation
which is the maximum number of times $\Ek3$ can occur.

Now we can show how to apply the above lemma to $\Ek3$.

\begin{lemma}
    Let Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\beta_j = \beta$, $L_j = L$, and $\Gamma_j = \Gamma$ for all $j=0,\dotsc, k$. Let 
    \bequationNN
        \balpha_{\min} := \frac{\beta \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max} := \frac{\beta \bxi_{\min} \btau_{-1}}{\btau_{-1}L + \Gamma}.
    \eequationNN
    Let $\delta \in (0,1)$. Then, with probability at least $1-\delta$,
    \begin{align}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top (\bar{d}_j-d_j)]
        &\leq (\btau_{-1} (\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3}(1 + \ell(s_{\btau_{\min}},\delta))\\
    &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}, \nonumber
    \end{align}
    where
    \bequationNN
        \ell(s_{\btau_{\min}},\delta) := s_{\btau_{\min}} + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s_{\btau_{\min}} \log(1/\delta)}.
    \eequationNN
\end{lemma}

\begin{proof}
    By Lemma \ref{lem:innerprod},
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq \sum_{j=0}^k (\btau_{j-1}(\balpha_{\max,j} + \theta \beta_j^2) - \btau_{\min} \balpha_{\min,j}) \kappa_g \kappa_d \kappa_{E_3} \Prob_j[E_{j,3}]\\
        &\quad+ \theta \beta_j^2 \btau_{j-1} \kappa_g \kappa_d \sqrt{M}.
    \end{align*}
    Using our assumption on $\beta$, $L$, and $\Gamma$, we can upper bound this inequality as
    \begin{align} \label{eq:ipproof1}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} \sum_{j=0}^k \Prob_j[E_{j,3}]\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}. \nonumber
    \end{align}
   
    To show the final result, we need to apply Lemma \ref{lem:depbernoulli}. To do this, let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_k$ and for all $i=0,\dotsc,k$, let $Z_i = 1$ if $E_{i,3}$ occurs and let $Z_i = 0$ otherwise. Recall that $\Prob_i[\cdot]$ is conditioned on the event $E_{\tau,low}$ occurring as well as the filtration $\mathcal{F}_i$.
    
    Now, let $s = s_{\btau_{\min}}$, so that $s$ is the maximum number of iterations in which $\Ek3$ can occur by Assumption \ref{assum:taulow}. Then, it is easy to verify that by the definition of our filtration, the probability that $\Ek3$ occurs is independent of the $E_{i,3}$ for all other $i$, whenever $\Ek3$ can occur without contradicting Assumption \ref{assum:taulow}. This holds whenever $E_{\hat{k},i}$ occurs, so that the first property of $Z_i$ in Lemma \ref{lem:depbernoulli} holds. On the other hand, when $E_{\hat{k},i}^c$ occurs it is clear that if $\Ek3$ occurs as well that Assumption \ref{assum:taulow} must be contradicted. Thus, second property of $Z_i$ in Lemma \ref{lem:depbernoulli} is satisfied as well.
    
    Now, presume that $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s_{\btau_{\min}},\delta)$. Then, by Lemma \ref{lem:depbernoulli},
    \bequationNN
        \Prob[K_{stop} \leq k_{s_{\btau_{\min}},\delta}] \geq 1 - \delta.
    \eequationNN
    In addition, by the definition of $s_{\btau_{\min}}$ and $K_{stop}$, it follows that whenever $K_{stop}$ is finite,
    \bequationNN
        \sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] =
        \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}].
    \eequationNN
    Thus, with probability at least $1 - \delta$,
     \bequationNN
        \sum_{i=0}^{k} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq \sum_{i=0}^{k_{s_{\btau_{\min}}}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]
        \leq 1 + \ell(s_{\btau_{\min}},\delta).
    \eequationNN
    
    On the other hand, if $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] < \ell(s_{\btau_{\min}},\delta)$, it is clear that $\sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq 1 + \ell(s_{\btau_{\min}},\delta)$. Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_k} \Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_k} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
    
    Combining this with (\ref{eq:ipproof1}),
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} (1 + \ell(s_{\btau_{\min}},\delta))\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M},
    \end{align*}
    holds with probability at least $1-\delta$.
\end{proof}

\begin{theorem}
Suppose that Assumption 4 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} holds. Define 
\bequationNN
\bar{A}_{\min} := \frac{\bar{\xi}_{\min} \bar{\tau}_{\min}}{\tau_{-1}L + \gamma} \mbox{ and }
\bar{A}_{\max} := \frac{\xi_{-1} \tau_{-1}}{\bar{\tau}_{\min}L + \gamma}
\eequationNN
as well as
\bequationNN
\bar{M} := \tau_{-1} \left(\frac12 (\bar{A}_{\max} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{K+1}}
\eequationNN
for some
\bequationNN
\gamma \leq \min\left\{\frac{\bar{A}_{\min}}{\bar{A}_{\max} + \theta},
\frac{1}{\bar{A}_{\min}}\right\}.
\eequationNN
Then,
\begin{equation}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + c_0 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation}
\end{theorem}

\begin{proof}
Let
\bequationNN
\bar{A}_k = \frac{\bar{\xi}_{k} \bar{\tau}_{k}}{\bar{\tau_{k}}L + \gamma} \mbox{ and }
\bar{M}_k = \bar{\tau}_{k} \left(\frac12 (\bar{A}_{k} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
It follows that $\bar{A}_k \beta \leq \bar{\alpha}_k \leq (\bar{A}_k + \theta)\beta$. Using  Lemmas 3.2(d), 3.5, 3.8, and 3.9 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} (with the replacement of $\bar{\tau}_{\min}$ by $\bar{\tau}_k$), we have
\begin{align*}
    &\E_k[\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\leq \E_k [-\bar{\alpha}_k \Delta q(x_k, \bar{\tau_k}, g_k, H_k, d_k) + \frac12 \bar{\alpha}_k \beta \Delta q(x_k, \bar{\tau_k}, \bar{g}_k, H_k, \bar{d}_k) + \bar{\alpha}_k \bar{\tau}_k g_k^\top (\bar{d}_k - d_k)] \\
    &\leq -\beta(\bar{A}_k - \frac12(\bar{A}_k + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}_k \\
    &\leq -\beta(\bar{A}_{\min} - \frac12(\bar{A}_{\max} + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M} \\
    &\leq -\frac12 \beta \bar{A}_{\min} \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}
\end{align*}
Summing this inequality from $0$ to $K$,
\begin{align}
&\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \nonumber \\ 
&\leq -\frac12 \bar{A}_{\min} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)] + (K+1) \beta^2 \bar{M}. \label{eq:stochasticproof1old}
\end{align}
Now, we work with the left hand side of this inequality,
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k f(x_k + \bar{\alpha}_k \bar{d}_k) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k f_k + c_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k (f(x_k + \bar{\alpha}_k \bar{d}_k) - f_{\min}) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k].
\end{align*}
Now, conditioned on the algorithm reaching $x_k$, it follows by the monotonicity of $\tau$
that
\bequationNN
-\E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k] \geq - \E_k[\bar{\tau}_{k-1} (f_k - f_{\min}) + c_k].
\eequationNN
Therefore, summing this inequality yields
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\geq \E_K [\bar{\tau}_K (f_{K+1} - f_{\min}) + \|c_K\|_1] - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1.
\end{align*}
Using this lower bound with \eqref{eq:stochasticproof1old}
\begin{equation*}
    \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min}}.
\end{equation*}
Dividing both sides by the summation of $\beta$,
\begin{equation*}
    \frac{1}{\sum_{k=0}^K \beta} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Now, by the definition of $x_{k^*}$, the left hand side is simply
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Using the definition of $\beta$, this becomes
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation*}
\end{proof}

\newpage
\appendix

\section{FEC Notes}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)\},
\eequationNN
where
\bitemize
  \item $\Xbar_k$ is the algorithm iterate in iteration $k$,
  \item $\Gbar_k$ is the stochastic gradient in iteration $k$,
  \item $\Dbar_k$ is the search direction in iteration $k$,
  \item $\overline\Tcal_k$ is the merit parameter in iteration $k$,
  \item $\Sbar_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\overline\Xi_k$ is the ratio parameter in iteration $k$, and
  \item $\overline\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)$ is denoted as
\bequationNN
  (\xbar_k,\gbar_k,\dbar_k,\bar\tau_k,\sbar_k,\bar\xi_k,\bar\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{\Gbar_0,\dots,\Gbar_{k-1}\}$, the realization of which (along with $\Xbar_0 = x_0$) determines the realization of
\bequationNN
  \{\Xbar_j\}_{j=1}^k\ \ \text{and}\ \ \{(\Dbar_j,\overline\Tcal_j,\Sbar_j,\overline\Xi_j,\overline\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

Let us consider a conditional model under the following assumption.
We introduce the following assumption.

\newpage

\bassumption\label{ass:FEC}
  Conditioned on the event $E := E(k_{\max},s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(k_{\max}+1)$th iterate is determined,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\bar\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$, and
    \item in every realization we have $\bar\xi_k = \bar\xi_{-1} = \bar\xi_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$,
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,k_{\max}\}$:
  \bequationNN
    \baligned
      \E[\Gbar_k &| E, \Fcal_k] = \nabla f(\xbar_k), \\
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ \text{and}\ \ 
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2 &| E, \Fcal_k, \nabla f(\xbar_k)^T(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0, \bar\tau_k < \bar\tau_{k-1}] \leq \kappa,
    \ealigned
  \eequationNN
  where $d(\xbar_k,\nabla f(\xbar_k))$ is the step that would be computed at an iterate $\xbar_k$ if the true gradient $\nabla f(\xbar_k)$ were used in the search direction computation.
\eassumption

Going forward, let us define the binary random variable
\bequation %\label{eq:zkdef}
  Z_k = \bcases 1 & \text{if $\nabla f(\xbar_k)^T(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0$ and $\bar\tau_k < \bar\tau_{k-1}$} \\ 0 & \text{otherwise.} \ecases
\eequation
Due to the definition of the event $E$, direct consequences of Assumption~\ref{ass:FEC} are
\bequation\label{eq:probz0}
  \baligned
    \P[Z_k = 1 &| E, \Fcal_k, \Sbar_{k-1} = s_{\max}] = 0 \\ \text{and}\ \ 
    \P[Z_k = 1 &| E, \Fcal_k, \Tbar_{k-1}(1 - \epsilon) < \tau_{\min}] = 0.
  \ealigned
\eequation

\bequationNN
  \P[Z_j = 1 | E, \Fcal_k, \Sbar_{k-1} < s_{\max}, \Tbar_{k-1}(1 - \epsilon) \geq \tau_{\min}]\ \ \text{for $j \in \{k,\dots,k_{\max}\}$}
\eequationNN

Our overall goal is to prove an upper bound (in high probability) on
\bequationNN
  \sum_{k=0}^{k_{\max}} p_k,\ \ \text{where}\ \ p_k := \P[Z_k = 1 | E, \Fcal_k].
\eequationNN
%From total probability and \eqref{temp}:
%\bequationNN
%  \baligned
%    \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k]
%    &= \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} < s_{\max}] \cdot \P[\Sbar_{k_{\max}} < s_{\max} | E, \Fcal_k] \\
%    &+ \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} = s_{\max}] \cdot \P[\Sbar_{k_{\max}} = s_{\max} | E, \Fcal_k]
%  \ealigned
%\eequationNN

As a first step, we prove the following.

\blemma\label{lem:chernoff_new}
  For any $k \in \N{}$, let $\{Y_0,\dots,Y_k\}$ be independent Bernoulli random variables.  Then, for any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, it follows that
  \bequationNN
    \mu := \sum_{j=0}^k \P[Y_j = 1] \geq \ell(s,\delta)\ \ \implies\ \ \P\left[\sum_{j=0}^k Y_j \leq s\right] \leq \delta,
  \eequationNN
  where
  \bequation\label{eq:lsd_new}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
  \eequation
\elemma
\bproof
  By the multiplicative form of Chernoff's bound, it follows for $\rho := 1 - s/\mu$ (which is in the interval $(0,1)$ by (\ref{eq:lsd_new})) that
  \bequationNN
    \P\left[\sum_{j=0}^{k} Y_j \leq s \right] \leq e^{-\frac{\mu \rho^2}{2}} = e^{-\frac{\mu (1-s/\mu)^2}{2}}.
  \eequationNN
  Hence, to prove the result, all that remains is to show that $e^{-\frac{\mu (1-s/\mu)^2}{2}} \leq \delta$, i.e.,
  \bequationNN
    -\frac{\mu(1-s/\mu)^2}{2} \leq \log(\delta)
  \eequationNN
  Using $\log(\delta) = -\log(1/\delta)$, this inequality is equivalent to
  \bequationNN
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta),
  \eequationNN
  which holds if and only if $\mu^2 - 2\mu (s+\log(1/\delta)) + s^2 \geq 0$.  Viewing the left-hand side of this inequality as a convex quadratic function in $\mu$, one finds that the inequality holds as long as $\mu$ is greater than or equal to the positive root of the quadratic, i.e.,
  \bequationNN
    \baligned
      \mu
        &\geq s + \log(1/\delta) + \sqrt{(s+\log(1/\delta))^2 - s^2} \\
        &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2s\log(1/\delta)}.
    \ealigned
  \eequationNN
  Since this holds under assumption in the lemma, the result is proved.
\eproof

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tau_k^{trial}$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ and $\xi_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tau_k^{trial}$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tau_k^{trial}$ occurs, we introduce the following assumption.

\begin{assumption} %\label{assum:ptau}
At every iteration $k$,
\bequation
    \Prob[\bar{g}_k^\top \bar{d}_k + \max\{\bar{d}_k^\top H_k \bar{d}_k,0\} \geq g_k^\top d_k + \max\{d_k^\top H_k d_k,0\} | E, \mathcal{F}_k] \geq p_{\tau}.
\eequation
\end{assumption}
This assumption is satisfied with $p_{\tau}$ when $\bar{g}_k$ is drawn from a Gaussian distrbution \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

This assumption is leads to the following lemma.

\blemma \label{lem:Etautrial_old}
    Let Assumptions \ref{ass:FEC} and \ref{assum:ptau} hold. Let $E_{\tau_k^{trial}}$ be the event that $\tau_k^{trial} < \bar{\tau}_{k-1}$. Then,
    \bequation
        \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, E_{\tau_k^{trial}}] \geq p_{\tau}.
    \eequation
\elemma

\bproof
    TODO: Copy proof from my notes.
\eproof

Due to the above lemma and Assumption \ref{ass:FEC}, it follows that
\bequationNN
    \Prob[E_{\tau_k^{trial}} | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN
In addition, by the definition of $\bar{\tau}_k$,
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, E_{\tau_{k}^{trial}}^c] = 0,
\eequationNN
so 
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN

Now, by Lemma \ref{lem:Etautrial} and the fact that $E_{\tau_{k}^{trial}}$ is not dependent on $\bar{g}_k$, it follows that
\bequation \label{eq:Etrialtaudec_old}
    \Prob[E_{\tau_{k}^{trial}} | \mathcal{F}_k, E, \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E] < p_{\tau}] = 0.
\eequation

Idea from here: Let $\bar{P}_k = \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, \bar{S}_{k-1} < s_{\max}]$ and let $Z_k$ be the indicator of the event that $\bar{\tau}_k < \bar{\tau}_{k-1}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}

Then, by \eqref{eq:Etrialtaudec}, with probability $1-\delta$, the number of occurrences of $E_{\tau_{k}^{trial}}$ is bounded by
\bequationNN
    |E_{\tau_{k}^{trial}}| \leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil.
\eequationNN
Thus, by the definition of $\bar{\tau}_k$, it follows that
\bequationNN
    |\tau_k^{trial} < \bar{\tau}_k|\leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil. 
\eequationNN

\newpage

\section{Mike's Simpler Problem} \label{app:simple}

Let $Y_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:simple1}
  \baligned
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \geq s_{\max}\right] &= 0
  \ealigned
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in [0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:simple2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Y_k = s_{\max} \right].
\eequation

The following lemma proves \eqref{eq:simple2}.
\begin{lemma} \label{lem:simple1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
    \bequationNN
      \baligned
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] &= 0,
      \ealigned
    \eequationNN
    for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in (0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k = s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} p_k + \sum_{k=j}^{k_{\max}} 0 = \sum_{k=0}^{j-1} p_k.
    \end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
    \end{align*}
    which completes the proof.
\end{proof}

The left side of this equation is similar to our goal for the actual problem, while the right is potentially easier to work with. 
A good starting point would be to try to prove a bound on
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right]
\eequationNN
for any $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$.

It clearly follows that
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right] = 1 -  \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right].
\eequationNN
We can find a lower bound on the right hand side of this equation using the following lemma.
\begin{lemma} \label{lem:simple2}
    Let $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$ and let $\hat{Y}_0,\dotsc,\hat{Y}_{\ell}$ be independent \\Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then,
    \bequationNN
        \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    For all $k \in \{0,\dotsc,\ell\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,\ell\}$, let
    \bequationNN 
        \bar{y}_k := \bcases
        1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
        0 & \textrm{otherwise},
        \ecases
    \eequationNN
    and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    \begin{align*}
        \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ are equivalent in distribution to $Y_0, \dotsc, Y_{\ell}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} Y_k < s_{\max}\right],
    \eequationNN
    where the last equality holds because 
    $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ and $Y_0, \dotsc, Y_{\ell}$ are equivalent in distribution.
\end{proof}

We can use these lemmas as well as Lemma \ref{lem:chernoff_new} to get our desired bound in high probability.

\begin{lemma} \label{lem:simple3}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Y_k$ be Bernoulli random variables which satisfy \eqref{eq:simple1}, where $p_k \in (0,1]$. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $\sum_{k=0}^{k_{\max}} p_k \leq \ell(s_{\max},\delta) + 1$. Then, by the definition of $Y_k$, it is clear that
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1
    \eequationNN
    holds deterministically, so the result is trivial in this case. Thus, for the remainder of the proof, we assume that $\sum_{k=0}^{k_{\max}} p_k > \ell(s_{\max},\delta) + 1$.
    
    Now, let $k_{s_{\max},\delta}$ be the minimum integer such that
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} p_k \geq \ell(s_{\max},\delta).
    \eequationNN
    Let $\hat{Y}_0,\dotsc,\hat{Y}_{k_{s_{\max},\delta}}$ be independent Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then, by Lemma \ref{lem:simple2} and Lemma \ref{lem:chernoff_new},
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &\geq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}

%Since the $\hat{Y}_k$ variables are independent, we can use this lemma and the CDF of the binomial distribution to get an exact description of the summation of interest. Alternatively, we can derive a bound for it by using a tail bound, such as Hoeffding's inequality or Chernoff's bound. The second option is likely to be more relevant in the more general setting of our actual algorithm.

What I'd hope a final result to look like:
\bequationNN
    \Prob\left[\sum_{k=0}^{k_{\max}} \Prob\Big[Z_k = 1 \Big| \mathcal{F}_{k}\Big] \leq \ell(s_{\max},\delta)\right] \geq 1 -\delta.
\eequationNN

Update: 2/8/2021

Let $\bar{P}_k = \Prob[Z_k=1| E, \mathcal{F}_k, \bar{S}_{k-1} < s_{\max}]$ and let $\bar{p}_k \in [0,1]$ for all \\$k \in \{0,\dotsc,k_{\max}\}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$ such that $\Prob\left[\left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\right] \neq 0$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}


Old idea:

If
\bequation \label{eq:simple3}
    \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | E, \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] \geq 1-\delta
\eequation
holds for any $\bar{g}_0,\dotsc,\bar{g}_{k_{\max}}$, then we are done because:
\begin{align*}
    &\Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i = 1| \mathcal{F}_i] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{g} \in \mathcal{F}_{k_{\max}}} \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
    &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{k_{\max}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta).
\end{align*}
Unfortunately, when conditioning on a realization from the filtration, we fix both the probabilities as well as whether the events occurred. Thus, the probabilities on the left side of \eqref{eq:simple3} is always 0 or 1.

\section{A Different Problem}
Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:different1}
  \begin{split}
    &\Prob\Bigg[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0,\dotsc,Z_{k-1}\Bigg] \in [0,1] \\ \text{and}\ \
    &\Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] = 0
  \end{split}
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:different2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
\eequation
We prove this inequality in the following lemma.

\begin{lemma} \label{lem:different1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy \eqref{eq:different1}, for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k \geq s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] + \sum_{k=j}^{k_{\max}} 0 \\
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right].
    \end{align*}
    
    %Now, letting $E_j^c$ denote the complement of $E_j$, the definition of $Z_k$ yields
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c \right] = \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \textrm{ for all $k \leq j$.}
    %\eequationNN
    %Thus,
    %\begin{align*}
    %    \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right]
    %    &\geq \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right] \\
    %    &= \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right].
    %\end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
\end{align*}
which completes the proof.
\end{proof}

Next, we would like to derive an analog to Lemma \ref{lem:simple2}.
\begin{lemma} \label{lem:different2}
    Let $p \in \{s_{\max}-1,\dotsc,k_{\max}\}$. Then, there exist independent Bernoulli random variables $\hat{Z}_0, \dotsc, \hat{Z}_p$ which satisfy
    \begin{align*}
        &\Prob\left[\sum_{k=0}^{p} Z_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{p} \hat{Z}_k < s_{\max} \right] \\
        \textrm{and } &\sum_{k=0}^p \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \sum_{k=0}^p \Prob\left[ \hat{Z}_k = 1\right].
    \end{align*}
\end{lemma}

\begin{proof}
    General idea: For any sequence of $\Prob\left[Z_k = 1 \Big| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right]$, there exists a fixed sequence of independent random variables that could generate this sequence in the same way that $\bar{Y}_k$ was generated in Lemma \ref{lem:simple2}. If we can get to that point, believe we can verbatim copy the rest of the proof.
    
    %To begin, note that for all $Z_0,\dotsc,Z_{k_{\max}}$ satisfying \eqref{eq:different1}, there exists a set of independent Bernoulli random variables 
    %$\hat{Z}_0, \dotsc, \hat{Z}_p$ such that
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right].
    %\eequationNN

    %For all $k \in \{0,\dotsc,p\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,p\}$, let
    %\bequationNN 
    %    \bar{y}_k := \bcases
    %    1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
    %    0 & \textrm{otherwise},
    %    \ecases
    %\eequationNN
    %and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    %and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    %\begin{align*}
    %    \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
    %    \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    %\end{align*}
    
    %Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{p}$ are equivalent in distribution to $Y_0, \dotsc, Y_{p}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{p} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{p} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    %\bequationNN
    %    \Prob\left[ \sum_{k=0}^{p} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} Y_k < s_{\max}\right],
    %\eequationNN
    %where the last equality holds because 
    %$\bar{Y}_0, \dotsc, \bar{Y}_{p}$ and $Y_0, \dotsc, Y_{p}$ are equivalent in distribution.
\end{proof}

\begin{lemma}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Z_k$ be Bernoulli random variables which satisfy \eqref{eq:different1}. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1} \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $E$ be the event that 
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}\right] > \ell(s_{\max},\delta).
    \eequationNN
    
    Then, let $K_{s_{\max},\delta}$ be the random variable whose realization $k_{s_{\max},\delta}$ is the minimum integer that satisfies
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}, E\right] \geq \ell(s_{\max},\delta).
    \eequationNN

    Now, for any $Z_0,\dotsc, Z_p$ which satisfies \eqref{eq:different1} and $E$, there exist independent Bernoulli random variables $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s_{\max}},\delta}$ such that
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, E, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right] \textrm{ for all } k \in \{0,\dotsc,k_{s_{\max},\delta}\}.
    \eequationNN

    Then, let $\bar{Z}_0,\dotsc,\bar{Z}_{k_{s_{\max},\delta}}$ be Bernoulli random variables such that
    \begin{align*}
        \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &= \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}


%DETERMINISTIC ANALYSIS BELOW
Given an objective function $f : \R{n} \rightarrow \R{}$ and a
constraint function $c : \R{n} \rightarrow \R{m}$, consider the optimization problem
\begin{equation} \label{eq:fdef}
    \underset{x \in \R{n}}{\min} \enspace f(x) \; \mbox{ s.t. } c(x)=0.
\end{equation}
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) = f(x) + c(x)^\top y$, the first-order stationarity conditions
for \eqref{eq:fdef} are given by
\begin{equation} \label{eq:1on}
    0 = \left[
    \begin{matrix}
    \nabla_x \ell(x,y) \\ \nabla_y \ell(x,y)
    \end{matrix}
    \right]
    = \left[
    \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\ c(x)
    \end{matrix}
    \right].
\end{equation}
Letting $f_k := f(x_k)$, $g_k := \nabla f(x_k)$, $c_k := c(x_k)$, and $J_k := \nabla c(x_k)^\top$ for all $k \in \mathbb{N}$ and given a sequence $\{H_k\}$ satisfying a standard type of sufficiency condition for equality constrained optimization, the SQP subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}
The optimal solution $d_k$ of this subproblem, and an associated Lagrange multiplier $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}
At each iteration, the algorithm uses a merit function with the $\ell_1$-norm penalty function $\phi : \R{n} \times \R{}_+ \rightarrow \R{}$ defined by
\begin{equation} \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1
\end{equation}
where $\tau \in \R{}_+$ is a merit parameter that is updated at each iteration of the algorithm. We use a local model of the merit function $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A useful quantity is the reduction in is model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}

For the purposes of this note, we will declare $x_k$ an approximate solution of (\ref{eq:fdef}) when
\begin{equation} \label{eq:eps1on}
    \|g_k + J_k^\top y_k\| \leq \epsilon  \quad \mbox{ and } \quad \|c_k\| \leq \epsilon,
\end{equation}
both hold for some $k \in \mathbb{N}$. We will derive a worst-case complexity result
in terms of the maximum number of iterations required to find a point statisfying \eqref{eq:eps1on}. We refer the reader to \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the
full definition of the algorithms. To prove our complexity result, we will use the following results which were proven in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}:
\begin{itemize}
    \item The merit parameter $\tau_k$ has an upper and lower bound given by $\tau_{-1} \geq \tau_k \geq \tau_{\min}$ (Lemma 2.14).
    \item The stepsize $\alpha_k$ is lower bounded by $\alpha_{\min}$ (Lemma 2.15).
    \item Let $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$ for all $k \in \mathbb{N}$. Then, by Lemma 2.7,
    \begin{equation} \label{eq:vltc}
        \max\left\{\|v_k\|,\|v_k\|^2\right\} \leq \kappa_v \|c_k\|,
    \end{equation}
    for some $\kappa_v > 0$.
    \item Let $\kappa_{uv}$ and $\zeta$ be strictly positive scalars. Then, by Lemma 2.8,
    \begin{equation} \label{eq:dposcurve}
        \|u_k\|^2 \geq \kappa_{uv} \|v_k\|^2 \implies d_k^\top H_k d_k \geq \frac14 \zeta \|u_k\|^2.
    \end{equation}
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:deltabound}
        \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \frac12 \tau_k \max\{d_k^\top H_k d_k, 0\} + \sigma\|c_k\|_1,
    \end{equation}
    (equation 2.9 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:meritdecrease}
        \phi(x_k + \alpha_k d_k, \tau_k) \leq \phi(x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k),
    \end{equation}
    (Lemma 2.12).
\end{itemize}

Armed with these results, we will prove the following lemma about sufficient decrease in the merit function whenever \eqref{eq:eps1on} does not hold.
\begin{lemma} \label{lem:suffdecrease}
Define
\begin{equation} \label{eq:kappahat}
    \hat{\kappa} := \frac{1}{\sqrt{1+\kappa_{uv}}\max\{\kappa_J,\kappa_H\}\kappa_v}
\end{equation}
and
\begin{equation} \label{eq:kappadec}
    \kappadec := \min\left\{\sigma \hat{\kappa},
    \frac18 \tau_{\min}\zeta\kappa_{uv}\kappa_v^2 \hat{\kappa}^2\right\}.
\end{equation}
Let $\epsilon < 1$ and let at least one of $\|g_k + J_k^\top y_k\| > \epsilon$ and/or $\|c_k\| > \epsilon$ hold. Then,
\begin{equation} \label{eq:suffdecrease}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\end{equation}
\end{lemma}

\begin{proof}
To begin, assume for contradiction that
\bequationNN
\|d_k\| \leq \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\eequationNN
Then, by the definitions of $d_k$ and $y_k$ as well as $\|H_k\| \leq \kappa_H$,
\bequationNN
\|g_k + J_k^\top y_k\| = \|H_k d_k\| \leq \kappa_H \|d_k\| \leq \frac{\epsilon \kappa_H}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
In addition, by the definition of $d_k$ and $\|J_k\| \leq \kappa_J$,
\bequationNN
\|c_k\| = \|J_k d_k\| \leq \kappa_J \|d_k\| \leq \frac{\epsilon \kappa_J}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
Therefore, \eqref{eq:eps1on} holds at $k$, which is a contradiction and we must
have
\begin{equation} \label{eq:dlength}
\|d_k\| > \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\end{equation}

We consider two cases in the rest of the proof. First, let $\|c_k\| \leq \hat{\kappa} \epsilon$. Then, by \eqref{eq:vltc} and $\|c_k\| \leq \hat{\kappa} \epsilon$,
\bequationNN
\|v_k\|^2 \leq \kappa_v^2 \|c_k\|^2 \leq \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
On the other hand, by \eqref{eq:dlength},
\begin{align*}
    \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} &< \|d_k\|^2 \\
    &= \|u_k\|^2 + \|v_k\|^2 \\
    &\leq \|u_k\|^2 + \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies
\begin{align*} \label{eq:ulb}
    \|u_k\|^2 &\geq \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &= \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \frac{ \epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \frac{\kappa_{uv}\epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &\geq \kappa_{uv} \|v_k\|^2.
\end{align*}
Thus, by \eqref{eq:dposcurve}, we have
\bequationNN
d_k^\top H_k d_k \geq \frac14 \zeta\|u_k\|^2 \geq \frac14 \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
Therefore,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} \\
    &\geq \frac18 \tau_{\min} \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies \eqref{eq:suffdecrease} in this case.

Now, presume that $\|c_k\| > \hat{\kappa} \epsilon$ holds. Then, by \eqref{eq:deltabound} and $\epsilon < 1$,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \sigma \|c_k\|_1 \\
    &\geq \sigma \hat{\kappa} \epsilon^2.
\end{align*}
Thus, (\ref{eq:suffdecrease}) holds in this case as well.
\end{proof}

We can use this lemma to prove the following complexity result.

\begin{theorem}
Let
\begin{equation} \label{eq:kbar}
    \bK := \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec} \epsilon^{-2},
\end{equation}
where $\kappadec$ is defined in \eqref{eq:kappadec}.
Presume Assumptions 1 and 2 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} hold.
Then, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in no more than $\bK$ iterations (a similar result holds for Algorithm 2.2 with a revised definition of $\alpha_{\min}$).
\end{theorem}

\begin{proof}
Assume for contradiction that for all iterations $k = 0,1, \dotsc, \bK$, \eqref{eq:eps1on}
does not hold. Then, by Lemma \ref{lem:suffdecrease}, we have
\bequationNN
\Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\eequationNN
Then, at each iteration, by \eqref{eq:meritdecrease},
\begin{align*}
    \phi (x_k + \alpha_k d_k, \tau_k) &\leq \phi (x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k) \\
    &\leq \phi(x_k, \tau_k) - \eta \alpha_{\min} \kappadec \epsilon^2.
\end{align*}
Using the definition of $\phi$ in \eqref{eq:phidef} as well as $x_{k+1} = x_k + \alpha_k d_k$, the above inequality becomes,
\bequationNN
\tau_k f_{k+1} + \|c_{k+1}\|_1 \leq \tau_k f_k + \|c_k\|_1 - \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Summing this inequality for all iterations $k = 0,1, \dotsc, \bK$, we have
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \sum_{k=0}^{\bK} \tau_k (f_{k+1}-f_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Now, by removing the first and last term of the summation, this inequality can be rewritten
as
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \tau_{\bK}f_{\bK+1} - \tau_0 f_0
+ \sum_{k=1}^{\bK} f_k (\tau_{k-1} - \tau_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
By definition, $\tau_k$ is a decreasing sequence. Therefore, we have $\tau_{k-1} - \tau_k \geq 0$
for all $k$. Then, since $\|c_{\bK+1}\|_1 \geq 0$ and $f_k \geq \flow$ holds for all $k$, we have
\bequationNN
- \|c_0\|_1 + \tau_{\bK}\flow - \tau_0 f_0
+ \flow (\tau_{0} - \tau_{\bK}) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Rearranging this inequality, we have
\bequationNN
\bK+1 \leq \frac{\tau_0 (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
\leq \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
= \bK,
\eequationNN
which is a contradiction. Therefore, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in
at most $\bK$ iterations.
\end{proof}
\fi



==> archived_versions/2021-09-16/abstract.tex <==
A worst-case complexity bound is proved for a sequential quadratic optimization (commonly known as SQP) algorithm that has been designed for solving optimization problems involving a stochastic objective function and deterministic nonlinear equality constraints.  Barring additional terms that arise due to the adaptivity of the monotonically nonincreasing merit parameter sequence, the proved complexity bound is comparable to that known for the stochastic gradient algorithm for unconstrained nonconvex optimization.  The overall complexity bound, which accounts for the adaptivity of the merit parameter sequence, shows that a result comparable to the unconstrained setting (ignoring log factors) holds with high probability.

==> archived_versions/2021-09-16/body.tex <==
%******************************************
% Paper-dependent macros here
%******************************************
\newcommand{\flow}{f_{\text{\rm low}}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\kappadec}{\kappa_{\text{\rm dec}}}
\newcommand{\bK}{\bar{K}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\btau}{\bar{\tau}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bg}{\bar{g}}
\newcommand{\bxi}{\bar{\xi}}

\newcommand{\xiktri}{\xi_k^{\rm trial}}
\newcommand{\ktaudec}{\kappa_{\tau_{\rm dec}}}
\newcommand{\kmax}{k_{\max}}
\newcommand{\smax}{s_{\max}}

\newcommand{\dktrue}{d_k^{\text{\rm true}}}
\newcommand{\uktrue}{u_k^{\text{\rm true}}}
\newcommand{\wktrue}{w_k^{\text{\rm true}}}
\newcommand{\yktrue}{y_k^{\text{\rm true}}}
\newcommand{\tktritrue}{\tau_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Dktrue}{D_k^{\text{\rm true}}}

\newcommand{\strue}{s^{\text{\rm true}}}

\newcommand{\Lbad}{\Lcal_{\text{\rm bad}}}
\newcommand{\Lgood}{\Lcal_{\text{\rm good}}}
\newcommand{\Ebad}{E_{\text{\rm bad}}}
\newcommand{\Cdec}{C_{\text{\rm dec}}}
\newcommand{\Idec}{\Ical_{\text{\rm dec}}}
\newcommand{\ktau}{k_{\tau}}
\newcommand{\tcalktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}



\def\Ek#1{E_{k,#1}}
\def\tred#1{\textcolor{red}{#1}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%*********
% Section
%*********

%\newtheorem{assumption}{Assumption}

%\def\proof{\par{\it Proof}. \ignorespaces}
%\def\endproof{{\ \vbox{\hrule\hbox{%
% \vrule height1.3ex\hskip0.8ex\vrule}\hrule
%}}\par}
%\def\noprint#1{}

\section{Introduction} \label{sec:intro}

We present a worst-case complexity analysis of an algorithm for minimizing a smooth objective function subject to nonlinear equality constraints.  Problems of this type arise in various important applications throughout science and engineering, including optimal control, PDE-constrained optimization, and resource allocation \cite{DPBertsekas_1998,JTBetts_2010,FSKupfer_EWSachs_1992,TRees_HSDollar_AJWathen_2010}.  However, unlike the vast majority of the literature on equality constrained optimization, the algorithm that we consider has been designed to solve problems in which the objective function is stochastic, in the sense that it may be viewed as the expectation of a function that has a random variable argument.  The algorithm that we consider assumes that evaluations of the objective function and its gradient are intractable to obtain, but that it has access to (unbiased) stochastic gradient estimates.

A few algorithms have been proposed recently for solving problems of this type.  These approaches fall into two categories: penalty methods \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018} (which includes the class of augmented Lagrangian methods) and sequential quadratic optimization (commonly known as SQP) methods \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}.  Penalty methods aim to solve the constrained optimization problem by adding a term to the objective function, weighted by a penalty parameter, that penalizes constraint violation.  Unconstrained optimization techniques are then applied to minimize the resulting penalty function, after which the penalty parameter may be modified and the minimization performed again in an iterative manner until a solution is obtained that (approximately) satisfies the original constraints.  Methods of this type perform well in some situations, but in others they perform poorly due to ill-conditioning and/or nonsmoothness of the subproblems. Such methods also often suffer due to their sensitivity to the particular scheme used for updating the penalty parameter.

In practice in both deterministic and stochastic optimization contexts, penalty methods are frequently outperformed by SQP-based methods.  Indeed, it is commonly accepted in the deterministic optimization literature that a state-of-the-art algorithm is an SQP method that chooses stepsizes based on a line search applied to a merit function.  In this deterministic setting, such an algorithm is intimately connected with applying Newton's method to the first-order primal-dual necessary conditions for optimality of the problem~\cite{RBWilson_1963}.

In this paper, we present a worst-case complexity analysis of the SQP method proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.  For one thing, our analysis shows that in an idealized setting in which one knows a threshold for the merit parameter beyond which the merit function is \emph{exact}, the number of iterations required until the method generates a point at which first-order necessary conditions for optimality hold in expectation with accuracy $\varepsilon \in (0,\infty)$ is $\Ocal(\varepsilon^{-4})$.  This is arguably the best result that one can expect given the bound that one can prove for a (projected) stochastic gradient method employed to solve an unconstrained nonconvex problem~\cite{DDavis_DDrusvyatskiy_2019}.  However, \emph{our analysis does not only consider this idealized setting}; we go further and prove a worst-case complexity bound for the algorithm when the merit parameter threshold is unknown, and instead the algorithm adaptively updates a monotonically nonincreasing merit parameter sequence.  We prove that under reasonable assumptions the aforementioned worst-case bound, with additional log factors, holds with high probability.  The high-probability aspect of this result arises purely due to the uncertainty of the behavior of the adaptive merit parameter sequence, and does not reflect any uncertainty of the behavior of the method during situations in which the merit parameter sequence remains constant.

To the best of our knowledge, ours is the first known worst-case complexity result for an SQP algorithm that operates in the \emph{highly stochastic regime} for solving stochastic optimization problems involving deterministic nonlinear equality constraints.  Prior to this work, the only known complexity results for stochastic constrained optimization were for algorithms for solving problems with simple constraint sets that enable projection-based methods \cite{DDavis_DDrusvyatskiy_2019,SGhadimi_GLan_HZhang_2016} and Frank-Wolfe type methods \cite{EHazan_HLuo_2016}.  (One exception is a complexity bound proved for the SQP algorithm proposed in \cite{SNa_MAnitescu_KMladen_2021}, although this result only holds for the idealized setting in which the algorithm has \emph{a priori} knowledge of a threshold for the merit function parameter.)  Our analysis focuses a great deal on the complications that arise due to the adaptivity of the merit parameter sequence, which essentially means that the algorithm in our consideration is aiming to reduce a merit function that \emph{changes} during the optimization process.  Hence, many aspects of our analysis are quite distinct from the analyses that have been presented for stochastic gradient methods in the context of unconstrained optimization or optimization over simple constraint sets.

%************
% Subsection
%************
\subsection{Problem formulation}

The algorithm that we consider is designed to solve problems of the form
\bequation \label{eq:fdef}
  \min_{x \in \R{n}} f(x)\ \ \st\ \ c(x) = 0,\ \ \text{with}\ \ f(x) = \E[F(x,\omega)],
\eequation
where $f : \R{n} \rightarrow \R{}$, $c : \R{n} \rightarrow \R{m}$, $\omega$ is a random variable with associated probability space $(\Omega,\mathcal{F}, P)$, $F : \R{n} \times \Omega \rightarrow \R{}$, and $\E$ represents expectation with respect to $P$.  In particular, following \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, we make the following assumption about problem \eqref{eq:fdef} and the algorithm that we analyze (stated later on as Algorithm~\ref{alg:ssqp} on page~\pageref{alg:ssqp}), which generates a sequence of iterates $\{x_k\} \subset \R{n}$.

\begin{assumption}\label{assum:fcsmooth}
  Let $\Xcal \subseteq \R{n}$ be an open convex set that contains $\{x_k\}$ for all realizations of Algorithm \ref{alg:ssqp}.  The objective function $f : \R{n} \rightarrow \R{}$ is continuously differentiable and bounded below by $\flow \in \R{}$ over $\Xcal$ and the corresponding gradient function $\nabla f: \R{n} \rightarrow \R{n}$ is bounded and Lipschitz continuous with constant $L \in (0,\infty)$ over $\Xcal$. The constraint function $c : \R{n} \rightarrow \R{m}$ $($where $m \leq n$$)$ and the corresponding Jacobian function $J := \nabla c^\top : \R{n} \rightarrow \R{m\times n}$ are bounded over $\Xcal$, each gradient function $\nabla c_i : \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $\gamma_i$ over $\Xcal$ for all $i \in \{1,\dots,m\}$, and the singular values of $J \equiv \nabla c^\top$ are bounded below and away from zero over $\Xcal$.
\end{assumption}

Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) := f(x) + c(x)^\top y$, first-order primal-dual stationarity conditions for~\eqref{eq:fdef}, which are necessary for optimality under Assumption~\ref{assum:fcsmooth}, are given by
\bequation \label{eq:optconds}
  0 =
  \left[ \begin{matrix}
    \nabla_x \ell(x,y) \\
    \nabla_y \ell(x,y)
  \end{matrix} \right]
  =
  \left[ \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\
    c(x)
  \end{matrix} \right].
\eequation

%************
% Subsection
%************
\subsection{Notation}

We adopt the notation that $\|\cdot\|$ denotes the $\ell_2$-norm for vectors and the vector-induced $\ell_2$-norm for matrices.  We denote by $\mathbb{S}^{n}$ the set of $n \times n$ dimensional real symmetric matrices. The set of nonnegative integers is denoted as $\N{} := \{0,1,2,\dots,\}$. For any integer $k \in \N{}$, we use $[k]$ to denote the subset of nonnegative integers up to $k$, namely, $[k] := \{0,\dots,k\}$.  Correspondingly, to represent a set of vectors $\{v_0,\dots,v_k\}$, we define $v_{[k]} := \{v_0,\dots,v_k\}$.

Algorithm~\ref{alg:ssqp} is iterative, generating in each realization a sequence of iterates $\{x_k\}$.  For our analysis, we also append the iteration number to other quantities corresponding to each iteration, e.g., $f_k := f(x_k)$ for all $k \in \N{}$.

When discussing stochastic quantities, we use capital letters to denote random variables and corresponding lower case letters to denote a realization of a random variable. For example, a stochastic gradient in iteration $k \in \N{}$ is denoted as $G_k$, a realization of which is written as $g_k$.

%************
% Subsection
%************
\subsection{Outline}

Section~\ref{sec:complexitypreview} provides a worst-case complexity result for the algorithm from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the deterministic setting, and uses this result and further commentary to motivate our main result for the stochastic setting.  Details of the algorithm for the stochastic setting are presented in Section~\ref{sec.algorithm}, followed by our main result and analysis provided in Section~\ref{sec:complexity}.  Finally, we provide some concluding thoughts and future directions in Section~\ref{sec:conclusion}.

%*********
% Section
%*********
\section{Outline of Main Results} \label{sec:complexitypreview}

Our algorithm of consideration, namely, that from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, is derived from an algorithm presented for the deterministic setting, which is also proposed and analyzed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} as a precursor for the stochastic setting.  To motivate our main result for the stochastic setting, it is instructive to consider a worst-case complexity bound for the deterministic algorithm.  Such a result is the following; further details and a proof is provided in Appendix~\ref{app.deterministic}.

\btheorem\label{th.deterministic}
  Consider Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} and suppose that Assumption~\ref{assum:fcsmooth} holds along with Assumption~2.4 from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.  Let $\tau_{-1} \in \R{}_{>0}$ be the initial value of the merit parameter sequence and let $\tau_{\min} \in (0,\tau_{-1}]$ be a lower bound for the merit parameter sequence (the existence of which follows from Lemma 2.16 in~\cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).  Then, for any $\epsilon \in (0,1)$, there exists $(\kappa_1,\kappa_2) \in \R{}_{>0} \times \R{}_{>0}$ such that the algorithm reaches an iterate $(x_k,y_k) \in \R{n} \times \R{m}$ satisfying
  \bequationNN  
    \|g_k + J_k^\top y_k\| \leq \epsilon\ \ \text{and}\ \ \|c_k\| \leq \epsilon
  \eequationNN
  in a number of iterations no more than
  \bequationNN
    \(\frac{\tau_{-1}(f_0 - \flow) + \|c_0\|_1}{\min\{\kappa_1,\tau_{\min} \kappa_2\}}\) \epsilon^{-2}.
  \eequationNN
\etheorem

The major technical hurdle in proving a complexity result for stochastic SQP methods arises from their use of an adaptive merit function. Merit functions are a commonly used tools in deterministic constrained optimization, as they provide a way to assess the quality of a step in terms of two (often competing) goals: minimizing the objective function $f$ and reducing the constraint violation in $c$. In our algorithm, we use the $\ell$-1 norm penalty  function $\phi : \R{n} \times \R{}_{>0}$ defined by,
\bequation \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1.
\eequation
Here, $\tau \in \R{}_{>0}$ is the merit parameter which, in our algorithm, is a positive non-increasing sequence $\{\tau_k\}$ that is adaptively chosen at each iteration $k$. The updating behavior of $\tau$ is the core difficulty in providing a complexity result, as the function being optimized at each iteration is modified based on stochastic information. Given that our algorithm uses only a single stochastic gradient at each iteration, the updates to $\tau$ may be based on very poor approximations to the true gradient, causing erratic behavior. We note that even when the sequence $\{\tau_k\}$ is deterministically lower bounded, such as when the noise is deterministically bounded, the complexity analysis is non-trivial as the number of iterations until the sequence $\{\tau_k\}$ settles near its lower bound is itself a random process. The behavior of $\tau$ is difficult to characterize, so previous analyses rely on ``fast-forwarding" to an iterate at which the merit parameter remains constant, greatly simplifying the theoretical challenges \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020,SNa_MAnitescu_KMladen_2021}. This strategy is not possible when a complexity result is desired however, as the behavior of the full iterate sequence must be analyzed instead.

We wish to stress here that while our techniques are developed for an SQP method which uses the merit function in \eqref{eq:phidef}, they may be applicable to a wide variety of algorithmic frameworks for stochastic optimization with deterministic constraints. The approaches used can be modified to apply to methods which adaptively update critical parameters at each iteration, such as adaptive penalty methods \cite{RHByrd_GLopez-Calva_JNocedal_2012,RHByrd_JNocedal_RAWaltz,MMongeau_ASartenaer_1995}, adaptive augmented Lagrangian \cite{FECurtis_HJiang_DPRobinson_2015}, adaptive barrier methods \cite{JNocedal_AWachter_RAWaltz_2009}, and penalty-interior point methods \cite{FECurtis_2012}. In addition, many constrained algorithms generate repeated (often unconstrained) subproblems defined by an auxilliary parameter sequence which is updated dynamically based off of the solution to the previous subproblem. Algorithms of this type include penalty methods, augmented Lagrangian methods, and interior point methods \cite{JNocedal_SJWright_2006}. In the case where the objective is stochastic, this auxilliary sequence would also be a random variable, the behavior of which would be paramount to proving a complexity result for this type of method. Thus, we believe that the techniques we derive for our SQP method are broadly applicable and foundational for performing a  complexity analysis of deterministically constrained stochastic optimization methods.

We note here that other stochastic SQP methods have been proposed in the literature \cite{SNa_MAnitescu_KMladen_2021}. These methods are either non-adaptive, in the sense that the merit parameter must be fixed a-priori, or require high-accuracy gradient estimates at each iteration. Due to this, we focus on the algorithmic framework developed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

In this section, we provide a sketch of our complexity result and describe how it compares to other results in the literature. Our result is proved under relatively common smoothness conditions on $f$ and $c$ as well as the linear independence constraint qualification (LICQ). We assume that, conditioned on some event $E$, the stochastic gradients are unbiased estimators of $\nabla f(x)$ with variance bounded by $M$, as is standard in the literature. Additionally, we assume that the stochastic gradients exhibit a bounded measure of asymmetry, the merit parameter sequence $\{\tau_k\}$ is lower bounded by some $\tau_{\min} > 0$, and the number of iterations at which $\tau_k$ is decreased is bounded by a positive integer $s_{\max}$ (this last condition is gauranteed by the definition of our algorithm under the rest of the assumptions). These last three assumptions are required to ensure that the merit function is well behaved with high probability, even though it is being updated based on stochastic gradient information. Exact definitions of these assumptions can be found in Section \ref{subsec:assumptions}.

Under the conditions listed above, after performing $k_{\max}+1$ iterations, our algorithm generates a point $x_{k^*}$ which satisfies, with probability at least $1-\delta$,
\bequation \label{eq:bigOcomplexity}
    \begin{split}
   \E[\|\nabla f(x_{k^*}) &+ J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c(x_{k^*})\| |
    E] \\
   &= \mathcal{O}\left(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c(x_0)\|_1 + M + (\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\right),
   \end{split}
\eequation
where $J_{k^*}$ is the Jacobian of the constraints at the point $x_{k^*}$, $y_{k^*}^{true}$ is the Lagrange multiplier at $x_{k^*}$, and $f_{\min}$ is a lower bound on $f(x)$.

The form of this result is commonly referred to as a convergence rate, however it can be easily manipulated into a worst-case complexity result. In terms of finding a point, $x_{k^*}$, such that $\E[\| \nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\| |E] \leq \varepsilon$ and $\E[\sqrt{\|c(x_{k^*})\|}|E] \leq \varepsilon$, by Jensen's inequality, our algorithm requires at most $\Ocal(\varepsilon^{-4})$ iterations.
As such, we use the terms complexity and convergence rate interchangably throughout.

The first three quantities in this result are essentially the same as those for the stochastic gradient method, representing the initial function gap as well as the variance. This is to be expected, given our mild assumptions on the matrices used in the quadratic subproblem at each iteration as well as the use of a single stochastic gradient at each iteration.

The final two terms are unique to our setting and arise due to the having a potentially poor initial estimate of $\tau_{\min}$. Given oracle knowledge of $\tau_{\min}$, these last two terms could be removed by choosing $\tau_{-1} \leq \tau_{\min}$ (as is done in the non-adaptive algorithm of \cite{SNa_MAnitescu_KMladen_2021}). However, this quantity is unknown so careful attention must be paid to the behaivor of the $\{\tau_k\}$ sequence to obtain a complexity result. The result holds in high probability due to the possibility of having an excessive number of iterations at which the computed $\tau_k$ is significantly larger than the value that the merit parameter would take if the step direction and merit parameter update were computed using the full gradient. On these types of iterations, the requirement for a bounded measure of asymmetry in the distribution of the stochastic gradients guarantees that there is always some nonzero probability of decreasing $\tau$. However, there still may exist realizations (which are guaranteed to occur with probability no more than $\delta$), where $\tau$ is ``too large" for enough iterations that the above complexity result does not hold.

We note that in terms of an overall complexity result with respect to the gradient of the Lagrangian, with probability at least $1-\delta$, we obtain a result which is the same order as the complexity result derived in \cite{DDavis_DDrusvyatskiy_2019}, whenever $s_{\max}$ satisfies a reasonable bound. Due to the definition of our algorithm, $s_{\max} = \mathcal{O}(\log(\tau_{\min}))$ for all sufficiently large $k_{\max}$. Thus, it follows that this complexity result gives an informative bound whenever $\tau_{\min}$ does not grow exponentially in $k_{\max}$. We prove that this is the case for sub-Gaussian distributions in Section \ref{subsec:subgauss}, where we show that, with probability at least $1-\delta$, $\tau_{\min} = \mathcal{O}(\log(\frac{k_{\max}}{\delta}))$ and
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O}\left(\frac{\log \log \frac{k_{\max}}{\delta}}{\sqrt{k_{\max}+1}}\right).
\eequationNN

%*********
% Section
%*********
\section{Algorithm}\label{sec.algorithm}

\subsection{Merit Function}

In Section \ref{sec:intro}, we introduced our $\ell$-1 penalty merit function in \eqref{eq:phidef}. The merit parameter $\tau$ is adaptively updated at each iteration and is used to define our line search procedure. We use a local model of the merit function $q : \R{n} \times \R{}_{>0} \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A key quantity in our algorithm is the reduction in the model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\Delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation} \label{eq:deltadef}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}
The reduction in the model of the merit function is a critical component of our complexity analysis. We will show that this can be used to give an upper bound on the merit function decrease at each iteration and thus it plays a similar role to the norm of the gradient squared in the analysis of stochastic gradient methods.

\subsection{Algorithm Preliminaries}

The algorithm that we develop for solving \eqref{eq:fdef} is based on a stochastic SQP paradigm. Specifically, at iteration $k$, a stochastic gradient estimate, $g_k$, is obtained (assumptions on the properties of $g_k$ can be found in Section \ref{subsec:assumptions}). Then, a search direction is computed by solving a quadratic optimization subproblem based on a stochastic local quadratic model of $f$ and a local affine model of $c$ about $x_k$. Letting $f_k := f(x_k)$, $c_k = c(x_k)$, and $J_k := \nabla c(x_k)^\top$ and given a sequence $\{H_k\}$ satisfying Assumption \ref{assum:Hk} below (a standard type of sufficiency condition for equality constrained optimization), this subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}

The optimal solution, $d_k$, of this subproblem, and an associated Lagrange multiplier, $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}


\begin{assumption} \label{assum:Hk}
    The sequence $\{H_k\}$ is bounded in norm by $\kappa_H \in \R{}_{>0}$. In addition, there exists a constant $\zeta \in \R{}_{>0}$ such that, for all $k = \{0,\dots,k_{\max}\}$, the matrix $H_k$ has the property $u^\top H_k u \geq \zeta \|u\|_2^2$ for all $u \in \R{n}$ such that $J_k u = 0$.
\end{assumption}

We stress that our algorithm and analysis does {\it not} assume that $H_k$ is a stochastic approximation of the Hessian of the Lagriangian at $x_k$ for some multiplier $y_k$. We merely assume that the sequence $\{H_k\}$ satisfies Assumption \ref{assum:Hk}.

Under Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk}, the following result is well known in the literature.

\blemma
    The linear system \eqref{eq:sqpsystem} has a unique solution.
\elemma

\subsection{Algorithm}

\begin{algorithm}[ht]
  \caption{Stochastic SQP Algorithm}
  \label{alg:ssqp}
  \begin{algorithmic}[1]
    \Require $x_0 \in \R{n}$; $\tau_{-1} \in \R{}_{>0}$; $\epsilon \in (0,1)$; $\sigma \in (0,1)$; $\xi_{-1} \in \R{}_{>0}$; $\kmax \in \N{}$; $\{\beta_k\} \subset (0,1]$; $\theta \in \R{}_{\geq0}$; $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$
    \For{\textbf{all} $k \in \{0,1,\dotsc,\kmax\}$}
	  \State Compute $(d_k,y_k)$ as the solution of \eqref{eq:sqpsystem}
	  \If{$d_k = 0$}
	    \State Set $\tau_k^{trial} \gets \infty$, $\tau_k \gets \tau_{k-1}$, $\xi_k^{trial} \gets \infty$, and $\xi_k \gets \xi_{k-1}$
	    \State Set $\widehat\alpha_{k,\text{init}} \gets 1$, $\widetilde\alpha_{k,\text{init}} \gets 1$, and $\alpha_k \leftarrow 1$
	  \Else\ (if $d_k \neq 0$)
	    \State Set $\tau_k^{trial}$ by \eqref{eq:tautrial} and $\tau_k$ by \eqref{eq:taudef} %\label{step.tau_stochastic}
	    \State Set $\xi_k^{trial}$  and $\xi_k$ by \eqref{eq:xidef} %\label{step.xi}
        \State Set
        \bequationNN
          \widehat\alpha_{k,\text{init}} \gets \tfrac{\beta_k\Delta q(x_k,\tau_k,g_k,H_k,d_k)}{(\tau_k L_k + \Gamma_k)\|d_k\|_2^2}\ \ \text{and}\ \  \widetilde\alpha_{k,\text{init}} \gets \widehat\alpha_{k,\text{init}} - \tfrac{4\|c_k\|_1}{(\tau_k L_k +  \Gamma_k)\|d_k\|_2^2}
        \eequationNN
        \State Set $\widehat\alpha_k \gets \proj_k(\widehat\alpha_{k,\text{init}})$ and $\widetilde\alpha_k \gets \proj_k(\widetilde\alpha_{k,\text{init}})$, then \label{step.alpha_projection_stochastic} \label{step.alpha_stochastic}
        \bequationNN
          \alpha_k \gets
		    \bcases
		      \widehat\alpha_k & \text{if $\widehat\alpha_k < 1$} \\
		      1 & \text{if $\widetilde\alpha_k \leq 1 \leq \widehat\alpha_k$} \\
		      \widetilde\alpha_k & \text{if $\widetilde\alpha_k > 1$}
		    \ecases
        \eequationNN
      \EndIf
      \State Set $x_{k+1} \gets x_k + \alpha_k d_k$
    \EndFor
    \State Sample $k^* \in \{0, \dotsc, \kmax\}$ according to the probability distribution
    \bequationNN
        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
    \eequationNN
    \Return $x_{k^*}$
  \end{algorithmic}
\end{algorithm}

After the search direction $d_k$ is computed, the merit parameter $\tau_k$ is updated. This is done by first setting, for some $\sigma \in (0,1)$, a trial value $\tau_k^{trial} \in \R{}_{>0} \cup  \{\infty\}$ by 
\bequation \label{eq:tautrial}
    \tau_k^{trial}\gets
    \begin{cases}
        \infty & \mbox{if $g_k^\top d_k + \max\{d_k^\top H_k d_k, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{g_k^\top d_k + \max\{d_k^\top H_k d_k,0\}} & \mbox{otherwise,}
    \end{cases}
\eequation
(If $c_k = 0$, then it follows from \eqref{eq:sqpsystem} and Assumption \ref{assum:Hk} that $d_k^\top H_k d_k \geq 0$ and $g_k^\top d_k + d_k^\top H_k d_k = 0$, meaning $\tau_k^{trial} \gets \infty$. Hence, $\tau_k^{trial} < \infty$ requires $\|c_k\|_1 > 0$, in which case $\tau_k^{trial} > 0$.) Then, the merit parameter is set, for some $\epsilon \in (0,1)$, by
\bequation \label{eq:taudef}
    \tau_k \gets \bcases
        \tau_{k-1} & \mbox{if $\tau_{k-1} \leq \tau_k^{trial}$} \\
        (1-\epsilon)\tau_k^{trial} & \mbox{otherwise,}
    \ecases
\eequation
which ensures that $\tau_k \leq \tau_k^{trial}$ and,
\bequation \label{eq:qquadlb}
    \Delta q(x_k,\tau,g_k,H_k,d_k) \geq \frac12 \tau \max\{d_k^\top H_k d_k, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
for any $\tau \leq \tau_k$.

Our algorithm adaptively estimates a lower bound for the ratio between the reduction in the model of the merit function and the merit parameter times the squared norm of the search direction. This is used to determine an interval into which the stepsize will be projected; control of this parameter is paramount to ensure convergence in expectation. We set
\bequation \label{eq:xidef}
    \xiktri \gets \frac{\Delta q(x_k, \tau_k, g_k, H_k, d_k)}{\tau_k \|d_k\|^2}
    \; \mbox{ then } \;
    \xi_k \gets \bcases
        \xi_{k-1} & \mbox{if }\xi_{k-1} \leq \xiktri \\
        (1-\epsilon)\xiktri & \mbox{otherwise,}
    \ecases
\eequation
which ensures $\xi_k \leq \xiktri$ for all $kb$. In previous work, it was show that $\{\xi_k\}$ is bounded away from zero {\it deterministically} \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

For generality, Algorithm \ref{alg:ssqp} is stated with Lipschitz constant estimates $\{L_k\}$ and $\{\Gamma_k\}$ given as inputs (with the idea that $\Gamma_k := \sum_{i \in 1,\dots,m} \gamma_{k,i}$ for all $k$). Our analysis in the next section presumes that Lipschitz constants are known, although in practice these can be estimated using standard techniques (see, e.g., \cite{FECurtis_DPRobinson_2019}) in an attempt to ensure that the same convergence results hold for the case where the constants are known. The sequence $\{\beta_k\}$ is introduced to control the setpsizes. Throughout most of the analysis, the sequence $\{\beta_k\}$ can be chosen arbitrarily. However, our final complexity result is established for a fixed step size of $\beta_k = \mathcal{O}(1/\sqrt{k_{\max}+1})$ for all $k\in\{0,\dots,k_{\max}\}$. We define
\bequationNN
    \mbox{Proj}_k(\cdot) := \mbox{Proj}\left(\cdot \; \Bigg| \left[\frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k}, \frac{\beta_k \xi_k \tau_k}{\tau_k L_k + \Gamma_k} + \theta \beta_k^2 \right]\right),
\eequationNN
where $\mbox{Proj}(\cdot \; | \; \mathcal{I})$ represents the projection operator onto the interval $\mathcal{I} \subset \R{}$.

We remark that the only substational changes from Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} are the fixed iteration count, $k_{\max}$, and the inclusion of a return value, $x_{k^*}$. Our method of sampling $k^*$ is consistent with the literature \cite{DDavis_DDrusvyatskiy_2019} and amounts to uniform sampling when a fixed step size sequence is employed.

%\balgorithm
%\caption{A Stochastic SQP Algorithm}
%\label{alg:ssqp}
%    \balgorithmic[1ht!]
%        \Require $x_0 \in \R{n};$ $\bar{\tau}_{-1} \in \R{}_{>0}$; $\epsilon \in (0, 1)$; $\sigma \in (0, 1);$ $\bar{\xi}_{-1} \in \R{}_{>0}$; $\{\beta_k\} \subset \R{}_{>0}$; $\theta \in \R{}_{>0};$ $\{L_k\} \subset \R{}_{>0}$; $\{\Gamma_k\} \subset \R{}_{>0}$; $K \in \N{}$
%        \State Run Algorithm 3.1 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for $k = 0, \dotsc, K$
%        \State Sample $k^* \in \{0, \dotsc, K\}$ according to the probability distribution
%        \bequationNN
%        \Prob(k^* = k) = \frac{\beta_k}{\sum_{k=0}^K \beta_k}
%        \eequationNN
%        \Return $x_{k^*}$
%    \ealgorithmic
%\ealgorithm

\section{Complexity Analysis} \label{sec:complexity}

In this section, we will prove our complexity result. We begin by describing our algorithm as a random process as well as the assumptions that we make on our stochastic gradient estimates (Section \ref{subsec:assumptions}). Then, we repeat (and sometimes slightly modify) a number of key lemmas from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} about Algorithm \ref{alg:ssqp} (Section \ref{subsec:algprops}). Afterwards, we present our complexity analysis and prove the result previewed in Section \ref{subsec:complexitypreview} (Section \ref{subsec:complexity}). We conclude this section by discussing distributions for which our assumptions are satisfied with high-probability (Section \ref{subsec:subgauss}) and outline a complexity result which relaxes one of our assumptions slightly (Section \ref{subsec:ratioparam}).

Our analysis relies on the orthogonal decomposition of the search directions given by $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$. We note here that conditioned on the algorithm having reached $x_k$ at iteration $k$, the normal component, $v_k$, is {\it deterministic}, depending only on the constraint value $c_k$ and the Jacobian $J_k$.

In addition to the quantities $d_k$, $y_k$, and $\tau_k^{trial}$ which are computed at each iteration using the stochastic gradient $g_k$, the following analysis relies on the quantities $\dktrue$, $\yktrue$, and $\tktritrue$ which are computed using the true gradient, $\nabla f(x_k)$. Specifically, let
\bequation \label{eq:sqpsystemdet}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    \dktrue \\ \yktrue
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    \nabla f(x_k) \\ c_k
    \end{matrix}
    \right]
\eequation
and
\bequationNN
    \tktritrue \gets
    \begin{cases}
        \infty & \mbox{if $\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue, 0\} \leq 0$} \\
        \frac{(1-\sigma)\|c_k\|_1}{\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}} & \mbox{otherwise}.
    \end{cases}
\eequationNN
Finally, we let $\dktrue = \uktrue + v_k$, where $\uktrue \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.

The definition of $\tktritrue$ guarantees that
\bequation \label{eq:qquadlbtrue}
    \Delta q(x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \frac12 \tau \max\{(\dktrue)^\top H_k \dktrue, 0\} + \sigma \|c_k\|_1 \geq 0,
\eequation
holds for any $\tau \leq \tktritrue$.

\subsection{Algorithm \ref{alg:ssqp} as a Stochastic Process and Assumptions} \label{subsec:assumptions}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(X_k,G_k,D_k,\Tcal_k,S_k,\Xi_k,R_k,\Acal_k)\},
\eequationNN
where
\bitemize
  \item $X_k$ is the algorithm iterate in iteration $k$,
  \item $G_k$ is the stochastic gradient in iteration $k$,
  \item $D_k$ is the search direction in iteration $k$,
  \item $\Tcal_k$ is the merit parameter in iteration $k$,
  \item $S_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\Xi_k$ is the ratio parameter in iteration $k$,
  \item $R_k$ is the number of ratio parameter decreases up to the end of iteration $k$, and
  \item $\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(X_k,G_k,D_k,\Tcal_k, S_k,\Xi_k,R_k,\Acal_k)$ is denoted as
\bequationNN
  (x_k,g_k,d_k,\tau_k,s_k,\xi_k,r_k,\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{G_0,\dots,G_{k-1}\}$, the realization of which (along with $X_0 = x_0$) determines the realization of
\bequationNN
  \{X_j\}_{j=1}^k\ \ \text{and}\ \ \{(D_j,\Tcal_j,S_j,\Xi_j,R_j,\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{0} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq 0}$ is a filtration. We condition on a specific realization of Algorithm \ref{alg:ssqp} up to iteration $k$, using the notation $g_{[k-1]}$, while we condition on $\Fcal_{k}$ to denote conditioning on all realizations of $G_{[k-1]}$ that are measurable with respect to the filtration $\Fcal_{k}$.

We consider a conditional model under the following assumption.

\bassumption\label{assum:eventE}
  Conditioned on the event $E := E(\kmax,s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    %\item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\xi_k = \xi_{\min} > 0$ for all $k \in \{0,\dots,\kmax\}$, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E, g_{[k-1]}] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E, g_{[k-1]}] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E, g_{[k-1]}, \nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \leq \ktaudec.
    \ealigned
  \eequationNN
\eassumption


The requirements on $G_k$ to be an unbiased estimator of $\nabla f(x_k)$ with bounded variance are standard for stochastic gradient methods. However, unlike the unconstrained setting, additional assumptions are required. The assumption on the existence of a $\tau_{\min} > 0$ is similar to Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, under which a global convergence result was proven. In Lemma 2.16 of the same work, it was proven that $\tktritrue$ has a deterministic lower bound. Based on this result, without loss of generality, we assume that $\tktritrue \geq \tau_{\min}$ holds for all $k$. In Proposition 3.18 of the same paper, the authors show that $\tau_{\min}$ exists with probability 1 whenever $G_k$ is a bounded random variable. We extend this result to show that $\tau_{\min}$ exists with high probability when $G_k$ follows a sub-Gaussian distribution in Section \ref{subsec:subgauss}.

By the definition of Algorithm \ref{alg:ssqp}, it should be clear that $s_{\max}$ in Assumption \ref{assum:eventE} must exist. Under the condition that $\tau_{\min} > 0$ exists, it follows that
\bequation \label{eq:smaxbound}
    s_{\max} \leq \min\left\{\kmax+1, \left\lceil\frac{\log(\tau_{\min}/\tau_{-1})}{\log(1-\epsilon)}\right\rceil\right\}.
\eequation
For the purposes of our analysis and results, we keep $s_{\max}$ decoupled from the above inequality as it is a fundamentally necessary component in order to guarantee that our results holds with high probability.

For convenience in the analysis, we make the assumption that the ratio parameter sequence $\{\xi_k\}$ is fixed. This sequence has a deterministic lower bound, as proven in Lemma 3.5 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, unlike the merit parameter sequence. In addition, this sequence is unique to our algorithm (and the algorithm in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}), while merit functions are a commonly used tool in constrained optimization. For this reason, we focus our attention on the properties of the merit parameter sequence instead. The approaches we develop for the merit parameter sequence can be applied to ratio parameter sequence as well. We outline a complexity result where both parameters are adaptively updated in Section \ref{subsec:ratioparam}.

Our final assumption requires that the stochastic gradient estimate is bounded in absolute value when conditioned on the event that $\tau_k < \tau_{k-1}$ and $\nabla f(x_k)^\top (d_k - \dktrue) < 0$ hold simultaneously. This event is fundamental in the analysis, as it arises naturally using $\Delta q(\cdot)$ as a measure of decrease in $\phi$ (see Lemma \ref{lem:phidecrease}). 
We remark that this inequality holds with high-probability whenever $G_k$ follows a sub-Guassian distribution with $\ktaudec = \Ocal(\log (k_{\max}))$. We prove this result in Section \ref{subsec:subgauss}.

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tktritrue$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tktritrue$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tktritrue$ occurs, we introduce the following assumption.

\begin{assumption} \label{assum:ptau}
At every iteration $k \in \{0,\dots,k_{\max}\}$,
\bequation
    \begin{split}
        \Prob[G_k^\top D_k &+ \max\{D_k^\top H_k D_k,0\} \\
        &\geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | E, g_{[k-1]}] \geq p_{\tau},
    \end{split}
\eequation
for some $p_{\tau} \in (0,1]$.
\end{assumption}
This assumption boils down to the distribution of $G_k$ having a bounded measure of asymmetry and is unique to our setting. It guarantees that there is always at least $p_{\tau}$ probability that $\tau_k$ decreases at any iteration for which $\tau_k$ would decrease if the step (and $\tau$ update) were computed using the full gradient, $\nabla f(x_k)$, as opposed to the stochastic gradient, $g_k$. This property ensures that, with high probability, $\tau_k$ is not larger than it ``should" be on too many iterations.

In \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, it was shown that this assumption is satisfied with $p_{\tau} = \frac12$ when $G_k$ is drawn from a Gaussian distribution. We show that this result can be extended to all distributions that obey a mild form of symmetry in Section \ref{subsec:subgauss}.

\subsection{Properties of Algorithm \ref{alg:ssqp}} \label{subsec:algprops}

Here we repeat a number of key results from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} that will be integral to our complexity analysis.

By Lemma 2.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for all $k = \{0,\dots,k_{\max}\}$, there exists $\kappa_{uv} \in \R{}_{>0}$ such that, if $\|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2$, then $\frac12 (\dktrue)^\top H_k \dktrue \geq \frac14 \zeta \|\uktrue\|^2$, where $\zeta$ is defined in Assumption \ref{assum:Hk}. Then, let
\bequationNN
    \Psi_k := \begin{cases}
        \|\uktrue\|^2 + \|c_k\| & \mbox{if } \|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2 \\
        \|c_k\| & \mbox{otherwise.}
    \end{cases}
\eequationNN
Now we can state a few lemmas which are relevant to our final complexity result.
\begin{lemma} \label{lem:kappapsi}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_{\Psi} \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$, the search true direction and constraint violation satisfy $\|\dktrue\|^2 + \|c_k\| \leq (\kappa_{\Psi} + 1) \Psi_k$.
\end{lemma}

\begin{proof}
    The result follows directly from Lemma 2.11 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

\begin{lemma} \label{lem:kappaq}
    Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_q \in \R{}_{>0}$ such that, for all $k \in \{0,\dots,k_{\max}\}$ and any $\tau \leq \tktritrue$, the reduction in the model of the merit function satisfies $\Delta q (x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \kappa_q \tau \Psi_k$.
\end{lemma}

\begin{proof}
    The proof follows from \eqref{eq:qquadlbtrue} combined with the proof of Lemma 2.12 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\end{proof}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and the a specific realization $g_{[k-1]}$.

Now, we can state a lemma about the expected values of a number of random variables in our algorithm.

\blemma \label{lem:dexpectation}
Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. For all $k = \{0,\dots,k_{\max}\}$, $\E_k[D_k] = \dktrue$, $\E_k[U_k] = \uktrue$, and $\E_k[Y_k] = \yktrue$.  Moreover, there exists $\kappa_d \in \R{}_{>0}$, independent of $k$, such that,
\bequationNN
\left\|\left[\begin{matrix}
H_k & J_k^\top \\
J_k & 0
\end{matrix}\right]\right\| \leq \kappa_d.
\eequationNN
In addition, $\E_k[\|D_k - \dktrue\|] \leq \kappa_d \sqrt{M}$, and $\E_k[\|D_k - \dktrue\| | E, \mathcal{F}_k, \nabla f(x_k)^\top (D_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \leq \kappa_d \ktaudec$.
\elemma

\bproof
    Except for the final inequality, the result is proven in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. To see the final inequality, we note that by the same argument as in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2020}, for any realization of $G_k$ and $D_k$,
    \bequationNN
        \|d_k - \dktrue\| \leq \kappa_d \|g_k - \nabla f(x_k)\|.
    \eequationNN
    Therefore,
    \begin{align*}
        &\E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \E_k[\|G_k - \nabla f(x_k)\| | \nabla f(x_k)^\top (d_k - \dktrue) < 0, \tau_k < \tau_{k-1}] \\
        &\quad \leq \kappa_d \ktaudec.
    \end{align*}
\eproof

Next, we provide some bounds on the expectation of a few key quantities.

\blemma\label{lem:product_bounds}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequationNN 
    \begin{split}
        \nabla f(x_k)^\top \dktrue &\geq \E_k[G_k^\top D_k] \geq \nabla f(x_k)^\top \dktrue - \zeta^{-1}M\ \ \text{and} \\ \E_k[D_k^\top H_k D_k] &\geq (\dktrue)^\top H_k \dktrue.
    \end{split}
  \eequationNN
\elemma

\bproof
    The result is proven in Lemma \cite[Lemma 3.9]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

We conclude this section with a lemma that will allow us to characterize descent in $\phi$ in terms of $\Delta q(\cdot)$.

\blemma\label{lem:phidecrease}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Suppose that $\{\beta_k\}$ is chosen such that $\beta_k \xi_k \tau_k/(\tau_k L + \Gamma) \in (0,1]$ for all $k \in \{0,\dots,k_{\max}\}$.  Then, for all $k \in \{0,\dots,k_{\max}\}$, it follows that
  \bequation \label{eq:phidecrease}
    \baligned
      \phi(x_k + \alpha_k d_k, \tau_k) - \phi(x_k, \tau_k)
      &\leq -\alpha_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue) \\
      &\quad + \thalf \alpha_k \beta_k  \Delta q(x_k,\tau_k,g_k,H_k,d_k) \\
      &\quad + \alpha_k \tau_k \nabla f(x_k)^\top (d_k - \dktrue),
    \ealigned
  \eequation
  where $d_k$ and $\dktrue$ are respectively defined by \eqref{eq:sqpsystem} and \eqref{eq:sqpsystemdet}.
\elemma

\bproof
    The result follows directly from Lemma 3.7 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}.
\eproof

\subsection{Complexity Result} \label{subsec:complexity}

In this section, we present our complexity result under the condition that Assumption \ref{assum:eventE} occurs. We derive our result in largely the same way as the global convergence result in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}, with two major changes, which stem from the need to characterize the behavior of the algorithm with respect to the merit parameter updating. At a high-level, the two modifications are as follows:
\begin{enumerate}
    \item We derive a new upper bound for the last term in \eqref{eq:phidecrease}. This inequality allows us to characterize decrease in the merit function and is central to the overall analysis. A new upper bound is needed in our setting, as this final term is the product of three random variables while $\tau$ is still being adaptively updated and has not settled at a lower bound. To handle this, we show that this term is bounded, under Assumption \ref{assum:eventE}, in terms of the probability that the event $\Ek3$ (defined formally below) occurs at iteration $k$. This event only occurs on iterations $k$ where $\tau_k < \tau_{k-1}$ which, when combined with a maximum of $s_{\max}$ decreases of $\tau$ due to Assumption \ref{assum:eventE}, allows us to obtain a bound on this quantity that holds with high-probability. The new upper bound is derived in Lemma \ref{lem:innerprod} while our high-probability bound on the summation (over $k=0,\dots,k_{\max}$) of the probabilities of $\Ek3$ occuring is presented in Lemma \ref{lem:Eksumlsmax}.
    \item We characterize iterations at which $\tktritrue < \tau_k$ occurs. These iterations are problematic for the analysis due to the inclusion of $\tau_k$ in $\Delta q(x_k,\tau_k,\nabla f(x_k), H_k, \dktrue)$, which is used during the analysis to measure progress in the algorithm. One particular concern arises in the final complexity result; if $k^*$ occurs at an iterate such that $\tau_{k^*}^{trial,\text{true}} < \tau_{k^*}$, then $\Delta q(x_{k^*},\tau_{k^*},\nabla f(x_{k^*}), H_{k^*}, d^{\text{true}}_{k^*})$ cannot be related to our optimality conditions \eqref{eq:optconds}. To solve this issue, we introduce a theoretical sequence, $\hat{\tau}_k$, which, for all $k$, is the minimum of $\tau_k$ and $\tktritrue$, and analyze the algorithm's progress with respect to this sequence. Due to Assumption \ref{assum:ptau}, whenever the event $\tktritrue < \tau_k$ occurs, there is at least $p_{\tau}$ probability of decreasing $\tau$. Taken in combination with $s_{\max}$ from Assumption \ref{assum:eventE}, this enables us to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ occurs. We introduce Lemma \ref{lem:dqbound} and Lemma \ref{lem:hattaudiff} to handle iterations such that $\tktritrue < \tau_k$. Additionally, we derive Lemma \ref{lem:Ktaulsmax} to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ can occur.
\end{enumerate}

Now, we analyze the first modification mentioned above. As in the previous section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event $E$ and a specific realization $g_{[k-1]}$.

Our analysis relies on the following three events. For all $k \in \{0,\dotsc,\kmax\}$, let $\Ek1$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) \geq 0$, let $\Ek2$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} = \tau_{k-1}$, and let $\Ek3$ be the event that $\nabla f(x_k)^\top(D_k - \dktrue)$ and $\Tcal_{k} < \tau_{k-1}$.

Now, we derive a bound on the final term in \eqref{eq:phidecrease}.

\begin{lemma} \label{lem:innerprod}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$, the existence of which follows under Assumption \ref{assum:fcsmooth}. Let
\bequationNN
\alpha_{\min,k} := \frac{\beta_k \xi_{\min} \tau_{\min}}{\tau_{\min}L_k + \Gamma_k} \mbox{ and } \alpha_{\max,k} := \frac{\beta_k \xi_{\min} \tau_{k-1}}{\tau_{k-1}L_k + \Gamma_k},
\eequationNN
where $\tau_{\min}$ and $\xi_{\min}$ are defined as in Assumption \ref{assum:eventE}.

Then, with $\kappa_d \in \R{}_{>0}$ defined by Lemma \ref{lem:dexpectation},
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq  (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek1], \\
\E_{k,2} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek2], \\
\E_{k,3} &= \E_k[\nabla f(x_k)^\top(D_k - \dktrue)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\tau_{\min}$, $\alpha_{\min,k}$, and $\alpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &= \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek1] \Prob_k[\Ek1] + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By the Law of Total Expectation and Lemma \ref{lem:dexpectation}, this means that
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\tau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob_k[\Ek2]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, we have
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{k-1} \alpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{k-1} \alpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{k-1} \alpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \tau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob_k[\Ek1]
    + (\tau_{\min} \alpha_{\min,k} - \tau_{k-1} \alpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    &\leq \tau_{\min} \alpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \tau_{\min} \alpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \tau_{\min} \alpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\tau_{k-1} (\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \\
    &\quad+ (\tau_{k-1} \alpha_{\max,k} - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}
Summing these three inequalities,
\begin{align}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \nonumber \\
    &\leq \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+\frac13(\tau_{k-1} (\alpha_{\max,k} - \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+\frac13(2 \tau_{\min} \alpha_{\min,k} - \tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \nonumber \\
    &= \frac13(\tau_{k-1}(\alpha_{\max,k} + 2\theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -\theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-\frac13(\tau_{k-1}(2\alpha_{\max,k} + \theta \beta_k^2) - 2 \tau_{\min} \alpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]. \label{eq:innerprodproof1}
\end{align}
Now, by Lemma \ref{lem:dexpectation},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|\nabla f(x_k)\| \E_k[\|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[\nabla f(x_k)^\top(D_k - \dktrue)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek2] \Prob_k [\Ek2] \\
    &= \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \\
    &\leq \kappa_g \E_k[\|D_k - \dktrue\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma \ref{lem:dexpectation}. Using these three inequalities with
\eqref{eq:innerprodproof1}, yields
\begin{align*}
    \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)]
    &\leq (\tau_{k-1}(\alpha_{\max,k} + \theta \beta_k^2) - \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
which proves the result.
\end{proof}

Now, we turn our attention to the second modification mentioned in the outline of this section. Our complexity result is derived through the use of \eqref{eq:phidecrease}, which relates decrease in our merit function to $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$. On any iteration for which $\tau_k \leq \tktritrue$ holds, $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$ can be directly related to the optimality conditions defined in \eqref{eq:optconds}. Unfortunately, the same is not true for $k$ such that $\tau_k > \tktritrue$. Thus, in order to provide an informative bound on such iterations, we introduce the following sequence:
\bequation \label{eq:hattaudef}
    \hat{\Tcal}_k := \min\{\Tcal_k, \tktritrue\},
\eequation
which we will use throughout the rest of the analysis (note that because we are conditioned on the history up to the start of iteration $k$, $\Tcal_k$ is a random variable, while $\tktritrue$ is not).

Now, we derive a bound on the conditional expectation of $\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)$ using the definition of $\hat{\Tcal}_k$.

\begin{lemma} \label{lem:dqbound}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|\nabla f(x_k)\|_2\}$ and let $\kappa_d$ be defined as in Lemma \ref{lem:dexpectation}. Let $\hat{\Tcal}_k$ be defined in \eqref{eq:hattaudef}. Then,
\begin{align*}
    \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)]
    &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
    +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
    &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
    &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)).
\end{align*}
\end{lemma}

\begin{proof}
    To begin, by the definition of \eqref{eq:deltadef},
    \begin{align}
        &\E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \nonumber \\ &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k, 0\}) + \|c_k\|_1] \nonumber \\
        &= \E_k[-\hat{\Tcal}_k(G_k^\top D_k - \nabla f(x_k)^\top \dktrue  + \frac12 \max\{D_k^\top H_k D_k, 0\} \nonumber \\
        &\quad- \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] \nonumber \\ &\quad+ \E_k[-\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\})] + \|c_k\|_1 \nonumber \\
        &= \E_k[\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} \nonumber \\
        &\quad- \frac12 \max\{D_k^\top H_k D_k, 0\})] + \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]. \label{eq:dqbound1}
    \end{align}
    Now, for simplicity of notation, let \tred{TODO: Figure out if there's a better name than $Z_k$.}
    \bequationNN
        Z_k =  \nabla f(x_k)^\top \dktrue - G_k^\top D_k + \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12 \max\{D_k^\top H_k D_k, 0\}.
    \eequationNN
    Let $E_Z$ denote the event that $Z_k \geq 0$ occurs and let $E_Z^c$ denote the event that $Z_k < 0$ occurs. Then, by the Law of Total Expectation,
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k] &= \E_k[\hat{\Tcal}_k Z_k | E_Z] \Prob_k[E_Z] + \E_k[\hat{\Tcal}_k Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Therefore, by the Law of Total Probability, Lemma \ref{lem:product_bounds}, Jensen's inequality, and convexity of $\max\{\cdot,0\}$, it follows that
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{k-1} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{k-1} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} \E_k[Z_k] + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &= \tau_{k-1} (\nabla f(x_k)^\top \dktrue - \E_k[G_k^\top D_k] \\
        &\quad+ \frac12 \max\{(\dktrue)^\top H_k \dktrue, 0\} - \frac12\E_k[\max\{D_k^\top H_k D_k, 0\}]) \\
        &\quad+ (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\leq \tau_{k-1} \zeta^{-1} M + (\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c].
    \end{align*}
    Similarly, we have
    \begin{align*}
        \E_k[\hat{\Tcal}_k Z_k]  &\leq \tau_{\min} \E_k[Z_k | E_Z] \Prob_k[E_Z] + \tau_{\min} \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &= \tau_{\min} \E_k[Z_k] + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \\
        &\leq \tau_{\min} \zeta^{-1} M + (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z].
    \end{align*}
    Summing these two inequalities yields
    \begin{align}
        \E_k[\hat{\Tcal}_k Z_k] &\leq \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M + \frac12 (\tau_{k-1} - \tau_{\min}) \E_k[Z_k | E_Z] \Prob_k[E_Z] \nonumber \\
        &\quad+ \frac12(\tau_{\min} - \tau_{k-1}) \E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] \label{eq:dqbound2}.
    \end{align}
    Next, we note that by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, Jensen's inequality, and the concavity of the square root,
    \begin{align*}
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] &\leq 
        \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top \dktrue|] +\E_k[|G_k^\top \dktrue - G_k^\top D_k|] \\
        &\leq \|\dktrue\| \E_k [\|\nabla f(x_k) - G_k\|] + \E_k[\|G_k\|\|\dktrue - D_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]} \\ &\quad+ \kappa_d \E_k[(\|G_k - \nabla f(x_k)\| + \|\nabla f(x_k)\|) \|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d \E_k[\|\nabla f(x_k) - G_k\|^2] \\
        &\quad+ \kappa_d \|\nabla f(x_k)\| \E_k[\|\nabla f(x_k) - G_k\|] \\
        &\leq \kappa_d \kappa_g \sqrt{M} + \kappa_d (M + \kappa_g \sqrt{M}) = \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}).
    \end{align*}
    In addition, by the Cauchy-Schwarz inequality, Lemma \ref{lem:dexpectation}, Assumption \ref{assum:eventE}, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
        &\leq \|H_k\|\|\dktrue\|^2 + \|H_k\|\E_k[\|D_k\|^2] \\
        &\leq \kappa_H \kappa_d^2 \kappa_g^2 + 2\kappa_H \kappa_d^2 (\E_k [\|G_k - \nabla f(x_k)\|^2] + \kappa_g^2) \\
        &\leq \kappa_H \kappa_d^2 (3\kappa_g^2 + 2 M).
    \end{align*}
    Now, by the Law of Total Expectation and the above two inequalities,
    \begin{align*}
         \E_k[Z_k | E_z] \Prob_k[E_Z] &= \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    By the same argument,
    \begin{align*}
         -\E_k[Z_k | E_Z^c] \Prob_k[E_Z^c] &\leq \E_k[|Z_k| | E_Z^c] \Prob_k[E_Z^c] \\
         &= \E_k[|Z_k|] - \E_k[|Z_k| | E_Z] \Prob_k[E_Z] \\
         &\leq \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \\
         &\quad+ \frac12\E_k[|\max\{(\dktrue)^\top H_k \dktrue, 0\} - \max\{D_k^\top H_k D_k, 0\}|] \\
         &\leq \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M).
    \end{align*}
    Thus, combining this with \eqref{eq:dqbound1} and \eqref{eq:dqbound2},
    \begin{align*}
        \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] &\leq \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]
        +  \frac{\tau_{k-1} + \tau_{\min}}{2} \zeta^{-1} M \\
        &\quad+ (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) \\
        &\quad+ \frac12\kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)),
    \end{align*}
    proving the result.
\end{proof}

Next, we introduce a lemma which controls the difference in $\Delta q(\cdot)$ on iterations where $\tktritrue < \Tcal_k$.
\begin{lemma} \label{lem:hattaudiff}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d),
    \end{align*}
    and
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k, \Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \kappa_d (M + \kappa_g^2) (2 + \kappa_H \kappa_d),
    \end{align*}
    where $\alpha_{\min,k}$ and $\alpha_{\max,k}$ are defined in Lemma \ref{lem:innerprod}.
\end{lemma}

\begin{proof}
    By the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
        &= \E_k[\Acal_k (\Tcal_k - \hat{\Tcal}_k) (\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) |\nabla f(x_k)^\top \dktrue + \frac12 \max\{(\dktrue)^\top H_k \dktrue,0\}| \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \kappa_g^2 + \thalf\kappa_H \kappa_d^2 \kappa_g^2).
    \end{align*}
    Next, by the definitions of $\kappa_H$, $\kappa_g$, $\kappa_d$, and $\|a+b\|^2 \leq 2\|a\|^2 + 2\|b\|^2$,
    \begin{align*}
        &\E_k[\Acal_k \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
        &= \E_k[\Acal_k (\hat{\Tcal}_k - \Tcal_k) (G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\})] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) \E_k[|G_k^\top D_k + \frac12 \max\{D_k^\top H_k D_k,0\}|] \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (\kappa_d \E_k[\|G_k\|^2] + \thalf \kappa_d^2 \kappa_H \E_k[\|G_k\|^2]) \\
        &\leq (\alpha_{\max,k} \tau_{k-1} - \alpha_{\min,k} \tau_{\min}) (2\kappa_d (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2) \\
        &\quad+ \kappa_d^2 \kappa_H (\E_k[\|G_k - \nabla f(x_k)\|^2] + \|\nabla f(x_k)\|^2)) \\
        &\leq (\alpha_{\max,k} \tau_k - \alpha_{\min,k} \hat{\tau}_k) (2\kappa_d (M + \kappa_g^2) + \kappa_d^2 \kappa_H (M + \kappa_g^2)).
    \end{align*}
\end{proof}

Next, we present the statements of two lemmas, which provide upper bounds, in high probability, on key components of the complexity result. The proofs of these lemmas are relegated to Appendix \ref{app:simple} for presentation purposes. Both of these lemmas use the following function in their statement. For any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, let
\bequation \label{eq:lsd}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\eequation

Now we can state the first lemma, which gives a high-probability bound on the sum of the probabilities from applying Lemma \ref{lem:innerprod} at each iteration.

\begin{lemma} \label{lem:Eksumlsmax}
    Let Assumption \ref{assum:eventE} hold. Then,
    \bequation \label{eq:Ek3lsmax}
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob [E_{k,3} | E, \mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\Bigg | E \right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Before stating the next lemma, recall the definition of $\hat{\Tcal}_k$ in \eqref{eq:hattaudef} and let
$k_{\tau}$ denote the index set
\bequation \label{eq:smallktau}
    k_{\tau} := \{k : \tktritrue < \tau_{k-1}\}.
\eequation
In addition, we let
$\mathcal{K}_{\tau}$ denote the associated random index set
\bequation \label{eq:Ktau}
    \mathcal{K}_{\tau} := \{k : \tcalktritrue < \Tcal_{k-1}\}.
\eequation
By the definitions of $\Tcal_k$, $\tcalktritrue$, and $\hat{\Tcal}_k$, this set of iterations is a superset of the iterations at which $\hat{\Tcal}_k < \Tcal_k$ occurs and can therefore be used to characterize the number of iterations at which this event occurs. In addition, the event $\tktritrue < \tau_{k-1}$ does {\it not} depend on $G_k$, which makes it more convenient to work with analytically. In particular, this means that $G_k$ is conditionally independent of the event $\tktritrue < \tau_{k-1}$ given $g_{[k-1]}$ and $E$.

In the following lemma, we bound the cardinality of $\Kcal_{\tau}$ with high probability.

\begin{lemma} \label{lem:Ktaulsmax}
    Let Assumptions \ref{assum:eventE} and \ref{assum:ptau} hold. Let $\mathcal{K}_{\tau} = \{k : \tcalktritrue < \Tcal_{k-1}\}$. Then,
    \bequation \label{eq:Ktaulsmax}
        \Prob\left[|\mathcal{K}_{\tau}| \leq \left\lceil \frac{\ell(s_{\max},\delta)+1}{p_{\tau}}\right\rceil \Bigg| E\right] \geq 1-\delta.
    \eequation
\end{lemma}

\begin{proof}
    This result is proven in Appendix \ref{app:simple}.
\end{proof}

Now we are prepared to state our complexity result in terms of $\Delta q(\cdot)$.

\begin{theorem} \label{thm:complexity}
Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold. 
Let the sequence $\{\hat{\Tcal}_k\}$ be defined in \eqref{eq:hattaudef}.

Define 
\bequationNN
A_{\min} := \frac{\xi_{\min} \tau_{\min}}{\tau_{\min}L + \gamma} \mbox{ and }
A_{\max} := \frac{\xi_{-1} \tau_{-1}}{\tau_{-1}L + \gamma}
\eequationNN
as well as
\begin{align*}
\hat{M} &:= \frac12 A_{\max} (\tau_{-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M})
+ \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M))\\ 
&\quad \ + \frac{\tau_{-1} + \tau_{\min}}{4} A_{\max} \zeta^{-1} M + \theta \tau_{-1} \kappa_g \kappa_d \sqrt{M},
\end{align*}
and
\begin{align*}
    \kappa_{\Delta q} &:= \beta (A_{\max} \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d (2M + 3\kappa_g^2) (1 + \frac12 \kappa_H \kappa_d), \\
    \kappa_{E_3} &:= \beta (\tau_{-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec.
\end{align*}
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{k_{\max}+1}} \quad \mbox{ for some } \quad \gamma \leq \frac{A_{\min}}{A_{\max} + \theta}.
\eequationNN
Then,
\begin{align}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \nonumber \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \nonumber \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil. \label{eq:complexity}
\end{align}
\end{theorem}

\begin{proof}
By Lemma \ref{lem:phidecrease} and Lemma \ref{lem:innerprod},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) \\
    &\quad + \Acal_k \Tcal_k \nabla f(x_k)^\top (D_k - \dktrue)] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}

First, we focus on iterations where $k \in k_{\tau}^c$ so that $\tktritrue \geq \tau_{k-1}$ and thus, $\tau_k \leq \tktritrue$. We mention once again that $G_k$ is conditionally independent of the event $\tktritrue \geq \tau_{k-1}$ given $E$ and $g_{[k-1]}$. Therefore, by \eqref{eq:qquadlb}, \eqref{eq:qquadlbtrue}, and Lemma \ref{lem:dqbound},
\begin{align*}
    &\E_k [\phi(x_k + \alpha_k D_k, \Tcal_k) | k \in k_{\tau}^c] - \E_k [\phi(x_k, \Tcal_k) | k \in k_{\tau}^c] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in k_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &=\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in k_{\tau}^c] \\
    &\quad +(\tau_{k-1}(\alpha_{\max,k} + \theta \beta^2) -    \tau_{\min} \alpha_{\min,k}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3 | k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}. \\
    &\leq -\beta (A_{\min} - \frac12 (A_{\max}+\theta) \beta) \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] + \frac{\tau_{k-1} + \tau_{\min}}{4} \beta^2 A_{\max} \zeta^{-1} M \\
    &\quad+ \frac12 \beta^2 A_{\max} (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \frac12 \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)) \\
    &\quad+ \beta (\tau_{k-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d \ktaudec \Prob_k[\Ek3| k \in k_{\tau}^c]
    + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] + \kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}^c] + \beta^2 \hat{M}.
\end{align*}

Now, we condition on $k \in k_{\tau}$. Once again, $G_k$ is conditionally independent of this event given $g_{[k-1]}$ and $E$. By (\ref{eq:qquadlb}), (\ref{eq:qquadlbtrue}), Lemma \ref{lem:dqbound}, and Lemma \ref{lem:hattaudiff},
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) | k \in k_{\tau}] - \E_k [\phi(x_k, \Tcal_k) | k \in k_{\tau}] \\
    &\leq \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | k \in k_{\tau}] \\
    &\quad+\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in k_{\tau}] \\
    &\quad-\E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)
    + \frac12 \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | k \in k_{\tau}] \\
    &\quad+ \kappa_{E_3} \Prob_k[\Ek3 | k \in k_{\tau}] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}] + \kappa_{\Delta q} \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}] + \beta^2 \hat{M}.
\end{align*}

Now by the law of total probability and the law of total expectation,
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &=\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] \\
    &\quad+ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in k_{\tau}] \Prob_k[k \in k_{\tau}] \\
    &\leq -\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}] \Prob_k[k \in k_{\tau}] + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}] \Prob_k[k \in k_{\tau}] + \beta^2 \hat{M} \Prob_k[k \in k_{\tau}] \\
    &\quad-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] + \beta^2 \hat{M} \Prob_k[k \in k_{\tau}^c] \\
    &=-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3}] + \beta^2 \hat{M} + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}]
\end{align*}

Summing this inequality for all $k \in \{0,\dots,k_{\max}\}$,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \sum_{k=0}^{k_{\max}} (-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{E_3} \Prob_k[E_{k,3}] + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}]) \\
    &\quad+ (k_{\max}+1) \beta^2 \hat{M}.
\end{align*}

Now, let $g_{[\kmax]} : = \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that are measurable with respect to the filtration $\mathcal{F}_{k_{\max}+1}$. Note that $\Prob_k[k \in k_{\tau}] \in \{0,1\}$ since the event $k \in k_{\tau}$ does not depend on $G_k$ when conditioned on $\Fcal_k$ and $E$. Therefore, by total expectation, the definition of $\Fcal_{\kmax+1}$, Lemma \ref{lem:Eksumlsmax}, Lemma \ref{lem:Ktaulsmax}, and the union bound, with probability at least $1-\hat{\delta}$,
\begin{align}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k)| E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \nonumber \\
    &= \int_{g_{[\kmax]} \in \mathcal{F}_{k_{\max}+1}} \sum_{k=0}^{k_{\max}} \E [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k,\Tcal_k) | E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] f_{G}(g) dg \nonumber \\
    &\leq \int_{g_{[\kmax]} \in \mathcal{F}_{k_{\max}+1}} \Bigg(-\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)|E,G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \nonumber \\
    &\quad+ \kappa_{\Delta q} \sum_{k=0}^{k_{\max}} \Prob[k \in k_{\tau}|E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] + \kappa_{E_3}\sum_{k=0}^{\kmax} \Prob[\Ek3 |  E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \Bigg) f_{G}(g) dg \nonumber \\
    &\quad+(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &= -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E, \Fcal_k] + \kappa_{\Delta q} \E\big[|\mathcal{K}_{\tau}|\big|E\big] \nonumber \\
    &\quad+ \kappa_{E_3}\sum_{k=0}^{\kmax} \Prob[\Ek3 | E, \Fcal_k] +(k_{\max}+1) \beta^2 \hat{M} \nonumber \\
    &\leq -\frac12 \beta A_{\min} \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E, \Fcal_k] + \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\hat{\delta}/2)+1}{p_{\tau}}\right\rceil \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(s_{\max},\hat{\delta}/2)+1) +(k_{\max}+1) \beta^2 \hat{M}, \label{eq:complexityproof1}
\end{align}
where $f_{G}(g)$ is the probability density function of the random variable $G$. Working with left side of this inequality,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k f(X_k + \Acal_k D_k) + \|c(X_k + \Acal_k D_k)\|_1 | E,\Fcal_k] - \E[\Tcal_k f(X_k) + \|c(X_k)\|_1 | E,\Fcal_k] \\
    &= \sum_{k=0}^{k_{\max}} \E [\Tcal_k (f(X_k + \Acal_k D_k) - f_{\min}) + \|c(X_k + \Acal_k D_k)\|_1 | E,\Fcal_k] - \E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E,\Fcal_k].
\end{align*}
It follows by the monotonicity of the $\Tcal_k$ sequence that
\bequationNN
-\E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_k] \geq - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_k].
\eequationNN
Thus,
\begin{align*}
    &\sum_{k=0}^{k_{\max}} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \\
    &\geq \E [\Tcal_{k_{\max}} (f(X_{k_{\max}+1}) - f_{\min}) + \|c(X_{k_{\max}+1})\|_1 | E,\Fcal_k] - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1.
\end{align*}
Combining this with \eqref{eq:complexityproof1},
\begin{align*}
    &\beta \sum_{k=0}^{k_{\max}} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E,\Fcal_k] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min}} \\
    &\quad+ \frac{2 (k_{\max}+1) \beta^2 \hat{M}}{A_{\min}} + \frac{2}{A_{\min}} \kappa_{\Delta q} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
Dividing both sides of this inequality by the summation of $\beta$,
\begin{align*}
    &\frac{1}{\sum_{k=0}^{k_{\max}} \beta} \sum_{k=0}^{k_{\max}} \beta \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E,\Fcal_k] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 (k_{\max}+1) \beta^2 \hat{M} + \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \sum_{k=0}^{k_{\max}} \beta} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil,
\end{align*}
so that by the definitions of $K^*$ and $\beta$,
\begin{align*}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1)}{A_{\min} \gamma \sqrt{k_{\max}+1}} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
\end{proof}

Now we convert this into a result in terms of our optimality conditions \eqref{eq:optconds}.

\begin{corollary} \label{coro:complexity}
    Let the assumptions of Theorem \ref{thm:complexity} hold. Then, with probability at least $1-\delta$,
    \begin{align}
        &\E\left[\frac{\|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\|^2}{\kappa_H^2} + \|c(X_{K^*})\| \Bigg| E\right] \nonumber \\
        &\leq \frac{(\kappa_{\Psi} + 1)(2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(s_{\max},\delta/2)+1))}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \label{eq:coro} \\
        &\quad+ \frac{2 (\kappa_{\Psi} + 1) \kappa_{\Delta q}}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{k_{\max}+1}} \left\lceil\frac{\ell(s_{\max},\delta/2)+1}{p_{\tau}}\right\rceil \nonumber. 
    \end{align}
\end{corollary}

\begin{proof}
    The result follows by Lemma \ref{lem:kappapsi}, Lemma \ref{lem:kappaq}, and Theorem \ref{thm:complexity} combined with \eqref{eq:sqpsystemdet}, which implies that
    \bequationNN
        \|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\| = \|H_{k^*} D^{true}_{K^*}\| \leq \kappa_H \|D^{true}_{K^*}\|.
    \eequationNN
\end{proof}

We remark again that this result, in terms of the norm of the gradient of the Lagrangian, matches the worst-case complexity of the projected stochastic gradient method \cite{DDavis_DDrusvyatskiy_2019}.

\subsection{Complexity Result for Symmetric Sub-Gaussian Distributions} \label{subsec:subgauss}

In this section, we show that Assumptions \ref{assum:eventE} and \ref{assum:ptau} occur with high probability when the stochastic gradient $G_k$ follows a symmetric, sub-Gaussian distribution.

Throughout this section, we work with the following assumption.

\begin{assumption} \label{assum:symmsubgauss}
    At every iteration $k = \{0,\dots,k_{\max}\}$, the stochastic gradient $G_k$ satisfies
    \bequation
        \E[G_k | g_{[k-1]}] = \nabla f(x_k),
    \eequation
    \bequation \label{eq:subgauss}
        \E[\exp(\|\nabla f(x_k)-G_k\|^2/M) | g_{[k-1]}] \leq \exp(1),
    \eequation
    and the quantities $G_k - \nabla f(x_k)$ and $\nabla f(x_k) - G_k$ are equivalent in distribution. Finally, for all $k = \{0,\dots,k_{\max}\}$, the ratio parameter $\xi_k$ satisfies $\xi_k = \xi_{\min}$.
\end{assumption}

The above assumption has a number of important implications. The first is that Assumption \ref{assum:ptau} occurs (without conditioning on event $E$) with $p_{\tau} = \frac12$, as we show in the following lemma.

\blemma \label{lem:subgptau}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then,
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | g_{[k-1]}] \geq \frac12.
    \eequationNN
\elemma

\bproof
    Let $Z_k$ be a basis for the null space of $J_k$, which under Assumption \ref{assum:fcsmooth} is a matrix in $\R{n\times(n-m)}$. Then, let $W_k$ be such that $U_k = Z_k W_k$ and $\wktrue$ be such that $\uktrue = Z_k \wktrue$. It follows from the first block in \eqref{eq:sqpsystem} that 
    \bequationNN
        H_k (Z_k W_k + v_k) + J_k^\top Y_k = -G_k \Longleftrightarrow Z_k W_k = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (G_k + H_k v_k).
    \eequationNN
    Using this equality and simplifying,
    \bequationNN
        G_k^\top D_k + D_k^\top H_k D_k = v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} G_k + H_k^{1/2} v_k).
    \eequationNN
    In a similar fashion, by \eqref{eq:sqpsystemdet},
    \bequationNN
        Z_k \wktrue = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (\nabla f(x_k) + H_k v_k)
    \eequationNN
    so that
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + (\dktrue)^\top H_k \dktrue \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} \nabla f(x_k) + H_k^{1/2} v_k).
    \end{align*}

    Then,
    \begin{align*}
        &G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (G_k -\nabla f(x_k))),
    \end{align*}
    and,
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (\nabla f(x_k) - G_k)),
    \end{align*}
    are equivalent in distribution by Assumption \ref{assum:symmsubgauss}. Therefore,
    \begin{align*}
        &\Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &=\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}].
    \end{align*}
    In addition, we have
    \begin{align*}
        1 &= \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &+\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}] \\
        &-\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} = 0 | g_{[k-1]}].
    \end{align*}
    Taking these two together, it follows that
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \geq \frac12,
    \eequationNN
    proving the claim.
\eproof

Next, we repeat a well known property of sub-Gaussian random variables.
\blemma \label{lem:subgboundedrv}
    Suppose Assumption \ref{assum:symmsubgauss} holds. Then, for any $\delta \in (0,1)$,
    \bequation \label{eq:subgboundedrv}
        \Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} | g_{[k-1]}\right] \geq 1 - \delta.
    \eequation
\elemma

\bproof
    By Markov's inequality and Assumption \ref{assum:symmsubgauss},
    \begin{align*}
        &\Prob\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2 > M \left(1 + \log \frac{k_{\max}+1}{\delta}\right) \bigg| g_{[k-1]}\right] \\
        &= \Prob\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) > \exp\left(1 + \log \frac{k_{\max}+1}{\delta}\right) \bigg| g_{[k-1]}\right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\exp\left(\underset{k \in \{0,\dots,k_{\max}\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]}\right] \\
        &= \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\E\left[\underset{k \in \{0,\dots,k_{\max}\}}{\max} \exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]}\right] \\
        &\leq \exp\left(-1 - \log \frac{k_{\max}+1}{\delta}\right)\sum_{k=0}^{k_{\max}} \E\left[\exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]} \right] \\
        &\leq \exp(-1) \frac{\delta}{k_{\max}+1} (k_{\max}+1)\exp(1) = \delta.
    \end{align*}
\eproof

We conclude this section by showing that under Assumption \ref{assum:symmsubgauss}, event $E$ as defined in Assumption \ref{assum:eventE} occurs with high probability.

\blemma \label{lem:subgeventE}
    Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then, there exists a constant $\kappa_{\tau_{\min}}$ such that, with probability at least $1-\delta$, event $E$ of Assumption \ref{assum:eventE} occurs with
    \bequationNN
        \ktaudec = \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)}.
    \eequationNN
    and
    \bequation \label{eq:sgtaumin}
        \tau_{\min} = \frac{(1-\sigma)(1-\epsilon)}{\kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \kappa_{\tau_{\min}}}, \quad  s_{\max} = \left\lceil\frac{\log \frac{(1-\sigma)(1-\epsilon)}{\tau_{-1} \kappa_v \sqrt{M \left(1 + \log \frac{k_{\max}+1}{\delta}\right)} + \tau_{-1}\kappa_{\tau_{\min}}}}{\log 1-\epsilon }\right\rceil.
    \eequation
\elemma

\bproof
    We begin the proof by noting that by Jensen's inequality and the convexity of $\exp(\cdot)$,
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2| g_{[k-1]}] \leq M.
    \eequationNN
    The bound on $\ktaudec$ follows directly from Lemma \ref{lem:subgboundedrv}. Finally, the bound on $\tau_{\min}$ follows from \cite[Lemma 2.16]{ABerahas_FECurtis_DPRobinson_BZhou_2020} combined with \ref{lem:subgboundedrv} and the bound on $s_{\max}$ follows from combining the bound on $\tau_{\min}$ with \eqref{eq:smaxbound}.
\eproof

\iffalse
\tred{Update 4/20 that I don't know where to put right now.}

We can also get a similar (though looser bound) for the case where we just have bounded variance!

\blemma \label{lem:boundeddiffvariance}
    For all $k \in \{0,\dots,k_{\max}\}$, let
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2 | \mathcal{F}_k] \leq M.
    \eequationNN
   Then,
    \bequationNN
        \Prob\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{\frac{(k_{\max}+1)M}{\delta}}\right] \geq 1-\delta.
    \eequationNN
\elemma

\bproof
    Let $g := \{g_0,\dots,g_{k_{\max}}\}$ denote any sequence of stochastic gradients that is measurable with respect to the filtration $\mathcal{F}_{k_{\max}}$. Then, by Markov's inequality, concavity of the square root, Jensen's inequality, and the law of total expectation,
    \begin{align*}
        &\Prob\Bigg[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2 > \frac{(k_{\max}+1)M}{\delta}\Bigg] \\
        &\leq \E\left[\underset{0 \leq k \leq k_{\max}}{\max} \|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &\leq \sum_{k=0}^{k_{\max}} \E\left[\|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(k_{\max}+1)M} \\
        &= \frac{\delta}{(k_{\max}+1)M} \sum_{k=0}^{k_{\max}} \int_{g \in \mathcal{F}_{k_{\max}}} \E\left[\|G_{k} - \nabla f(x_k)\|^2 | G_{0} = g_{0}, \dots, G_{k-1} = g_{k-1}\right] f_{G} dg \\
        &\leq \frac{\delta}{(k_{\max}+1)M} (k_{\max} + 1) M \int_{g \in \mathcal{F}_{k_{\max}}} f_{G}(g) dg = \delta,
    \end{align*}
    where $f_G(g)$ is the probability density function of the random variable $G$.
\eproof

What does this mean for our results? We can repeat the proof of Lemma \ref{lem:subgeventE} so that with probability at least $1-\delta$,
\bequationNN
    \tau_{\min} = \mathcal{O}\left(\sqrt{\frac{\delta}{k_{\max}+1}}\right)
\eequationNN
and, for sufficiently large $k_{\max}$,
\bequationNN
    s_{\max} = \mathcal{O}\left(\log \sqrt{\frac{k_{\max}+1}{\delta}}\right). 
\eequationNN
Thus,
\bequationNN
    \frac{s_{\max}}{\sqrt{k_{\max}+1}} = \mathcal{O} \left(\frac{\log \sqrt{\frac{k_{\max}+1}{\delta}}}{\sqrt{k_{\max}+1}} \right),
\eequationNN
which means we can always get a useful complexity result, so long as $k_{\max}$ is sufficently large.

Unfortunately, because the bound from Lemma \ref{lem:boundeddiffvariance} is $\mathcal{O}(\sqrt{k_{\max}+1})$, we cannot use this approach to directly bound $\ktaudec$ and obtain a meaningful complexity result. Thus, additional assumptions are still needed in this case.
\fi

\subsection{Complexity Result with Decreasing Ratio Parameter} \label{subsec:ratioparam}

In this section, we relax Assumption \ref{assum:eventE} with respect to the random variable $\{\Xi_k\}$ and allow it to be adaptive over the course of the algorithm. Due to the definition of $\{\Xi_k\}$, it satisfies a deterministic lower-bound, $\xi_{\min}$, such that $\xi_k \geq \xi_{\min} > 0$ holds for all $k$ \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Therefore, it follows that there exists a maximum number of decreases of $\xi$, which we denote by $r_{\max}$, that satisfies
\bequationNN
    r_{\max} \leq \min\left\{k_{\max}+1, \left\lceil \frac{\log(\xi_{\min}/\xi_{-1})}{\log(1-\epsilon)} \right\rceil\right\}.
\eequationNN

Now, we can state our new assumption.

\bassumption\label{assum:eventExi}
  Conditioned on the event $E_{\xi} := E(\kmax,s_{\max},\tau_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E_{\xi}, \Fcal_k] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E_{\xi}, \Fcal_k] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k = \xi_{k-1}] \leq \kappa_1, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k = \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_2, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_3.
    \ealigned
  \eequationNN
\eassumption

This assumption is largely the same as Assumption \ref{assum:eventE}. The major new requirement due to the adaptive $\{\Xi_k\}$ sequence is the addition of two more events under which the norm difference of $\nabla f(x_k)$ and $G_k$ is bounded.

We remark that this assumption holds with high-probability under Assumption \ref{assum:symmsubgauss} (without the condition that $\xi_k = \xi_{\min}$), a result which can easily be derived by simple modification of the techniques used in Section \ref{subsec:subgauss}. We leave this derivation as an exercise for the reader.

The complexity analysis for this case follows by essentially the same arguments as those used to derive a complexity result under Assumption \ref{assum:eventE}. A slight modification of Lemma \ref{lem:innerprod} is needed to include the three events related to $\nabla f(x_k)^\top(d_k-\dktrue)$ that appear in Assumption \ref{assum:eventExi} (as opposed to the one in Assumption \ref{assum:eventE}), which yields a result in terms of the probabilities of these three events. Then, a slightly modified Lemma \ref{lem:Eksumlsmax} and the union bound can be applied two additional times to derive a complexity result. Since the analysis is a relatively straightforward extension of the results in Section \ref{subsec:complexity}, we simply state our complexity result here.
\begin{theorem}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:ptau}, and \ref{assum:eventExi} hold. Then, with probability at least $1-\delta$,
    \begin{align*}
        &\E[\|\nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c_{k^*}\| |
        E_{\xi}] \\
        &= \mathcal{O}\Bigg(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c_0\|_1 + M}{\sqrt{k_{\max}+1}} \\
        &\quad+ \frac{(\tau_{-1} - \tau_{\min})(s_{\max} + \log(1/\delta)) + (\xi_{-1} - \xi_{\min})(r_{\max} + \log(1/\delta))}{\sqrt{k_{\max}+1}}\Bigg).
    \end{align*}
\end{theorem}

\bproof
    We leave the proof as an exercise for the reader.
\eproof

\section{Conclusion} \label{sec:conclusion}

In this work, we derived the first worst-case complexity result for an adaptive stochastic algorithm for equality constrained optimization. We developed a stochastic SQP algorithm with an adaptive $\ell$-1 merit function, based on the framework proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}. While key to a practical algorithm, the adaptivity in the merit function introduced a number of theoretical challenges to overcome. Under mostly standard assumptions, we prove that, with high probability, the expected value of the norm of the gradient of the Lagrangian decays at a rate of $k^{-4}$, matching the worst-case complexity of the projected stochastic gradient method. We believe the theoretical tools developed within may be applicable to a broad class of constrained stochastic optimization methods that utilize an adaptive merit function. 

\iffalse
OLD STUFF BELOW:
\subsection{Quick Complexity Highlight}
Quick highlight of the main complexity result for meeting on 3/9/2021:

Let $\mathcal{I} \subseteq \{0,1,\dots,\kmax\}$ denote the index set of ``good" iterations. Overall analysis will lead to a result of the form (with $\beta_k := \beta = \gamma/\sqrt{\kmax+1}$:
\begin{align*}
    &\sum_{k \in \mathcal{I}} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\quad\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &\quad+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau}.
\end{align*}
To get the expectation that we want, we need to add and subtract:
\begin{align*}
    &\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &+ C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + \sum_{k \in \mathcal{I}^c} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)].
\end{align*}
Then, because the number of ``bad" iterations is bounded by $\ell(s_{\max},\delta)/p_{\tau}$,
\begin{align*}
    &\frac{\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)]}{\sum_{k=0}^{\kmax} \beta} \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\sum_{k=0}^{\kmax} \beta} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sum_{k=0}^{\kmax} \beta}.
\end{align*}
So that,
\begin{align*}
    &\E [\Delta q(x^*, \tau^*, \nabla f(x^*), H^*, d^{*,true})] \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\sqrt{\kmax + 1}} \\
    &+ \frac{C_1 \ell(s_{\max},\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(s_{\max},\delta)/p_{\tau} + C_4 \ell(s_{\max},\delta)/p_{\tau}}{\sqrt{\kmax+1}}.
\end{align*}

Algorithm \ref{alg:ssqp} generates a random process $\{\bar{G}_k,X_k,\bar{D}_k,\bar{\mathcal{T}}_k,\bar{\Xi}_k,\bar{\mathcal{A}}_k\}$. We will denote all random quantities by capital letters and their realizations by small letters. The random gradient estimate is denoted by $\bar{G}_k$ and its realizations by $\bar{g}_k = \bar{G}_k(\omega)$. Similarly, let the random quantities $x_k = X_k(\omega)$ (iterates), $\bar{d}_k = \bar{D}_k(\omega)$ (search directions), $\btau_k = \bar{\mathcal{T}}_k(\omega)$ (merit parameter), $\bxi_k = \bar{\Xi}_k(\omega)$ (reduction ratio), and $\bar{\alpha}_k = \bar{\mathcal{A}}_k(\omega)$ (step sizes) denote their respective realizations. We will assume that the estimates $\bar{G}_k$ obey some standard properties, conditioned on the past.

To formalize conditioning on the past, let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by the random variables $\bar{G}_0, \dotsc \bar{G}_{k-1}$. For completness, we set $\mathcal{F}_{-1} = \sigma(x_0)$. As a result, we have that $\mathcal{F}_{k}$ for $k \geq -1$ is a filtration.

Let $E_{\tau,low}$ denote the event that the merit parameter sequence eventually remains constant at a sufficiently small positive value.
We will derive our complexity result under the assumption that this event occurs.

\begin{assumption} \label{assum:taulow}
Event $E_{\tau,low}$ occurs in the sense that there exists an iteration
number $\bar{k}_{\tau,\xi} \in \mathbb{N}$ and a merit parameter value
$\btau_{\min} \in \R{}_{>0}$ such that
\begin{equation} \label{eq:taumin}
    \btau_k = \btau_{\min} \leq \btau_k^{trial} \quad and \quad
    \xi_k = \xi_{\min} \quad for \; all \quad k \geq \bar{k}_{\tau,\xi}.
\end{equation}
In addition, the sequence of random gradients $\bar{G}_k$ generated by Algorithm \ref{alg:ssqp} satisfies
\begin{equation*}
    \E_{k,\tau,small}[\bar{G}_k] = g_k \quad and \quad \E_{k,\tau,small}[\|\bar{G}_k - g_k\|^2] \leq M
\end{equation*}
where $\E_{k,\tau,small}$ denotes expectation with respect to the distribution of $\omega$ conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_{k}$.
\end{assumption}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k$, let $\Ek1$ be the event that $g_k^\top(\bd_k - d_k) \geq 0$, let $\Ek2$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} = \btau_{k-1}$, and let $\Ek3$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} < \btau_{k-1}$.

We require an additonal assumption to obtain our complexity result:
\begin{assumption} \label{assum:boundedrv}
There exists $\kappa_{\Ek3} > 0$ such that
\begin{equation} \label{eq:boundedrv}
    \E_k [\|\bar{g}_k-g_k\||\Ek3] \leq \kappa_{E_3}.
\end{equation}
\end{assumption}
The above assumption holds under a number of conditions, including when
$\bar{g}_k$ is a bounded random vector.

%NEW
\textcolor{red}{TODO:} Ignoring $\xi_k$ for now. Will probably need additional cases in the proof eventually...

\begin{lemma} \label{lem:innerprodold}
Suppose that Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|g_k\|_2\}$, the existence of which follows under \cite[Assumption 1]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\bxi_k = \bxi_{\min}$ and define
\bequationNN
\balpha_{\min,k} := \frac{\beta_k \bxi_{\min} \btau_{\min}}{\btau_{\min}L_k + \Gamma_k} \mbox{ and } \balpha_{\max,k} := \frac{\beta_k \bxi_{\min} \btau_{k-1}}{\btau_{k-1}L_k + \Gamma_k}.
\eequationNN

Then, with $\kappa_d \in \R{}_{>0}$ from Lemma 3.6 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} which satisfies
$\|\bar{d}_k-d_k\| \leq \kappa_d \|\bar{g}_k-g_k\|$,
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq  (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek1] \\
\E_{k,2} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek2] \\
\E_{k,3} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\btau_{\min}$, $\balpha_{\min,k}$, and $\balpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &= \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek1] \Prob_k[\Ek1] + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By Lemma 3.6, this means that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, by Lemma 3.6, we have
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} \balpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} \balpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{\min} \balpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{\min} \balpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}

Summing these three inequalities yields

\begin{align}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \nonumber \\
    &\leq \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+(\btau_{k-1} (\balpha_{\max,k} - \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+(2 \btau_{\min} \balpha_{\min,k} - \btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3]) \nonumber \\
    &= \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -3 \theta \beta_k^2 \btau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-(\btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2) - 2 \btau_{\min} \balpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]). \label{eq:innerprodproof1old}
\end{align}
Now, by Assumption \ref{assum:boundedrv},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|g_k\| \E_k[\|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \E_k[\|\bar{g}_k - g_k\| | \Ek3] \Prob_k[\Ek3]  \\
    &\leq \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[g_k^\top(\bd_k - d_k)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek2] \\
    &= \E_k[\|g_k\| \|\bar{d}_k - d_k\|] - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \E_k[\|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma 3.6. Using these three inequalities with
\eqref{eq:innerprodproof1old}, yields
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
which proves the result.
\end{proof}

The above result provides an upper bound in terms of the probability that the event $\Ek3$ occurs. Due to the assumed lower bound on $\btau_k$, this event can only occur a finite number of times. To obtain our final result, we need an upper bound on the summation of the probability that $\Ek3$ occurs. The first component of this upper bound comes from the Chernoff bound.

\begin{lemma} \label{lem:chernoff}
Let $Z_0, \dotsc, Z_{k}$ be independent Bernoulli random variables and let $s \in \mathbb{N}_{>0}$.
%Let
%\begin{equation} \label{eq:lsd}
%    \ell(s,\delta) := S + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 S \log(1/\delta)}.
%\end{equation}
Then, for any $\delta \in (0, 1)$,%\todo{FEC: I suggest ``Let ... random variables for any $k \in \mathbb{N}_{\geq0}$.  Then, for any $s \in \mathbb{N}_{\geq0}$ and $\delta \in (0,1)$, ....}
\begin{equation}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s\right] \leq \delta,
\end{equation}
whenever
\begin{equation} \label{eq:lsdold}
    \sum_{i=0}^{k} \Prob[Z_i = 1] \geq \ell(s,\delta) \quad where \quad \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\end{equation}
\end{lemma}

\begin{proof}
Denote $\mu = \sum_{i=0}^{k} \Prob[Z_i = 1]$.%\todo{FEC: In the general form, the definition of $\mu$ is in terms of expected value.  Maybe for clarity we should write $\mu = \sum_{i=0}^k E[Z_i] = \sum_{i=0}^k \Prob[Z_i = 1]$, where the latter is true only because we have Bernoulli random variables.} Then by Chernoff's bound, for any $\rho \in (0,1)$,
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq (1-\rho) \mu \right]
    \leq e^{-\mu \rho^2/2}.
\end{equation*}
Now, setting $\rho = 1 - s/\mu$ (which is in $(0,1)$ by (\ref{eq:lsd})), we have
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s \right]
    \leq e^{-\mu (1-s/\mu)^2/2}.
\end{equation*}
To prove the result, we need to show that%\todo{FEC: In the proof, you start with what we need, then work backwards to show what we want.  I'd prefer if we start with what we have (assumed in the statement) and prove that it gives what we want.  Does that make sense?}
\begin{equation*}
    e^{-\mu (1-s/\mu)^2/2} \leq \delta
\end{equation*}
holds. Therefore, we need
\begin{equation*}
    -\mu(1-s/\mu)^2/2 \leq \log(\delta)
\end{equation*}
to be satisfied. Rearranging this inequality, and using $\log(\delta) = -\log(1/\delta)$,%\todo{FEC: I don't see where the last equation comes from.  Did you scale it by $2\mu$?  I'm not seeing it.}
\begin{equation*}
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta) = \mu^2 - 2\mu (s+\log(1/\delta)) + s^2. 
\end{equation*}
Therefore, using the quadratic equation and taking the positive root,
\begin{align*}
    \mu &\geq s + \log(1/\delta) + \frac12\sqrt{4(s+\log(1/\delta))^2 - 4 s^2} \\
    &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)},
\end{align*}
which proves the result.
\end{proof}

Unfortunately, the events $\Ek3$ are not independent of each other so we can not directly apply Chernoff's bound. However, we can use this result in combination with an observation about the limited nature of the dependency between these events to prove the following result.

%IDEA: Rewrite lemma to prove that $K_stop <= k_{S,\delta}$ w.h.p. when $k_{s,\delta}$ exists. Gets rid of this whole J_i,stop nonsense

%This rewrite sucks, should just do it instance-wise.

%Essential components:
%   Independence when the leave one out sum is less than s.
%   Conclusion: w.h.p K_stop <= k_s,delta (or something similar).

%Crappy parts:
%   Conditioning on k_s,delta being well defined. Any better way to handle it? Yes if we do it instance wise. But then that notation is a bit frustrating
%   Top part is fine, gets rough as soon as we introduce E_s,delta.

\begin{lemma} \label{lem:depbernoulli}
For any $k \in \mathbb{N}_{\geq 0}$, let $Z_0, \dotsc, Z_{k}$ be Bernoulli random variables. Let $s \in \mathbb{N}_{>0}$.%\todo{FEC: Is it right to say that $Z_i$ is Bernoulli upfront?  Or should we be saying that, conditioned on ${\cal F}_i$, the random variable $Z_i$ is Bernoulli?  I guess technically it's Bernoulli in any case, since it's 0--1, but maybe we should say the condition since we always talk about conditional probabilities?}
For any $\hat{k} \in \{0,\dotsc,k\}$ and $i \in \{0,\dotsc,\hat{k}\}$, let $E_{\hat{k},i}$ be the event that $\sum_{j\leq \hat{k},j\neq i} Z_j < s$. We assume the following about the random variable $Z_i$ for each $i \in \{0,\dotsc,k\}$:
\begin{enumerate}
    \item $\Prob[Z_i = 1 | \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\hat{k}}]$.
    \item $\Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}^c] = 0.$
\end{enumerate}
%Let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_{k}$. %and let $\bar{G}_{i}$ be measurable with respect to $\mathcal{F}_i$ for all $i \in \{-1,\dotsc,\hat{k}-1\}$.
Let $\delta \in (0,1)$ and let $\ell(s,\delta)$ be defined as in (\ref{eq:lsd}). Let $K_{s,\delta}$ be the random variable such that, for any realization of $\bar{G}_0,\dotsc,\bar{G}_{k-1}$ that is measurable with respect to $\mathcal{F}_k$,
\bequationNN
    k_{s,\delta} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta) \right\},
\eequationNN
($k_{s,\delta} = \infty$ for any realization such that $\sum_{i=0}^k \Prob[Z_i=1|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta)$ does not occur).
In addition, let $K_{stop}$ be the random variable
\bequationNN
K_{stop} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} Z_i = s\right\},
\eequationNN
($k_{stop} = \infty$ for any realization of $Z$ such that $\sum_{i=0}^{k} z_i < s$).

We define two events:%\todo{FEC: How do these events depend on $k$?  Should we take it that $k$ is ``fixed'' in some sense, but we are considering the events for any $s$?  But shouldn't we be proving the result ``for any $k$'' as well, in which case the events should depend on $k$, too?}
\begin{enumerate}
    \item Let $E_{k,s,\delta}$ be the event that 
    $\sum_{i=0}^k \Prob[Z_i=1|\mathcal{F}_i] \geq \ell(s,\delta)$.
    \item Let $E_{k,s,\delta,stop}$ be the event that $K_{stop} > K_{s,\delta}$.
\end{enumerate}
Then,
\begin{equation*}
    \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
\end{equation*}
%We assume the following:
%\begin{enumerate}
%    \item For any $i \in \{0,\dotsc,\hat{k}\}$, let $J_{i,stop}$ be the event that $i > K_{stop}$ and  
%    \bequationNN
%    \Prob[(Z_i = 1) \cap J_{i,stop} | \mathcal{F}_i] = 0.
%    \eequationNN
%    (high level idea: once a realization of $Z$ has $s$ successes, the probability of $Z_i = 1$ is $0$.)
    %and thus $\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] = \sum_{i=0}^{K_{stop}} \Prob[Z_i = 1 | \mathcal{F}_i]$.
%the minimum integer such that $\sum_{i=0}^{k_{stop}} Z_i = s$ (set $k_{stop} = \infty$ if $\sum_{i=0}^{\hat{k}} Z_i < s$). Let $Y_i = 0$ for all $i > k_{stop}$.
%    \item For any $\bar{k} \in \{0,\dotsc,\hat{k}\}$, let $J_{\bar{k},i}$ be the event that $\sum_{j\leq \bar{k},j\neq i} Z_j < s$. Then, $\Prob[Z_i = 1| \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, J_{\bar{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\bar{k}}]$. (high level idea: if the summation leaving out $Z_i$ does not equal $s$, then $Z_i$ is independent of all other $Z_j$.)
%\end{enumerate}

%$\Prob[Z_i = 1|\nu_i] = \Prob[Z_i = 1|\nu_i, Z_0, %\dotsc, Z_{i-1}$.
%let $\Prob[Z_i=1|\nu_i] = \Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}]$ hold unless $\sum_{j=0}^{\bar{k}} Z_j = s$ in which case $\Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}] = 0$ holds for any $i$ such that $\sum_{j\leq \bar{k}, j\neq i} Z_j = s$.
%Then, for any $\delta \in (0,1)$,
%\begin{equation}
%    \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \geq 1 - \delta,
%\end{equation}
%where $\ell(s,\delta)$ is defined in (\ref{eq:lsd}).
\end{lemma}

\begin{proof}
    %We work with any fixed sequence $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ satisfying these conditions.
    %Note that by the definition of our filtration, it should be clear that $\Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{k-1}] = \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]$ for any $i \in \{0,\dotsc,k\}$.
    
    %We begin the proof by showing that
    %\begin{equation*}
    %    \Prob\left[ \right] \geq 1 - \delta,
    %\end{equation*}
    %holds for any fixed $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$. To prove this, we assume that $\sum_{i=0}^{\hat{k}} \Prob[Z_i| \bar{g_0}, \dotsc, \bar{g}_{i-1}] \geq \ell(s,\delta)$ (as the result is trivial otherwise).
    
    Let $E_{k,s,\delta}$ and $E_{k,s,\delta,stop}$ both occur. Then, since $E_{k,s,\delta}$ occurs, $k_{s,\delta}$ is finite. In addition, because $E_{k,s,\delta,stop}$ occurs,
    we have that
    \bequationNN
        \sum_{i=0}^{k_{s,\delta}} z_i < s.
    \eequationNN
    Therefore, for all $i \in \{0,\dotsc,k_{s,\delta}\}$, $E_{k_{s,\delta},i}$ occurs. Thus, for all $i,j \in \{0,\dotsc,k_{s,\delta}\}$, $Z_i$ and $Z_j$ were mutually independent.
    
    Due to the independence $Z$ in this case, by Lemma \ref{lem:chernoff},
    \bequationNN
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s\right] \leq \delta,
    \eequationNN
    and thus,
    \bequationNN
        \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
    \eequationNN
    
    Now, let $\hat{Z}_0, \dotsc, \hat{Z}_{k}$ be independent Bernoulli random variables such that $\Prob[\hat{Z}_i = 1] = \Prob[Z_i = 1|\mathcal{F}_i]$ for all $i=0,\dotsc,k$. Let $E$ be the event that $\sum_{i=0}^{k_{s,\delta}} Z_i < s$ and let $E_{k,s,\delta}$ occur. Now, for each $i=0,\dotsc,k_{s,\delta}$, it follows that if event $E$ occurs, $E_{k_{s,\delta},i}$ must occur as well, so $Z_i$ is independent of $Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{k_{s,\delta}}$ conditioned on the event $E$. Thus, whenever $E$ occurs, $Z_0,\dotsc,Z_{k_{s,\delta}}$ are identical in distribution to $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s,\delta}}$. Therefore, by Lemma \ref{lem:chernoff},
    \begin{equation}
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = \Prob\left[\sum_{i=0}^{k_{s,\delta}} \hat{Z}_i < s\right] \leq
        \delta.
    \end{equation}
    It follows that
    \begin{equation*}
           \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i \geq s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = 1 -    \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] \geq 1 - \delta,
    \end{equation*}
    and thus
    \begin{equation*}
        \Prob[k_{stop} \leq k_{S,\delta}] \geq 1 - \delta.
    \end{equation*}
    In addition, by the definition of $k_{stop}$ and $J_{i,stop}$, with probability at least $1-\delta$,
    \begin{align*}
        \sum_{i=0}^{\hat{k}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}]
        &= \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq \sum_{i=0}^{k_{S,\delta}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq 1 + \ell(s,\delta),
    \end{align*}
    and thus,
    \begin{equation*}
        \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1|\bar{g}_0, \dotsc, \bar{g}_{i-1}] \leq 1 + \ell(s,\delta) \right] \geq 1 - \delta.
    \end{equation*}
    Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_{\hat{k}}} \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{\hat{k}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\hat{k}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\hat{k}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
\end{proof}

This setup applies to $\Ek3$ under Assumption \ref{assum:taulow} due to the definitions of $\btau$ and $\btau_{\min}$. In particular, at each iteration where $\Ek3$ occurs, $\btau_{k} \leq (1-\varepsilon)\btau_{k-1}$ holds. Therefore, if we perform this process $s$ times, until
\begin{equation*}
    \btau_{\min} \geq (1-\varepsilon)^s \btau_{-1},
\end{equation*}
it follows that $\Ek3$ cannot occur again by Assumption \ref{assum:taulow}. Thus, solving this inequality for $s$, we have
\bequation \label{eq:Stmin}
    s_{\btau_{\min}} := \left\lceil\frac{\log(\btau_{\min}/\tau_{-1})}{\log(1-\varepsilon)}\right\rceil
\eequation
which is the maximum number of times $\Ek3$ can occur.

Now we can show how to apply the above lemma to $\Ek3$.

\begin{lemma}
    Let Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\beta_j = \beta$, $L_j = L$, and $\Gamma_j = \Gamma$ for all $j=0,\dotsc, k$. Let 
    \bequationNN
        \balpha_{\min} := \frac{\beta \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max} := \frac{\beta \bxi_{\min} \btau_{-1}}{\btau_{-1}L + \Gamma}.
    \eequationNN
    Let $\delta \in (0,1)$. Then, with probability at least $1-\delta$,
    \begin{align}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top (\bar{d}_j-d_j)]
        &\leq (\btau_{-1} (\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3}(1 + \ell(s_{\btau_{\min}},\delta))\\
    &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}, \nonumber
    \end{align}
    where
    \bequationNN
        \ell(s_{\btau_{\min}},\delta) := s_{\btau_{\min}} + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s_{\btau_{\min}} \log(1/\delta)}.
    \eequationNN
\end{lemma}

\begin{proof}
    By Lemma \ref{lem:innerprod},
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq \sum_{j=0}^k (\btau_{j-1}(\balpha_{\max,j} + \theta \beta_j^2) - \btau_{\min} \balpha_{\min,j}) \kappa_g \kappa_d \kappa_{E_3} \Prob_j[E_{j,3}]\\
        &\quad+ \theta \beta_j^2 \btau_{j-1} \kappa_g \kappa_d \sqrt{M}.
    \end{align*}
    Using our assumption on $\beta$, $L$, and $\Gamma$, we can upper bound this inequality as
    \begin{align} \label{eq:ipproof1}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} \sum_{j=0}^k \Prob_j[E_{j,3}]\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}. \nonumber
    \end{align}
   
    To show the final result, we need to apply Lemma \ref{lem:depbernoulli}. To do this, let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_k$ and for all $i=0,\dotsc,k$, let $Z_i = 1$ if $E_{i,3}$ occurs and let $Z_i = 0$ otherwise. Recall that $\Prob_i[\cdot]$ is conditioned on the event $E_{\tau,low}$ occurring as well as the filtration $\mathcal{F}_i$.
    
    Now, let $s = s_{\btau_{\min}}$, so that $s$ is the maximum number of iterations in which $\Ek3$ can occur by Assumption \ref{assum:taulow}. Then, it is easy to verify that by the definition of our filtration, the probability that $\Ek3$ occurs is independent of the $E_{i,3}$ for all other $i$, whenever $\Ek3$ can occur without contradicting Assumption \ref{assum:taulow}. This holds whenever $E_{\hat{k},i}$ occurs, so that the first property of $Z_i$ in Lemma \ref{lem:depbernoulli} holds. On the other hand, when $E_{\hat{k},i}^c$ occurs it is clear that if $\Ek3$ occurs as well that Assumption \ref{assum:taulow} must be contradicted. Thus, second property of $Z_i$ in Lemma \ref{lem:depbernoulli} is satisfied as well.
    
    Now, presume that $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s_{\btau_{\min}},\delta)$. Then, by Lemma \ref{lem:depbernoulli},
    \bequationNN
        \Prob[K_{stop} \leq k_{s_{\btau_{\min}},\delta}] \geq 1 - \delta.
    \eequationNN
    In addition, by the definition of $s_{\btau_{\min}}$ and $K_{stop}$, it follows that whenever $K_{stop}$ is finite,
    \bequationNN
        \sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] =
        \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}].
    \eequationNN
    Thus, with probability at least $1 - \delta$,
     \bequationNN
        \sum_{i=0}^{k} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq \sum_{i=0}^{k_{s_{\btau_{\min}}}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]
        \leq 1 + \ell(s_{\btau_{\min}},\delta).
    \eequationNN
    
    On the other hand, if $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] < \ell(s_{\btau_{\min}},\delta)$, it is clear that $\sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq 1 + \ell(s_{\btau_{\min}},\delta)$. Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_k} \Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_k} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
    
    Combining this with (\ref{eq:ipproof1}),
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} (1 + \ell(s_{\btau_{\min}},\delta))\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M},
    \end{align*}
    holds with probability at least $1-\delta$.
\end{proof}

\begin{theorem}
Suppose that Assumption 4 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} holds. Define 
\bequationNN
\bar{A}_{\min} := \frac{\bar{\xi}_{\min} \bar{\tau}_{\min}}{\tau_{-1}L + \gamma} \mbox{ and }
\bar{A}_{\max} := \frac{\xi_{-1} \tau_{-1}}{\bar{\tau}_{\min}L + \gamma}
\eequationNN
as well as
\bequationNN
\bar{M} := \tau_{-1} \left(\frac12 (\bar{A}_{\max} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{K+1}}
\eequationNN
for some
\bequationNN
\gamma \leq \min\left\{\frac{\bar{A}_{\min}}{\bar{A}_{\max} + \theta},
\frac{1}{\bar{A}_{\min}}\right\}.
\eequationNN
Then,
\begin{equation}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + c_0 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation}
\end{theorem}

\begin{proof}
Let
\bequationNN
\bar{A}_k = \frac{\bar{\xi}_{k} \bar{\tau}_{k}}{\bar{\tau_{k}}L + \gamma} \mbox{ and }
\bar{M}_k = \bar{\tau}_{k} \left(\frac12 (\bar{A}_{k} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
It follows that $\bar{A}_k \beta \leq \bar{\alpha}_k \leq (\bar{A}_k + \theta)\beta$. Using  Lemmas 3.2(d), 3.5, 3.8, and 3.9 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} (with the replacement of $\bar{\tau}_{\min}$ by $\bar{\tau}_k$), we have
\begin{align*}
    &\E_k[\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\leq \E_k [-\bar{\alpha}_k \Delta q(x_k, \bar{\tau_k}, g_k, H_k, d_k) + \frac12 \bar{\alpha}_k \beta \Delta q(x_k, \bar{\tau_k}, \bar{g}_k, H_k, \bar{d}_k) + \bar{\alpha}_k \bar{\tau}_k g_k^\top (\bar{d}_k - d_k)] \\
    &\leq -\beta(\bar{A}_k - \frac12(\bar{A}_k + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}_k \\
    &\leq -\beta(\bar{A}_{\min} - \frac12(\bar{A}_{\max} + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M} \\
    &\leq -\frac12 \beta \bar{A}_{\min} \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}
\end{align*}
Summing this inequality from $0$ to $K$,
\begin{align}
&\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \nonumber \\ 
&\leq -\frac12 \bar{A}_{\min} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)] + (K+1) \beta^2 \bar{M}. \label{eq:stochasticproof1old}
\end{align}
Now, we work with the left hand side of this inequality,
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k f(x_k + \bar{\alpha}_k \bar{d}_k) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k f_k + c_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k (f(x_k + \bar{\alpha}_k \bar{d}_k) - f_{\min}) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k].
\end{align*}
Now, conditioned on the algorithm reaching $x_k$, it follows by the monotonicity of $\tau$
that
\bequationNN
-\E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k] \geq - \E_k[\bar{\tau}_{k-1} (f_k - f_{\min}) + c_k].
\eequationNN
Therefore, summing this inequality yields
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\geq \E_K [\bar{\tau}_K (f_{K+1} - f_{\min}) + \|c_K\|_1] - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1.
\end{align*}
Using this lower bound with \eqref{eq:stochasticproof1old}
\begin{equation*}
    \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min}}.
\end{equation*}
Dividing both sides by the summation of $\beta$,
\begin{equation*}
    \frac{1}{\sum_{k=0}^K \beta} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Now, by the definition of $x_{k^*}$, the left hand side is simply
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Using the definition of $\beta$, this becomes
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation*}
\end{proof}

\newpage
\appendix

\section{FEC Notes}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)\},
\eequationNN
where
\bitemize
  \item $\Xbar_k$ is the algorithm iterate in iteration $k$,
  \item $\Gbar_k$ is the stochastic gradient in iteration $k$,
  \item $\Dbar_k$ is the search direction in iteration $k$,
  \item $\overline\Tcal_k$ is the merit parameter in iteration $k$,
  \item $\Sbar_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\overline\Xi_k$ is the ratio parameter in iteration $k$, and
  \item $\overline\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)$ is denoted as
\bequationNN
  (\xbar_k,\gbar_k,\dbar_k,\bar\tau_k,\sbar_k,\bar\xi_k,\bar\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{\Gbar_0,\dots,\Gbar_{k-1}\}$, the realization of which (along with $\Xbar_0 = x_0$) determines the realization of
\bequationNN
  \{\Xbar_j\}_{j=1}^k\ \ \text{and}\ \ \{(\Dbar_j,\overline\Tcal_j,\Sbar_j,\overline\Xi_j,\overline\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

Let us consider a conditional model under the following assumption.
We introduce the following assumption.

\newpage

\bassumption\label{ass:FEC}
  Conditioned on the event $E := E(k_{\max},s_{\max},\tau_{\min},\xi_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(k_{\max}+1)$th iterate is determined,
    \item in every realization there are at most $s_{\max}$ decreases of the merit parameter,
    \item in every realization we have $\bar\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$, and
    \item in every realization we have $\bar\xi_k = \bar\xi_{-1} = \bar\xi_{\min}$ for all $k \in \{0,\dots,k_{\max}\}$,
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,k_{\max}\}$:
  \bequationNN
    \baligned
      \E[\Gbar_k &| E, \Fcal_k] = \nabla f(\xbar_k), \\
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ \text{and}\ \ 
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2 &| E, \Fcal_k, \nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0, \bar\tau_k < \bar\tau_{k-1}] \leq \kappa,
    \ealigned
  \eequationNN
  where $d(\xbar_k,\nabla f(\xbar_k))$ is the step that would be computed at an iterate $\xbar_k$ if the true gradient $\nabla f(\xbar_k)$ were used in the search direction computation.
\eassumption

Going forward, let us define the binary random variable
\bequation %\label{eq:zkdef}
  Z_k = \bcases 1 & \text{if $\nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0$ and $\bar\tau_k < \bar\tau_{k-1}$} \\ 0 & \text{otherwise.} \ecases
\eequation
Due to the definition of the event $E$, direct consequences of Assumption~\ref{ass:FEC} are
\bequation\label{eq:probz0}
  \baligned
    \P[Z_k = 1 &| E, \Fcal_k, \Sbar_{k-1} = s_{\max}] = 0 \\ \text{and}\ \ 
    \P[Z_k = 1 &| E, \Fcal_k, \Tbar_{k-1}(1 - \epsilon) < \tau_{\min}] = 0.
  \ealigned
\eequation

\bequationNN
  \P[Z_j = 1 | E, \Fcal_k, \Sbar_{k-1} < s_{\max}, \Tbar_{k-1}(1 - \epsilon) \geq \tau_{\min}]\ \ \text{for $j \in \{k,\dots,k_{\max}\}$}
\eequationNN

Our overall goal is to prove an upper bound (in high probability) on
\bequationNN
  \sum_{k=0}^{k_{\max}} p_k,\ \ \text{where}\ \ p_k := \P[Z_k = 1 | E, \Fcal_k].
\eequationNN
%From total probability and \eqref{temp}:
%\bequationNN
%  \baligned
%    \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k]
%    &= \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} < s_{\max}] \cdot \P[\Sbar_{k_{\max}} < s_{\max} | E, \Fcal_k] \\
%    &+ \sum_{k=0}^{k_{\max}} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{k_{\max}} = s_{\max}] \cdot \P[\Sbar_{k_{\max}} = s_{\max} | E, \Fcal_k]
%  \ealigned
%\eequationNN

As a first step, we prove the following.

\blemma\label{lem:chernoff_new}
  For any $k \in \N{}$, let $\{Y_0,\dots,Y_k\}$ be independent Bernoulli random variables.  Then, for any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, it follows that
  \bequationNN
    \mu := \sum_{j=0}^k \P[Y_j = 1] \geq \ell(s,\delta)\ \ \implies\ \ \P\left[\sum_{j=0}^k Y_j \leq s\right] \leq \delta,
  \eequationNN
  where
  \bequation\label{eq:lsd_new}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
  \eequation
\elemma
\bproof
  By the multiplicative form of Chernoff's bound, it follows for $\rho := 1 - s/\mu$ (which is in the interval $(0,1)$ by (\ref{eq:lsd_new})) that
  \bequationNN
    \P\left[\sum_{j=0}^{k} Y_j \leq s \right] \leq e^{-\frac{\mu \rho^2}{2}} = e^{-\frac{\mu (1-s/\mu)^2}{2}}.
  \eequationNN
  Hence, to prove the result, all that remains is to show that $e^{-\frac{\mu (1-s/\mu)^2}{2}} \leq \delta$, i.e.,
  \bequationNN
    -\frac{\mu(1-s/\mu)^2}{2} \leq \log(\delta)
  \eequationNN
  Using $\log(\delta) = -\log(1/\delta)$, this inequality is equivalent to
  \bequationNN
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta),
  \eequationNN
  which holds if and only if $\mu^2 - 2\mu (s+\log(1/\delta)) + s^2 \geq 0$.  Viewing the left-hand side of this inequality as a convex quadratic function in $\mu$, one finds that the inequality holds as long as $\mu$ is greater than or equal to the positive root of the quadratic, i.e.,
  \bequationNN
    \baligned
      \mu
        &\geq s + \log(1/\delta) + \sqrt{(s+\log(1/\delta))^2 - s^2} \\
        &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2s\log(1/\delta)}.
    \ealigned
  \eequationNN
  Since this holds under assumption in the lemma, the result is proved.
\eproof

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tau_k^{trial}$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ and $\xi_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tau_k^{trial}$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tau_k^{trial}$ occurs, we introduce the following assumption.

\begin{assumption} %\label{assum:ptau}
At every iteration $k$,
\bequation
    \Prob[\bar{g}_k^\top \bar{d}_k + \max\{\bar{d}_k^\top H_k \bar{d}_k,0\} \geq g_k^\top d_k + \max\{d_k^\top H_k d_k,0\} | E, \mathcal{F}_k] \geq p_{\tau}.
\eequation
\end{assumption}
This assumption is satisfied with $p_{\tau}$ when $\bar{g}_k$ is drawn from a Gaussian distrbution \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

This assumption is leads to the following lemma.

\blemma \label{lem:Etautrial_old}
    Let Assumptions \ref{ass:FEC} and \ref{assum:ptau} hold. Let $E_{\tau_k^{trial}}$ be the event that $\tau_k^{trial} < \bar{\tau}_{k-1}$. Then,
    \bequation
        \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, E_{\tau_k^{trial}}] \geq p_{\tau}.
    \eequation
\elemma

\bproof
    TODO: Copy proof from my notes.
\eproof

Due to the above lemma and Assumption \ref{ass:FEC}, it follows that
\bequationNN
    \Prob[E_{\tau_k^{trial}} | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN
In addition, by the definition of $\bar{\tau}_k$,
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, E_{\tau_{k}^{trial}}^c] = 0,
\eequationNN
so 
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, \bar{S}_{k-1} = s_{\max}] = 0.
\eequationNN

Now, by Lemma \ref{lem:Etautrial} and the fact that $E_{\tau_{k}^{trial}}$ is not dependent on $\bar{g}_k$, it follows that
\bequation \label{eq:Etrialtaudec_old}
    \Prob[E_{\tau_{k}^{trial}} | \mathcal{F}_k, E, \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E] < p_{\tau}] = 0.
\eequation

Idea from here: Let $\bar{P}_k = \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, \bar{S}_{k-1} < s_{\max}]$ and let $Z_k$ be the indicator of the event that $\bar{\tau}_k < \bar{\tau}_{k-1}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s_{\max},\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}

Then, by \eqref{eq:Etrialtaudec}, with probability $1-\delta$, the number of occurrences of $E_{\tau_{k}^{trial}}$ is bounded by
\bequationNN
    |E_{\tau_{k}^{trial}}| \leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil.
\eequationNN
Thus, by the definition of $\bar{\tau}_k$, it follows that
\bequationNN
    |\tau_k^{trial} < \bar{\tau}_k|\leq \left\lceil\frac{ \ell(s_{\max},\delta) + 1 }{p_{\tau}}\right\rceil. 
\eequationNN

\newpage

\section{Mike's Simpler Problem} \label{app:simple}

Let $Y_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:simple1}
  \baligned
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \geq s_{\max}\right] &= 0
  \ealigned
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in [0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:simple2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Y_k = s_{\max} \right].
\eequation

The following lemma proves \eqref{eq:simple2}.
\begin{lemma} \label{lem:simple1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
    \bequationNN
      \baligned
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}\right] &= p_k \\ \text{and}\ \ 
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] &= 0,
      \ealigned
    \eequationNN
    for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$, where $p_k \in (0,1]$ for all $k \in \{0,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k = s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} p_k + \sum_{k=j}^{k_{\max}} 0 = \sum_{k=0}^{j-1} p_k.
    \end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
    \end{align*}
    which completes the proof.
\end{proof}

The left side of this equation is similar to our goal for the actual problem, while the right is potentially easier to work with. 
A good starting point would be to try to prove a bound on
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right]
\eequationNN
for any $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$.

It clearly follows that
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = s_{\max} \right] = 1 -  \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right].
\eequationNN
We can find a lower bound on the right hand side of this equation using the following lemma.
\begin{lemma} \label{lem:simple2}
    Let $\ell \in \{s_{\max}-1,\dotsc,k_{\max}\}$ and let $\hat{Y}_0,\dotsc,\hat{Y}_{\ell}$ be independent \\Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then,
    \bequationNN
        \Prob\left[\sum_{k=0}^{\ell} Y_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    For all $k \in \{0,\dotsc,\ell\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,\ell\}$, let
    \bequationNN 
        \bar{y}_k := \bcases
        1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
        0 & \textrm{otherwise},
        \ecases
    \eequationNN
    and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    \begin{align*}
        \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ are equivalent in distribution to $Y_0, \dotsc, Y_{\ell}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\ell} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{\ell} Y_k < s_{\max}\right],
    \eequationNN
    where the last equality holds because 
    $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ and $Y_0, \dotsc, Y_{\ell}$ are equivalent in distribution.
\end{proof}

We can use these lemmas as well as Lemma \ref{lem:chernoff_new} to get our desired bound in high probability.

\begin{lemma} \label{lem:simple3}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Y_k$ be Bernoulli random variables which satisfy \eqref{eq:simple1}, where $p_k \in (0,1]$. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $\sum_{k=0}^{k_{\max}} p_k \leq \ell(s_{\max},\delta) + 1$. Then, by the definition of $Y_k$, it is clear that
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(s_{\max},\delta) + 1
    \eequationNN
    holds deterministically, so the result is trivial in this case. Thus, for the remainder of the proof, we assume that $\sum_{k=0}^{k_{\max}} p_k > \ell(s_{\max},\delta) + 1$.
    
    Now, let $k_{s_{\max},\delta}$ be the minimum integer such that
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} p_k \geq \ell(s_{\max},\delta).
    \eequationNN
    Let $\hat{Y}_0,\dotsc,\hat{Y}_{k_{s_{\max},\delta}}$ be independent Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then, by Lemma \ref{lem:simple2} and Lemma \ref{lem:chernoff_new},
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &\geq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}

%Since the $\hat{Y}_k$ variables are independent, we can use this lemma and the CDF of the binomial distribution to get an exact description of the summation of interest. Alternatively, we can derive a bound for it by using a tail bound, such as Hoeffding's inequality or Chernoff's bound. The second option is likely to be more relevant in the more general setting of our actual algorithm.

What I'd hope a final result to look like:
\bequationNN
    \Prob\left[\sum_{k=0}^{k_{\max}} \Prob\Big[Z_k = 1 \Big| \mathcal{F}_{k}\Big] \leq \ell(s_{\max},\delta)\right] \geq 1 -\delta.
\eequationNN

Update: 2/8/2021

Let $\bar{P}_k = \Prob[Z_k=1| E, \mathcal{F}_k, \bar{S}_{k-1} < s_{\max}]$ and let $\bar{p}_k \in [0,1]$ for all \\$k \in \{0,\dotsc,k_{\max}\}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$ such that $\Prob\left[\left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\right] \neq 0$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{k_{\max}} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{k_{\max} + 1}} \Prob\Bigg[\sum_{k=0}^{k_{\max}} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{k_{\max}}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{k_{\max}}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{k_{\max} + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}


Old idea:

If
\bequation \label{eq:simple3}
    \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | E, \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] \geq 1-\delta
\eequation
holds for any $\bar{g}_0,\dotsc,\bar{g}_{k_{\max}}$, then we are done because:
\begin{align*}
    &\Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i = 1| \mathcal{F}_i] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{g} \in \mathcal{F}_{k_{\max}}} \Prob\left[\sum_{i=0}^{k_{\max}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | \left\{\bar{G}_0,\dotsc,\bar{G}_{k_{\max}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k_{\max}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
    &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{k_{\max}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta).
\end{align*}
Unfortunately, when conditioning on a realization from the filtration, we fix both the probabilities as well as whether the events occurred. Thus, the probabilities on the left side of \eqref{eq:simple3} is always 0 or 1.

\section{A Different Problem}
Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:different1}
  \begin{split}
    &\Prob\Bigg[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0,\dotsc,Z_{k-1}\Bigg] \in [0,1] \\ \text{and}\ \
    &\Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq s_{\max}\right] = 0
  \end{split}
\eequation
for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$
\bequation \label{eq:different2}
    \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
\eequation
We prove this inequality in the following lemma.

\begin{lemma} \label{lem:different1}
    Let $Z_k$ for $k \in \{0,\dotsc,k_{\max}\}$ be Bernoulli random variables which satisfy \eqref{eq:different1}, for some $s_{\max} \in \{1,\dotsc,k_{\max}\}$. Then, for any $j \in \{s_{\max}, \dotsc, k_{\max}\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = s_{\max} \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k \geq s_{\max}$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] + \sum_{k=j}^{k_{\max}} 0 \\
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right].
    \end{align*}
    
    %Now, letting $E_j^c$ denote the complement of $E_j$, the definition of $Z_k$ yields
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c \right] = \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \textrm{ for all $k \leq j$.}
    %\eequationNN
    %Thus,
    %\begin{align*}
    %    \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right]
    %    &\geq \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right] \\
    %    &= \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right].
    %\end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \right] \\
        &= \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max} \right] \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
\end{align*}
which completes the proof.
\end{proof}

Next, we would like to derive an analog to Lemma \ref{lem:simple2}.
\begin{lemma} \label{lem:different2}
    Let $p \in \{s_{\max}-1,\dotsc,k_{\max}\}$. Then, there exist independent Bernoulli random variables $\hat{Z}_0, \dotsc, \hat{Z}_p$ which satisfy
    \begin{align*}
        &\Prob\left[\sum_{k=0}^{p} Z_k < s_{\max} \right] = \Prob\left[\sum_{k=0}^{p} \hat{Z}_k < s_{\max} \right] \\
        \textrm{and } &\sum_{k=0}^p \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \sum_{k=0}^p \Prob\left[ \hat{Z}_k = 1\right].
    \end{align*}
\end{lemma}

\begin{proof}
    General idea: For any sequence of $\Prob\left[Z_k = 1 \Big| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right]$, there exists a fixed sequence of independent random variables that could generate this sequence in the same way that $\bar{Y}_k$ was generated in Lemma \ref{lem:simple2}. If we can get to that point, believe we can verbatim copy the rest of the proof.
    
    %To begin, note that for all $Z_0,\dotsc,Z_{k_{\max}}$ satisfying \eqref{eq:different1}, there exists a set of independent Bernoulli random variables 
    %$\hat{Z}_0, \dotsc, \hat{Z}_p$ such that
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right].
    %\eequationNN

    %For all $k \in \{0,\dotsc,p\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,p\}$, let
    %\bequationNN 
    %    \bar{y}_k := \bcases
    %    1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < s_{\max} \\
    %    0 & \textrm{otherwise},
    %    \ecases
    %\eequationNN
    %and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    %and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    %\begin{align*}
    %    \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < s_{\max}\right] &= p_k \\
    %    \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq s_{\max}\right] &= 0
    %\end{align*}
    
    %Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{p}$ are equivalent in distribution to $Y_0, \dotsc, Y_{p}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{p} \hat{Y}_k < s_{\max}$ occurs if and only if the event $\sum_{k=0}^{p} \bar{Y}_k < s_{\max}$ occurs as well. Thus,
    %\bequationNN
    %    \Prob\left[ \sum_{k=0}^{p} \hat{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} \bar{Y}_k < s_{\max}\right] = \Prob\left[ \sum_{k=0}^{p} Y_k < s_{\max}\right],
    %\eequationNN
    %where the last equality holds because 
    %$\bar{Y}_0, \dotsc, \bar{Y}_{p}$ and $Y_0, \dotsc, Y_{p}$ are equivalent in distribution.
\end{proof}

\begin{lemma}
    Let $s_{\max} \in \{1,\dotsc,k_{\max}\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,k_{\max}\}$, let $Z_k$ be Bernoulli random variables which satisfy \eqref{eq:different1}. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{k_{\max}} \Prob \left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1} \right] \leq \ell(s_{\max},\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(s_{\max},\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $E$ be the event that 
    \bequationNN
        \sum_{k=0}^{k_{\max}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}\right] > \ell(s_{\max},\delta).
    \eequationNN
    
    Then, let $K_{s_{\max},\delta}$ be the random variable whose realization $k_{s_{\max},\delta}$ is the minimum integer that satisfies
    \bequationNN
        \sum_{k=0}^{k_{s_{\max},\delta}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}, E\right] \geq \ell(s_{\max},\delta).
    \eequationNN

    Now, for any $Z_0,\dotsc, Z_p$ which satisfies \eqref{eq:different1} and $E$, there exist independent Bernoulli random variables $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s_{\max}},\delta}$ such that
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < s_{\max}, E, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right] \textrm{ for all } k \in \{0,\dotsc,k_{s_{\max},\delta}\}.
    \eequationNN

    Then, let $\bar{Z}_0,\dotsc,\bar{Z}_{k_{s_{\max},\delta}}$ be Bernoulli random variables such that
    \begin{align*}
        \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i < s_{\max}\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i \geq s_{\max}\right] &= 0
    \end{align*}
    
    
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max}\right] = \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k < s_{\max}\right] \leq \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} \hat{Y}_k \leq s_{\max}\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{k_{\max}} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{s_{\max},\delta}} p_k \right] &= \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k = s_{\max} \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{s_{\max},\delta}} Y_k < s_{\max} \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{s_{\max},\delta}} p_k \leq \ell(s_{\max},\delta) + 1$.
\end{proof}


%DETERMINISTIC ANALYSIS BELOW
Given an objective function $f : \R{n} \rightarrow \R{}$ and a
constraint function $c : \R{n} \rightarrow \R{m}$, consider the optimization problem
\begin{equation} \label{eq:fdef}
    \underset{x \in \R{n}}{\min} \enspace f(x) \; \mbox{ s.t. } c(x)=0.
\end{equation}
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) = f(x) + c(x)^\top y$, the first-order stationarity conditions
for \eqref{eq:fdef} are given by
\begin{equation} \label{eq:1on}
    0 = \left[
    \begin{matrix}
    \nabla_x \ell(x,y) \\ \nabla_y \ell(x,y)
    \end{matrix}
    \right]
    = \left[
    \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\ c(x)
    \end{matrix}
    \right].
\end{equation}
Letting $f_k := f(x_k)$, $g_k := \nabla f(x_k)$, $c_k := c(x_k)$, and $J_k := \nabla c(x_k)^\top$ for all $k \in \mathbb{N}$ and given a sequence $\{H_k\}$ satisfying a standard type of sufficiency condition for equality constrained optimization, the SQP subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}
The optimal solution $d_k$ of this subproblem, and an associated Lagrange multiplier $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}
At each iteration, the algorithm uses a merit function with the $\ell_1$-norm penalty function $\phi : \R{n} \times \R{}_+ \rightarrow \R{}$ defined by
\begin{equation} \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1
\end{equation}
where $\tau \in \R{}_+$ is a merit parameter that is updated at each iteration of the algorithm. We use a local model of the merit function $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + \nabla c(x)^\top d\|_1.
\end{equation}
A useful quantity is the reduction in is model for a given $d \in \R{n}$ with $c(x) + \nabla c(x)^\top d = 0$, i.e., $\delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}

For the purposes of this note, we will declare $x_k$ an approximate solution of (\ref{eq:fdef}) when
\begin{equation} \label{eq:eps1on}
    \|g_k + J_k^\top y_k\| \leq \epsilon  \quad \mbox{ and } \quad \|c_k\| \leq \epsilon,
\end{equation}
both hold for some $k \in \mathbb{N}$. We will derive a worst-case complexity result
in terms of the maximum number of iterations required to find a point statisfying \eqref{eq:eps1on}. We refer the reader to \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the
full definition of the algorithms. To prove our complexity result, we will use the following results which were proven in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}:
\begin{itemize}
    \item The merit parameter $\tau_k$ has an upper and lower bound given by $\tau_{-1} \geq \tau_k \geq \tau_{\min}$ (Lemma 2.14).
    \item The stepsize $\alpha_k$ is lower bounded by $\alpha_{\min}$ (Lemma 2.15).
    \item Let $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$ for all $k \in \mathbb{N}$. Then, by Lemma 2.7,
    \begin{equation} \label{eq:vltc}
        \max\left\{\|v_k\|,\|v_k\|^2\right\} \leq \kappa_v \|c_k\|,
    \end{equation}
    for some $\kappa_v > 0$.
    \item Let $\kappa_{uv}$ and $\zeta$ be strictly positive scalars. Then, by Lemma 2.8,
    \begin{equation} \label{eq:dposcurve}
        \|u_k\|^2 \geq \kappa_{uv} \|v_k\|^2 \implies d_k^\top H_k d_k \geq \frac14 \zeta \|u_k\|^2.
    \end{equation}
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:deltabound}
        \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \frac12 \tau_k \max\{d_k^\top H_k d_k, 0\} + \sigma\|c_k\|_1,
    \end{equation}
    (equation 2.9 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:meritdecrease}
        \phi(x_k + \alpha_k d_k, \tau_k) \leq \phi(x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k),
    \end{equation}
    (Lemma 2.12).
\end{itemize}

Armed with these results, we will prove the following lemma about sufficient decrease in the merit function whenever \eqref{eq:eps1on} does not hold.
\begin{lemma} \label{lem:suffdecrease}
Define
\begin{equation} \label{eq:kappahat}
    \hat{\kappa} := \frac{1}{\sqrt{1+\kappa_{uv}}\max\{\kappa_J,\kappa_H\}\kappa_v}
\end{equation}
and
\begin{equation} \label{eq:kappadec}
    \kappadec := \min\left\{\sigma \hat{\kappa},
    \frac18 \tau_{\min}\zeta\kappa_{uv}\kappa_v^2 \hat{\kappa}^2\right\}.
\end{equation}
Let $\epsilon < 1$ and let at least one of $\|g_k + J_k^\top y_k\| > \epsilon$ and/or $\|c_k\| > \epsilon$ hold. Then,
\begin{equation} \label{eq:suffdecrease}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\end{equation}
\end{lemma}

\begin{proof}
To begin, assume for contradiction that
\bequationNN
\|d_k\| \leq \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\eequationNN
Then, by the definitions of $d_k$ and $y_k$ as well as $\|H_k\| \leq \kappa_H$,
\bequationNN
\|g_k + J_k^\top y_k\| = \|H_k d_k\| \leq \kappa_H \|d_k\| \leq \frac{\epsilon \kappa_H}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
In addition, by the definition of $d_k$ and $\|J_k\| \leq \kappa_J$,
\bequationNN
\|c_k\| = \|J_k d_k\| \leq \kappa_J \|d_k\| \leq \frac{\epsilon \kappa_J}{\max\{\kappa_J,\kappa_H\}} \leq \epsilon.
\eequationNN
Therefore, \eqref{eq:eps1on} holds at $k$, which is a contradiction and we must
have
\begin{equation} \label{eq:dlength}
\|d_k\| > \frac{\epsilon}{\max\{\kappa_J,\kappa_H\}}.
\end{equation}

We consider two cases in the rest of the proof. First, let $\|c_k\| \leq \hat{\kappa} \epsilon$. Then, by \eqref{eq:vltc} and $\|c_k\| \leq \hat{\kappa} \epsilon$,
\bequationNN
\|v_k\|^2 \leq \kappa_v^2 \|c_k\|^2 \leq \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
On the other hand, by \eqref{eq:dlength},
\begin{align*}
    \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} &< \|d_k\|^2 \\
    &= \|u_k\|^2 + \|v_k\|^2 \\
    &\leq \|u_k\|^2 + \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies
\begin{align*} \label{eq:ulb}
    \|u_k\|^2 &\geq \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &= \frac{\epsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \frac{ \epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \frac{\kappa_{uv}\epsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2 \\
    &\geq \kappa_{uv} \|v_k\|^2.
\end{align*}
Thus, by \eqref{eq:dposcurve}, we have
\bequationNN
d_k^\top H_k d_k \geq \frac14 \zeta\|u_k\|^2 \geq \frac14 \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2.
\eequationNN
Therefore,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} \\
    &\geq \frac18 \tau_{\min} \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \epsilon^2,
\end{align*}
which implies \eqref{eq:suffdecrease} in this case.

Now, presume that $\|c_k\| > \hat{\kappa} \epsilon$ holds. Then, by \eqref{eq:deltabound} and $\epsilon < 1$,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \sigma \|c_k\|_1 \\
    &\geq \sigma \hat{\kappa} \epsilon^2.
\end{align*}
Thus, (\ref{eq:suffdecrease}) holds in this case as well.
\end{proof}

We can use this lemma to prove the following complexity result.

\begin{theorem}
Let
\begin{equation} \label{eq:kbar}
    \bK := \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec} \epsilon^{-2},
\end{equation}
where $\kappadec$ is defined in \eqref{eq:kappadec}.
Presume Assumptions 1 and 2 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} hold.
Then, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in no more than $\bK$ iterations (a similar result holds for Algorithm 2.2 with a revised definition of $\alpha_{\min}$).
\end{theorem}

\begin{proof}
Assume for contradiction that for all iterations $k = 0,1, \dotsc, \bK$, \eqref{eq:eps1on}
does not hold. Then, by Lemma \ref{lem:suffdecrease}, we have
\bequationNN
\Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \epsilon^2.
\eequationNN
Then, at each iteration, by \eqref{eq:meritdecrease},
\begin{align*}
    \phi (x_k + \alpha_k d_k, \tau_k) &\leq \phi (x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k) \\
    &\leq \phi(x_k, \tau_k) - \eta \alpha_{\min} \kappadec \epsilon^2.
\end{align*}
Using the definition of $\phi$ in \eqref{eq:phidef} as well as $x_{k+1} = x_k + \alpha_k d_k$, the above inequality becomes,
\bequationNN
\tau_k f_{k+1} + \|c_{k+1}\|_1 \leq \tau_k f_k + \|c_k\|_1 - \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Summing this inequality for all iterations $k = 0,1, \dotsc, \bK$, we have
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \sum_{k=0}^{\bK} \tau_k (f_{k+1}-f_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Now, by removing the first and last term of the summation, this inequality can be rewritten
as
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \tau_{\bK}f_{\bK+1} - \tau_0 f_0
+ \sum_{k=1}^{\bK} f_k (\tau_{k-1} - \tau_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
By definition, $\tau_k$ is a decreasing sequence. Therefore, we have $\tau_{k-1} - \tau_k \geq 0$
for all $k$. Then, since $\|c_{\bK+1}\|_1 \geq 0$ and $f_k \geq \flow$ holds for all $k$, we have
\bequationNN
- \|c_0\|_1 + \tau_{\bK}\flow - \tau_0 f_0
+ \flow (\tau_{0} - \tau_{\bK}) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \epsilon^2.
\eequationNN
Rearranging this inequality, we have
\bequationNN
\bK+1 \leq \frac{\tau_0 (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
\leq \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \epsilon^2}
= \bK,
\eequationNN
which is a contradiction. Therefore, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in
at most $\bK$ iterations.
\end{proof}
\fi



==> archived_versions/2021-10-19/abstract.tex <==
A worst-case complexity bound is proved for a sequential quadratic optimization (commonly known as SQP) algorithm that has been designed for solving optimization problems involving a stochastic objective function and deterministic nonlinear equality constraints.  Barring additional terms that arise due to the adaptivity of the monotonically nonincreasing merit parameter sequence, the proved complexity bound is comparable to that known for the stochastic gradient algorithm for unconstrained nonconvex optimization.  The overall complexity bound, which accounts for the adaptivity of the merit parameter sequence, shows that a result comparable to the unconstrained setting (with additional logarithmic factors) holds with high probability.

==> archived_versions/2021-10-19/body.tex <==
%******************************************
% Paper-dependent macros here
%******************************************
\newcommand{\flow}{f_{\text{\rm low}}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\kappadec}{\kappa_{\text{\rm dec}}}
\newcommand{\bK}{\bar{K}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\btau}{\bar{\tau}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bg}{\bar{g}}
\newcommand{\bxi}{\bar{\xi}}

\newcommand{\xiktri}{\xi_k^{\rm trial}}
\newcommand{\ktaudec}{\kappa_{\tau_{\rm dec}}}
\newcommand{\kmax}{k_{\max}}
\newcommand{\smax}{s_{\max}}
\newcommand{\tauktri}{\tau_k^{\rm trial}}

\newcommand{\dktrue}{d_k^{\text{\rm true}}}
\newcommand{\uktrue}{u_k^{\text{\rm true}}}
\newcommand{\wktrue}{w_k^{\text{\rm true}}}
\newcommand{\yktrue}{y_k^{\text{\rm true}}}
\newcommand{\ykstartrue}{y_{k^*}^{\text{\rm true}}}
\newcommand{\tktritrue}{\tau_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Tktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Dktrue}{D_k^{\text{\rm true}}}
\newcommand{\Yktrue}{Y_k^{\text{\rm true}}}
\newcommand{\Uktrue}{U_k^{\text{\rm true}}}
\newcommand{\Uk}{U_k}
\newcommand{\Vk}{V_k}

\newcommand{\strue}{s^{\text{\rm true}}}

\newcommand{\Lbad}{\Lcal_{\text{\rm bad}}}
\newcommand{\Lgood}{\Lcal_{\text{\rm good}}}
\newcommand{\Ebad}{E_{\text{\rm bad}}}
\newcommand{\Cdec}{C_{\text{\rm dec}}}
\newcommand{\Idec}{\Ical_{\text{\rm dec}}}
\newcommand{\ktau}{k_{\tau}}
\newcommand{\tcalktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}

\def\Ek#1{E_{k,#1}}
\def\tred#1{\textcolor{red}{#1}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%*********
% Section
%*********
\section{Introduction} \label{sec:intro}

We present a worst-case complexity analysis of an algorithm for minimizing a smooth objective function subject to nonlinear equality constraints.  Problems of this type arise in various important applications throughout science and engineering, including optimal control, PDE-constrained optimization, and resource allocation \cite{DPBertsekas_1998,JTBetts_2010,FSKupfer_EWSachs_1992,TRees_HSDollar_AJWathen_2010}.  However, unlike the vast majority of the literature on equality constrained optimization, the algorithm that we consider has been designed to solve problems in which the objective function is stochastic, in the sense that it is defined by the expectation of a function that has a random variable argument.  The algorithm that we consider assumes that evaluations of the objective function and its gradient are intractable to obtain, but that it has access to (unbiased) stochastic gradient estimates.

A few algorithms have been proposed recently for solving problems of this type.  These approaches fall into two categories: penalty methods \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018} (which includes the class of augmented Lagrangian methods) and sequential quadratic optimization (commonly known as SQP) methods \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021,SNa_MAnitescu_KMladen_2021}.  Penalty methods aim to solve the constrained optimization problem by adding a term to the objective function, weighted by a penalty parameter, that penalizes constraint violation.  Unconstrained optimization techniques are then applied to minimize the resulting penalty function, after which the penalty parameter may be modified and the minimization performed again in an iterative manner until a solution is obtained that (approximately) satisfies the original constraints.  Methods of this type perform well in some situations, but in others they perform poorly, e.g., due to ill-conditioning and/or nonsmoothness of the subproblems. Such methods also often suffer due to their sensitivity to the particular scheme used for updating the penalty parameter.

In practice in both deterministic and stochastic optimization contexts, penalty methods are frequently outperformed by SQP methods.  Indeed, it is commonly accepted in the deterministic optimization literature that a state-of-the-art algorithm is an SQP method that chooses stepsizes based on a line search applied to a merit function.  In this deterministic setting, such an algorithm is intimately connected with applying Newton's method to the first-order primal-dual necessary conditions for optimality of the problem~\cite{RBWilson_1963}.

In this paper, we present a worst-case complexity analysis of the SQP method proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which can be seen as an extension of an SQP method from the deterministic to the stochastic setting.  A consequence of our analysis is that, in an idealized setting in which one knows a threshold for the merit parameter beyond which the merit function is \emph{exact} \cite{HanM79}, the number of iterations required until the method generates a point at which first-order necessary conditions for optimality hold in expectation with accuracy $\varepsilon \in (0,\infty)$ is $\Ocal(\varepsilon^{-4})$.  This is arguably the best result that one can expect given this is the same bound proved to hold for a stochastic gradient method employed to solve an unconstrained nonconvex problem~\cite{DDavis_DDrusvyatskiy_2019}.  However, \emph{our analysis does not only consider this idealized setting}; we go further and prove a worst-case complexity bound for the algorithm when the merit parameter threshold is unknown, and instead the algorithm adaptively updates a monotonically nonincreasing merit parameter sequence.  We prove under reasonable assumptions that the aforementioned worst-case bound, with additional logarithmic factors, holds with high probability.  The high-probability aspect of this result arises purely due to the uncertainty of the behavior of the adaptive merit parameter sequence, and does not reflect any uncertainty of the behavior of the method during situations in which the merit parameter sequence remains constant.

To the best of our knowledge, ours is the first worst-case complexity result for an SQP algorithm that operates in the \emph{highly stochastic regime} (where one merely presumes that the stochastic gradient estimates have bounded variance) for solving stochastic optimization problems involving deterministic nonlinear equality constraints.  Prior to this work, the only known complexity results for stochastic constrained optimization were for algorithms for solving problems with simple constraint sets that enable projection-based methods \cite{DDavis_DDrusvyatskiy_2019,SGhadimi_GLan_HZhang_2016} and Frank-Wolfe type methods \cite{EHazan_HLuo_2016}.  (One exception is a complexity bound proved for the SQP algorithm proposed in \cite{SNa_MAnitescu_KMladen_2021}, although that result only holds for the idealized setting in which the algorithm has \emph{a priori} knowledge of a threshold for the merit function parameter.)  Our analysis focuses a great deal on the complications that arise due to the adaptivity of the merit parameter sequence, which essentially means that the algorithm in our consideration is aiming to reduce a merit function that \emph{changes} during the optimization process.  Hence, many aspects of our analysis are quite distinct from the analyses that have been presented for stochastic gradient methods in the context of unconstrained optimization or optimization over simple constraint sets, for which the tool for measuring the progress of an algorithm---namely, the objective function itself---remains the same throughout the optimization.

%************
% Subsection
%************
\subsection{Problem formulation}

The algorithm that we consider is designed to solve problems of the form
\bequation \label{eq:fdef}
  \min_{x \in \R{n}} f(x)\ \ \st\ \ c(x) = 0,\ \ \text{with}\ \ f(x) = \E[F(x,\omega)],
\eequation
where $f : \R{n} \rightarrow \R{}$, $c : \R{n} \rightarrow \R{m}$, $\omega$ is a random variable with associated probability space $(\Omega,\mathcal{F}, P)$, $F : \R{n} \times \Omega \rightarrow \R{}$, and $\E$ represents expectation with respect to $P$.  In particular, following \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, we make the following assumption about problem \eqref{eq:fdef} and the algorithm that we analyze (stated as Algorithm~\ref{alg:ssqp} on page~\pageref{alg:ssqp}), which in any run generates a sequence of iterates $\{x_k\} \subset \R{n}$.

\begin{assumption}\label{assum:fcsmooth}
  Let $\Xcal \subseteq \R{n}$ be an open convex set that contains $\{x_k\}$ for all realizations of Algorithm \ref{alg:ssqp}.  The objective function $f : \R{n} \rightarrow \R{}$ is continuously differentiable and bounded below by $\flow \in \R{}$ over $\Xcal$ and the corresponding gradient function $\nabla f: \R{n} \rightarrow \R{n}$ is bounded and Lipschitz continuous with constant $L \in (0,\infty)$ over $\Xcal$. The constraint function $c : \R{n} \rightarrow \R{m}$ $($where $m \leq n$$)$ and the corresponding Jacobian function $J := \nabla c^\top : \R{n} \rightarrow \R{m\times n}$ are bounded over $\Xcal$, each gradient function $\nabla c_i : \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $\gamma_i$ over $\Xcal$ for all $i \in \{1,\dots,m\}$, and the singular values of $J \equiv \nabla c^\top$ are bounded below and away from zero over $\Xcal$.
\end{assumption}

A consequence of Assumption~\ref{assum:fcsmooth} is that there exists $\kappa_g \in \R{}_{>0}$ such that
\bequation\label{eq.kappa_g}
  \|\nabla f(x_k)\| \leq \kappa_g\ \ \text{for any iterate $x_k$}.
\eequation
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) := f(x) + c(x)^\top y$, first-order primal-dual stationarity conditions for~\eqref{eq:fdef}, which are necessary for optimality under Assumption~\ref{assum:fcsmooth}, are given by
\bequation \label{eq:optconds}
  0 =
  \left[ \begin{matrix}
    \nabla_x \ell(x,y) \\
    \nabla_y \ell(x,y)
  \end{matrix} \right]
  =
  \left[ \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\
    c(x)
  \end{matrix} \right].
\eequation

%************
% Subsection
%************
\subsection{Notation}

We adopt the notation that $\|\cdot\|$ denotes the $\ell_2$-norm for vectors and the vector-induced $\ell_2$-norm for matrices.  We denote by $\mathbb{S}^{n}$ the set of $n \times n$ dimensional real symmetric matrices. The set of nonnegative integers is denoted as $\N{} := \{0,1,2,\dots,\}$. For any integer $k \in \N{}$, we use $[k]$ to denote the subset of nonnegative integers up to $k$, namely, $[k] := \{0,\dots,k\}$.  Correspondingly, to represent a set of vectors $\{v_0,\dots,v_k\}$, we define $v_{[k]} := \{v_0,\dots,v_k\}$.

Given $\phi : \R{} \to \R{}$ and $\varphi : \R{} \to [0,\infty)$, we write $\phi(\cdot) = \Ocal(\varphi(\cdot))$ to indicate that $|\phi(\cdot)| \leq C\varphi(\cdot)$ for some $C \in (0,\infty)$.  Similarly, we write $\phi(\cdot) = \widetilde\Ocal(\varphi(\cdot))$ to indicate that $|\phi(\cdot)| \leq C\varphi(\cdot)|\log^c(\cdot)|$ for some $C \in (0,\infty)$ and $c \in (0,\infty)$.  In this manner, one finds that $\Ocal(\varphi(\cdot)\log^c(\cdot)) \equiv \widetilde\Ocal(\varphi(\cdot))$ for any $c \in (0,\infty)$.

Algorithm~\ref{alg:ssqp} is iterative, generating in each realization a sequence of iterates $\{x_k\}$.  For our analysis, we also append the iteration number to other quantities corresponding to each iteration, e.g., $f_k := f(x_k)$ for all $k \in \N{}$.

When discussing stochastic quantities, we use capital letters to denote random variables and corresponding lower case letters to denote a realization of a random variable. For example, a stochastic gradient in iteration $k \in \N{}$ is denoted as $G_k$, a realization of which is written as $g_k$.

%************
% Subsection
%************
\subsection{Outline}

Section~\ref{sec:complexitypreview} provides a worst-case complexity result for the algorithm from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} for the deterministic setting, and uses this result and further commentary to provide an overview of our main result for the stochastic setting.  Details of the algorithm for the stochastic setting are presented in Section~\ref{sec.algorithm}, followed by our main result and analysis, which are provided in Section~\ref{sec:complexity}.  Finally, we provide some concluding thoughts and future directions in Section~\ref{sec:conclusion}.

%*********
% Section
%*********
\section{Outline of Main Results} \label{sec:complexitypreview}

Our algorithm of consideration, namely, Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, is derived from Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which is proposed and analyzed for the deterministic setting as a precursor for the stochastic setting (of Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}).  In the deterministic algorithm, the $k$th search direction $d_k \in \R{n}$ is computed by solving an optimization subproblem defined by a quadratic approximation of the objective function and an affine approximation of the constraints using derivative information at the current iterate $x_k \in \R{n}$.  This computation also results in a Lagrange multiplier value $y_k \in \R{m}$.  The subsequent iterate is set by $x_{k+1} \gets x_k + \alpha_k d_k$, where $\alpha_k \in (0,\infty)$ is a stepsize determined by a procedure to reduce the merit function $\phi : \R{n} \times (0,\infty) \to \R{}$ defined by
\bequation \label{eq:phidef}
  \phi(x,\tau) = \tau f(x) + \|c(x)\|_1.
\eequation
In particular, based on properties of the search direction $d_k$, a value of the merit parameter $\tau_k \in (0,\tau_{k-1}]$ is set by the algorithm, after which $\alpha_k \in (0,\infty)$ is computed to ensure that $\phi(x_k,\tau_k) - \phi(x_{k+1},\tau_k)$ is sufficiently positive.

%************
% Subsection
%************
\subsection{Complexity of Deterministic Algorithm}

To motivate our main result for the stochastic setting, it is instructive to state a worst-case complexity bound for the deterministic algorithm.  Such a result is the following; further details and a proof is provided in Appendix~\ref{app.deterministic}.

\btheorem\label{th.deterministic}
  Consider Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} and suppose that Assumption~\ref{assum:fcsmooth} holds along with Assumption~2.4 from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}.  Let $\tau_{-1} \in \R{}_{>0}$ be the initial value of the merit parameter sequence and let $\tau_{\min} \in (0,\tau_{-1}]$ be a positive lower bound for the merit parameter sequence $($the existence of which follows from Lemma~2.16 in~\cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}$)$.  Then, for any $\varepsilon \in (0,1)$, there exists $(\kappa_1,\kappa_2) \in \R{}_{>0} \times \R{}_{>0}$ such that the algorithm reaches an iterate $(x_k,y_k) \in \R{n} \times \R{m}$ satisfying
  \bequation\label{eq:eps1lon}  
    \|g_k + J_k^\top y_k\| \leq \varepsilon\ \ \text{and}\ \ \sqrt{\|c_k\|_1} \leq \varepsilon
  \eequation
  in a number of iterations no more than
  \bequation\label{eq.deterministic_complexity}
    \(\frac{\tau_{-1}(f_0 - \flow) + \|c_0\|_1}{\min\{\kappa_1,\tau_{\min} \kappa_2\}}\) \varepsilon^{-2}.
  \eequation
\etheorem

Theorem~\ref{th.deterministic} is not surprising.  After all, such a complexity bound of $\Ocal(\varepsilon^{-2})$ is well-known for gradient-based algorithms in unconstrained nonconvex optimization.  Since Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} and its corresponding analysis do not consider the use of exact second-order derivative information, this complexity bound is on the order of what could be expected for such a method.

%************
% Subsection
%************
\subsection{Preview of Complexity of Stochastic Algorithm}

Moving to the stochastic setting, there are a few major technical hurdles that need to be addressed, all of which relate to the adaptivity of the merit parameter sequence.  In particular, the analysis for the deterministic setting relies heavily on the facts that $(i)$ each step of the algorithm yields a sufficient reduction in the merit function for the current value of the merit parameter, $(ii)$ each such reduction in the merit function can be tied to a first-order primal-dual stationarity measure for each iterate, and $(iii)$ under Assumption~\ref{assum:fcsmooth}, one can be certain of the existence of a positive lower bound for the merit parameter sequence.  This lower bound for the merit parameter is referenced directly in the proof of the worst-case bound for the deterministic algorithm; in particular, it is shown (see Lemma~\ref{lem:suffdecrease} and the beginning of the proof of Theorem~\ref{th.deter_complex}) that the improvement in the merit function from any iterate that is not $\varepsilon$-stationary is at least proportional to $\min\{1,\tau_{\min}\} \varepsilon^{-2}$, even if the current value of the merit parameter is greater than $\tau_{\min}$.  Unfortunately, these properties of the steps and merit parameter sequence are not certain in the stochastic setting.  For example, as discussed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, it is possible---even under Assumption~\ref{assum:fcsmooth}---for the merit parameter sequence to vanish or for it to eventually remain constant at a value that is not sufficiently small, and for there to be iterations in which the expected reduction in the merit function cannot be tied to a first-order primal-dual stationarity measure.  As a result, we have had to devise new analytical approaches that confront the fact that $\{\tau_k\}$ is a random process, the ultimate behavior of which is uncertain.

To aid the reader, we provide here an overview and commentary about our ultimate complexity bound; see Corollary~\ref{coro:complexity} on page~\pageref{coro:complexity}.  Our result is proved under Assumption~\ref{assum:fcsmooth} along with others that are introduced in the subsequent sections. For one thing, as is common in SQP methods for deterministic optimization, we assume that the subproblem defining the search direction in each iteration is defined by a matrix that is positive definite in the null space of the constraint Jacobian; see Assumption~\ref{assum:Hk} on page~\pageref{assum:Hk}.  In addition, we make the assumption that a particular event $E$ occurs related to the overall behavior of the algorithm; see Assumption~\ref{assum:eventE} on page~\pageref{assum:eventE}.  This event $E$ captures situations in which, over a total of $\kmax+1 \in \N{}$ iterations, the merit parameter is reduced at most $\smax \in [\kmax]$ times, the merit parameter is bounded below by $\tau_{\min} \in (0,\infty)$, the stochastic gradient estimates are unbiased with variance bounded by $M \in (0,\infty)$, and the stochastic gradient estimates exhibit a certain bounded measure of asymmetry about their means; see Assumption~\ref{assum:eventE} for further details.  Under these conditions, our main complexity result shows that, within $\kmax + 1$ iterations, it holds with probability $1-\delta \in (0,1)$ that the algorithm generates $x_{k^*} \in \R{n}$ corresponding to which there exists an associated Lagrange multiplier $\ykstartrue \in \R{m}$ such that
\begin{align}
     &\ \E[\|\nabla f_{k^*} + J_{k^*}^\top \ykstartrue\|^2 + \|c_{k^*}\|_1 | E] \nonumber \\
    =&\ \Ocal \Bigg(\frac{\tau_{-1}(f_0 - \flow) + \|c(x_0)\|_1 + M}{\sqrt{\kmax+1}} \label{eq.like_sg} \\
     &\qquad + \frac{(\tau_{-1} - \tau_{\min})(\smax\log(\kmax) + \log(1/\delta))}{\sqrt{\kmax+1}}\Bigg). \label{eq.new_terms}
\end{align}
This form of the result is commonly called a convergence rate since it bounds the expected stationarity error from above by a function that decreases with the number of iterations performed, namely, $\kmax+1$.  This bound can be used to form a worst-case complexity result.  Specifically, the result above and Jensen's inequality imply that, within $\kmax+1$ iterations and as long as $\smax = \Ocal(\log(\kmax))$ (more on this below), it holds with probability $1-\delta$ that the algorithm requires at most $\widetilde\Ocal(\varepsilon^{-4})$ iterations to generate~$x_{k^*}$ with corresponding $\ykstartrue$ such that $\E[\|\nabla f_{k^*} + J_{k^*}^\top \ykstartrue\| |E] \leq \varepsilon$ and $\E[\sqrt{\|c_{k^*}\|_1}|E] \leq \varepsilon$.

The first three quantities on the right-hand side of the convergence rate, namely, in \eqref{eq.like_sg}, representing the initial objective function gap, initial constraint violation, and the variance of the stochastic gradient estimates, mirror the presence of similar terms that appear for comparable results for the stochastic gradient method in an unconstrained or simple-constraint-set setting.  The final term in \eqref{eq.new_terms}, on the other hand, as well as the fact that the result is stated as a high-probability result, are unique to our setting and arise due to the adaptivity of the merit parameter sequence.  If one were to have prior knowledge of $\tau_{\min}$, then one could set $\tau_{-1} = \tau_{\min}$ (and disable the update mechanism for the merit parameter in the algorithm), in which case our analysis would show that the expected stationarity error is bounded above by \eqref{eq.like_sg} (surely, not only with high probability).

In the context of an adaptive merit parameter sequence, the particular form of our complexity result depends on the magnitude of $\smax$ relative to $\kmax+1$, i.e., the bound on the number of times that the merit parameter is decreased relative to the total number of iterations performed.  One setting in which our result is relatively straightforward is when, over all realizations of the algorithm, the differences between the stochastic gradient estimates and the true gradients are bounded deterministically, in which case $\smax$ is bounded by a value that is independent from $\kmax+1$; this follows from the fact that whenever the merit parameter is decreased, it is done so by a constant factor.  Beyond this setting, for another concrete example of a situation in which $\smax$ is guaranteed to be sufficiently small relative to $\kmax$, we prove in Section~\ref{subsec:subgauss} that if the distributions of the stochastic gradient estimates are sub-Gaussian, then with probability $1-\delta$ one finds that $\tau_{\min} = \mathcal{O}(\log(\frac{\kmax}{\delta}))$, meaning\footnote{dpr:I do not follow why the next displayed equation holds.  Is this a typo?  If you think this is correct, then I need an explanation.  FEC: I also think it was a typo.  Previously, it said ``$\log\log(\kmax/\delta)$.'' I think it's correct now.  Mike, please check.}
\bequationNN
  \frac{\smax}{\sqrt{\kmax+1}} = \mathcal{O}\left(\frac{\log(\frac{\kmax}{\delta}) \log(\kmax)}{\sqrt{\kmax+1}}\right).
\eequationNN
As a result, one finds in such a setting that our proved convergence rate is indeed comparable to the unconstrained or simple-constraint-set setting, in the sense that the rate is not ruined by the presence of the term in \eqref{eq.new_terms}.

Before proceeding to the details of the algorithm and our analysis, we remark in passing that while our analytical approach has been developed for an SQP method that uses the merit function in \eqref{eq:phidef}, it may be applicable to a wide variety of algorithmic frameworks for constrained stochastic optimization.  For example, our approach may be modified to apply to methods that  adaptively update critical parameters at each iteration, such as adaptive penalty methods \cite{RHByrd_GLopez-Calva_JNocedal_2012,RHByrd_JNocedal_RAWaltz,MMongeau_ASartenaer_1995}, adaptive augmented Lagrangian methods \cite{FECurtis_HJiang_DPRobinson_2015}, adaptive barrier methods \cite{JNocedal_AWachter_RAWaltz_2009}, and penalty-interior point methods \cite{FECurtis_2012}.  In addition, many constrained optimization algorithms generate repeated (often unconstrained) subproblems defined by an auxilliary parameter sequence that is updated dynamically based off of the solution to the previous subproblem.  Algorithms of this type include penalty methods, augmented Lagrangian methods, and interior point methods \cite{JNocedal_SJWright_2006}.  In cases when the objective is stochastic, this auxilliary sequence would also be a random process, in which case analyzing the behavior of such a process would be paramount to proving a complexity result for such a method.  We believe that the techniques that we have devised for this paper are broadly applicable and foundational for performing complexity analyses of deterministically constrained stochastic optimization methods.

%*********
% Section
%*********
\section{Algorithm}\label{sec.algorithm}

For ease of reference, in this section we present Algorithm~3.1 from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which is designed to solve problems of the form~\eqref{eq:fdef} and is our focus for the remainder of the paper.  In the spirit of an SQP method, the algorithm computes a search direction $d_k$ and Lagrange multiplier vector $y_k$ in iteration $k \in \N{}$ by solving
\begin{equation} \label{eq:sqpsubproblem}
  \min_{d \in \R{n}}\ f_k + g_k^\top d + \thalf d^\top H_k d\ \ \st\ \ c_k + J_k d = 0,
\end{equation}
where $H_k \in \mathbb{S}^n$ is chosen independently from $g_k$, and we remind the reader that $g_k$ is a realization of the stochastic gradient $G_k$. Under Assumption~\ref{assum:fcsmooth} and the following Assumption~\ref{assum:Hk} (that we make throughout the remainder of the paper), the solution of \eqref{eq:sqpsubproblem} can be obtained from the unique solution of
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}

\begin{assumption} \label{assum:Hk}
  The sequence $\{\|H_k\|\}$ is bounded by $\kappa_H \in \R{}_{>0}$.  In addition, there exists $\zeta \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, the matrix $H_k \in \mathbb{S}^n$ has the property that $u^\top H_k u \geq \zeta \|u\|_2^2$ for all $u \in \R{n}$ such that $J_k u = 0$.
\end{assumption}

After computation of $(d_k,y_k)$, the remainder of the $k$th iteration involves $(i)$ updating the merit parameter, $(ii)$ updating an auxiliary parameter needed for the stepsize computation, and $(iii)$ computing a positive stepsize.  These algorithmic components are designed with the aim of yielding a sufficiently positive reduction in a model of the merit function, which in turn is aimed at yielding a sufficiently positive reduction in the merit function itself.  The algorithm employs the model $q : \R{n} \times (0,\infty) \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\bequationNN
  q(x, \tau, g, H, d) = \tau (f(x) + g^\top d + \thalf \max\{d^\top H d,0\}) + \|c(x) + J(x) d\|_1,
\eequationNN
and the reduction function $\Delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$, for a given $d \in \R{n}$ satisfying $c(x) + J(x) d = 0$, defined by
\begin{equation} \label{eq:deltadef}
  \baligned
    \Delta q(x, \tau, g, H, d)
      :=&\ q(x, \tau, g, H, 0) - q(x, \tau, g, H, d) \\
       =&\ -\tau (g^\top d + \thalf \max\{d^\top H d,0\}) + \|c(x)\|_1.
  \ealigned
\end{equation}
Specifically, in order to ensure in iteration $k$ that $\tau_k \leq \tau_{k-1}$ and
\bequation \label{eq:qquadlb}
  \Delta q(x_k,\tau,g_k,H_k,d_k) \geq \thalf \tau \max\{d_k^\top H_k d_k, 0\} + \sigma \|c_k\|_1 \geq 0
\eequation
holds for all $\tau \leq \tau_k$, the algorithm sets, for user-defined $\sigma \in (0,1)$, the value
\bequation \label{eq:tautrial}
  \tauktri\gets
  \begin{cases}
    \infty & \mbox{if $g_k^\top d_k + \max\{d_k^\top H_k d_k, 0\} \leq 0$} \\
    \frac{(1-\sigma)\|c_k\|_1}{g_k^\top d_k + \max\{d_k^\top H_k d_k,0\}} & \mbox{otherwise,}
  \end{cases}
\eequation
and then sets, for some $\epsilon_\tau \in (0,1)$, the merit parameter value
\bequation \label{eq:taudef}
  \tau_k \gets \bcases \tau_{k-1} & \mbox{if $\tau_{k-1} \leq \tauktri$} \\ (1-\epsilon_\tau)\tauktri & \mbox{otherwise.} \ecases
\eequation
Then, for use in the stepsize computation (as motivated in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}) it sets
\bequation \label{eq:xidef}
  \xiktri \gets \frac{\Delta q(x_k, \tau_k, g_k, H_k, d_k)}{\tau_k \|d_k\|^2}\ \ \text{then}\ \ \xi_k \gets \bcases \xi_{k-1} & \mbox{if }\xi_{k-1} \leq \xiktri \\ (1-\epsilon_\xi)\xiktri & \mbox{otherwise} \ecases
\eequation
for some $\epsilon_\xi \in (0,1)$, which, for one thing, ensures $\xi_k \leq \xiktri$.  The last component in the $k$th iteration is to set the stepsize, the magnitude of which is controlled by prescribed $\{\beta_k\} \subset (0,1]$, which is employed in the following projection interval that is used in the stepsize computation:
\bequationNN
    \mbox{Proj}_k(\cdot) := \mbox{Proj}\left(\cdot \; \Bigg| \left[\frac{\beta_k \xi_k \tau_k}{\tau_k L + \Gamma}, \frac{\beta_k \xi_k \tau_k}{\tau_k L + \Gamma} + \theta \beta_k^2 \right]\right),
\eequationNN
where $\mbox{Proj}(\cdot \; | \; \mathcal{I})$ represents the projection operator onto the interval $\mathcal{I} \subset \R{}$.  As in other stochastic-gradient-based methods, the convergence properties of the method depend on properties of $\{\beta_k\}$, which in many analyses is considered to be a constant or diminishing sequence.  In our analysis, we establish our result for the case of $\beta_k = \Ocal(1/\sqrt{\kmax+1})$ for all $k \in [\kmax]$.

Overall, the algorithm that we consider is stated as Algorithm~\ref{alg:ssqp} below.  The only changes from Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} are the fixed iteration limit ($\kmax$) and the concluding step for producing the return value ($x_{k^*}$).  This method of sampling $k^*$ to produce the return value is consistent with other approaches in the literature on complexity analyses for algorithms for solving nonconvex optimization problems; see, e.g., \cite{DDavis_DDrusvyatskiy_2019}.  It amounts to uniform sampling over the iterates when constant $\{\beta_k\}$ is considered, as in our analysis.  Finally, we remark that Algorithm~\ref{alg:ssqp} presumes knowledge of Lipschitz constants for the objective and constraint gradients, although in practice one might only estimate these values, for which standard procedures can be employed~\cite{FECurtis_DPRobinson_2019}.

\begin{algorithm}[ht]
  \caption{Stochastic SQP Algorithm}
  \label{alg:ssqp}
  \begin{algorithmic}[1]
    \Require $x_0 \in \R{n}$; $\kmax \in \N{}$; $\tau_{-1} \in \R{}_{>0}$; $\epsilon_\tau \in (0,1)$; $\epsilon_\xi \in (0,1)$; $\sigma \in (0,1)$; $\xi_{-1} \in \R{}_{>0}$; $\{\beta_k\} \subset (0,1]$; $\theta \in \R{}_{\geq0}$; $L \in (0,\infty)$, a Lipschitz constant for $\nabla f$; $\Gamma \in [\sum_{i=1}^m \gamma_i,\infty)$, where $\gamma_i \in (0,\infty)$ is a Lipschitz constant for $\nabla c_i$ for all $i \in [m]$
    \For{\textbf{all} $k \in [\kmax]$}
	  \State Compute $(d_k,y_k)$ as the solution of \eqref{eq:sqpsystem}
	  \If{$d_k = 0$}
	    \State Set $\tauktri \gets \infty$, $\tau_k \gets \tau_{k-1}$, $\xiktri \gets \infty$, and $\xi_k \gets \xi_{k-1}$
	    \State Set $\widehat\alpha_{k,\text{init}} \gets 1$, $\widetilde\alpha_{k,\text{init}} \gets 1$, and $\alpha_k \leftarrow 1$
	  \Else\ (if $d_k \neq 0$)
	    \State Set $\tauktri$ by \eqref{eq:tautrial} and $\tau_k$ by \eqref{eq:taudef} %\label{step.tau_stochastic}
	    \State Set $\xiktri$  and $\xi_k$ by \eqref{eq:xidef} %\label{step.xi}
        \State Set
        \bequationNN
          \widehat\alpha_{k,\text{init}} \gets \tfrac{\beta_k\Delta q(x_k,\tau_k,g_k,H_k,d_k)}{(\tau_k L + \Gamma)\|d_k\|_2^2}\ \ \text{and}\ \  \widetilde\alpha_{k,\text{init}} \gets \widehat\alpha_{k,\text{init}} - \tfrac{4\|c_k\|_1}{(\tau_k L +  \Gamma)\|d_k\|_2^2}
        \eequationNN
        \State Set $\widehat\alpha_k \gets \proj_k(\widehat\alpha_{k,\text{init}})$ and $\widetilde\alpha_k \gets \proj_k(\widetilde\alpha_{k,\text{init}})$, then \label{step.alpha_projection_stochastic} \label{step.alpha_stochastic}
        \bequationNN
          \alpha_k \gets
		    \bcases
		      \widehat\alpha_k & \text{if $\widehat\alpha_k < 1$} \\
		      1 & \text{if $\widetilde\alpha_k \leq 1 \leq \widehat\alpha_k$} \\
		      \widetilde\alpha_k & \text{if $\widetilde\alpha_k > 1$}
		    \ecases
        \eequationNN
      \EndIf
      \State Set $x_{k+1} \gets x_k + \alpha_k d_k$
    \EndFor
    \State Sample $k^* \in [\kmax]$ according to the probability distribution
    \bequationNN
        \Prob[k^* = k] = \frac{\beta_k}{\sum_{k=0}^{\kmax} \beta_k},
    \eequationNN
    then \Return $x_{k^*}$
  \end{algorithmic}
\end{algorithm}

%*********
% Section
%*********
\section{Complexity Analysis} \label{sec:complexity}

We begin our complexity analysis by describing the algorithm as a stochastic process (Section~\ref{subsec:process}), then formalizing the assumptions that we make about the stochastic gradient estimates (Section \ref{subsec:assumptions}).  We then state, in some cases in a slightly modified form, some key lemmas from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} that are needed for our analysis (Section \ref{subsec:algprops}).  Our generic complexity result, which has been outlined in Section~\ref{sec:complexitypreview}, is then stated and proved (Section \ref{subsec:complexity}).  Consequences and extensions of our generic complexity result are then discussed for some special cases of distributions for the stochastic gradient estimates for which our required assumptions hold with high-probability (Section \ref{subsec:subgauss}).  Finally, we conclude this section by outlining a form of our generic complexity result that relaxes one of our minor simplifying assumptions (Section \ref{subsec:ratioparam}).

Similarly as for the convergence analysis in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, our complexity analysis makes use of orthogonal decompositions of the search directions computed by the algorithm; in particular, for all $k \in \N{}$, we express $d_k = u_k + v_k$, where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.  We note here that conditioned on the algorithm having reached $x_k$ at iteration $k$, the normal component $v_k$ is {\it deterministic}, depending only on the constraint value $c_k$ and the Jacobian $J_k$.

In addition to the quantities that are computed explicitly in Algorithm~\ref{alg:ssqp}, our analysis also refers to the quantities that would have been computed in each iteration $k \in \N{}$, conditioned on the event that the algorithm has reached~$x_k$ as the $k$th iterate, if the true gradient $\nabla f(x_k)$ in place of the stochastic gradient $g_k$.  These quantities are denoted by a ``true'' superscript.  For example, in iteration $k$, the true search direction and corresponding true Lagrange multiplier estimate are the solution of the linear system
\bequation \label{eq:sqpsystemdet}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    \dktrue \\ \yktrue
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    \nabla f(x_k) \\ c_k
    \end{matrix}
    \right],
\eequation
which may be decomposed as $\dktrue = \uktrue + v_k$, where $\uktrue \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.  Here, we write $v_k$ (without a superscript) since the normal component of the search direction is defined in a manner that makes it independent of the objective gradient (estimate).  Similarly, the true value of the merit parameter that would have been computed is denoted
\bequationNN
    \tktritrue \gets
    \begin{cases}
        \infty\ \ \text{if $\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue, 0\} \leq 0$} & \\
        \frac{(1-\sigma)\|c_k\|_1}{\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}}\ \  \text{otherwise}. &
    \end{cases}
\eequationNN
This definition of $\tktritrue$ guarantees that, for any $\tau \leq \tktritrue$, one finds
\bequation \label{eq:qquadlbtrue}
    \Delta q(x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \thalf \tau \max\{(\dktrue)^\top H_k \dktrue, 0\} + \sigma \|c_k\|_1.
\eequation

%************
% Subsection
%************
\subsection{Stochastic Process} \label{subsec:process}

Henceforth, for the sake of formality, we shall refer in our analysis to the stochastic process generated by Algorithm~\ref{alg:ssqp}.  Specifically, in terms of values that are computed by the algorithm itself, we have the stochastic process
\bequationNN
  \{(X_k,G_k,D_k,Y_k,\Tcal_k,\Xi_k,\Acal_k)\},
\eequationNN
where, for all $k \in \N{}$, the random variables are: the algorithm iterate $X_k$, stochastic gradient estimate $G_k$, search direction $D_k$, Lagrange multiplier estimate $Y_k$, merit parameter $\Tcal_k$, ratio parameter $\Xi_k$, and stepsize $\Acal_k$.  For all $k \in \N{}$, a realization of the corresponding element of this process is denoted $(x_k,g_k,d_k,y_k,\tau_k,\xi_k,\alpha_k)$.  Similarly, in terms of ``true'' values and step decomposition values that are not computed by the algorithm, but are defined for the sake of our analysis, we have the simultaneously generated process
\bequationNN
  \{(\Vk,\Uk,\Dktrue,\Uktrue,\Yktrue,\Tktritrue)\},
\eequationNN
where, for all $k \in \N{}$, the random variables are: the normal search direction component $\Vk$, the tangential search direction component $\Uk$, the true search direction $\Dktrue$, the true tangential search direction component $\Uktrue$, the true Lagrange multiplier estimate $\Yktrue$, and the true trial merit parameter $\Tktritrue$.  For all $k \in \N{}$, a realization of the corresponding element of this process is denoted $(v_k,u_k,\dktrue,\uktrue,\yktrue,\tktritrue)$.  Finally, for the sake of tracking the number of merit parameter updates that occur during runs of the algorithm, we define the stochastic process $\{S_k\}$, where for all $k \in \N{}$ the random variable $S_k$ represents the number of merit parameter decreases up to the end of the $k$th iteration, i.e., the number of iterations in which $\Tcal_k < \Tcal_{k-1}$.  For all $k \in \N{}$, a realization of $S_k$ is denoted $s_k$.

In any run, the behavior of Algorithm~\ref{alg:ssqp} is dictated entirely by the initial conditions and the sequence of stochastic gradient estimates that are generated.  Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{G_0,\dots,G_{k-1}\}$, a realization of which (along with all initial conditions of the algorithm, including $X_0 = x_0$) determines the realizations of
\bequationNN
  \{X_j\}_{j=1}^k\ \text{and}\ \{(D_j,Y_j,\Tcal_j,\Xi_j,\Acal_j,V_j,U_j,D_j^{\rm true},U_j^{\rm true},Y_j^{\rm true},\Tcal_j^{\rm trial, true},S_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{0} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq 0}$ is a filtration.  When conditioning on a specific realization of Algorithm~\ref{alg:ssqp} up to the beginning of iteration $k \in \N{}$, we condition on $G_{[k-1]} = g_{[k-1]}$, since these stochastic gradients determine $x_k$.  (Recall our notation that $g_{[k-1]}$ represents $\{g_0,\dots,g_{k-1}\}$.)  Similarly, later in our analysis when we condition on $\Fcal_{k}$, we are conditioning on all realizations of $G_{[k-1]}$ that are measurable with respect to the filtration~$\Fcal_{k}$.

%************
% Subsection
%************
\subsection{Assumptions} \label{subsec:assumptions}

Our analysis presumes certain good behavior of the sequences of merit and ratio parameters that are set adaptively by the algorithm.  Formally, given $(\kmax,\smax,\tau_{\min},\xi_{\min}) \in \N{} \times \N{} \times \R{}_{>0} \times \R{}_{>0}$, our main result characterizes the worst-case behavior of Algorithm~\ref{alg:ssqp} conditioned on the event denoted as
\bequation\label{def:E}
  E := E(\kmax,\smax,\tau_{\min},\xi_{\min}),
\eequation
which we define as the event such that, in every realization of the algorithm, the merit parameters $\{\tau_k\}_{k=0}^{\kmax}$ and ratio parameters $\{\xi_k\}_{k=0}^{\kmax}$ satisfy
\bitemize
  \item $\tau_k \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\tktritrue \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\xi_k = \xi_{\min} > 0$ for all $k \in [\kmax]$, and
  \item $|\{k \in [\kmax] : \tau_k < \tau_{k-1}\}| < \smax$.
\eitemize
Consideration of this event as a focus for proving a worst-case complexity result for Algorithm~\ref{alg:ssqp} is justifiable for the following reasons.

\bitemize
  \item The condition in $E$ that the ratio parameter sequence is constant over all iterations is not actually essential for our analysis; rather, it is made for the sake of simplicity.  Indeed, in Section \ref{subsec:ratioparam}, we present an extension of our main result to the setting in which this parameter sequence is not constant.  Observe that, as proved in \cite[Lemma~3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, the sequence $\{\Xi_k\}$ is bounded below by a positive real number whose value is deterministic, i.e., it is independent of the sequence of stochastic gradient estimates that are generated by the algorithm.  Hence, for the sake of simplicity, we assume for now that $\{\Xi_k\}$ is constant and leave the statement of the more complicated version of our main result to a subsection at the end of our analysis.
  \item The conditions in $E$ pertaining to the behavior of the merit parameter sequence are not necessarily minor.  That said, attention to this behavior of the algorithm is justified by arguments made in \cite{BeraCurtONeiRobi21,ABerahas_FECurtis_DPRobinson_BZhou_2021}, which under the same kinds of assumptions made in this paper argue that, in any run of the algorithm, the probability is zero that the merit parameter vanishes.  Furthermore, in Section~\ref{subsec:subgauss}, we consider a particular setting of interest in which the distributions of the stochastic gradient estimates are sub-Gaussin over any run of the algorithm, in which case we show that the merit parameter remains bounded below with high probability, meaning that our main worst-case complexity bound---which holds with high probability due to the adaptivity of the merit parameter sequence---remains essentially unchanged in this setting when we do not presume upfront that the merit parameter sequence remains bounded above a positive real number.
  \item The condition in $E$ pertaining to the existence of $\smax$ is not actually an additional requirement beyond the existence of $\tau_{\min}$ in the event.  After all, by the construction of Algorithm~\ref{alg:ssqp}, it follows that when the merit parameter is decreased, it is decreased by at least a constant factor, from which it follows (under the existence of $\tau_{\min}$) that $\smax$ exists and satisfies
  \bequation \label{eq:smaxbound}
    \smax \leq \min\left\{\kmax+1, \left\lceil\frac{\log(\tau_{\min}/\tau_{-1})}{\log(1-\epsilon_\tau)}\right\rceil\right\}.
  \eequation
  That said, for simplicity and generality in our analysis, we define $\smax$ as a quantity that is decoupled from the above (conservative) inequality.
\eitemize

Conditioned on $E$, we assume the following about the stochastic gradient estimates.  Such an assumption, namely, that conditioned on the event that a given iterate has been reached the stochastic gradient is unbiased and has bounded variance, is common in analyses of stochastic optimization methods.  Here and throughout the remainder of the paper, Henceforth, we let $\Prob_k[\cdot]$ (respectively, $\E_k[\cdot]$) denote probabilty (respectively, expectation) conditioned on event $E$ and, for a given $g_{[k-1]}$, that $G_{[k-1]} = g_{[k-1]}$, i.e.,
\bequationNN
  \P_k[\cdot] := \P[\cdot | E, G_{[k-1]} = g_{[k-1]}]\ \ \text{and}\ \ \E_k[\cdot] := \E[\cdot | E, G_{[k-1]} = g_{[k-1]}].
\eequationNN

\bassumption\label{assum:eventE}
  There exists $M \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequation\label{eq.sg}
    \E_k[G_k] = \nabla f(x_k)\ \ \text{and}\ \ \E_k[\|G_k - \nabla f(x_k)\|_2^2] \leq M.
  \eequation
  In addition, there exists $M_\tau \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequation\label{eq.sg+}
    \baligned
      \text{either}\ \ \P_k[\nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &= 0 \\
      \text{or}\ \ \E_k[\|G_k - \nabla f(x_k)\|_2 | \nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &\leq M_\tau.
    \ealigned
  \eequation
\eassumption

Observe that the second inequality in \eqref{eq.sg} can imply \eqref{eq.sg+}, such as when there exists $p \in (0,1]$ such that, for all $k \in [\kmax]$ and $g_{[k-1]}$, one finds that
\bequationNN
  \P_k[\nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \geq p
\eequationNN
whenever this probability is nonzero.  This occurs, for example, when the objective of \eqref{eq:fdef} is a finite sum of $N$ terms and each stochastic gradient estimate is computed as a so-called mini-batch estimate through the uniform (random) selection of $b$ indices, in which case the above holds with $p = b/N$.

We make one additional assumption for our analysis, namely, the following.

\begin{assumption} \label{assum:ptau}
  There exists $p_{\tau} \in (0,1]$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequationNN
    \baligned
      \P_k[& G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \\
      & \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}] \geq p_{\tau}.
    \ealigned
  \eequationNN
\end{assumption}

Similar to \cite[Proposition~3.16]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, Assumption~\ref{assum:ptau} allows us to prove that, with high probability, the number of iterations in which $\tau_k > \tktritrue$ is not too large.  In \cite[Example 3.17]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, it was shown that the inequality in this assumption holds with $p_{\tau} = \frac12$ when, conditioned on having reached $x_k$, the stochastic gradient $G_k$ has a Gaussian distribution.  We show in in Section~\ref{subsec:subgauss} that this result can be extended to other settings in which the stochastic gradient distributions obey a mild form of symmetry.

%************
% Subsection
%************
\subsection{Properties of Algorithm \ref{alg:ssqp}} \label{subsec:algprops}

In this section, we state key results from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} that are needed for our analysis.

By \cite[Lemma 2.10]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, there exists $\kappa_{uv} \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, if $\|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2$, then $\frac12 (\dktrue)^\top H_k \dktrue \geq \frac14 \zeta \|\uktrue\|^2$, where $\zeta$ is defined in Assumption \ref{assum:Hk}.  Correspondingly, let us define
\bequationNN
  \Psi_k := \begin{cases}
        \|\uktrue\|^2 + \|c_k\| & \mbox{if } \|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2 \\
        \|c_k\| & \mbox{otherwise.}
    \end{cases}
\eequationNN

\begin{lemma}[{\cite[Lemma 2.11]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}] \label{lem:kappapsi}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold.  Then, there exists $\kappa_{\Psi} \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, the true search direction and constraint violation satisfy $\|\dktrue\|^2 + \|c_k\| \leq (\kappa_{\Psi} + 1) \Psi_k$.
\end{lemma}

\begin{lemma}[{\cite[Lemma 2.12]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}] \label{lem:kappaq}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_q \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any $\tau \leq \tktritrue$, the true reduction in the merit model satisfies $\Delta q (x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \kappa_q \tau \Psi_k$.
\end{lemma}

\blemma[{\cite[Lemma~3.7]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}]\label{lem:phidecrease}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold and suppose that $\{\beta_k\}$ is chosen such that $\beta_k \xi_k \tau_k/(\tau_k L + \Gamma) \in (0,1]$ for all $k \in [\kmax]$.  Then, for all $k \in [\kmax]$, it follows that
  \bequation \label{eq:phidecrease}
    \baligned
      \phi(x_k + \alpha_k d_k, \tau_k) - \phi(x_k, \tau_k)
      &\leq -\alpha_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue) \\
      &\quad + \thalf \alpha_k \beta_k  \Delta q(x_k,\tau_k,g_k,H_k,d_k) \\
      &\quad + \alpha_k \tau_k \nabla f(x_k)^\top (d_k - \dktrue).
    \ealigned
  \eequation
\elemma

\blemma \label{lem:dexpectation}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in [\kmax]$, it follows that $\E_k[D_k] = \dktrue$, $\E_k[U_k] = \uktrue$, and $\E_k[Y_k] = \yktrue$.  Moreover, there exists $\kappa_d \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, one finds that
  \bequationNN
    \left\|\begin{bmatrix} H_k & J_k^\top \\ J_k & 0 \end{bmatrix}^{-1}\right\| \leq \kappa_d,
  \eequationNN
  from which it follows that
  \bequationNN
    \baligned
      \|\dktrue\| \leq \kappa_d \|\nabla f(x_k)\| &\leq \kappa_d \kappa_g, \\
      \E_k[\|D_k - \dktrue\|] \leq \kappa_d \|G_k - \nabla f(x_k)\| &\leq \kappa_d \sqrt{M},\ \ \text{and} \\
      \E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &\leq \kappa_d M_\tau.
    \ealigned
  \eequationNN
\elemma
\bproof
  Except for the final inequality, the result follows from \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2021}.  As for the final inequality, observe by the arguments in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2021} that for any realization of $G_k$ and $D_k$ one finds $\|d_k - \dktrue\| \leq \kappa_d \|g_k - \nabla f(x_k)\|$, so
  \begin{align*}
    &\ \E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \\
    \leq&\ \kappa_d \E_k[\|G_k - \nabla f(x_k)\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \leq \kappa_d M_\tau,
  \end{align*}
  as desired. \qed
\eproof


\blemma[{\cite[Lemma~3.9]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}]\label{lem:product_bounds}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in [\kmax]$, it follows that
  \bequationNN
    \baligned
      \nabla f(x_k)^\top \dktrue \geq \E_k[G_k^\top D_k] &\geq \nabla f(x_k)^\top \dktrue - \zeta^{-1}M \\
      \text{and}\ \ \E_k[D_k^\top H_k D_k] &\geq (\dktrue)^\top H_k \dktrue.
    \ealigned
  \eequationNN
\elemma

%************
% Subsection
%************
\subsection{Complexity Result} \label{subsec:complexity}

In this section, we present our main complexity results. We derive our result in largely the same manner as the global convergence result in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, but with two major changes that stem from the need to characterize the behavior of the algorithm in the context of the adaptive merit parameter sequence.  At a high level, the two modifications are as follows:\footnote{FEC: Will come back to this after going through analysis.}
\begin{enumerate}
    \item \textcolor{blue}{We derive a new upper bound for the last term in \eqref{eq:phidecrease}. This inequality allows us to characterize decrease in the merit function and is central to the overall analysis. A new upper bound is needed in our setting, which is complicated by the fact that this term is the product of three correlated random variables: $\alpha_k$, $\tau_k$, and $\nabla f(x_k)^\top (D_k - \dktrue)$.  To handle this, we show under our assumptions that this term is bounded in terms of the probability that an event, which we denote as $\Ek3$ (defined formally below), occurs in iteration $k \in \N{}$.  This event only occurs on iterations $k$ when $\tau_k < \tau_{k-1}$ which, when combined with a maximum of $\smax$ decreases of $\tau$ due to Assumption \ref{assum:eventE}, allows us to obtain a bound on this quantity that holds with high-probability. The new upper bound is derived in Lemma \ref{lem:innerprod} while our high-probability bound on the summation (over $k=0,\dots,\kmax$) of the probabilities of $\Ek3$ occuring is presented in Lemma \ref{lem:Eksumlsmax}.}
    \item \textcolor{blue}{We characterize iterations at which $\tktritrue < \tau_k$ occurs. These iterations are problematic for the analysis due to the inclusion of $\tau_k$ in $\Delta q(x_k,\tau_k,\nabla f(x_k), H_k, \dktrue)$, which is used during the analysis to measure progress in the algorithm. One particular concern arises in the final complexity result; if $k^*$ occurs at an iterate such that $\tau_{k^*}^{trial,\text{true}} < \tau_{k^*}$, then $\Delta q(x_{k^*},\tau_{k^*},\nabla f(x_{k^*}), H_{k^*}, d^{\text{true}}_{k^*})$ cannot be related to our optimality conditions \eqref{eq:optconds}. To solve this issue, we introduce a theoretical sequence, $\hat{\tau}_k$, which, for all $k$, is the minimum of $\tau_k$ and $\tktritrue$, and analyze the algorithm's progress with respect to this sequence. Due to Assumption \ref{assum:ptau}, whenever the event $\tktritrue < \tau_k$ occurs, there is at least $p_{\tau}$ probability of decreasing $\tau$. Taken in combination with $\smax$ from Assumption \ref{assum:eventE}, this enables us to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ occurs. We introduce Lemma \ref{lem:dqbound} and Lemma \ref{lem:hattaudiff} to handle iterations such that $\tktritrue < \tau_k$. Additionally, we derive Lemma \ref{lem:Ktaulsmax} to provide a high-probability bound on the number of iterations at which $\tktritrue < \tau_k$ can occur.}
\end{enumerate}

Given $k \in [\kmax]$ and $g_{[k-1]}$, values generated by the algorithm have been determined value up to the beginning of iteration $k$, including $x_k$, $\dktrue$, and~$\tau_{k-1}$.  Given these quantities, let us define three events:
\bitemize
  \item $\Ek1$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) \geq 0$;
  \item $\Ek2$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} = \tau_{k-1}$; and
  \item $\Ek3$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} < \tau_{k-1}$.
\eitemize

We now derive an upper bound on the final term in \eqref{eq:phidecrease}.  In the following lemma, we make use, for given $k \in [\kmax]$ and $g_{[k-1]}$, of the stepsize values
\bequation\label{eq.alpha_mins}
  \baligned
    \alpha_{\min,k}^{<} := \frac{\beta_k \xi_{\min} \tau_{\min}}{\tau_{\min}L + \Gamma},\ \ \alpha_{\min,k}^{=} &:= \frac{\beta_k \xi_{\min} \tau_{k-1}}{\tau_{k-1}L + \Gamma}, \\
    \text{and}\ \ \varsigma_{\max,k} &:= \alpha_{\min,k}^{=} + \theta \beta_k^2.
  \ealigned
\eequation
The first two values here represent the smallest stepsizes that may be computed in the event that $\Tcal_k < \tau_{k-1}$ and in the event that $\Tcal_k = \tau_{k-1}$, respectively, for which it is easily verified that $\alpha_{\min,k}^{<} < \alpha_{\min,k}^{=}$.  Hence, $\varsigma_{\max,k}$ represents the largest stepsize that may be computed.

\begin{lemma} \label{lem:innerprod}
  Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold, let $\tau_{\min} \in \R{}_{>0}$ and $\xi_{\min} \in \R{}_{>0}$ be defined as for the event $E$ in \eqref{def:E}, and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$ with $(\alpha_{\min,k}^{<},\alpha_{\min,k}^{=},\varsigma_{\max,k})$ defined as in \eqref{eq.alpha_mins}, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ (\varsigma_{\max,k}\tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
  \end{align*}
\end{lemma}
\begin{proof}
  Consider arbitrary $k \in [\kmax]$ and $g_{[k-1]}$, and for ease of exposition, let us denote $\E_{k,j} = \E_k[\nabla f(x_k)^\top(D_k - \dktrue) | E_{k,j}]$ for all $j \in \{1,2,3\}$.  By the Law of Total Expectation, the fact that $0 < \tau_{\min} \leq \Tcal_k \leq \tau_{k-1}$ under $E$, and the definitions of $\alpha_{\min,k}^{<}$, $\alpha_{\min,k}^{=}$, and $\varsigma_{\max,k}$, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    =&\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek1] \Prob_k[\Ek1] \\
     &\ + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek2] \\
     &\ + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek3] \Prob_k[\Ek3] \\
    \leq&\ \varsigma_{\max,k} \tau_{k-1}  \E_{k,1} \Prob_k[\Ek1] + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,3} \Prob_k[\Ek3].
  \end{align*}
  Using this inequality, the Law of Total Expectation, and Lemma \ref{lem:dexpectation}, one obtains three distinct upper bounds by adding subtracting terms in multiple ways:
  \begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \varsigma_{\max,k} \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \varsigma_{\max,k} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \varsigma_{\max,k} \tau_{k-1} \E_{k,3} \Prob_k[\Ek3] + (\alpha_{\min,k}^{<} \tau_{\min} - \varsigma_{\max,k} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \\
    =&\ - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] + (\alpha_{\min,k}^{<} \tau_{\min} - \varsigma_{\max,k} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3]; \\
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \theta \beta_k^2 \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,3} \Prob_k[\Ek3] + (\alpha_{\min,k}^{<} \tau_{\min} - \alpha_{\min,k}^{=} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \\
    =&\ \theta \beta_k^2 \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + (\alpha_{\min,k}^{<} \tau_{\min} - \alpha_{\min,k}^{=} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3];\ \ \text{and} \\
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \alpha_{\min,k}^{<} \tau_{\min} \E_{k,1} \Prob_k[\Ek1] + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \\
    &\ + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,2} \Prob_k[\Ek2] + (\alpha_{\min,k}^{=} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,3} \Prob_k[\Ek3] \\
    =&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \\
    &\ + (\alpha_{\min,k}^{=} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2].
  \end{align*}
  Averaging these three upper bounds, one obtains
  \begin{align}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \nonumber \\
    \leq&\ \tfrac13 ((\alpha_{\min,k}^{=} + 2\theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\ + \tfrac13 ((\alpha_{\min,k}^{=} - \theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\ + \tfrac13 (2\alpha_{\min,k}^{<} \tau_{\min} - (2\alpha_{\min,k}^{=} + \theta \beta_k^2) \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \nonumber \\
    =&\ \tfrac13 ((\alpha_{\min,k}^{=} + 2\theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\ - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\ - \tfrac13 ((2\alpha_{\min,k}^{=} + \theta \beta_k^2) \tau_{k-1} - 2\alpha_{\min,k}^{<} \tau_{\min}) \E_{k,3} \Prob_k[\Ek3]. \label{eq:innerprodproof1}
  \end{align}
  This bound can be rewritten as follows.  By the Law of Total expectation,
  \begin{align}
    &\ \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    =&\ \E_k[\nabla f(x_k)^\top(D_k - \dktrue)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3], \label{eq.new1}
  \end{align}
  and along with Lemma \ref{lem:dexpectation} one finds
  \begin{align}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek2] \Prob_k [\Ek2] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek2] \Prob_k [\Ek2] \nonumber \\
    &= \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \nonumber \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek1]\Prob_k [\Ek1] \nonumber \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek3] \Prob_k [\Ek3] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \nonumber \\
    &\leq \kappa_g \E_k[\|D_k - \dktrue\|] \leq \kappa_g \kappa_d \sqrt{M}. \label{eq.new2}
  \end{align}
  In addition, Lemma \ref{lem:dexpectation} also yields that
  \begin{align}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek3] \Prob_k[\Ek3] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \nonumber \\
    &\leq \kappa_g \kappa_d M_{\tau} \Prob_k[\Ek3]. \label{eq.new3}
  \end{align}
  Combining \eqref{eq:innerprodproof1}, \eqref{eq.new1}, \eqref{eq.new2}, and \eqref{eq.new3}, the desired result follows. \qed
\end{proof}

\textcolor{blue}{Now, we turn our attention to the second modification mentioned in the outline of this section. Our complexity result is derived through the use of \eqref{eq:phidecrease}, which relates decrease in our merit function to $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$. On any iteration for which $\tau_k \leq \tktritrue$ holds, $\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)$ can be directly related to the optimality conditions defined in \eqref{eq:optconds}. Unfortunately, the same is not true for $k$ such that $\tau_k > \tktritrue$. Thus, in order to provide an informative bound on such iterations, we introduce the following sequence:
\bequation \label{eq:hattaudef}
    \hat{\Tcal}_k := \min\{\Tcal_k, \tktritrue\},
\eequation
which we will use throughout the rest of the analysis (note that because we are conditioned on the history up to the start of iteration $k$, $\Tcal_k$ is a random variable, while $\tktritrue$ is not).}

\textcolor{blue}{Now, we derive a bound on the conditional expectation of $\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)$ using the definition of $\hat{\Tcal}_k$.}

\begin{lemma} \label{lem:dqbound}
  Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$, one finds that
  \begin{align*}
    &\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \\
    \leq&\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)] + \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M \\
    &\ + (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)).
  \end{align*}
\end{lemma}
\begin{proof}
  By the definition of $\Delta q$ in \eqref{eq:deltadef}, one has that
  \begin{align}
    &\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \nonumber \\
    =&\ \E_k[-\hat{\Tcal}_k(G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k, 0\}) + \|c_k\|_1] \nonumber \\
    =&\ \E_k[-\hat{\Tcal}_k(G_k^\top D_k - \nabla f(x_k)^\top \dktrue  + \thalf \max\{D_k^\top H_k D_k, 0\} \nonumber \\
    &\qquad - \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\})] \nonumber \\
    &\ + \E_k[-\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\}) + \|c_k\|_1] \nonumber \\
    =&\ \E_k[\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue - G_k^\top D_k + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} \nonumber \\
    &\ - \thalf \max\{D_k^\top H_k D_k, 0\})] + \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]. \label{eq:dqbound1}
  \end{align}
  Now, for simplicity of notation, define
  \begin{align*}
    Q_k :=&\ \nabla f(x_k)^\top \dktrue - G_k^\top D_k \\
    &\ + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \max\{D_k^\top H_k D_k, 0\}.
  \end{align*}
  Let $E_Q$ denote the event that $Q_k \geq 0$ and let $E_Q^c$ denote the event that $Q_k < 0$ occurs.  By the Law of Total Expectation, one has that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
      &= \E_k[\hat{\Tcal}_k Q_k | E_Q] \Prob_k[E_Q] + \E_k[\hat{\Tcal}_k Q_k | E_Q^c] \Prob_k[E_Q^c] \\
      &\leq \tau_{k-1} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{\min} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c].
  \end{align*}
  Therefore, by the Law of Total Probability, Lemma \ref{lem:product_bounds}, Jensen's inequality, and convexity of $\max\{\cdot,0\}$, it follows that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
    \leq&\ \tau_{k-1} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{k-1} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    &\ + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    =&\ \tau_{k-1} \E_k[Q_k] + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    =&\ \tau_{k-1} (\nabla f(x_k)^\top \dktrue - \E_k[G_k^\top D_k] \\
    &\ + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \E_k[\max\{D_k^\top H_k D_k, 0\}]) \\
    &\ + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    \leq&\ \tau_{k-1} \zeta^{-1} M + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c],
  \end{align*}
  and by similar reasoning one finds that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
    \leq&\ \tau_{\min} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{\min} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    &\ + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \\
    =&\ \tau_{\min} \E_k[Q_k] + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \\
    \leq&\ \tau_{\min} \zeta^{-1} M + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q].
  \end{align*}
  Averaging these two upper bounds, one finds that
  \begin{align}
    \E_k[\hat{\Tcal}_k Q_k] 
    \leq&\ \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M + \thalf (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \nonumber \\
    &\ + \thalf (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \label{eq:dqbound2}.
  \end{align}
  Our goal now is to bound the latter two terms in \eqref{eq:dqbound2}.  Toward this end, observe that by the Cauchy-Schwarz inequality, Lemma~\ref{lem:dexpectation}, Assumption~\ref{assum:eventE}, Jensen's inequality, and concavity of the square root over $\R{}_{\geq0}$, one finds that
  \begin{align}
    &\ \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \nonumber \\
    \leq&\ \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top \dktrue|] +\E_k[|G_k^\top \dktrue - G_k^\top D_k|] \nonumber \\
    \leq&\ \|\dktrue\| \E_k [\|\nabla f(x_k) - G_k\|] + \E_k[\|G_k\|\|\dktrue - D_k\|] \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]} + \kappa_d \E_k[\|G_k\| \|\nabla f(x_k) - G_k\|]  \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]}  \nonumber \\
    &\ + \kappa_d \E_k[(\|G_k - \nabla f(x_k)\| + \|\nabla f(x_k)\|) \|\nabla f(x_k) - G_k\|] \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{M} + \kappa_d (M + \kappa_g \sqrt{M}) = \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}). \label{eq.wednesday1}
  \end{align}
  In addition, by the Cauchy-Schwarz inequality, Lemma~\ref{lem:dexpectation}, and Assumption~\ref{assum:eventE}, and the fact that $\|a\|^2 \leq 2(\|a - b\|^2 + \|b\|^2)$ for any $(a,b) \in \R{n} \times \R{n}$, one finds
  \begin{align}
    &\ \E_k[|\thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \max\{D_k^\top H_k D_k, 0\}|] \nonumber \\
    \leq&\ |\thalf \max\{(\dktrue)^\top H_k \dktrue, 0\}| + \E_k[|\thalf \max\{D_k^\top H_k D_k, 0\}|] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \thalf \|H_k\|\E_k[\|D_k\|^2] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \thalf \kappa_d^2 \|H_k\|\E_k[\|G_k\|^2] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \kappa_d^2 \|H_k\|\E_k[\|G_k - \nabla f(x_k)\|^2 + \|\nabla f(x_k)\|^2] \nonumber \\
    \leq&\ \thalf \kappa_H \kappa_d^2 \kappa_g^2 + \kappa_H \kappa_d^2 (M + \kappa_g^2) \nonumber \\
    \leq&\ \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2). \label{eq.wednesday2}
  \end{align}
  By the Law of Total Expectation, \eqref{eq.wednesday1}, and \eqref{eq.wednesday2}, it follows that
  \begin{align*}
    \E_k[Q_k | E_Q] \Prob_k[E_Q] &= \E_k[|Q_k| | E_Q] \Prob_k[E_Q] \\
    &= \E_k[|Q_k|] - \E_k[|Q_k| | E_Q^c] \Prob_k[E_Q^c] \\
    &\leq \kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2),
  \end{align*}
  and by a similar argument, one finds that
  \begin{align*}
    -\E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] &= \E_k[|Q_k| | E_Q^c] \Prob_k[E_Q^c] \\
    &= \E_k[|Q_k|] - \E_k[|Q_k| | E_Q] \Prob_k[E_Q] \\
    \leq&\ \kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2).
  \end{align*}
  The conclusion follows by combining these equations, \eqref{eq:dqbound1}, and \eqref{eq:dqbound2}. \qed
\end{proof}

\textcolor{blue}{Next, we introduce a lemma which controls the difference in $\Delta q(\cdot)$ on iterations where $\tktritrue < \Tcal_k$.}

\begin{lemma} \label{lem:hattaudiff}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$, with $(\alpha_{\min,k}^{<},\alpha_{\min,k}^{=},\varsigma_{\max,k})$ defined as in \eqref{eq.alpha_mins} and $\hat{\Tcal}_k$ defined in \eqref{eq:hattaudef}, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d)
  \end{align*}
  and
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k, \Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d(2 + \kappa_d \kappa_H) (M + \kappa_g^2).
  \end{align*}
\end{lemma}
\begin{proof}
  Under the stated assumptions, it follows from the stated lemma and definitions, along with the definition of $\Delta q$ in \eqref{eq:deltadef}, that
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
    =&\ \E_k[\Acal_k (\Tcal_k - \hat{\Tcal}_k) (\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue,0\})] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) |\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue,0\}| \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d \kappa_g^2 + \thalf\kappa_H \kappa_d^2 \kappa_g^2),
  \end{align*}
  and, along with $\|a\|^2 \leq 2(\|a - b\|^2 + \|b\|^2)$ for any $(a,b) \in \R{n} \times \R{n}$, one finds
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
    =&\ \E_k[\Acal_k (\hat{\Tcal}_k - \Tcal_k) (G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k,0\})] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_k[|G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k,0\}|] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d + \thalf \kappa_d^2 \kappa_H) \E_k[\|G_k\|^2] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d + \thalf \kappa_d^2 \kappa_H) (2(M + \kappa_g^2)),
  \end{align*}
  which together are the desired conclusions. \qed
\end{proof}

\textcolor{blue}{Next, we present the statements of two lemmas, which provide upper bounds, in high probability, on key components of the complexity result. The proofs of these lemmas are relegated to Appendix \ref{app:simple} for presentation purposes. Both of these lemmas use the following function in their statement. For any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, let
\bequation \label{eq:lsd}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\eequation
Now we can state the first lemma, which gives a high-probability bound on the sum of the probabilities from applying Lemma \ref{lem:innerprod} at each iteration.}

\begin{lemma} \label{lem:Eksumlsmax}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for any $\delta \in (0,1)$,
  \bequation \label{eq:Ek3lsmax}
    \Prob\left[\sum_{k=0}^{\kmax} \Prob [E_{k,3} | E, \mathcal{F}_k] \leq \ell(\smax,\delta) + 1\Bigg | E \right] \geq 1-\delta.
  \eequation
\end{lemma}
\begin{proof}
  This result is proved in Appendix~\ref{app:simple}.
\end{proof}

\textcolor{blue}{Before stating the next lemma, recall the definition of $\hat{\Tcal}_k$ in \eqref{eq:hattaudef} and let
$k_{\tau}$ denote the index set
\bequation \label{eq:smallktau}
    k_{\tau} := \{k : \tktritrue < \tau_{k-1}\}.
\eequation
In addition, we let
$\mathcal{K}_{\tau}$ denote the associated random index set
\bequation \label{eq:Ktau}
    \mathcal{K}_{\tau} := \{k : \tcalktritrue < \Tcal_{k-1}\}.
\eequation
By the definitions of $\Tcal_k$, $\tcalktritrue$, and $\hat{\Tcal}_k$, this set of iterations is a superset of the iterations at which $\hat{\Tcal}_k < \Tcal_k$ occurs and can therefore be used to characterize the number of iterations at which this event occurs. In addition, the event $\tktritrue < \tau_{k-1}$ does {\it not} depend on $G_k$, which makes it more convenient to work with analytically. In particular, this means that $G_k$ is conditionally independent of the event $\tktritrue < \tau_{k-1}$ given $g_{[k-1]}$ and $E$.}

\textcolor{blue}{In the following lemma, we bound the cardinality of $\Kcal_{\tau}$ with high probability.}

\begin{lemma} \label{lem:Ktaulsmax}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold and let $\Kcal_\tau$ be defined as in \eqref{eq:Ktau}.  Then, for any $\delta \in (0,1)$, it follows that
  \bequation \label{eq:Ktaulsmax}
    \Prob\left[|\mathcal{K}_{\tau}| \leq \left\lceil \frac{\ell(\smax,\delta)+1}{p_{\tau}}\right\rceil \Bigg| E\right] \geq 1-\delta.
  \eequation
\end{lemma}
\begin{proof}
  This result is proved in Appendix~\ref{app:simple}.
\end{proof}

We are now prepared to prove a convergence rate result.

\begin{theorem} \label{thm:complexity}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold, let $\tau_{\min} \in \R{}_{>0}$ and $\xi_{\min} \in \R{}_{>0}$ be defined as for the event $E$ in \eqref{def:E}, let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}, define
  \bequationNN
    \baligned
      A_{\min} :=&\ \frac{\xi_{\min} \tau_{\min}}{\tau_{\min}L + \Gamma},\ \ A_{\max} := \frac{\xi_{-1} \tau_{-1}}{\tau_{-1}L + \Gamma}, \\
      \Mbar :=&\ \thalf (A_{\max} + \theta\beta) \beta^2 \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M \\
    &\ + \thalf (A_{\max} + \theta\beta) \beta^2 (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)), \\
      \kappa_{\Delta q} :=&\ (A_{\max} \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d (2M + 3\kappa_g^2) (1 + \thalf \kappa_H \kappa_d), \\
      \text{and}\ \ \kappa_{E_3} :=&\ ((A_{\max} + \theta \beta)\tau_{-1} - A_{\min} \tau_{\min}) \kappa_g \kappa_d \ktaudec,
    \ealigned
  \eequationNN
  and, for all $k \in [\kmax]$ and $g_{[k-1]}$, let $\hat{\Tcal}_k$ be defined as in \eqref{eq:hattaudef} and
  \bequationNN
    \beta_k = \beta := \frac{\gamma}{\sqrt{\kmax+1}}\ \ \text{for some}\ \ \gamma \in \(0,\frac{A_{\min}}{A_{\max} + \theta}\right].
  \eequationNN
  Then, with $K^*$ having a discrete uniform distribution over $[\kmax]$, one finds
  \begin{align}
    &\ \E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \nonumber \\
    \leq&\ \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(\smax,\delta/2)+1)}{A_{\min} \gamma \sqrt{\kmax+1}} \nonumber \\
    &\ + \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{\kmax+1}} \left\lceil\frac{\ell(\smax,\delta/2)+1}{p_{\tau}}\right\rceil. \label{eq:complexity}
  \end{align}
\end{theorem}
\begin{proof}
  First, consider arbitrary $k \in [\kmax]$.  By Lemmas~\ref{lem:phidecrease} and \ref{lem:innerprod}, one has that
  \begin{align*}
    &\ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) \\
    &\ + \Acal_k \Tcal_k \nabla f(x_k)^\top (D_k - \dktrue)] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] \\
    &\ + (\varsigma_{\max,k}\tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
  \end{align*}
  Let $E_{k,\tau}$ be the event that $\Tktritrue \geq \tau_{k-1}$ and let $E_{k,\tau}^c$ be the complementary event that $\Tktritrue < \tau_{k-1}$.  Observe that whether $E_{k,\tau}$ or $E_{k,\tau}^c$ occurs is determined by events leading up to iteration $k$.  Hence, the bound in Lemma~\ref{lem:dqbound} holds even if one conditions on the occurence of event $E_{k,\tau}$ or on the occurence of $E_{k,\tau}^c$.  This means that, with the bound above, \eqref{eq:qquadlb}, and \eqref{eq:qquadlbtrue}, one finds
  \begin{align*}
    &\ \E_k [\phi(x_k + \alpha_k D_k, \Tcal_k) | E_{\tau,k}^c] - \E_k [\phi(x_k, \Tcal_k) | E_{\tau,k}^c] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    =&\ \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ -A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \thalf (A_{\max}\beta + \theta\beta^2) \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + ((A_{\max}\beta + \theta\beta^2) \tau_{k-1} - A_{\min} \beta \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ -(A_{\min} - \thalf (A_{\max} + \theta\beta) \beta) \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \thalf (A_{\max} + \theta\beta) \beta^2 \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M \\
    &\ + \thalf (A_{\max} + \theta\beta) \beta^2 (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)) \\
    &\ + ((A_{\max} + \theta\beta) \tau_{k-1} - A_{\min} \tau_{\min}) \beta \kappa_g \kappa_d M_\tau \Prob_k[\Ek3 | E_{\tau,k}^c] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ - \thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \kappa_{E_3} \beta \Prob_k[\Ek3 | E_{\tau,k}^c] + \Mbar \beta^2,
    \\
    \\
    \\
    \\
    \leq&\ -\beta (A_{\min} - \thalf (A_{\max}+\theta) \beta) \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] + \frac{\tau_{k-1} + \tau_{\min}}{4} \beta^2 A_{\max} \zeta^{-1} M \\
    &\ + \thalf \beta^2 A_{\max} (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}) + \thalf \kappa_H \kappa_d^2 (3\kappa_g^2 + 2M)) \\
    &\ + \beta (\tau_{k-1}(A_{\max} + \theta \beta) -\tau_{\min} A_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3| E_{\tau,k}^c] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}\\ 
    \leq&\ -\thalf \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] + \kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}^c] + \beta^2 \hat{M}.
  \end{align*}
  and, similarly, since $\Tktritrue \geq \tau_{k-1} \geq \Tcal_k$ in event~$E_{k,\tau}$, one finds that
  \begin{align*}
    &\ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) | E_{k,\tau}] - \E_k [\phi(x_k, \Tcal_k) | E_{k,\tau}] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    +&\ \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    -&\ \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    +&\ \kappa_{E_3} \Prob_k[\Ek3 | E_{k,\tau}] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\ 
    \leq&\ -\thalf \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}] + \kappa_{\Delta q} \\
    &\ + \kappa_{E_3} \Prob_k[E_{k,3} | E_{k,\tau}] + \beta^2 \hat{M}.
  \end{align*}


Now by the law of total probability and the law of total expectation,
\begin{align*}
    &\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &=\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] \\
    &\quad+ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k, \Tcal_k)| k \in k_{\tau}] \Prob_k[k \in k_{\tau}] \\
    &\leq -\thalf \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}] \Prob_k[k \in k_{\tau}] + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}] \Prob_k[k \in k_{\tau}] + \beta^2 \hat{M} \Prob_k[k \in k_{\tau}] \\
    &\quad-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3} | k \in k_{\tau}^c] \Prob_k[k \in k_{\tau}^c] + \beta^2 \hat{M} \Prob_k[k \in k_{\tau}^c] \\
    &=-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] \\
    &\quad+\kappa_{E_3} \Prob_k[E_{k,3}] + \beta^2 \hat{M} + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}]
\end{align*}

Summing this inequality for all $k \in \{0,\dots,\kmax\}$,
\begin{align*}
    &\sum_{k=0}^{\kmax} \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    &\leq \sum_{k=0}^{\kmax} (-\frac12 \beta A_{\min} \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] + \kappa_{E_3} \Prob_k[E_{k,3}] + \kappa_{\Delta q} \Prob_k[k \in k_{\tau}]) \\
    &\quad+ (\kmax+1) \beta^2 \hat{M}.
\end{align*}

Now, let $g_{[\kmax]} : = \{g_0,\dots,g_{\kmax}\}$ denote any sequence of stochastic gradients that are measurable with respect to the filtration $\mathcal{F}_{\kmax+1}$. Note that $\Prob_k[k \in k_{\tau}] \in \{0,1\}$ since the event $k \in k_{\tau}$ does not depend on $G_k$ when conditioned on $\Fcal_k$ and $E$. Therefore, by total expectation, the definition of $\Fcal_{\kmax+1}$, Lemma \ref{lem:Eksumlsmax}, Lemma \ref{lem:Ktaulsmax}, and the union bound, with probability at least $1-\hat{\delta}$,
\begin{align}
    &\sum_{k=0}^{\kmax} \E [\phi(X_k + \Acal_k D_k, \Tcal_k)| E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \nonumber \\
    &= \int_{g_{[\kmax]} \in \mathcal{F}_{\kmax+1}} \sum_{k=0}^{\kmax} \E [\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k,\Tcal_k) | E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] f_{G}(g) dg \nonumber \\
    &\leq \int_{g_{[\kmax]} \in \mathcal{F}_{\kmax+1}} \Bigg(-\frac12 \beta A_{\min} \sum_{k=0}^{\kmax} \E[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)|E,G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \nonumber \\
    &\quad+ \kappa_{\Delta q} \sum_{k=0}^{\kmax} \Prob[k \in k_{\tau}|E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] + \kappa_{E_3}\sum_{k=0}^{\kmax} \Prob[\Ek3 |  E, G_0 = g_0,\dots,G_{k-1} = g_{k-1}] \Bigg) f_{G}(g) dg \nonumber \\
    &\quad+(\kmax+1) \beta^2 \hat{M} \nonumber \\
    &= -\frac12 \beta A_{\min} \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E, \Fcal_k] + \kappa_{\Delta q} \E\big[|\mathcal{K}_{\tau}|\big|E\big] \nonumber \\
    &\quad+ \kappa_{E_3}\sum_{k=0}^{\kmax} \Prob[\Ek3 | E, \Fcal_k] +(\kmax+1) \beta^2 \hat{M} \nonumber \\
    &\leq -\frac12 \beta A_{\min} \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E, \Fcal_k] + \kappa_{\Delta q} \left\lceil\frac{\ell(\smax,\hat{\delta}/2)+1}{p_{\tau}}\right\rceil \nonumber \\
    &\quad+ \kappa_{E_3}(\ell(\smax,\hat{\delta}/2)+1) +(\kmax+1) \beta^2 \hat{M}, \label{eq:complexityproof1}
\end{align}
where $f_{G}(g)$ is the probability density function of the random variable $G$. Working with left side of this inequality,
\begin{align*}
    &\sum_{k=0}^{\kmax} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \\
    &= \sum_{k=0}^{\kmax} \E [\Tcal_k f(X_k + \Acal_k D_k) + \|c(X_k + \Acal_k D_k)\|_1 | E,\Fcal_k] - \E[\Tcal_k f(X_k) + \|c(X_k)\|_1 | E,\Fcal_k] \\
    &= \sum_{k=0}^{\kmax} \E [\Tcal_k (f(X_k + \Acal_k D_k) - f_{\min}) + \|c(X_k + \Acal_k D_k)\|_1 | E,\Fcal_k] - \E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E,\Fcal_k].
\end{align*}
It follows by the monotonicity of the $\Tcal_k$ sequence that
\bequationNN
-\E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_k] \geq - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_k].
\eequationNN
Thus,
\begin{align*}
    &\sum_{k=0}^{\kmax} \E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_k] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_k] \\
    &\geq \E [\Tcal_{\kmax} (f(X_{\kmax+1}) - f_{\min}) + \|c(X_{\kmax+1})\|_1 | E,\Fcal_k] - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1.
\end{align*}
Combining this with \eqref{eq:complexityproof1},
\begin{align*}
    &\beta \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E,\Fcal_k] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \kappa_{E_3}(\ell(\smax,\delta/2)+1)}{A_{\min}} \\
    &\quad+ \frac{2 (\kmax+1) \beta^2 \hat{M}}{A_{\min}} + \frac{2}{A_{\min}} \kappa_{\Delta q} \left\lceil\frac{\ell(\smax,\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
Dividing both sides of this inequality by the summation of $\beta$,
\begin{align*}
    &\frac{1}{\sum_{k=0}^{\kmax} \beta} \sum_{k=0}^{\kmax} \beta \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue)|E,\Fcal_k] \\
    &\leq 2\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 (\kmax+1) \beta^2 \hat{M} + \kappa_{E_3}(\ell(\smax,\delta/2)+1)}{A_{\min} \sum_{k=0}^{\kmax} \beta} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \sum_{k=0}^{\kmax} \beta} \left\lceil\frac{\ell(\smax,\delta/2)+1}{p_{\tau}}\right\rceil,
\end{align*}
so that by the definitions of $K^*$ and $\beta$,
\begin{align*}
    &\E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{true})|E] \\
    &\leq \frac{2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(\smax,\delta/2)+1)}{A_{\min} \gamma \sqrt{\kmax+1}} \\
    &\quad+ \frac{2 \kappa_{\Delta q}}{A_{\min} \gamma \sqrt{\kmax+1}} \left\lceil\frac{\ell(\smax,\delta/2)+1}{p_{\tau}}\right\rceil.
\end{align*}
\end{proof}

Now we convert this into a result in terms of our optimality conditions \eqref{eq:optconds}.

\begin{corollary} \label{coro:complexity}
    Let the assumptions of Theorem \ref{thm:complexity} hold. Then, with probability at least $1-\delta$,
    \begin{align}
        &\E\left[\frac{\|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\|^2}{\kappa_H^2} + \|c(X_{K^*})\| \Bigg| E\right] \nonumber \\
        &\leq \frac{(\kappa_{\Psi} + 1)(2\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + 2 \gamma^2 \hat{M} +  \kappa_{E_3}(\ell(\smax,\delta/2)+1))}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{\kmax+1}} \label{eq:coro} \\
        &\quad+ \frac{2 (\kappa_{\Psi} + 1) \kappa_{\Delta q}}{\tau_{\min} \kappa_q A_{\min} \gamma \sqrt{\kmax+1}} \left\lceil\frac{\ell(\smax,\delta/2)+1}{p_{\tau}}\right\rceil \nonumber. 
    \end{align}
\end{corollary}

\begin{proof}
    The result follows by Lemma \ref{lem:kappapsi}, Lemma \ref{lem:kappaq}, and Theorem \ref{thm:complexity} combined with \eqref{eq:sqpsystemdet}, which implies that
    \bequationNN
        \|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\| = \|H_{k^*} D^{true}_{K^*}\| \leq \kappa_H \|D^{true}_{K^*}\|.
    \eequationNN
\end{proof}

We remark again that this result, in terms of the norm of the gradient of the Lagrangian, matches the worst-case complexity of the projected stochastic gradient method \cite{DDavis_DDrusvyatskiy_2019}.

%************
% Subsection
%************
\subsection{Complexity Result for Symmetric Sub-Gaussian Distributions} \label{subsec:subgauss}

In this section, we show that Assumptions \ref{assum:eventE} and \ref{assum:ptau} occur with high probability when the stochastic gradient $G_k$ follows a symmetric, sub-Gaussian distribution.

Throughout this section, we work with the following assumption.

\begin{assumption} \label{assum:symmsubgauss}
    At every iteration $k = \{0,\dots,\kmax\}$, the stochastic gradient $G_k$ satisfies
    \bequation
        \E[G_k | g_{[k-1]}] = \nabla f(x_k),
    \eequation
    \bequation \label{eq:subgauss}
        \E[\exp(\|\nabla f(x_k)-G_k\|^2/M) | g_{[k-1]}] \leq \exp(1),
    \eequation
    and the quantities $G_k - \nabla f(x_k)$ and $\nabla f(x_k) - G_k$ are equivalent in distribution. Finally, for all $k = \{0,\dots,\kmax\}$, the ratio parameter $\xi_k$ satisfies $\xi_k = \xi_{\min}$.
\end{assumption}

The above assumption has a number of important implications. The first is that Assumption \ref{assum:ptau} occurs (without conditioning on event $E$) with $p_{\tau} = \frac12$, as we show in the following lemma.

\blemma \label{lem:subgptau}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then,
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | g_{[k-1]}] \geq \frac12.
    \eequationNN
\elemma

\bproof
    Let $Z_k$ be a basis for the null space of $J_k$, which under Assumption \ref{assum:fcsmooth} is a matrix in $\R{n\times(n-m)}$. Then, let $W_k$ be such that $U_k = Z_k W_k$ and $\wktrue$ be such that $\uktrue = Z_k \wktrue$. It follows from the first block in \eqref{eq:sqpsystem} that 
    \bequationNN
        H_k (Z_k W_k + v_k) + J_k^\top Y_k = -G_k \Longleftrightarrow Z_k W_k = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (G_k + H_k v_k).
    \eequationNN
    Using this equality and simplifying,
    \bequationNN
        G_k^\top D_k + D_k^\top H_k D_k = v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} G_k + H_k^{1/2} v_k).
    \eequationNN
    In a similar fashion, by \eqref{eq:sqpsystemdet},
    \bequationNN
        Z_k \wktrue = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (\nabla f(x_k) + H_k v_k)
    \eequationNN
    so that
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + (\dktrue)^\top H_k \dktrue \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} \nabla f(x_k) + H_k^{1/2} v_k).
    \end{align*}

    Then,
    \begin{align*}
        &G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (G_k -\nabla f(x_k))),
    \end{align*}
    and,
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (\nabla f(x_k) - G_k)),
    \end{align*}
    are equivalent in distribution by Assumption \ref{assum:symmsubgauss}. Therefore,
    \begin{align*}
        &\Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &=\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}].
    \end{align*}
    In addition, we have
    \begin{align*}
        1 &= \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &+\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}] \\
        &-\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} = 0 | g_{[k-1]}].
    \end{align*}
    Taking these two together, it follows that
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \geq \frac12,
    \eequationNN
    proving the claim.
\eproof

Next, we repeat a well known property of sub-Gaussian random variables.
\blemma \label{lem:subgboundedrv}
    Suppose Assumption \ref{assum:symmsubgauss} holds. Then, for any $\delta \in (0,1)$,
    \bequation \label{eq:subgboundedrv}
        \Prob\left[\underset{k \in \{0,\dots,\kmax\}}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{M \left(1 + \log \frac{\kmax+1}{\delta}\right)} | g_{[k-1]}\right] \geq 1 - \delta.
    \eequation
\elemma

\bproof
    By Markov's inequality and Assumption \ref{assum:symmsubgauss},
    \begin{align*}
        &\Prob\left[\underset{k \in \{0,\dots,\kmax\}}{\max} \|G_k - \nabla f(x_k)\|^2 > M \left(1 + \log \frac{\kmax+1}{\delta}\right) \bigg| g_{[k-1]}\right] \\
        &= \Prob\left[\exp\left(\underset{k \in \{0,\dots,\kmax\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) > \exp\left(1 + \log \frac{\kmax+1}{\delta}\right) \bigg| g_{[k-1]}\right] \\
        &\leq \exp\left(-1 - \log \frac{\kmax+1}{\delta}\right)\E\left[\exp\left(\underset{k \in \{0,\dots,\kmax\}}{\max} \|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]}\right] \\
        &= \exp\left(-1 - \log \frac{\kmax+1}{\delta}\right)\E\left[\underset{k \in \{0,\dots,\kmax\}}{\max} \exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]}\right] \\
        &\leq \exp\left(-1 - \log \frac{\kmax+1}{\delta}\right)\sum_{k=0}^{\kmax} \E\left[\exp\left(\|G_k - \nabla f(x_k)\|^2/M\right) \bigg| g_{[k-1]} \right] \\
        &\leq \exp(-1) \frac{\delta}{\kmax+1} (\kmax+1)\exp(1) = \delta.
    \end{align*}
\eproof

We conclude this section by showing that under Assumption \ref{assum:symmsubgauss}, event $E$ as defined in Assumption \ref{assum:eventE} occurs with high probability.

\blemma \label{lem:subgeventE}
    Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then, there exists a constant $\kappa_{\tau_{\min}}$ such that, with probability at least $1-\delta$, event $E$ of Assumption \ref{assum:eventE} occurs with
    \bequationNN
        \ktaudec = \sqrt{M \left(1 + \log \frac{\kmax+1}{\delta}\right)}.
    \eequationNN
    and
    \bequation \label{eq:sgtaumin}
        \tau_{\min} = \frac{(1-\sigma)(1-\epsilon_\tau)}{\kappa_v \sqrt{M \left(1 + \log \frac{\kmax+1}{\delta}\right)} + \kappa_{\tau_{\min}}}, \quad  \smax = \left\lceil\frac{\log \frac{(1-\sigma)(1-\epsilon_\tau)}{\tau_{-1} \kappa_v \sqrt{M \left(1 + \log \frac{\kmax+1}{\delta}\right)} + \tau_{-1}\kappa_{\tau_{\min}}}}{\log 1-\epsilon_\tau }\right\rceil.
    \eequation
\elemma

\bproof
    We begin the proof by noting that by Jensen's inequality and the convexity of $\exp(\cdot)$,
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2| g_{[k-1]}] \leq M.
    \eequationNN
    The bound on $\ktaudec$ follows directly from Lemma \ref{lem:subgboundedrv}. Finally, the bound on $\tau_{\min}$ follows from \cite[Lemma 2.16]{ABerahas_FECurtis_DPRobinson_BZhou_2021} combined with \ref{lem:subgboundedrv} and the bound on $\smax$ follows from combining the bound on $\tau_{\min}$ with \eqref{eq:smaxbound}.
\eproof

\iffalse
\tred{Update 4/20 that I don't know where to put right now.}

We can also get a similar (though looser bound) for the case where we just have bounded variance!

\blemma \label{lem:boundeddiffvariance}
    For all $k \in \{0,\dots,\kmax\}$, let
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2 | \mathcal{F}_k] \leq M.
    \eequationNN
   Then,
    \bequationNN
        \Prob\left[\underset{0 \leq k \leq \kmax}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{\frac{(\kmax+1)M}{\delta}}\right] \geq 1-\delta.
    \eequationNN
\elemma

\bproof
    Let $g := \{g_0,\dots,g_{\kmax}\}$ denote any sequence of stochastic gradients that is measurable with respect to the filtration $\mathcal{F}_{\kmax}$. Then, by Markov's inequality, concavity of the square root, Jensen's inequality, and the law of total expectation,
    \begin{align*}
        &\Prob\Bigg[\underset{0 \leq k \leq \kmax}{\max} \|G_{k} - \nabla f(x_k)\|^2 > \frac{(\kmax+1)M}{\delta}\Bigg] \\
        &\leq \E\left[\underset{0 \leq k \leq \kmax}{\max} \|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(\kmax+1)M} \\
        &\leq \sum_{k=0}^{\kmax} \E\left[\|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(\kmax+1)M} \\
        &= \frac{\delta}{(\kmax+1)M} \sum_{k=0}^{\kmax} \int_{g \in \mathcal{F}_{\kmax}} \E\left[\|G_{k} - \nabla f(x_k)\|^2 | G_{0} = g_{0}, \dots, G_{k-1} = g_{k-1}\right] f_{G} dg \\
        &\leq \frac{\delta}{(\kmax+1)M} (\kmax + 1) M \int_{g \in \mathcal{F}_{\kmax}} f_{G}(g) dg = \delta,
    \end{align*}
    where $f_G(g)$ is the probability density function of the random variable $G$.
\eproof

What does this mean for our results? We can repeat the proof of Lemma \ref{lem:subgeventE} so that with probability at least $1-\delta$,
\bequationNN
    \tau_{\min} = \mathcal{O}\left(\sqrt{\frac{\delta}{\kmax+1}}\right)
\eequationNN
and, for sufficiently large $\kmax$,
\bequationNN
    \smax = \mathcal{O}\left(\log \sqrt{\frac{\kmax+1}{\delta}}\right). 
\eequationNN
Thus,
\bequationNN
    \frac{\smax}{\sqrt{\kmax+1}} = \mathcal{O} \left(\frac{\log \sqrt{\frac{\kmax+1}{\delta}}}{\sqrt{\kmax+1}} \right),
\eequationNN
which means we can always get a useful complexity result, so long as $\kmax$ is sufficently large.

Unfortunately, because the bound from Lemma \ref{lem:boundeddiffvariance} is $\mathcal{O}(\sqrt{\kmax+1})$, we cannot use this approach to directly bound $\ktaudec$ and obtain a meaningful complexity result. Thus, additional assumptions are still needed in this case.
\fi

%************
% Subsection
%************
\subsection{Complexity Result with Decreasing Ratio Parameter} \label{subsec:ratioparam}

In this section, we relax Assumption \ref{assum:eventE} with respect to the random variable $\{\Xi_k\}$ and allow it to be adaptive over the course of the algorithm. Due to the definition of $\{\Xi_k\}$, it satisfies a deterministic lower-bound, $\xi_{\min}$, such that $\xi_k \geq \xi_{\min} > 0$ holds for all $k$ \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2021}. Therefore, it follows that there exists a maximum number of decreases of $\xi$, which we denote by $r_{\max}$, that satisfies
\bequationNN
    r_{\max} \leq \min\left\{\kmax+1, \left\lceil \frac{\log(\xi_{\min}/\xi_{-1})}{\log(1-\epsilon_\xi)} \right\rceil\right\}.
\eequationNN

Now, we can state our new assumption.

\bassumption\label{assum:eventExi}
  Conditioned on the event $E_{\xi} := E(\kmax,\smax,\tau_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization we have $\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
    \item in every realization there are at most $\smax$ decreases of the merit parameter, and
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[G_k &| E_{\xi}, \Fcal_k] = \nabla f(x_k), \\
      \E[\|G_k - \nabla f(x_k)\|_2^2 &| E_{\xi}, \Fcal_k] \leq M, \\ %\text{and}\ \ 
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k = \xi_{k-1}] \leq \kappa_1, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k = \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_2, \\
      \E[\|G_k - \nabla f(x_k)\|_2 &| E_{\xi}, \Fcal_k, \nabla f(x_k)^\top(d_k - \dktrue)) < 0, \tau_k < \tau_{k-1}, \xi_k < \xi_{k-1}] \leq \kappa_3.
    \ealigned
  \eequationNN
\eassumption

This assumption is largely the same as Assumption \ref{assum:eventE}. The major new requirement due to the adaptive $\{\Xi_k\}$ sequence is the addition of two more events under which the norm difference of $\nabla f(x_k)$ and $G_k$ is bounded.

We remark that this assumption holds with high-probability under Assumption \ref{assum:symmsubgauss} (without the condition that $\xi_k = \xi_{\min}$), a result which can easily be derived by simple modification of the techniques used in Section \ref{subsec:subgauss}. We leave this derivation as an exercise for the reader.

The complexity analysis for this case follows by essentially the same arguments as those used to derive a complexity result under Assumption \ref{assum:eventE}. A slight modification of Lemma \ref{lem:innerprod} is needed to include the three events related to $\nabla f(x_k)^\top(d_k-\dktrue)$ that appear in Assumption \ref{assum:eventExi} (as opposed to the one in Assumption \ref{assum:eventE}), which yields a result in terms of the probabilities of these three events. Then, a slightly modified Lemma \ref{lem:Eksumlsmax} and the union bound can be applied two additional times to derive a complexity result. Since the analysis is a relatively straightforward extension of the results in Section \ref{subsec:complexity}, we simply state our complexity result here.
\begin{theorem}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:ptau}, and \ref{assum:eventExi} hold. Then, with probability at least $1-\delta$,
    \begin{align*}
        &\E[\|\nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c_{k^*}\| |
        E_{\xi}] \\
        &= \mathcal{O}\Bigg(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c_0\|_1 + M}{\sqrt{\kmax+1}} \\
        &\quad+ \frac{(\tau_{-1} - \tau_{\min})(\smax + \log(1/\delta)) + (\xi_{-1} - \xi_{\min})(r_{\max} + \log(1/\delta))}{\sqrt{\kmax+1}}\Bigg).
    \end{align*}
\end{theorem}

\bproof
    We leave the proof as an exercise for the reader.
\eproof

%*********
% Section
%*********
\section{Conclusion} \label{sec:conclusion}

In this work, we derived the first worst-case complexity result for an adaptive stochastic algorithm for equality constrained optimization. We developed a stochastic SQP algorithm with an adaptive $\ell$-1 merit function, based on the framework proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}. While key to a practical algorithm, the adaptivity in the merit function introduced a number of theoretical challenges to overcome. Under mostly standard assumptions, we prove that, with high probability, the expected value of the norm of the gradient of the Lagrangian decays at a rate of $k^{-4}$, matching the worst-case complexity of the projected stochastic gradient method. We believe the theoretical tools developed within may be applicable to a broad class of constrained stochastic optimization methods that utilize an adaptive merit function. 

\iffalse
OLD STUFF BELOW:

%************
% Subsection
%************
\subsection{Quick Complexity Highlight}
Quick highlight of the main complexity result for meeting on 3/9/2021:

Let $\mathcal{I} \subseteq \{0,1,\dots,\kmax\}$ denote the index set of ``good" iterations. Overall analysis will lead to a result of the form (with $\beta_k := \beta = \gamma/\sqrt{\kmax+1}$:
\begin{align*}
    &\sum_{k \in \mathcal{I}} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\quad\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &\quad+ C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau}.
\end{align*}
To get the expectation that we want, we need to add and subtract:
\begin{align*}
    &\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &+ C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + \sum_{k \in \mathcal{I}^c} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)].
\end{align*}
Then, because the number of ``bad" iterations is bounded by $\ell(\smax,\delta)/p_{\tau}$,
\begin{align*}
    &\frac{\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)]}{\sum_{k=0}^{\kmax} \beta} \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\sum_{k=0}^{\kmax} \beta} \\
    &+ \frac{C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + C_4 \ell(\smax,\delta)/p_{\tau}}{\sum_{k=0}^{\kmax} \beta}.
\end{align*}
So that,
\begin{align*}
    &\E [\Delta q(x^*, \tau^*, \nabla f(x^*), H^*, d^{*,true})] \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\sqrt{\kmax + 1}} \\
    &+ \frac{C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + C_4 \ell(\smax,\delta)/p_{\tau}}{\sqrt{\kmax+1}}.
\end{align*}

Algorithm \ref{alg:ssqp} generates a random process $\{\bar{G}_k,X_k,\bar{D}_k,\bar{\mathcal{T}}_k,\bar{\Xi}_k,\bar{\mathcal{A}}_k\}$. We will denote all random quantities by capital letters and their realizations by small letters. The random gradient estimate is denoted by $\bar{G}_k$ and its realizations by $\bar{g}_k = \bar{G}_k(\omega)$. Similarly, let the random quantities $x_k = X_k(\omega)$ (iterates), $\bar{d}_k = \bar{D}_k(\omega)$ (search directions), $\btau_k = \bar{\mathcal{T}}_k(\omega)$ (merit parameter), $\bxi_k = \bar{\Xi}_k(\omega)$ (reduction ratio), and $\bar{\alpha}_k = \bar{\mathcal{A}}_k(\omega)$ (step sizes) denote their respective realizations. We will assume that the estimates $\bar{G}_k$ obey some standard properties, conditioned on the past.

To formalize conditioning on the past, let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by the random variables $\bar{G}_0, \dotsc \bar{G}_{k-1}$. For completness, we set $\mathcal{F}_{-1} = \sigma(x_0)$. As a result, we have that $\mathcal{F}_{k}$ for $k \geq -1$ is a filtration.

Let $E_{\tau,low}$ denote the event that the merit parameter sequence eventually remains constant at a sufficiently small positive value.
We will derive our complexity result under the assumption that this event occurs.

\begin{assumption} \label{assum:taulow}
Event $E_{\tau,low}$ occurs in the sense that there exists an iteration
number $\bar{k}_{\tau,\xi} \in \mathbb{N}$ and a merit parameter value
$\btau_{\min} \in \R{}_{>0}$ such that
\begin{equation} \label{eq:taumin}
    \btau_k = \btau_{\min} \leq \btau_k^{trial} \quad and \quad
    \xi_k = \xi_{\min} \quad for \; all \quad k \geq \bar{k}_{\tau,\xi}.
\end{equation}
In addition, the sequence of random gradients $\bar{G}_k$ generated by Algorithm \ref{alg:ssqp} satisfies
\begin{equation*}
    \E_{k,\tau,small}[\bar{G}_k] = g_k \quad and \quad \E_{k,\tau,small}[\|\bar{G}_k - g_k\|^2] \leq M
\end{equation*}
where $\E_{k,\tau,small}$ denotes expectation with respect to the distribution of $\omega$ conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_{k}$.
\end{assumption}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k$, let $\Ek1$ be the event that $g_k^\top(\bd_k - d_k) \geq 0$, let $\Ek2$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} = \btau_{k-1}$, and let $\Ek3$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} < \btau_{k-1}$.

We require an additonal assumption to obtain our complexity result:
\begin{assumption} \label{assum:boundedrv}
There exists $\kappa_{\Ek3} > 0$ such that
\begin{equation} \label{eq:boundedrv}
    \E_k [\|\bar{g}_k-g_k\||\Ek3] \leq \kappa_{E_3}.
\end{equation}
\end{assumption}
The above assumption holds under a number of conditions, including when
$\bar{g}_k$ is a bounded random vector.

%NEW
\textcolor{red}{TODO:} Ignoring $\xi_k$ for now. Will probably need additional cases in the proof eventually...

\begin{lemma} \label{lem:innerprodold}
Suppose that Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|g_k\|_2\}$, the existence of which follows under \cite[Assumption 1]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\bxi_k = \bxi_{\min}$ and define
\bequationNN
\balpha_{\min,k} := \frac{\beta_k \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max,k} := \frac{\beta_k \bxi_{\min} \btau_{k-1}}{\btau_{k-1}L + \Gamma}.
\eequationNN

Then, with $\kappa_d \in \R{}_{>0}$ from Lemma 3.6 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} which satisfies
$\|\bar{d}_k-d_k\| \leq \kappa_d \|\bar{g}_k-g_k\|$,
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq  (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek1] \\
\E_{k,2} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek2] \\
\E_{k,3} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\btau_{\min}$, $\balpha_{\min,k}$, and $\balpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &= \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek1] \Prob_k[\Ek1] + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By Lemma 3.6, this means that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, by Lemma 3.6, we have
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} \balpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} \balpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{\min} \balpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{\min} \balpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}

Summing these three inequalities yields

\begin{align}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \nonumber \\
    &\leq \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+(\btau_{k-1} (\balpha_{\max,k} - \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+(2 \btau_{\min} \balpha_{\min,k} - \btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3]) \nonumber \\
    &= \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -3 \theta \beta_k^2 \btau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-(\btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2) - 2 \btau_{\min} \balpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]). \label{eq:innerprodproof1old}
\end{align}
Now, by Assumption \ref{assum:boundedrv},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|g_k\| \E_k[\|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \E_k[\|\bar{g}_k - g_k\| | \Ek3] \Prob_k[\Ek3]  \\
    &\leq \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[g_k^\top(\bd_k - d_k)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek2] \\
    &= \E_k[\|g_k\| \|\bar{d}_k - d_k\|] - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \E_k[\|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma 3.6. Using these three inequalities with
\eqref{eq:innerprodproof1old}, yields
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
which proves the result.
\end{proof}

The above result provides an upper bound in terms of the probability that the event $\Ek3$ occurs. Due to the assumed lower bound on $\btau_k$, this event can only occur a finite number of times. To obtain our final result, we need an upper bound on the summation of the probability that $\Ek3$ occurs. The first component of this upper bound comes from the Chernoff bound.

\begin{lemma} \label{lem:chernoff}
Let $Z_0, \dotsc, Z_{k}$ be independent Bernoulli random variables and let $s \in \mathbb{N}_{>0}$.
%Let
%\begin{equation} \label{eq:lsd}
%    \ell(s,\delta) := S + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 S \log(1/\delta)}.
%\end{equation}
Then, for any $\delta \in (0, 1)$,%\todo{FEC: I suggest ``Let ... random variables for any $k \in \mathbb{N}_{\geq0}$.  Then, for any $s \in \mathbb{N}_{\geq0}$ and $\delta \in (0,1)$, ....}
\begin{equation}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s\right] \leq \delta,
\end{equation}
whenever
\begin{equation} \label{eq:lsdold}
    \sum_{i=0}^{k} \Prob[Z_i = 1] \geq \ell(s,\delta) \quad where \quad \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\end{equation}
\end{lemma}

\begin{proof}
Denote $\mu = \sum_{i=0}^{k} \Prob[Z_i = 1]$.%\todo{FEC: In the general form, the definition of $\mu$ is in terms of expected value.  Maybe for clarity we should write $\mu = \sum_{i=0}^k E[Z_i] = \sum_{i=0}^k \Prob[Z_i = 1]$, where the latter is true only because we have Bernoulli random variables.} Then by Chernoff's bound, for any $\rho \in (0,1)$,
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq (1-\rho) \mu \right]
    \leq e^{-\mu \rho^2/2}.
\end{equation*}
Now, setting $\rho = 1 - s/\mu$ (which is in $(0,1)$ by (\ref{eq:lsd})), we have
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s \right]
    \leq e^{-\mu (1-s/\mu)^2/2}.
\end{equation*}
To prove the result, we need to show that%\todo{FEC: In the proof, you start with what we need, then work backwards to show what we want.  I'd prefer if we start with what we have (assumed in the statement) and prove that it gives what we want.  Does that make sense?}
\begin{equation*}
    e^{-\mu (1-s/\mu)^2/2} \leq \delta
\end{equation*}
holds. Therefore, we need
\begin{equation*}
    -\mu(1-s/\mu)^2/2 \leq \log(\delta)
\end{equation*}
to be satisfied. Rearranging this inequality, and using $\log(\delta) = -\log(1/\delta)$,%\todo{FEC: I don't see where the last equation comes from.  Did you scale it by $2\mu$?  I'm not seeing it.}
\begin{equation*}
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta) = \mu^2 - 2\mu (s+\log(1/\delta)) + s^2. 
\end{equation*}
Therefore, using the quadratic equation and taking the positive root,
\begin{align*}
    \mu &\geq s + \log(1/\delta) + \frac12\sqrt{4(s+\log(1/\delta))^2 - 4 s^2} \\
    &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)},
\end{align*}
which proves the result.
\end{proof}

Unfortunately, the events $\Ek3$ are not independent of each other so we can not directly apply Chernoff's bound. However, we can use this result in combination with an observation about the limited nature of the dependency between these events to prove the following result.

%IDEA: Rewrite lemma to prove that $K_stop <= k_{S,\delta}$ w.h.p. when $k_{s,\delta}$ exists. Gets rid of this whole J_i,stop nonsense

%This rewrite sucks, should just do it instance-wise.

%Essential components:
%   Independence when the leave one out sum is less than s.
%   Conclusion: w.h.p K_stop <= k_s,delta (or something similar).

%Crappy parts:
%   Conditioning on k_s,delta being well defined. Any better way to handle it? Yes if we do it instance wise. But then that notation is a bit frustrating
%   Top part is fine, gets rough as soon as we introduce E_s,delta.

\begin{lemma} \label{lem:depbernoulli}
For any $k \in \mathbb{N}_{\geq 0}$, let $Z_0, \dotsc, Z_{k}$ be Bernoulli random variables. Let $s \in \mathbb{N}_{>0}$.%\todo{FEC: Is it right to say that $Z_i$ is Bernoulli upfront?  Or should we be saying that, conditioned on ${\cal F}_i$, the random variable $Z_i$ is Bernoulli?  I guess technically it's Bernoulli in any case, since it's 0--1, but maybe we should say the condition since we always talk about conditional probabilities?}
For any $\hat{k} \in \{0,\dotsc,k\}$ and $i \in \{0,\dotsc,\hat{k}\}$, let $E_{\hat{k},i}$ be the event that $\sum_{j\leq \hat{k},j\neq i} Z_j < s$. We assume the following about the random variable $Z_i$ for each $i \in \{0,\dotsc,k\}$:
\begin{enumerate}
    \item $\Prob[Z_i = 1 | \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\hat{k}}]$.
    \item $\Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}^c] = 0.$
\end{enumerate}
%Let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_{k}$. %and let $\bar{G}_{i}$ be measurable with respect to $\mathcal{F}_i$ for all $i \in \{-1,\dotsc,\hat{k}-1\}$.
Let $\delta \in (0,1)$ and let $\ell(s,\delta)$ be defined as in (\ref{eq:lsd}). Let $K_{s,\delta}$ be the random variable such that, for any realization of $\bar{G}_0,\dotsc,\bar{G}_{k-1}$ that is measurable with respect to $\mathcal{F}_k$,
\bequationNN
    k_{s,\delta} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta) \right\},
\eequationNN
($k_{s,\delta} = \infty$ for any realization such that $\sum_{i=0}^k \Prob[Z_i=1|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta)$ does not occur).
In addition, let $K_{stop}$ be the random variable
\bequationNN
K_{stop} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} Z_i = s\right\},
\eequationNN
($k_{stop} = \infty$ for any realization of $Z$ such that $\sum_{i=0}^{k} z_i < s$).

We define two events:%\todo{FEC: How do these events depend on $k$?  Should we take it that $k$ is ``fixed'' in some sense, but we are considering the events for any $s$?  But shouldn't we be proving the result ``for any $k$'' as well, in which case the events should depend on $k$, too?}
\begin{enumerate}
    \item Let $E_{k,s,\delta}$ be the event that 
    $\sum_{i=0}^k \Prob[Z_i=1|\mathcal{F}_i] \geq \ell(s,\delta)$.
    \item Let $E_{k,s,\delta,stop}$ be the event that $K_{stop} > K_{s,\delta}$.
\end{enumerate}
Then,
\begin{equation*}
    \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
\end{equation*}
%We assume the following:
%\begin{enumerate}
%    \item For any $i \in \{0,\dotsc,\hat{k}\}$, let $J_{i,stop}$ be the event that $i > K_{stop}$ and  
%    \bequationNN
%    \Prob[(Z_i = 1) \cap J_{i,stop} | \mathcal{F}_i] = 0.
%    \eequationNN
%    (high level idea: once a realization of $Z$ has $s$ successes, the probability of $Z_i = 1$ is $0$.)
    %and thus $\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] = \sum_{i=0}^{K_{stop}} \Prob[Z_i = 1 | \mathcal{F}_i]$.
%the minimum integer such that $\sum_{i=0}^{k_{stop}} Z_i = s$ (set $k_{stop} = \infty$ if $\sum_{i=0}^{\hat{k}} Z_i < s$). Let $Y_i = 0$ for all $i > k_{stop}$.
%    \item For any $\bar{k} \in \{0,\dotsc,\hat{k}\}$, let $J_{\bar{k},i}$ be the event that $\sum_{j\leq \bar{k},j\neq i} Z_j < s$. Then, $\Prob[Z_i = 1| \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, J_{\bar{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\bar{k}}]$. (high level idea: if the summation leaving out $Z_i$ does not equal $s$, then $Z_i$ is independent of all other $Z_j$.)
%\end{enumerate}

%$\Prob[Z_i = 1|\nu_i] = \Prob[Z_i = 1|\nu_i, Z_0, %\dotsc, Z_{i-1}$.
%let $\Prob[Z_i=1|\nu_i] = \Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}]$ hold unless $\sum_{j=0}^{\bar{k}} Z_j = s$ in which case $\Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}] = 0$ holds for any $i$ such that $\sum_{j\leq \bar{k}, j\neq i} Z_j = s$.
%Then, for any $\delta \in (0,1)$,
%\begin{equation}
%    \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \geq 1 - \delta,
%\end{equation}
%where $\ell(s,\delta)$ is defined in (\ref{eq:lsd}).
\end{lemma}

\begin{proof}
    %We work with any fixed sequence $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ satisfying these conditions.
    %Note that by the definition of our filtration, it should be clear that $\Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{k-1}] = \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]$ for any $i \in \{0,\dotsc,k\}$.
    
    %We begin the proof by showing that
    %\begin{equation*}
    %    \Prob\left[ \right] \geq 1 - \delta,
    %\end{equation*}
    %holds for any fixed $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$. To prove this, we assume that $\sum_{i=0}^{\hat{k}} \Prob[Z_i| \bar{g_0}, \dotsc, \bar{g}_{i-1}] \geq \ell(s,\delta)$ (as the result is trivial otherwise).
    
    Let $E_{k,s,\delta}$ and $E_{k,s,\delta,stop}$ both occur. Then, since $E_{k,s,\delta}$ occurs, $k_{s,\delta}$ is finite. In addition, because $E_{k,s,\delta,stop}$ occurs,
    we have that
    \bequationNN
        \sum_{i=0}^{k_{s,\delta}} z_i < s.
    \eequationNN
    Therefore, for all $i \in \{0,\dotsc,k_{s,\delta}\}$, $E_{k_{s,\delta},i}$ occurs. Thus, for all $i,j \in \{0,\dotsc,k_{s,\delta}\}$, $Z_i$ and $Z_j$ were mutually independent.
    
    Due to the independence $Z$ in this case, by Lemma \ref{lem:chernoff},
    \bequationNN
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s\right] \leq \delta,
    \eequationNN
    and thus,
    \bequationNN
        \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
    \eequationNN
    
    Now, let $\hat{Z}_0, \dotsc, \hat{Z}_{k}$ be independent Bernoulli random variables such that $\Prob[\hat{Z}_i = 1] = \Prob[Z_i = 1|\mathcal{F}_i]$ for all $i=0,\dotsc,k$. Let $E$ be the event that $\sum_{i=0}^{k_{s,\delta}} Z_i < s$ and let $E_{k,s,\delta}$ occur. Now, for each $i=0,\dotsc,k_{s,\delta}$, it follows that if event $E$ occurs, $E_{k_{s,\delta},i}$ must occur as well, so $Z_i$ is independent of $Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{k_{s,\delta}}$ conditioned on the event $E$. Thus, whenever $E$ occurs, $Z_0,\dotsc,Z_{k_{s,\delta}}$ are identical in distribution to $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s,\delta}}$. Therefore, by Lemma \ref{lem:chernoff},
    \begin{equation}
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = \Prob\left[\sum_{i=0}^{k_{s,\delta}} \hat{Z}_i < s\right] \leq
        \delta.
    \end{equation}
    It follows that
    \begin{equation*}
           \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i \geq s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = 1 -    \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] \geq 1 - \delta,
    \end{equation*}
    and thus
    \begin{equation*}
        \Prob[k_{stop} \leq k_{S,\delta}] \geq 1 - \delta.
    \end{equation*}
    In addition, by the definition of $k_{stop}$ and $J_{i,stop}$, with probability at least $1-\delta$,
    \begin{align*}
        \sum_{i=0}^{\hat{k}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}]
        &= \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq \sum_{i=0}^{k_{S,\delta}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq 1 + \ell(s,\delta),
    \end{align*}
    and thus,
    \begin{equation*}
        \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1|\bar{g}_0, \dotsc, \bar{g}_{i-1}] \leq 1 + \ell(s,\delta) \right] \geq 1 - \delta.
    \end{equation*}
    Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_{\hat{k}}} \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{\hat{k}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\hat{k}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\hat{k}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
\end{proof}

This setup applies to $\Ek3$ under Assumption \ref{assum:taulow} due to the definitions of $\btau$ and $\btau_{\min}$. In particular, at each iteration where $\Ek3$ occurs, $\btau_{k} \leq (1-\varepsilon)\btau_{k-1}$ holds. Therefore, if we perform this process $s$ times, until
\begin{equation*}
    \btau_{\min} \geq (1-\varepsilon)^s \btau_{-1},
\end{equation*}
it follows that $\Ek3$ cannot occur again by Assumption \ref{assum:taulow}. Thus, solving this inequality for $s$, we have
\bequation \label{eq:Stmin}
    s_{\btau_{\min}} := \left\lceil\frac{\log(\btau_{\min}/\tau_{-1})}{\log(1-\varepsilon)}\right\rceil
\eequation
which is the maximum number of times $\Ek3$ can occur.

Now we can show how to apply the above lemma to $\Ek3$.

\begin{lemma}
    Let Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\beta_j = \beta$, $L_j = L$, and $\Gamma_j = \Gamma$ for all $j=0,\dotsc, k$. Let 
    \bequationNN
        \balpha_{\min} := \frac{\beta \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max} := \frac{\beta \bxi_{\min} \btau_{-1}}{\btau_{-1}L + \Gamma}.
    \eequationNN
    Let $\delta \in (0,1)$. Then, with probability at least $1-\delta$,
    \begin{align}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top (\bar{d}_j-d_j)]
        &\leq (\btau_{-1} (\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3}(1 + \ell(s_{\btau_{\min}},\delta))\\
    &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}, \nonumber
    \end{align}
    where
    \bequationNN
        \ell(s_{\btau_{\min}},\delta) := s_{\btau_{\min}} + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s_{\btau_{\min}} \log(1/\delta)}.
    \eequationNN
\end{lemma}

\begin{proof}
    By Lemma \ref{lem:innerprod},
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq \sum_{j=0}^k (\btau_{j-1}(\balpha_{\max,j} + \theta \beta_j^2) - \btau_{\min} \balpha_{\min,j}) \kappa_g \kappa_d \kappa_{E_3} \Prob_j[E_{j,3}]\\
        &\quad+ \theta \beta_j^2 \btau_{j-1} \kappa_g \kappa_d \sqrt{M}.
    \end{align*}
    Using our assumption on $\beta$, $L$, and $\Gamma$, we can upper bound this inequality as
    \begin{align} \label{eq:ipproof1}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} \sum_{j=0}^k \Prob_j[E_{j,3}]\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}. \nonumber
    \end{align}
   
    To show the final result, we need to apply Lemma \ref{lem:depbernoulli}. To do this, let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_k$ and for all $i=0,\dotsc,k$, let $Z_i = 1$ if $E_{i,3}$ occurs and let $Z_i = 0$ otherwise. Recall that $\Prob_i[\cdot]$ is conditioned on the event $E_{\tau,low}$ occurring as well as the filtration $\mathcal{F}_i$.
    
    Now, let $s = s_{\btau_{\min}}$, so that $s$ is the maximum number of iterations in which $\Ek3$ can occur by Assumption \ref{assum:taulow}. Then, it is easy to verify that by the definition of our filtration, the probability that $\Ek3$ occurs is independent of the $E_{i,3}$ for all other $i$, whenever $\Ek3$ can occur without contradicting Assumption \ref{assum:taulow}. This holds whenever $E_{\hat{k},i}$ occurs, so that the first property of $Z_i$ in Lemma \ref{lem:depbernoulli} holds. On the other hand, when $E_{\hat{k},i}^c$ occurs it is clear that if $\Ek3$ occurs as well that Assumption \ref{assum:taulow} must be contradicted. Thus, second property of $Z_i$ in Lemma \ref{lem:depbernoulli} is satisfied as well.
    
    Now, presume that $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s_{\btau_{\min}},\delta)$. Then, by Lemma \ref{lem:depbernoulli},
    \bequationNN
        \Prob[K_{stop} \leq k_{s_{\btau_{\min}},\delta}] \geq 1 - \delta.
    \eequationNN
    In addition, by the definition of $s_{\btau_{\min}}$ and $K_{stop}$, it follows that whenever $K_{stop}$ is finite,
    \bequationNN
        \sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] =
        \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}].
    \eequationNN
    Thus, with probability at least $1 - \delta$,
     \bequationNN
        \sum_{i=0}^{k} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq \sum_{i=0}^{k_{s_{\btau_{\min}}}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]
        \leq 1 + \ell(s_{\btau_{\min}},\delta).
    \eequationNN
    
    On the other hand, if $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] < \ell(s_{\btau_{\min}},\delta)$, it is clear that $\sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq 1 + \ell(s_{\btau_{\min}},\delta)$. Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_k} \Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_k} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
    
    Combining this with (\ref{eq:ipproof1}),
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} (1 + \ell(s_{\btau_{\min}},\delta))\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M},
    \end{align*}
    holds with probability at least $1-\delta$.
\end{proof}

\begin{theorem}
Suppose that Assumption 4 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} holds. Define 
\bequationNN
\bar{A}_{\min} := \frac{\bar{\xi}_{\min} \bar{\tau}_{\min}}{\tau_{-1}L + \gamma} \mbox{ and }
\bar{A}_{\max} := \frac{\xi_{-1} \tau_{-1}}{\bar{\tau}_{\min}L + \gamma}
\eequationNN
as well as
\bequationNN
\bar{M} := \tau_{-1} \left(\frac12 (\bar{A}_{\max} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{K+1}}
\eequationNN
for some
\bequationNN
\gamma \leq \min\left\{\frac{\bar{A}_{\min}}{\bar{A}_{\max} + \theta},
\frac{1}{\bar{A}_{\min}}\right\}.
\eequationNN
Then,
\begin{equation}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + c_0 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation}
\end{theorem}

\begin{proof}
Let
\bequationNN
\bar{A}_k = \frac{\bar{\xi}_{k} \bar{\tau}_{k}}{\bar{\tau_{k}}L + \gamma} \mbox{ and }
\bar{M}_k = \bar{\tau}_{k} \left(\frac12 (\bar{A}_{k} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
It follows that $\bar{A}_k \beta \leq \bar{\alpha}_k \leq (\bar{A}_k + \theta)\beta$. Using  Lemmas 3.2(d), 3.5, 3.8, and 3.9 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} (with the replacement of $\bar{\tau}_{\min}$ by $\bar{\tau}_k$), we have
\begin{align*}
    &\E_k[\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\leq \E_k [-\bar{\alpha}_k \Delta q(x_k, \bar{\tau_k}, g_k, H_k, d_k) + \frac12 \bar{\alpha}_k \beta \Delta q(x_k, \bar{\tau_k}, \bar{g}_k, H_k, \bar{d}_k) + \bar{\alpha}_k \bar{\tau}_k g_k^\top (\bar{d}_k - d_k)] \\
    &\leq -\beta(\bar{A}_k - \frac12(\bar{A}_k + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}_k \\
    &\leq -\beta(\bar{A}_{\min} - \frac12(\bar{A}_{\max} + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M} \\
    &\leq -\frac12 \beta \bar{A}_{\min} \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}
\end{align*}
Summing this inequality from $0$ to $K$,
\begin{align}
&\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \nonumber \\ 
&\leq -\frac12 \bar{A}_{\min} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)] + (K+1) \beta^2 \bar{M}. \label{eq:stochasticproof1old}
\end{align}
Now, we work with the left hand side of this inequality,
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k f(x_k + \bar{\alpha}_k \bar{d}_k) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k f_k + c_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k (f(x_k + \bar{\alpha}_k \bar{d}_k) - f_{\min}) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k].
\end{align*}
Now, conditioned on the algorithm reaching $x_k$, it follows by the monotonicity of $\tau$
that
\bequationNN
-\E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k] \geq - \E_k[\bar{\tau}_{k-1} (f_k - f_{\min}) + c_k].
\eequationNN
Therefore, summing this inequality yields
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\geq \E_K [\bar{\tau}_K (f_{K+1} - f_{\min}) + \|c_K\|_1] - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1.
\end{align*}
Using this lower bound with \eqref{eq:stochasticproof1old}
\begin{equation*}
    \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min}}.
\end{equation*}
Dividing both sides by the summation of $\beta$,
\begin{equation*}
    \frac{1}{\sum_{k=0}^K \beta} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Now, by the definition of $x_{k^*}$, the left hand side is simply
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Using the definition of $\beta$, this becomes
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation*}
\end{proof}

\newpage
\appendix

%*********
% Section
%*********
\section{FEC Notes}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)\},
\eequationNN
where
\bitemize
  \item $\Xbar_k$ is the algorithm iterate in iteration $k$,
  \item $\Gbar_k$ is the stochastic gradient in iteration $k$,
  \item $\Dbar_k$ is the search direction in iteration $k$,
  \item $\overline\Tcal_k$ is the merit parameter in iteration $k$,
  \item $\Sbar_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\overline\Xi_k$ is the ratio parameter in iteration $k$, and
  \item $\overline\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)$ is denoted as
\bequationNN
  (\xbar_k,\gbar_k,\dbar_k,\bar\tau_k,\sbar_k,\bar\xi_k,\bar\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{\Gbar_0,\dots,\Gbar_{k-1}\}$, the realization of which (along with $\Xbar_0 = x_0$) determines the realization of
\bequationNN
  \{\Xbar_j\}_{j=1}^k\ \ \text{and}\ \ \{(\Dbar_j,\overline\Tcal_j,\Sbar_j,\overline\Xi_j,\overline\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

Let us consider a conditional model under the following assumption.
We introduce the following assumption.

\newpage

\bassumption\label{ass:FEC}
  Conditioned on the event $E := E(\kmax,\smax,\tau_{\min},\xi_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization there are at most $\smax$ decreases of the merit parameter,
    \item in every realization we have $\bar\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$, and
    \item in every realization we have $\bar\xi_k = \bar\xi_{-1} = \bar\xi_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[\Gbar_k &| E, \Fcal_k] = \nabla f(\xbar_k), \\
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ \text{and}\ \ 
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2 &| E, \Fcal_k, \nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0, \bar\tau_k < \bar\tau_{k-1}] \leq \kappa,
    \ealigned
  \eequationNN
  where $d(\xbar_k,\nabla f(\xbar_k))$ is the step that would be computed at an iterate $\xbar_k$ if the true gradient $\nabla f(\xbar_k)$ were used in the search direction computation.
\eassumption

Going forward, let us define the binary random variable
\bequation %\label{eq:zkdef}
  Z_k = \bcases 1 & \text{if $\nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0$ and $\bar\tau_k < \bar\tau_{k-1}$} \\ 0 & \text{otherwise.} \ecases
\eequation
Due to the definition of the event $E$, direct consequences of Assumption~\ref{ass:FEC} are
\bequation\label{eq:probz0}
  \baligned
    \P[Z_k = 1 &| E, \Fcal_k, \Sbar_{k-1} = \smax] = 0 \\ \text{and}\ \ 
    \P[Z_k = 1 &| E, \Fcal_k, \Tbar_{k-1}(1 - \epsilon_\tau) < \tau_{\min}] = 0.
  \ealigned
\eequation

\bequationNN
  \P[Z_j = 1 | E, \Fcal_k, \Sbar_{k-1} < \smax, \Tbar_{k-1}(1 - \epsilon_\tau) \geq \tau_{\min}]\ \ \text{for $j \in \{k,\dots,\kmax\}$}
\eequationNN

Our overall goal is to prove an upper bound (in high probability) on
\bequationNN
  \sum_{k=0}^{\kmax} p_k,\ \ \text{where}\ \ p_k := \P[Z_k = 1 | E, \Fcal_k].
\eequationNN
%From total probability and \eqref{temp}:
%\bequationNN
%  \baligned
%    \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k]
%    &= \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{\kmax} < \smax] \cdot \P[\Sbar_{\kmax} < \smax | E, \Fcal_k] \\
%    &+ \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{\kmax} = \smax] \cdot \P[\Sbar_{\kmax} = \smax | E, \Fcal_k]
%  \ealigned
%\eequationNN

As a first step, we prove the following.

\blemma\label{lem:chernoff_new}
  For any $k \in \N{}$, let $\{Y_0,\dots,Y_k\}$ be independent Bernoulli random variables.  Then, for any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, it follows that
  \bequationNN
    \mu := \sum_{j=0}^k \P[Y_j = 1] \geq \ell(s,\delta)\ \ \implies\ \ \P\left[\sum_{j=0}^k Y_j \leq s\right] \leq \delta,
  \eequationNN
  where
  \bequation\label{eq:lsd_new}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
  \eequation
\elemma
\bproof
  By the multiplicative form of Chernoff's bound, it follows for $\rho := 1 - s/\mu$ (which is in the interval $(0,1)$ by (\ref{eq:lsd_new})) that
  \bequationNN
    \P\left[\sum_{j=0}^{k} Y_j \leq s \right] \leq e^{-\frac{\mu \rho^2}{2}} = e^{-\frac{\mu (1-s/\mu)^2}{2}}.
  \eequationNN
  Hence, to prove the result, all that remains is to show that $e^{-\frac{\mu (1-s/\mu)^2}{2}} \leq \delta$, i.e.,
  \bequationNN
    -\frac{\mu(1-s/\mu)^2}{2} \leq \log(\delta)
  \eequationNN
  Using $\log(\delta) = -\log(1/\delta)$, this inequality is equivalent to
  \bequationNN
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta),
  \eequationNN
  which holds if and only if $\mu^2 - 2\mu (s+\log(1/\delta)) + s^2 \geq 0$.  Viewing the left-hand side of this inequality as a convex quadratic function in $\mu$, one finds that the inequality holds as long as $\mu$ is greater than or equal to the positive root of the quadratic, i.e.,
  \bequationNN
    \baligned
      \mu
        &\geq s + \log(1/\delta) + \sqrt{(s+\log(1/\delta))^2 - s^2} \\
        &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2s\log(1/\delta)}.
    \ealigned
  \eequationNN
  Since this holds under assumption in the lemma, the result is proved.
\eproof

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tauktri$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ and $\xi_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tauktri$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tauktri$ occurs, we introduce the following assumption.

\begin{assumption} %\label{assum:ptau}
At every iteration $k$,
\bequation
    \Prob[\bar{g}_k^\top \bar{d}_k + \max\{\bar{d}_k^\top H_k \bar{d}_k,0\} \geq g_k^\top d_k + \max\{d_k^\top H_k d_k,0\} | E, \mathcal{F}_k] \geq p_{\tau}.
\eequation
\end{assumption}
This assumption is satisfied with $p_{\tau}$ when $\bar{g}_k$ is drawn from a Gaussian distrbution \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

This assumption is leads to the following lemma.

\blemma \label{lem:Etautrial_old}
    Let Assumptions \ref{ass:FEC} and \ref{assum:ptau} hold. Let $E_{\tauktri}$ be the event that $\tauktri < \bar{\tau}_{k-1}$. Then,
    \bequation
        \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, E_{\tauktri}] \geq p_{\tau}.
    \eequation
\elemma

\bproof
    TODO: Copy proof from my notes.
\eproof

Due to the above lemma and Assumption \ref{ass:FEC}, it follows that
\bequationNN
    \Prob[E_{\tauktri} | \mathcal{F}_k, E, \bar{S}_{k-1} = \smax] = 0.
\eequationNN
In addition, by the definition of $\bar{\tau}_k$,
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, E_{\tau_{k}^{trial}}^c] = 0,
\eequationNN
so 
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, \bar{S}_{k-1} = \smax] = 0.
\eequationNN

Now, by Lemma \ref{lem:Etautrial} and the fact that $E_{\tau_{k}^{trial}}$ is not dependent on $\bar{g}_k$, it follows that
\bequation \label{eq:Etrialtaudec_old}
    \Prob[E_{\tau_{k}^{trial}} | \mathcal{F}_k, E, \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E] < p_{\tau}] = 0.
\eequation

Idea from here: Let $\bar{P}_k = \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, \bar{S}_{k-1} < \smax]$ and let $Z_k$ be the indicator of the event that $\bar{\tau}_k < \bar{\tau}_{k-1}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{\kmax} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{\kmax + 1}} \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{\kmax + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}

Then, by \eqref{eq:Etrialtaudec}, with probability $1-\delta$, the number of occurrences of $E_{\tau_{k}^{trial}}$ is bounded by
\bequationNN
    |E_{\tau_{k}^{trial}}| \leq \left\lceil\frac{ \ell(\smax,\delta) + 1 }{p_{\tau}}\right\rceil.
\eequationNN
Thus, by the definition of $\bar{\tau}_k$, it follows that
\bequationNN
    |\tauktri < \bar{\tau}_k|\leq \left\lceil\frac{ \ell(\smax,\delta) + 1 }{p_{\tau}}\right\rceil. 
\eequationNN

\newpage

%*********
% Section
%*********
\section{Mike's Simpler Problem} \label{app:simple}

Let $Y_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:simple1}
  \baligned
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i < \smax\right] &= p_k \\ \text{and}\ \ 
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \geq \smax\right] &= 0
  \ealigned
\eequation
for some $\smax \in \{1,\dotsc,\kmax\}$, where $p_k \in [0,1]$ for all $k \in \{0,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$
\bequation \label{eq:simple2}
    \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Y_k = \smax \right].
\eequation

The following lemma proves \eqref{eq:simple2}.
\begin{lemma} \label{lem:simple1}
    Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
    \bequationNN
      \baligned
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax\right] &= p_k \\ \text{and}\ \ 
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq \smax\right] &= 0,
      \ealigned
    \eequationNN
    for some $\smax \in \{1,\dotsc,\kmax\}$, where $p_k \in (0,1]$ for all $k \in \{0,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k = \smax$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} p_k + \sum_{k=j}^{\kmax} 0 = \sum_{k=0}^{j-1} p_k.
    \end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \\
        &= \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
    \end{align*}
    which completes the proof.
\end{proof}

The left side of this equation is similar to our goal for the actual problem, while the right is potentially easier to work with. 
A good starting point would be to try to prove a bound on
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = \smax \right]
\eequationNN
for any $\ell \in \{\smax-1,\dotsc,\kmax\}$.

It clearly follows that
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = \smax \right] = 1 -  \Prob\left[\sum_{k=0}^{\ell} Y_k < \smax \right].
\eequationNN
We can find a lower bound on the right hand side of this equation using the following lemma.
\begin{lemma} \label{lem:simple2}
    Let $\ell \in \{\smax-1,\dotsc,\kmax\}$ and let $\hat{Y}_0,\dotsc,\hat{Y}_{\ell}$ be independent \\Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then,
    \bequationNN
        \Prob\left[\sum_{k=0}^{\ell} Y_k < \smax \right] = \Prob\left[\sum_{k=0}^{\ell} \hat{Y}_k < \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    For all $k \in \{0,\dotsc,\ell\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,\ell\}$, let
    \bequationNN 
        \bar{y}_k := \bcases
        1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < \smax \\
        0 & \textrm{otherwise},
        \ecases
    \eequationNN
    and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    \begin{align*}
        \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < \smax\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq \smax\right] &= 0
    \end{align*}
    
    Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ are equivalent in distribution to $Y_0, \dotsc, Y_{\ell}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{\ell} \hat{Y}_k < \smax$ occurs if and only if the event $\sum_{k=0}^{\ell} \bar{Y}_k < \smax$ occurs as well. Thus,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\ell} \hat{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{\ell} \bar{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{\ell} Y_k < \smax\right],
    \eequationNN
    where the last equality holds because 
    $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ and $Y_0, \dotsc, Y_{\ell}$ are equivalent in distribution.
\end{proof}

We can use these lemmas as well as Lemma \ref{lem:chernoff_new} to get our desired bound in high probability.

\begin{lemma} \label{lem:simple3}
    Let $\smax \in \{1,\dotsc,\kmax\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,\kmax\}$, let $Y_k$ be Bernoulli random variables which satisfy \eqref{eq:simple1}, where $p_k \in (0,1]$. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{\kmax} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(\smax,\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(\smax,\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $\sum_{k=0}^{\kmax} p_k \leq \ell(\smax,\delta) + 1$. Then, by the definition of $Y_k$, it is clear that
    \bequationNN
        \sum_{k=0}^{\kmax} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(\smax,\delta) + 1
    \eequationNN
    holds deterministically, so the result is trivial in this case. Thus, for the remainder of the proof, we assume that $\sum_{k=0}^{\kmax} p_k > \ell(\smax,\delta) + 1$.
    
    Now, let $k_{\smax,\delta}$ be the minimum integer such that
    \bequationNN
        \sum_{k=0}^{k_{\smax,\delta}} p_k \geq \ell(\smax,\delta).
    \eequationNN
    Let $\hat{Y}_0,\dotsc,\hat{Y}_{k_{\smax,\delta}}$ be independent Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then, by Lemma \ref{lem:simple2} and Lemma \ref{lem:chernoff_new},
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax\right] = \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k < \smax\right] \leq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k \leq \smax\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{\smax,\delta}} p_k \right] &\geq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k = \smax \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{\smax,\delta}} p_k \leq \ell(\smax,\delta) + 1$.
\end{proof}

%Since the $\hat{Y}_k$ variables are independent, we can use this lemma and the CDF of the binomial distribution to get an exact description of the summation of interest. Alternatively, we can derive a bound for it by using a tail bound, such as Hoeffding's inequality or Chernoff's bound. The second option is likely to be more relevant in the more general setting of our actual algorithm.

What I'd hope a final result to look like:
\bequationNN
    \Prob\left[\sum_{k=0}^{\kmax} \Prob\Big[Z_k = 1 \Big| \mathcal{F}_{k}\Big] \leq \ell(\smax,\delta)\right] \geq 1 -\delta.
\eequationNN

Update: 2/8/2021

Let $\bar{P}_k = \Prob[Z_k=1| E, \mathcal{F}_k, \bar{S}_{k-1} < \smax]$ and let $\bar{p}_k \in [0,1]$ for all \\$k \in \{0,\dotsc,\kmax\}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$ such that $\Prob\left[\left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\right] \neq 0$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{\kmax} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{\kmax + 1}} \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{\kmax + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}


Old idea:

If
\bequation \label{eq:simple3}
    \Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | E, \left\{\bar{G}_0,\dotsc,\bar{G}_{\kmax-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\kmax-1}\right\}\right] \geq 1-\delta
\eequation
holds for any $\bar{g}_0,\dotsc,\bar{g}_{\kmax}$, then we are done because:
\begin{align*}
    &\Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i = 1| \mathcal{F}_i] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{g} \in \mathcal{F}_{\kmax}} \Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | \left\{\bar{G}_0,\dotsc,\bar{G}_{\kmax-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\kmax-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
    &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\kmax}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta).
\end{align*}
Unfortunately, when conditioning on a realization from the filtration, we fix both the probabilities as well as whether the events occurred. Thus, the probabilities on the left side of \eqref{eq:simple3} is always 0 or 1.

%*********
% Section
%*********
\section{A Different Problem}

Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:different1}
  \begin{split}
    &\Prob\Bigg[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0,\dotsc,Z_{k-1}\Bigg] \in [0,1] \\ \text{and}\ \
    &\Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq \smax\right] = 0
  \end{split}
\eequation
for some $\smax \in \{1,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$
\bequation \label{eq:different2}
    \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
\eequation
We prove this inequality in the following lemma.

\begin{lemma} \label{lem:different1}
    Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy \eqref{eq:different1}, for some $\smax \in \{1,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k \geq \smax$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] + \sum_{k=j}^{\kmax} 0 \\
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right].
    \end{align*}
    
    %Now, letting $E_j^c$ denote the complement of $E_j$, the definition of $Z_k$ yields
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c \right] = \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \textrm{ for all $k \leq j$.}
    %\eequationNN
    %Thus,
    %\begin{align*}
    %    \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right]
    %    &\geq \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right] \\
    %    &= \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right].
    %\end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \right] \\
        &= \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
\end{align*}
which completes the proof.
\end{proof}

Next, we would like to derive an analog to Lemma \ref{lem:simple2}.
\begin{lemma} \label{lem:different2}
    Let $p \in \{\smax-1,\dotsc,\kmax\}$. Then, there exist independent Bernoulli random variables $\hat{Z}_0, \dotsc, \hat{Z}_p$ which satisfy
    \begin{align*}
        &\Prob\left[\sum_{k=0}^{p} Z_k < \smax \right] = \Prob\left[\sum_{k=0}^{p} \hat{Z}_k < \smax \right] \\
        \textrm{and } &\sum_{k=0}^p \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] = \sum_{k=0}^p \Prob\left[ \hat{Z}_k = 1\right].
    \end{align*}
\end{lemma}

\begin{proof}
    General idea: For any sequence of $\Prob\left[Z_k = 1 \Big| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right]$, there exists a fixed sequence of independent random variables that could generate this sequence in the same way that $\bar{Y}_k$ was generated in Lemma \ref{lem:simple2}. If we can get to that point, believe we can verbatim copy the rest of the proof.
    
    %To begin, note that for all $Z_0,\dotsc,Z_{\kmax}$ satisfying \eqref{eq:different1}, there exists a set of independent Bernoulli random variables 
    %$\hat{Z}_0, \dotsc, \hat{Z}_p$ such that
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right].
    %\eequationNN

    %For all $k \in \{0,\dotsc,p\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,p\}$, let
    %\bequationNN 
    %    \bar{y}_k := \bcases
    %    1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < \smax \\
    %    0 & \textrm{otherwise},
    %    \ecases
    %\eequationNN
    %and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    %and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    %\begin{align*}
    %    \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < \smax\right] &= p_k \\
    %    \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq \smax\right] &= 0
    %\end{align*}
    
    %Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{p}$ are equivalent in distribution to $Y_0, \dotsc, Y_{p}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{p} \hat{Y}_k < \smax$ occurs if and only if the event $\sum_{k=0}^{p} \bar{Y}_k < \smax$ occurs as well. Thus,
    %\bequationNN
    %    \Prob\left[ \sum_{k=0}^{p} \hat{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{p} \bar{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{p} Y_k < \smax\right],
    %\eequationNN
    %where the last equality holds because 
    %$\bar{Y}_0, \dotsc, \bar{Y}_{p}$ and $Y_0, \dotsc, Y_{p}$ are equivalent in distribution.
\end{proof}

\begin{lemma}
    Let $\smax \in \{1,\dotsc,\kmax\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,\kmax\}$, let $Z_k$ be Bernoulli random variables which satisfy \eqref{eq:different1}. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{\kmax} \Prob \left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1} \right] \leq \ell(\smax,\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(\smax,\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $E$ be the event that 
    \bequationNN
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}\right] > \ell(\smax,\delta).
    \eequationNN
    
    Then, let $K_{\smax,\delta}$ be the random variable whose realization $k_{\smax,\delta}$ is the minimum integer that satisfies
    \bequationNN
        \sum_{k=0}^{k_{\smax,\delta}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}, E\right] \geq \ell(\smax,\delta).
    \eequationNN

    Now, for any $Z_0,\dotsc, Z_p$ which satisfies \eqref{eq:different1} and $E$, there exist independent Bernoulli random variables $\hat{Z}_0,\dotsc,\hat{Z}_{k_{\smax},\delta}$ such that
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, E, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right] \textrm{ for all } k \in \{0,\dotsc,k_{\smax,\delta}\}.
    \eequationNN

    Then, let $\bar{Z}_0,\dotsc,\bar{Z}_{k_{\smax,\delta}}$ be Bernoulli random variables such that
    \begin{align*}
        \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i < \smax\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i \geq \smax\right] &= 0
    \end{align*}
    
    
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax\right] = \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k < \smax\right] \leq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k \leq \smax\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{\smax,\delta}} p_k \right] &= \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k = \smax \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{\smax,\delta}} p_k \leq \ell(\smax,\delta) + 1$.
\end{proof}


%DETERMINISTIC ANALYSIS BELOW
Given an objective function $f : \R{n} \rightarrow \R{}$ and a
constraint function $c : \R{n} \rightarrow \R{m}$, consider the optimization problem
\begin{equation} \label{eq:fdef}
    \underset{x \in \R{n}}{\min} \enspace f(x) \; \mbox{ s.t. } c(x)=0.
\end{equation}
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) = f(x) + c(x)^\top y$, the first-order stationarity conditions
for \eqref{eq:fdef} are given by
\begin{equation} \label{eq:1on}
    0 = \left[
    \begin{matrix}
    \nabla_x \ell(x,y) \\ \nabla_y \ell(x,y)
    \end{matrix}
    \right]
    = \left[
    \begin{matrix}
    \nabla f(x) + J(x)^T y \\ c(x)
    \end{matrix}
    \right].
\end{equation}
Letting $f_k := f(x_k)$, $g_k := \nabla f(x_k)$, $c_k := c(x_k)$, and $J_k := J(x_k) := \nabla c(x_k)^\top$ for all $k \in \mathbb{N}$ and given a sequence $\{H_k\}$ satisfying a standard type of sufficiency condition for equality constrained optimization, the SQP subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}
The optimal solution $d_k$ of this subproblem, and an associated Lagrange multiplier $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}
At each iteration, the algorithm uses a merit function with the $\ell_1$-norm penalty function $\phi : \R{n} \times \R{}_+ \rightarrow \R{}$ defined by
\begin{equation} \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1
\end{equation}
where $\tau \in \R{}_+$ is a merit parameter that is updated at each iteration of the algorithm. We use a local model of the merit function $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + J(x) d\|_1.
\end{equation}
A useful quantity is the reduction in is model for a given $d \in \R{n}$ with $c(x) + J(x) d = 0$, i.e., $\delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}

For the purposes of this note, we will declare $x_k$ an approximate solution of (\ref{eq:fdef}) when
\begin{equation} \label{eq:eps1on}
    \|g_k + J_k^\top y_k\| \leq \varepsilon  \quad \mbox{ and } \quad \|c_k\| \leq \varepsilon,
\end{equation}
both hold for some $k \in \mathbb{N}$. We will derive a worst-case complexity result
in terms of the maximum number of iterations required to find a point statisfying \eqref{eq:eps1on}. We refer the reader to \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the
full definition of the algorithms. To prove our complexity result, we will use the following results which were proven in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}:
\begin{itemize}
    \item The merit parameter $\tau_k$ has an upper and lower bound given by $\tau_{-1} \geq \tau_k \geq \tau_{\min}$ (Lemma 2.14).
    \item The stepsize $\alpha_k$ is lower bounded by $\alpha_{\min}$ (Lemma 2.15).
    \item Let $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$ for all $k \in \mathbb{N}$. Then, by Lemma 2.7,
    \begin{equation} \label{eq:vltc}
        \max\left\{\|v_k\|,\|v_k\|^2\right\} \leq \kappa_v \|c_k\|,
    \end{equation}
    for some $\kappa_v > 0$.
    \item Let $\kappa_{uv}$ and $\zeta$ be strictly positive scalars. Then, by Lemma 2.8,
    \begin{equation} \label{eq:dposcurve}
        \|u_k\|^2 \geq \kappa_{uv} \|v_k\|^2 \implies d_k^\top H_k d_k \geq \frac14 \zeta \|u_k\|^2.
    \end{equation}
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:deltabound}
        \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \frac12 \tau_k \max\{d_k^\top H_k d_k, 0\} + \sigma\|c_k\|_1,
    \end{equation}
    (equation 2.9 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:meritdecrease}
        \phi(x_k + \alpha_k d_k, \tau_k) \leq \phi(x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k),
    \end{equation}
    (Lemma 2.12).
\end{itemize}

Armed with these results, we will prove the following lemma about sufficient decrease in the merit function whenever \eqref{eq:eps1on} does not hold.
\begin{lemma} \label{lem:suffdecrease}
Define
\begin{equation} \label{eq:kappahat}
    \hat{\kappa} := \frac{1}{\sqrt{1+\kappa_{uv}}\max\{\kappa_J,\kappa_H\}\kappa_v}
\end{equation}
and
\begin{equation} \label{eq:kappadec}
    \kappadec := \min\left\{\sigma \hat{\kappa},
    \frac18 \tau_{\min}\zeta\kappa_{uv}\kappa_v^2 \hat{\kappa}^2\right\}.
\end{equation}
Let $\varepsilon < 1$ and let at least one of $\|g_k + J_k^\top y_k\| > \varepsilon$ and/or $\|c_k\| > \varepsilon$ hold. Then,
\begin{equation} \label{eq:suffdecrease}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \varepsilon^2.
\end{equation}
\end{lemma}

\begin{proof}
To begin, assume for contradiction that
\bequationNN
\|d_k\| \leq \frac{\varepsilon}{\max\{\kappa_J,\kappa_H\}}.
\eequationNN
Then, by the definitions of $d_k$ and $y_k$ as well as $\|H_k\| \leq \kappa_H$,
\bequationNN
\|g_k + J_k^\top y_k\| = \|H_k d_k\| \leq \kappa_H \|d_k\| \leq \frac{\varepsilon \kappa_H}{\max\{\kappa_J,\kappa_H\}} \leq \varepsilon.
\eequationNN
In addition, by the definition of $d_k$ and $\|J_k\| \leq \kappa_J$,
\bequationNN
\|c_k\| = \|J_k d_k\| \leq \kappa_J \|d_k\| \leq \frac{\varepsilon \kappa_J}{\max\{\kappa_J,\kappa_H\}} \leq \varepsilon.
\eequationNN
Therefore, \eqref{eq:eps1on} holds at $k$, which is a contradiction and we must
have
\begin{equation} \label{eq:dlength}
\|d_k\| > \frac{\varepsilon}{\max\{\kappa_J,\kappa_H\}}.
\end{equation}

We consider two cases in the rest of the proof. First, let $\|c_k\| \leq \hat{\kappa} \varepsilon$. Then, by \eqref{eq:vltc} and $\|c_k\| \leq \hat{\kappa} \varepsilon$,
\bequationNN
\|v_k\|^2 \leq \kappa_v^2 \|c_k\|^2 \leq \kappa_v^2 \hat{\kappa}^2 \varepsilon^2.
\eequationNN
On the other hand, by \eqref{eq:dlength},
\begin{align*}
    \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} &< \|d_k\|^2 \\
    &= \|u_k\|^2 + \|v_k\|^2 \\
    &\leq \|u_k\|^2 + \kappa_v^2 \hat{\kappa}^2 \varepsilon^2,
\end{align*}
which implies
\begin{align*} \label{eq:ulb}
    \|u_k\|^2 &\geq \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \kappa_v^2 \hat{\kappa}^2 \varepsilon^2 \\
    &= \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \frac{ \varepsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \frac{\kappa_{uv}\varepsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2 \\
    &\geq \kappa_{uv} \|v_k\|^2.
\end{align*}
Thus, by \eqref{eq:dposcurve}, we have
\bequationNN
d_k^\top H_k d_k \geq \frac14 \zeta\|u_k\|^2 \geq \frac14 \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2.
\eequationNN
Therefore,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} \\
    &\geq \frac18 \tau_{\min} \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2,
\end{align*}
which implies \eqref{eq:suffdecrease} in this case.

Now, presume that $\|c_k\| > \hat{\kappa} \varepsilon$ holds. Then, by \eqref{eq:deltabound} and $\varepsilon < 1$,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \sigma \|c_k\|_1 \\
    &\geq \sigma \hat{\kappa} \varepsilon^2.
\end{align*}
Thus, (\ref{eq:suffdecrease}) holds in this case as well.
\end{proof}

We can use this lemma to prove the following complexity result.

\begin{theorem}
Let
\begin{equation} \label{eq:kbar}
    \bK := \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec} \varepsilon^{-2},
\end{equation}
where $\kappadec$ is defined in \eqref{eq:kappadec}.
Presume Assumptions 1 and 2 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} hold.
Then, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in no more than $\bK$ iterations (a similar result holds for Algorithm 2.2 with a revised definition of $\alpha_{\min}$).
\end{theorem}

\begin{proof}
Assume for contradiction that for all iterations $k = 0,1, \dotsc, \bK$, \eqref{eq:eps1on}
does not hold. Then, by Lemma \ref{lem:suffdecrease}, we have
\bequationNN
\Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \varepsilon^2.
\eequationNN
Then, at each iteration, by \eqref{eq:meritdecrease},
\begin{align*}
    \phi (x_k + \alpha_k d_k, \tau_k) &\leq \phi (x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k) \\
    &\leq \phi(x_k, \tau_k) - \eta \alpha_{\min} \kappadec \varepsilon^2.
\end{align*}
Using the definition of $\phi$ in \eqref{eq:phidef} as well as $x_{k+1} = x_k + \alpha_k d_k$, the above inequality becomes,
\bequationNN
\tau_k f_{k+1} + \|c_{k+1}\|_1 \leq \tau_k f_k + \|c_k\|_1 - \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Summing this inequality for all iterations $k = 0,1, \dotsc, \bK$, we have
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \sum_{k=0}^{\bK} \tau_k (f_{k+1}-f_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Now, by removing the first and last term of the summation, this inequality can be rewritten
as
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \tau_{\bK}f_{\bK+1} - \tau_0 f_0
+ \sum_{k=1}^{\bK} f_k (\tau_{k-1} - \tau_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
By definition, $\tau_k$ is a decreasing sequence. Therefore, we have $\tau_{k-1} - \tau_k \geq 0$
for all $k$. Then, since $\|c_{\bK+1}\|_1 \geq 0$ and $f_k \geq \flow$ holds for all $k$, we have
\bequationNN
- \|c_0\|_1 + \tau_{\bK}\flow - \tau_0 f_0
+ \flow (\tau_{0} - \tau_{\bK}) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Rearranging this inequality, we have
\bequationNN
\bK+1 \leq \frac{\tau_0 (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \varepsilon^2}
\leq \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \varepsilon^2}
= \bK,
\eequationNN
which is a contradiction. Therefore, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in
at most $\bK$ iterations.
\end{proof}
\fi



==> archived_versions/2021-11-11/abstract.tex <==
A worst-case complexity bound is proved for a sequential quadratic optimization (commonly known as SQP) algorithm that has been designed for solving optimization problems involving a stochastic objective function and deterministic nonlinear equality constraints.  Barring additional terms that arise due to the adaptivity of the monotonically nonincreasing merit parameter sequence, the proved complexity bound is comparable to that known for the stochastic gradient algorithm for unconstrained nonconvex optimization.  The overall complexity bound, which accounts for the adaptivity of the merit parameter sequence, shows that a result comparable to the unconstrained setting (with additional logarithmic factors) holds with high probability.

==> archived_versions/2021-11-11/body.tex <==
%******************************************
% Paper-dependent macros here
%******************************************
\newcommand{\flow}{f_{\text{\rm low}}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\E}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\kappadec}{\kappa_{\text{\rm dec}}}
\newcommand{\bK}{\bar{K}}
\newcommand{\balpha}{\bar{\alpha}}
\newcommand{\btau}{\bar{\tau}}
\newcommand{\bd}{\bar{d}}
\newcommand{\bg}{\bar{g}}
\newcommand{\bxi}{\bar{\xi}}
\newcommand{\hdelta}{\hat{\delta}}

\newcommand{\xiktri}{\xi_k^{\rm trial}}
\newcommand{\ktaudec}{\kappa_{\tau_{\rm dec}}}
\newcommand{\kmax}{k_{\max}}
\newcommand{\smax}{s_{\max}}
\newcommand{\tauktri}{\tau_k^{\rm trial}}

\newcommand{\dktrue}{d_k^{\text{\rm true}}}
\newcommand{\uktrue}{u_k^{\text{\rm true}}}
\newcommand{\wktrue}{w_k^{\text{\rm true}}}
\newcommand{\yktrue}{y_k^{\text{\rm true}}}
\newcommand{\ykstartrue}{y_{k^*}^{\text{\rm true}}}
\newcommand{\tktritrue}{\tau_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Tktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}
\newcommand{\Dktrue}{D_k^{\text{\rm true}}}
\newcommand{\Yktrue}{Y_k^{\text{\rm true}}}
\newcommand{\Uktrue}{U_k^{\text{\rm true}}}
\newcommand{\Uk}{U_k}
\newcommand{\Vk}{V_k}

\newcommand{\strue}{s^{\text{\rm true}}}

\newcommand{\Lbad}{\Lcal_{\text{\rm bad}}}
\newcommand{\Lgood}{\Lcal_{\text{\rm good}}}
\newcommand{\Ebad}{E_{\text{\rm bad}}}
\newcommand{\EbadB}{E_{\text{\rm bad},B}}
\newcommand{\Cdec}{C_{\text{\rm dec}}}
\newcommand{\Idec}{\Ical_{\text{\rm dec}}}
\newcommand{\ktau}{k_{\tau}}
\newcommand{\tcalktritrue}{\Tcal_k^{\rm \text{trial},\text{\rm true}}}

\def\Ek#1{E_{k,#1}}
\def\tred#1{\textcolor{red}{#1}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

%*********
% Section
%*********
\section{Introduction} \label{sec:intro}

We present a worst-case complexity analysis of an algorithm for minimizing a smooth objective function subject to nonlinear equality constraints.  (Due to the nature of the algorithm, this worst-case complexity analysis holds in terms of iterations, function evaluations, and derivative evaluations.)  Problems of this type arise in various important applications throughout science and engineering, including optimal control, PDE-constrained optimization, and resource allocation \cite{DPBertsekas_1998,JTBetts_2010,FSKupfer_EWSachs_1992,TRees_HSDollar_AJWathen_2010}.  However, unlike the vast majority of the literature on equality constrained optimization, the algorithm that we consider has been designed to solve problems in which the objective function is stochastic, in the sense that it is defined by the expectation of a function that has a random variable argument.  The algorithm that we consider assumes that evaluations of the objective function and its gradient are intractable to obtain, but that it has access to (unbiased) stochastic gradient estimates.

A few algorithms have been proposed recently for solving problems of this type.  These approaches fall into two categories: penalty methods \cite{CChen_FTung_NVedula_2018,YNandwani_PAbhishek_Mausam_PSingla,SKRoy_ZMhammedi_MHarandi_2018} (which includes the class of augmented Lagrangian methods) and sequential quadratic optimization (commonly known as SQP) methods \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021,SNa_MAnitescu_KMladen_2021}.  Penalty methods aim to solve the constrained optimization problem by adding a term to the objective function, weighted by a penalty parameter, that penalizes constraint violation.  Unconstrained optimization techniques are then applied to minimize the resulting penalty function, after which the penalty parameter may be modified and the minimization is performed again in an iterative manner until a solution is obtained that (approximately) satisfies the original constraints.  Methods of this type perform well in some situations, but in others they perform poorly, e.g., due to ill-conditioning and/or nonsmoothness of the subproblems. Such methods also often suffer due to their sensitivity to the particular scheme used for updating the penalty parameter.

In practice in both deterministic and stochastic optimization contexts, penalty methods are frequently outperformed by SQP methods.  Indeed, it is commonly accepted in the deterministic optimization literature that a state-of-the-art algorithm is an SQP method that chooses stepsizes based on a line search applied to a merit function.  In this deterministic setting, such an algorithm is intimately connected with applying Newton's method to the first-order primal-dual necessary conditions for optimality of the problem~\cite{RBWilson_1963}.

In this paper, we present a worst-case complexity analysis of the SQP method proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which can be seen as an extension of an SQP method from the deterministic to the stochastic setting.  A consequence of our analysis is that, in an idealized setting in which one knows a threshold for the merit parameter beyond which the merit function is \emph{exact} \cite{HanM79}, the number of iterations required until the method generates a point at which first-order necessary conditions for optimality hold in expectation with accuracy $\varepsilon \in (0,\infty)$ is $\Ocal(\varepsilon^{-4})$.  This is arguably the best result that one can expect given this is the same bound proved to hold for a stochastic gradient method employed to solve an unconstrained nonconvex problem~\cite{DDavis_DDrusvyatskiy_2019}.  However, \emph{our analysis does not only consider this idealized setting}; we go further and prove a worst-case complexity bound for the algorithm when the merit parameter threshold is unknown, and instead the algorithm adaptively updates a monotonically nonincreasing merit parameter sequence.  We prove under reasonable assumptions that the aforementioned worst-case bound, with additional logarithmic factors, holds with high probability.  The high-probability aspect of this result arises purely due to the uncertainty of the behavior of the adaptive merit parameter sequence, and does not reflect any uncertainty of the behavior of the method during situations in which the merit parameter sequence remains constant.

To the best of our knowledge, ours is the first worst-case complexity result for an SQP algorithm that operates in the \emph{highly stochastic regime} (where one merely presumes that the stochastic gradient estimates have bounded variance) for solving stochastic optimization problems involving deterministic nonlinear equality constraints.  Prior to this work, the only known complexity results for stochastic constrained optimization were for algorithms for solving problems with simple constraint sets that enable projection-based methods \cite{DDavis_DDrusvyatskiy_2019,SGhadimi_GLan_HZhang_2016} and Frank-Wolfe type methods \cite{EHazan_HLuo_2016}.  (One exception is a complexity bound proved for the SQP algorithm proposed in \cite{SNa_MAnitescu_KMladen_2021}, although that result only holds for the idealized setting in which the algorithm has \emph{a priori} knowledge of a threshold for the merit function parameter.)  Our analysis focuses a great deal on the complications that arise due to the adaptivity of the merit parameter sequence, which essentially means that the algorithm in our consideration is aiming to reduce a merit function that \emph{changes} during the optimization process.  Hence, many aspects of our analysis are quite distinct from the analyses that have been presented for stochastic gradient methods in the context of unconstrained optimization or optimization over simple constraint sets, for which the tool for measuring the progress of an algorithm---namely, the objective function itself---remains the same throughout the optimization.

%************
% Subsection
%************
\subsection{Problem formulation}

The algorithm that we consider is designed to solve problems of the form
\bequation \label{eq:fdef}
  \min_{x \in \R{n}} f(x)\ \ \st\ \ c(x) = 0,\ \ \text{with}\ \ f(x) = \E[F(x,\omega)],
\eequation
where $f : \R{n} \rightarrow \R{}$, $c : \R{n} \rightarrow \R{m}$, $\omega$ is a random variable with associated probability space $(\Omega,\mathcal{F}, P)$, $F : \R{n} \times \Omega \rightarrow \R{}$, and $\E$ represents expectation with respect to $P$.  In particular, following \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, we make the following assumption about problem \eqref{eq:fdef} and the algorithm that we analyze (stated as Algorithm~\ref{alg:ssqp} on page~\pageref{alg:ssqp}), which in any run generates a sequence of iterates $\{x_k\} \subset \R{n}$.

\begin{assumption}\label{assum:fcsmooth}
  Let $\Xcal \subseteq \R{n}$ be an open convex set that contains $\{x_k\}$ for all realizations of Algorithm \ref{alg:ssqp}.  The objective function $f : \R{n} \rightarrow \R{}$ is continuously differentiable and bounded below by $\flow \in \R{}$ over $\Xcal$ and the corresponding gradient function $\nabla f: \R{n} \rightarrow \R{n}$ is bounded and Lipschitz continuous with constant $L \in (0,\infty)$ over $\Xcal$. The constraint function $c : \R{n} \rightarrow \R{m}$ $($where $m \leq n$$)$ and the corresponding Jacobian function $J := \nabla c^\top : \R{n} \rightarrow \R{m\times n}$ are bounded over $\Xcal$, each gradient function $\nabla c_i : \R{n} \rightarrow \R{n}$ is Lipschitz continuous with constant $\gamma_i$ over $\Xcal$ for all $i \in \{1,\dots,m\}$, and the singular values of $J \equiv \nabla c^\top$ are bounded below and away from zero over $\Xcal$.
\end{assumption}

A consequence of Assumption~\ref{assum:fcsmooth} is that there exists $\kappa_g \in \R{}_{>0}$ such that
\bequation\label{eq.kappa_g}
  \|\nabla f(x_k)\| \leq \kappa_g\ \ \text{for any $k \in \N{}$ in any realization of Algorithm~\ref{alg:ssqp}}.
\eequation
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) := f(x) + c(x)^\top y$, first-order primal-dual stationarity conditions for~\eqref{eq:fdef}, which are necessary for optimality under Assumption~\ref{assum:fcsmooth}, are given by
\bequation \label{eq:optconds}
  0 =
  \left[ \begin{matrix}
    \nabla_x \ell(x,y) \\
    \nabla_y \ell(x,y)
  \end{matrix} \right]
  =
  \left[ \begin{matrix}
    \nabla f(x) + \nabla c(x) y \\
    c(x)
  \end{matrix} \right].
\eequation

%************
% Subsection
%************
\subsection{Notation}

We adopt the notation that $\|\cdot\|$ denotes the $\ell_2$-norm for vectors and the vector-induced $\ell_2$-norm for matrices.  We denote by $\mathbb{S}^{n}$ the set of $n \times n$ dimensional real symmetric matrices. The set of nonnegative integers is denoted as $\N{} := \{0,1,2,\dots,\}$. For any integer $k \in \N{}$, we use $[k]$ to denote the subset of nonnegative integers up to $k$, namely, $[k] := \{0,\dots,k\}$.  Correspondingly, to represent a set of vectors $\{v_0,\dots,v_k\}$, we define $v_{[k]} := \{v_0,\dots,v_k\}$.

Given $\phi : \R{} \to \R{}$ and $\varphi : \R{} \to [0,\infty)$, we write $\phi(\cdot) = \Ocal(\varphi(\cdot))$ to indicate that $|\phi(\cdot)| \leq C\varphi(\cdot)$ for some $C \in (0,\infty)$.  Similarly, we write $\phi(\cdot) = \widetilde\Ocal(\varphi(\cdot))$ to indicate that $|\phi(\cdot)| \leq C\varphi(\cdot)|\log^c(\cdot)|$ for some $C \in (0,\infty)$ and $c \in (0,\infty)$.  In this manner, one finds that $\Ocal(\varphi(\cdot)\log^c(\cdot)) \equiv \widetilde\Ocal(\varphi(\cdot))$ for any $c \in (0,\infty)$.

Algorithm~\ref{alg:ssqp} is iterative, generating in each realization a sequence $\{x_k\}$.  (See Section~\ref{subsec:process} for a complete description of the stochastic process generated by the algorithm.)  For our analysis, we also append the iteration number to other quantities corresponding to each iteration, e.g., $f_k := f(x_k)$ for all $k \in \N{}$.

When discussing stochastic quantities, we use capital letters to denote random variables and corresponding lower case letters to denote a realization of a random variable. For example, a stochastic gradient in iteration $k \in \N{}$ is denoted as $G_k$, a realization of which is written as $g_k$.

%************
% Subsection
%************
\subsection{Outline}

Section~\ref{sec:complexitypreview} provides a worst-case complexity result for the algorithm from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} for the deterministic setting, and uses this result and further commentary to provide an overview of our main result for the stochastic setting.  Details of the algorithm for the stochastic setting are presented in Section~\ref{sec.algorithm}, followed by our main result and analysis, which are provided in Section~\ref{sec:complexity}.  Finally, we provide some concluding thoughts and future directions in Section~\ref{sec:conclusion}.

%*********
% Section
%*********
\section{Outline of Main Results} \label{sec:complexitypreview}

Our algorithm of consideration, namely, Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, is derived from Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which is proposed and analyzed for the deterministic setting as a precursor for the stochastic setting (of Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}).  In the deterministic algorithm, the $k$th search direction $d_k \in \R{n}$ is computed by solving an optimization subproblem defined by a quadratic approximation of the objective function and an affine approximation of the constraints using derivative information at the current iterate $x_k \in \R{n}$.  This computation also results in a Lagrange multiplier value $y_k \in \R{m}$.  The subsequent iterate is set by $x_{k+1} \gets x_k + \alpha_k d_k$, where $\alpha_k \in (0,\infty)$ is a stepsize determined by a procedure to reduce the merit function $\phi : \R{n} \times (0,\infty) \to \R{}$ defined by
\bequation \label{eq:phidef}
  \phi(x,\tau) = \tau f(x) + \|c(x)\|_1.
\eequation
In particular, based on properties of the search direction $d_k$, a value of the merit parameter $\tau_k \in (0,\tau_{k-1}]$ is set by the algorithm, after which $\alpha_k \in (0,\infty)$ is computed to ensure that $\phi(x_k,\tau_k) - \phi(x_{k+1},\tau_k)$ is sufficiently positive.

%************
% Subsection
%************
\subsection{Complexity of Deterministic Algorithm}

To motivate our main result for the stochastic setting, it is instructive to state a worst-case complexity bound for the deterministic algorithm.  Such a result is the following; further details and a proof is provided in Appendix~\ref{app.deterministic}.

\btheorem\label{th.deterministic}
  Consider Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} and suppose that Assumption~\ref{assum:fcsmooth} holds along with Assumption~2.4 from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}.  Let $\tau_{-1} \in \R{}_{>0}$ be the initial value of the merit parameter sequence and let $\tau_{\min} \in (0,\tau_{-1}]$ be a positive lower bound for the merit parameter sequence $($the existence of which follows from Lemma~2.16 in~\cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}$)$.  Then, for any $\varepsilon \in (0,1)$, there exists $(\kappa_1,\kappa_2) \in \R{}_{>0} \times \R{}_{>0}$ such that the algorithm reaches an iterate $(x_k,y_k) \in \R{n} \times \R{m}$ satisfying
  \bequation\label{eq:eps1lon}  
    \|g_k + J_k^\top y_k\| \leq \varepsilon\ \ \text{and}\ \ \sqrt{\|c_k\|_1} \leq \varepsilon
  \eequation
  in a number of iterations no more than
  \bequation\label{eq.deterministic_complexity}
    \(\frac{\tau_{-1}(f_0 - \flow) + \|c_0\|_1}{\min\{\kappa_1,\tau_{\min} \kappa_2\}}\) \varepsilon^{-2}.
  \eequation
\etheorem

Theorem~\ref{th.deterministic} is not surprising.  After all, such a complexity bound of $\Ocal(\varepsilon^{-2})$ is well-known for gradient-based algorithms in unconstrained nonconvex optimization.  Since Algorithm~2.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} and its corresponding analysis do not consider the use of exact second-order derivative information, this complexity bound is on the order of what could be expected for such a method.

%************
% Subsection
%************
\subsection{Preview of Complexity of Stochastic Algorithm}\label{sec.preview}

Moving to the stochastic setting, there are a few major technical hurdles that need to be addressed, all of which relate to the adaptivity of the merit parameter sequence.  In particular, the analysis for the deterministic setting relies heavily on the facts that $(i)$ each step of the algorithm yields a sufficient reduction in the merit function for the current value of the merit parameter, $(ii)$ each such reduction in the merit function can be tied to a first-order primal-dual stationarity measure for each iterate, and $(iii)$ under Assumption~\ref{assum:fcsmooth}, one can be certain of the existence of a positive lower bound for the merit parameter sequence.  This lower bound for the merit parameter is referenced directly in the proof of the worst-case bound for the deterministic algorithm; in particular, it is shown (see Lemma~\ref{lem:suffdecrease} and the beginning of the proof of Theorem~\ref{th.deter_complex}) that the improvement in the merit function from any iterate that is not $\varepsilon$-stationary is at least proportional to $\min\{1,\tau_{\min}\} \varepsilon^{-2}$, even if the current value of the merit parameter is greater than $\tau_{\min}$.  Unfortunately, these properties of the steps and merit parameter sequence are not certain in the stochastic setting.  For example, as discussed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, it is possible---even under Assumption~\ref{assum:fcsmooth}---for the merit parameter sequence to vanish or for it to eventually remain constant at a value that is not sufficiently small, and for there to be iterations in which the expected reduction in the merit function cannot be tied to a first-order primal-dual stationarity measure.  As a result, we have had to devise new analytical approaches that confront the fact that $\{\tau_k\}$ is a random process, the ultimate behavior of which is uncertain.

To aid the reader, we provide here an overview and commentary about our ultimate complexity bound; see Corollary~\ref{coro:complexity} on page~\pageref{coro:complexity}.  Our result is proved under Assumption~\ref{assum:fcsmooth} along with others that are introduced in the subsequent sections. For one thing, as is common in SQP methods for deterministic optimization, we assume that the subproblem defining the search direction in each iteration is defined by a matrix that is positive definite in the null space of the constraint Jacobian; see Assumption~\ref{assum:Hk} on page~\pageref{assum:Hk}.  We also assume, as is common for stochastic gradient methods, that the stochastic gradient estimates are unbiased with variance bounded by $M \in (0,\infty)$, along with some related assumptions; see Assumption~\ref{assum:eventE} on page~\pageref{assum:eventE}.  Furthermore, our analysis conditions on the occurrence of an event that we call $E$ (see \eqref{def:E}); this event captures situations in which, over a total of $\kmax+1 \in \N{}$ iterations, the merit parameter is reduced at most $\smax \in [\kmax]$ times and the merit parameter is bounded below by $\tau_{\min} \in (0,\infty)$.  Under these conditions, our main complexity result shows that, within $\kmax + 1$ iterations, it holds with probability $1-\delta \in (0,1)$ that the algorithm generates $x_{k^*} \in \R{n}$ corresponding to which there exists an associated Lagrange multiplier $\ykstartrue \in \R{m}$ such that
\begin{align}
     &\ \E[\|\nabla f_{k^*} + J_{k^*}^\top \ykstartrue\|^2 + \|c_{k^*}\|_1 | E] \nonumber \\
    =&\ \Ocal \Bigg(\frac{\tau_{-1}(f_0 - \flow) + \|c(x_0)\|_1 + M}{\sqrt{\kmax+1}} \label{eq.like_sg} \\
     &\qquad + \frac{(\tau_{-1} - \tau_{\min})(\smax\log(\kmax) + \log(1/\delta))}{\sqrt{\kmax+1}}\Bigg). \label{eq.new_terms}
\end{align}
This form of the result is commonly called a convergence rate since it bounds the expected stationarity error from above by a function that decreases with the number of iterations performed, namely, $\kmax+1$.  This bound can be used to form a worst-case complexity result.  Specifically, the result above and Jensen's inequality imply that, within $\kmax+1$ iterations and as long as $\smax = \Ocal(\log(\kmax))$ (more on this below), it holds with probability $1-\delta$ that the algorithm requires at most $\widetilde\Ocal(\varepsilon^{-4})$ iterations to generate~$x_{k^*}$ with corresponding $\ykstartrue$ such that $\E[\|\nabla f_{k^*} + J_{k^*}^\top \ykstartrue\| |E] \leq \varepsilon$ and $\E[\sqrt{\|c_{k^*}\|_1}|E] \leq \varepsilon$.

The first three quantities on the right-hand side of the convergence rate, namely, in \eqref{eq.like_sg}, representing the initial objective function gap, initial constraint violation, and the variance of the stochastic gradient estimates, mirror the presence of similar terms that appear for comparable results for the stochastic gradient method in an unconstrained or simple-constraint-set setting.  The final term in \eqref{eq.new_terms}, on the other hand, as well as the fact that the result is stated as a high-probability result, are unique to our setting and arise due to the adaptivity of the merit parameter sequence.  If one were to have prior knowledge of $\tau_{\min}$, then one could set $\tau_{-1} = \tau_{\min}$ (and disable the update mechanism for the merit parameter in the algorithm), in which case our analysis would show that the expected stationarity error is bounded above by~\eqref{eq.like_sg} (surely, not only with high probability).

In the context of an adaptive merit parameter sequence, the particular form of our complexity result depends on the magnitude of $\smax$ relative to $\kmax+1$, i.e., the bound on the number of times that the merit parameter is decreased relative to the total number of iterations performed.  One setting in which our result is relatively straightforward is when, over all realizations of the algorithm, the differences between the stochastic gradient estimates and the true gradients are bounded deterministically, in which case $\smax$ is bounded by a value that is independent from $\kmax+1$; this follows from the fact that whenever the merit parameter is decreased, it is done so by a constant factor.  Beyond this setting, for another concrete example of a situation in which $\smax$ is guaranteed to be sufficiently small relative to $\kmax$, we prove in Section~\ref{subsec:subgauss} that if the distributions of the stochastic gradient estimates are sub-Gaussian, then with probability $1-\delta$ one finds that $\tau_{\min} = \textcolor{red}{\mathcal{O}(1/\log(\frac{\kmax}{\delta}))}$, meaning\footnote{\textcolor{blue}{dpr:I do not follow why the next displayed equation holds.  Is this a typo?  If you think this is correct, then I need an explanation.  FEC: I also think it was a typo.  Previously, it said ``$\log\log(\kmax/\delta)$.'' I think it's correct now.  Mike, please check. MON: It should be $\log(\log(\kmax/\delta))$ for the $\smax$ term. Check the updated sub-Gaussian section. It should be more clear now.}}
\bequationNN
  \frac{\textcolor{red}{\smax \log(\kmax)}}{\sqrt{\kmax+1}} = \mathcal{O}\left(\frac{\textcolor{red}{\log(\log(\frac{\kmax}{\delta}))\log(\kmax)}}{\sqrt{\kmax+1}}\right).
\eequationNN
As a result, one finds in such a setting that our proved convergence rate is indeed comparable to the unconstrained or simple-constraint-set setting, in the sense that the rate is not ruined by the presence of the term in \eqref{eq.new_terms}.

Before proceeding to the details of the algorithm and our analysis, we remark in passing that while our analytical approach has been developed for an SQP method that uses the merit function in \eqref{eq:phidef}, it may be applicable to a wide variety of algorithmic frameworks for constrained stochastic optimization.  For example, our approach may be modified to apply to methods that  adaptively update critical parameters at each iteration, such as adaptive penalty methods \cite{RHByrd_GLopez-Calva_JNocedal_2012,RHByrd_JNocedal_RAWaltz,MMongeau_ASartenaer_1995}, adaptive augmented Lagrangian methods \cite{FECurtis_HJiang_DPRobinson_2015}, adaptive barrier methods \cite{JNocedal_AWachter_RAWaltz_2009}, and penalty-interior point methods \cite{FECurtis_2012}.  In addition, many constrained optimization algorithms generate repeated (often unconstrained) subproblems defined by an auxilliary parameter sequence that is updated dynamically based off of the solution to the previous subproblem.  Algorithms of this type include penalty methods, augmented Lagrangian methods, and interior point methods \cite{JNocedal_SJWright_2006}.  In cases when the objective is stochastic, this auxilliary sequence would also be a random process, in which case analyzing the behavior of such a process would be paramount to proving a complexity result for such a method.  We believe that the techniques that we have devised for this paper are broadly applicable and foundational for performing complexity analyses of deterministically constrained stochastic optimization methods.

%*********
% Section
%*********
\section{Algorithm}\label{sec.algorithm}

For ease of reference, in this section we present Algorithm~3.1 from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, which is designed to solve problems of the form~\eqref{eq:fdef} and is our focus for the remainder of the paper.  In the spirit of an SQP method, the algorithm computes a search direction $d_k$ and Lagrange multiplier vector $y_k$ in iteration $k \in \N{}$ by solving
\begin{equation} \label{eq:sqpsubproblem}
  \min_{d \in \R{n}}\ f_k + g_k^\top d + \thalf d^\top H_k d\ \ \st\ \ c_k + J_k d = 0,
\end{equation}
where $H_k \in \mathbb{S}^n$ is chosen independently from $g_k$, and we remind the reader that $g_k$ is a realization of the stochastic gradient $G_k$. Under Assumption~\ref{assum:fcsmooth} and the following Assumption~\ref{assum:Hk} (that we make throughout the remainder of the paper), the solution of \eqref{eq:sqpsubproblem} can be obtained from the unique solution of
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}

\begin{assumption} \label{assum:Hk}
  The sequence $\{\|H_k\|\}$ is bounded by $\kappa_H \in \R{}_{>0}$.  In addition, there exists $\zeta \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, the matrix $H_k \in \mathbb{S}^n$ has the property that $u^\top H_k u \geq \zeta \|u\|_2^2$ for all $u \in \R{n}$ such that $J_k u = 0$.
\end{assumption}

After computation of $(d_k,y_k)$, the remainder of the $k$th iteration involves $(i)$ updating the merit parameter, $(ii)$ updating an auxiliary parameter needed for the stepsize computation, and $(iii)$ computing a positive stepsize.  These algorithmic components are designed with the aim of yielding a sufficiently positive reduction in a model of the merit function, which in turn is aimed at yielding a sufficiently positive reduction in the merit function itself.  The algorithm employs the model $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\bequationNN
  q(x, \tau, g, H, d) = \tau (f(x) + g^\top d + \thalf \max\{d^\top H d,0\}) + \|c(x) + J(x) d\|_1,
\eequationNN
and the reduction function $\Delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$, for a given $d \in \R{n}$ satisfying $c(x) + J(x) d = 0$, defined by
\begin{equation} \label{eq:deltadef}
  \baligned
    \Delta q(x, \tau, g, H, d)
      :=&\ q(x, \tau, g, H, 0) - q(x, \tau, g, H, d) \\
       =&\ -\tau (g^\top d + \thalf \max\{d^\top H d,0\}) + \|c(x)\|_1.
  \ealigned
\end{equation}
Specifically, in order to ensure in iteration $k$ that $\tau_k \leq \tau_{k-1}$ and
\bequation \label{eq:qquadlb}
  \Delta q(x_k,\tau,g_k,H_k,d_k) \geq \thalf \tau \max\{d_k^\top H_k d_k, 0\} + \sigma \|c_k\|_1 \geq 0
\eequation
holds for all $\tau \leq \tau_k$, the algorithm sets, for user-defined $\sigma \in (0,1)$, the value
\bequation \label{eq:tautrial}
  \tauktri\gets
  \begin{cases}
    \infty & \mbox{if $g_k^\top d_k + \max\{d_k^\top H_k d_k, 0\} \leq 0$} \\
    \frac{(1-\sigma)\|c_k\|_1}{g_k^\top d_k + \max\{d_k^\top H_k d_k,0\}} & \mbox{otherwise,}
  \end{cases}
\eequation
and then sets, for some $\epsilon_\tau \in (0,1)$, the merit parameter value
\bequation \label{eq:taudef}
  \tau_k \gets \bcases \tau_{k-1} & \mbox{if $\tau_{k-1} \leq \tauktri$} \\ (1-\epsilon_\tau)\tauktri & \mbox{otherwise.} \ecases
\eequation
Then, for use in the stepsize computation (as motivated in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}) it sets
\bequation \label{eq:xidef}
  \xiktri \gets \frac{\Delta q(x_k, \tau_k, g_k, H_k, d_k)}{\tau_k \|d_k\|^2}\ \ \text{then}\ \ \xi_k \gets \bcases \xi_{k-1} & \mbox{if }\xi_{k-1} \leq \xiktri \\ (1-\epsilon_\xi)\xiktri & \mbox{otherwise} \ecases
\eequation
for some $\epsilon_\xi \in (0,1)$, which, for one thing, ensures $\xi_k \leq \xiktri$.  The last component in the $k$th iteration is to set the stepsize, the magnitude of which is controlled by prescribed $\{\beta_k\} \subset (0,1]$, which is employed in the following projection interval that is used in the stepsize computation:
\bequationNN
    \mbox{Proj}_k(\cdot) := \mbox{Proj}\left(\cdot \; \Bigg| \left[\frac{\beta_k \xi_k \tau_k}{\tau_k L + \Gamma}, \frac{\beta_k \xi_k \tau_k}{\tau_k L + \Gamma} + \theta \beta_k^2 \right]\right),
\eequationNN
where $\mbox{Proj}(\cdot \; | \; \mathcal{I})$ represents the projection operator onto the interval $\mathcal{I} \subset \R{}$.  As in other stochastic-gradient-based methods, the convergence properties of the method depend on properties of $\{\beta_k\}$, which in many analyses is considered to be a constant or diminishing sequence.  In our analysis, we establish our result for the case of $\beta_k = \Ocal(1/\sqrt{\kmax+1})$ for all $k \in [\kmax]$.

Overall, the algorithm that we consider is stated as Algorithm~\ref{alg:ssqp}.  The only changes from Algorithm~3.1 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} are the fixed iteration limit ($\kmax$) and the concluding step for producing the return value ($x_{k^*}$).  This method of sampling $k^*$ to produce the return value is consistent with other approaches in the literature on complexity analyses for algorithms for solving nonconvex optimization problems; see, e.g., \cite{DDavis_DDrusvyatskiy_2019}.  It amounts to uniform sampling over the iterates when constant $\{\beta_k\}$ is considered, as in our analysis.  Finally, we remark that Algorithm~\ref{alg:ssqp} presumes knowledge of Lipschitz constants for the objective and constraint gradients, although in practice one might only estimate these values, for which standard procedures can be employed~\cite{FECurtis_DPRobinson_2019}.

\begin{algorithm}[ht]
  \caption{Stochastic SQP Algorithm}
  \label{alg:ssqp}
  \begin{algorithmic}[1]
    \Require $x_0 \in \R{n}$; $\kmax \in \N{}$; $\tau_{-1} \in \R{}_{>0}$; $\epsilon_\tau \in (0,1)$; $\epsilon_\xi \in (0,1)$; $\sigma \in (0,1)$; $\xi_{-1} \in \R{}_{>0}$; $\{\beta_k\} \subset (0,1]$; $\theta \in \R{}_{\geq0}$; $L \in (0,\infty)$, a Lipschitz constant for $\nabla f$; $\Gamma \in [\sum_{i=1}^m \gamma_i,\infty)$, where $\gamma_i \in (0,\infty)$ is a Lipschitz constant for $\nabla c_i$ for all $i \in [m]$
    \For{\textbf{all} $k \in [\kmax]$}
	  \State Compute $(d_k,y_k)$ as the solution of \eqref{eq:sqpsystem}
	  \If{$d_k = 0$}
	    \State Set $\tauktri \gets \infty$, $\tau_k \gets \tau_{k-1}$, $\xiktri \gets \infty$, and $\xi_k \gets \xi_{k-1}$
	    \State Set $\widehat\alpha_{k,\text{init}} \gets 1$, $\widetilde\alpha_{k,\text{init}} \gets 1$, and $\alpha_k \leftarrow 1$
	  \Else\ (if $d_k \neq 0$)
	    \State Set $\tauktri$ by \eqref{eq:tautrial} and $\tau_k$ by \eqref{eq:taudef} %\label{step.tau_stochastic}
	    \State Set $\xiktri$  and $\xi_k$ by \eqref{eq:xidef} %\label{step.xi}
        \State Set
        \bequationNN
          \widehat\alpha_{k,\text{init}} \gets \tfrac{\beta_k\Delta q(x_k,\tau_k,g_k,H_k,d_k)}{(\tau_k L + \Gamma)\|d_k\|_2^2}\ \ \text{and}\ \  \widetilde\alpha_{k,\text{init}} \gets \widehat\alpha_{k,\text{init}} - \tfrac{4\|c_k\|_1}{(\tau_k L +  \Gamma)\|d_k\|_2^2}
        \eequationNN
        \State Set $\widehat\alpha_k \gets \proj_k(\widehat\alpha_{k,\text{init}})$ and $\widetilde\alpha_k \gets \proj_k(\widetilde\alpha_{k,\text{init}})$, then \label{step.alpha_projection_stochastic} \label{step.alpha_stochastic}
        \bequationNN
          \alpha_k \gets
		    \bcases
		      \widehat\alpha_k & \text{if $\widehat\alpha_k < 1$} \\
		      1 & \text{if $\widetilde\alpha_k \leq 1 \leq \widehat\alpha_k$} \\
		      \widetilde\alpha_k & \text{if $\widetilde\alpha_k > 1$}
		    \ecases
        \eequationNN
      \EndIf
      \State Set $x_{k+1} \gets x_k + \alpha_k d_k$
    \EndFor
    \State Sample $k^* \in [\kmax]$ according to the probability distribution
    \bequationNN
        \Prob[k^* = k] = \frac{\beta_k}{\sum_{k=0}^{\kmax} \beta_k},
    \eequationNN
    then \Return $x_{k^*}$
  \end{algorithmic}
\end{algorithm}

%*********
% Section
%*********
\section{Complexity Analysis} \label{sec:complexity}

We begin our complexity analysis by describing the algorithm as a stochastic process (Section~\ref{subsec:process}), then formalizing the assumptions that we make about the stochastic gradient estimates (Section \ref{subsec:assumptions}).  We then state, in some cases in a slightly modified form, some key lemmas from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} that are needed for our analysis (Section \ref{subsec:algprops}).  Our generic complexity result, which has been outlined in Section~\ref{sec:complexitypreview}, is then stated and proved (Section \ref{subsec:complexity}).  Consequences and extensions of our generic complexity result are then discussed for some special cases of distributions for the stochastic gradient estimates for which our required assumptions hold with high-probability (Section \ref{subsec:subgauss}).  Finally, we conclude this section by outlining a form of our generic complexity result that relaxes one of our minor simplifying assumptions (Section \ref{subsec:ratioparam}).

Similarly as for the convergence analysis in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, our complexity analysis makes use of orthogonal decompositions of the search directions computed by the algorithm; in particular, for all $k \in \N{}$, we express $d_k = u_k + v_k$, where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.  We note here that conditioned on the algorithm having reached $x_k$ at iteration $k$, the normal component $v_k$ is {\it deterministic}, depending only on the constraint value $c_k$ and the Jacobian $J_k$.

In addition to the quantities that are computed explicitly in Algorithm~\ref{alg:ssqp}, our analysis also refers to the quantities that would have been computed in each iteration $k \in \N{}$, conditioned on the event that the algorithm has reached~$x_k$ as the $k$th iterate, if the true gradient $\nabla f(x_k)$ in place of the stochastic gradient $g_k$.  These quantities are denoted by a ``true'' superscript.  For example, in iteration $k$, the true search direction and corresponding true Lagrange multiplier estimate are the solution of the linear system
\bequation \label{eq:sqpsystemdet}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    \dktrue \\ \yktrue
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    \nabla f(x_k) \\ c_k
    \end{matrix}
    \right],
\eequation
which may be decomposed as $\dktrue = \uktrue + v_k$, where $\uktrue \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$.  Here, we write $v_k$ (without a superscript) since the normal component of the search direction is defined in a manner that makes it independent of the objective gradient (estimate).  Similarly, the true value of the merit parameter that would have been computed is denoted
\bequationNN
    \tktritrue \gets
    \begin{cases}
        \infty\ \ \text{if $\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue, 0\} \leq 0$} & \\
        \frac{(1-\sigma)\|c_k\|_1}{\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}}\ \  \text{otherwise}. &
    \end{cases}
\eequationNN
This definition of $\tktritrue$ guarantees that, for any $\tau \leq \tktritrue$, one finds
\bequation \label{eq:qquadlbtrue}
    \Delta q(x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \thalf \tau \max\{(\dktrue)^\top H_k \dktrue, 0\} + \sigma \|c_k\|_1.
\eequation

%************
% Subsection
%************
\subsection{Stochastic Process} \label{subsec:process}

Henceforth, for the sake of formality, we shall refer in our analysis to the stochastic process generated by Algorithm~\ref{alg:ssqp}.  Specifically, in terms of values that are computed by the algorithm itself, we have the stochastic process
\bequationNN
  \{(X_k,G_k,D_k,Y_k,\Tcal_k,\Xi_k,\Acal_k)\},
\eequationNN
where, for all $k \in \N{}$, the random variables are: the algorithm iterate $X_k$, stochastic gradient estimate $G_k$, search direction $D_k$, Lagrange multiplier estimate $Y_k$, merit parameter $\Tcal_k$, ratio parameter $\Xi_k$, and stepsize $\Acal_k$.  For all $k \in \N{}$, a realization of the corresponding element of this process is denoted $(x_k,g_k,d_k,y_k,\tau_k,\xi_k,\alpha_k)$.  Similarly, in terms of ``true'' values and step decomposition values that are not computed by the algorithm, but are defined for the sake of our analysis, we have the simultaneously generated process
\bequationNN
  \{(\Vk,\Uk,\Dktrue,\Uktrue,\Yktrue,\Tktritrue)\},
\eequationNN
where, for all $k \in \N{}$, the random variables are: the normal search direction component $\Vk$, the tangential search direction component $\Uk$, the true search direction $\Dktrue$, the true tangential search direction component $\Uktrue$, the true Lagrange multiplier estimate $\Yktrue$, and the true trial merit parameter $\Tktritrue$.  For all $k \in \N{}$, a realization of the corresponding element of this process is denoted $(v_k,u_k,\dktrue,\uktrue,\yktrue,\tktritrue)$.  Finally, for the sake of tracking the number of merit parameter updates that occur during runs of the algorithm, we define the stochastic process $\{S_k\}$, where for all $k \in \N{}$ the random variable $S_k$ represents the number of merit parameter decreases up to the end of the $k$th iteration, i.e., the number of iterations in which $\Tcal_k < \Tcal_{k-1}$.  For all $k \in \N{}$, a realization of $S_k$ is denoted $s_k$.

In any run, the behavior of Algorithm~\ref{alg:ssqp} is dictated entirely by the initial conditions and the sequence of stochastic gradient estimates that are generated.  Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{G_0,\dots,G_{k-1}\}$, a realization of which (along with all initial conditions of the algorithm, including $X_0 = x_0$) determines the realizations of
\bequationNN
  \{X_j\}_{j=1}^k\ \text{and}\ \{(D_j,Y_j,\Tcal_j,\Xi_j,\Acal_j,V_j,U_j,D_j^{\rm true},U_j^{\rm true},Y_j^{\rm true},\Tcal_j^{\rm trial, true},S_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{0} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq 0}$ is a filtration.  When conditioning on a specific realization of Algorithm~\ref{alg:ssqp} up to the beginning of iteration $k \in \N{}$, we condition on $G_{[k-1]} = g_{[k-1]}$, since these stochastic gradients determine $x_k$.  (Recall our notation that $g_{[k-1]}$ represents $\{g_0,\dots,g_{k-1}\}$.)  Similarly, later in our analysis when we condition on $\Fcal_{k}$, we are conditioning on all realizations of $G_{[k-1]}$ that are measurable with respect to the filtration~$\Fcal_{k}$.

%************
% Subsection
%************
\subsection{Assumptions} \label{subsec:assumptions}

Our analysis presumes certain good behavior of the sequences of merit and ratio parameters that are set adaptively by the algorithm.  Formally, given $(\kmax,\smax,\tau_{\min},\xi_{\min}) \in \N{} \times \N{} \times \R{}_{>0} \times \R{}_{>0}$, our main result characterizes the worst-case behavior of Algorithm~\ref{alg:ssqp} conditioned on the event denoted as
\bequation\label{def:E}
  E := E(\kmax,\smax,\tau_{\min},\xi_{\min}),
\eequation
which we define as the event such that, in every realization of the algorithm, the merit parameters $\{\tau_k\}_{k=0}^{\kmax}$ and ratio parameters $\{\xi_k\}_{k=0}^{\kmax}$ satisfy
\bitemize
  \item $\tau_k \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\tktritrue \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\xi_k = \xi_{\min} > 0$ for all $k \in [\kmax]$, and
  \item $|\{k \in [\kmax] : \tau_k < \tau_{k-1}\}| \leq \smax$.
\eitemize
Consideration of this event as a focus for proving a worst-case complexity result for Algorithm~\ref{alg:ssqp} is justifiable for the following reasons.

\bitemize
  \item The condition in $E$ that the ratio parameter sequence is constant over all iterations is not actually essential for our analysis; rather, it is made for the sake of simplicity.  Indeed, in Section \ref{subsec:ratioparam}, we present an extension of our main result to the setting in which this parameter sequence is not constant.  Observe that, as proved in \cite[Lemma~3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, the sequence $\{\Xi_k\}$ is bounded below by a positive real number whose value is deterministic, i.e., it is independent of the sequence of stochastic gradient estimates that are generated by the algorithm.  Hence, for the sake of simplicity, we assume for now that $\{\Xi_k\}$ is constant and leave the statement of the more complicated version of our main result to a subsection at the end of our analysis.
  \item The conditions in $E$ pertaining to the behavior of the merit parameter sequence are not necessarily minor.  That said, attention to this behavior of the algorithm is justified by arguments made in \cite{BeraCurtONeiRobi21,ABerahas_FECurtis_DPRobinson_BZhou_2021}, which under the same kinds of assumptions made in this paper argue that, in any run of the algorithm, the probability is zero that the merit parameter vanishes.  Furthermore, in Section~\ref{subsec:subgauss}, we consider a particular setting of interest in which the distributions of the stochastic gradient estimates are sub-Gaussian over any run of the algorithm, in which case we show that the merit parameter remains bounded below with high probability, meaning that our main worst-case complexity bound---which holds with high probability due to the adaptivity of the merit parameter sequence---remains essentially unchanged in this setting when we do not presume upfront that the merit parameter sequence remains bounded above a positive real number.
  \item The condition in $E$ pertaining to the existence of $\smax$ is not actually an additional requirement beyond the existence of $\tau_{\min}$ in the event.  After all, by the construction of Algorithm~\ref{alg:ssqp}, it follows that when the merit parameter is decreased, it is decreased by at least a constant factor, from which it follows (under the existence of $\tau_{\min}$) that $\smax$ exists and satisfies
  \bequation \label{eq:smaxbound}
    \smax \leq \min\left\{\kmax+1, \left\lceil\frac{\log(\tau_{\min}/\tau_{-1})}{\log(1-\epsilon_\tau)}\right\rceil\right\}.
  \eequation
  That said, for simplicity and generality in our analysis, we define $\smax$ as a quantity that is decoupled from the above (conservative) inequality.
\eitemize

Conditioned on $E$, we assume the following about the stochastic gradient estimates.  Such an assumption, namely, that conditioned on the event that a given iterate has been reached the stochastic gradient is unbiased and has bounded variance, is common in analyses of stochastic optimization methods.  Here and throughout the remainder of the paper, we let $\Prob_k[\cdot]$ (respectively, $\E_k[\cdot]$) denote probabilty (respectively, expectation) conditioned on event $E$ and that $G_{[k-1]} = g_{[k-1]}$ for a given $g_{[k-1]}$, i.e., we define
\bequationNN
  \P_k[\cdot] := \P[\cdot | E, G_{[k-1]} = g_{[k-1]}]\ \ \text{and}\ \ \E_k[\cdot] := \E[\cdot | E, G_{[k-1]} = g_{[k-1]}].
\eequationNN

\bassumption\label{assum:eventE}
  There exists $M \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequation\label{eq.sg}
    \E_k[G_k] = \nabla f(x_k)\ \ \text{and}\ \ \E_k[\|G_k - \nabla f(x_k)\|_2^2] \leq M.
  \eequation
  In addition, there exists $M_\tau \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequation\label{eq.sg+}
    \baligned
      \text{either}\ \ \P_k[\nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &= 0 \\
      \text{or}\ \ \E_k[\|G_k - \nabla f(x_k)\|_2 | \nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &\leq M_\tau.
    \ealigned
  \eequation
\eassumption

Observe that the second inequality in \eqref{eq.sg} can imply \eqref{eq.sg+}, such as when there exists $p \in (0,1]$ such that, for all $k \in [\kmax]$ and $g_{[k-1]}$, one finds that
\bequationNN
  \P_k[\nabla f(x_k)^\top(D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \geq p
\eequationNN
whenever this probability is nonzero.  This occurs, for example, when the objective of \eqref{eq:fdef} is a finite sum of $N$ terms and each stochastic gradient estimate is computed as a so-called mini-batch estimate through the uniform (random) selection of $b$ indices, in which case the above holds with $p = b/N$.

We make one additional assumption for our analysis, namely, the following.

\begin{assumption} \label{assum:ptau}
  There exists $p_{\tau} \in (0,1]$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequationNN
    \baligned
      \P_k[& G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \\
      & \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\}] \geq p_{\tau}.
    \ealigned
  \eequationNN
\end{assumption}

Similar to \cite[Proposition~3.16]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, Assumption~\ref{assum:ptau} allows us to prove that, with high probability, the number of iterations in which $\tau_k > \tktritrue$ is not too large.  In \cite[Example 3.17]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, it was shown that the inequality in this assumption holds with $p_{\tau} = \frac12$ when, conditioned on having reached $x_k$, the stochastic gradient $G_k$ has a Gaussian distribution.  We show in Section~\ref{subsec:subgauss} that this result can be extended to other settings in which the stochastic gradient distributions obey a mild form of symmetry.

%************
% Subsection
%************
\subsection{Properties of Algorithm \ref{alg:ssqp}} \label{subsec:algprops}

In this section, we state key results from \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} that are needed for our analysis.

By \cite[Lemma 2.10]{ABerahas_FECurtis_DPRobinson_BZhou_2021}, there exists $\kappa_{uv} \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, if $\|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2$, then $\frac12 (\dktrue)^\top H_k \dktrue \geq \frac14 \zeta \|\uktrue\|^2$, where $\zeta$ is defined in Assumption \ref{assum:Hk}.  Correspondingly, let us define
\bequationNN
  \Psi_k := \begin{cases}
        \|\uktrue\|^2 + \|c_k\| & \mbox{if } \|\uktrue\|^2 \geq \kappa_{uv} \|v_k\|^2 \\
        \|c_k\| & \mbox{otherwise.}
    \end{cases}
\eequationNN

The following lemma is stated using a different norm (for $c_k$) than in \cite[Lemma 2.11]{ABerahas_FECurtis_DPRobinson_BZhou_2021}\footnote{\textcolor{red}{MON: I'm a bit worried that this change adds a hidden $\sqrt{n}$ factor that should not be there. I believe if we updated $\Psi_k$ to use $\|c_k\|_1$, all of the results involving it still hold and we don't need to use equivalence of norms.}}.  The result holds in the same manner due the norm-equivalence between $\|\cdot\|$ and $\|\cdot\|_1$ in $\R{m}$.  We state the result in this manner for consistency in the measure of constraint violation stated in our final complexity bound. 

\begin{lemma}[{\cite[Lemma 2.11]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}] \label{lem:kappapsi}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold.  Then, there exists $\kappa_{\Psi} \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, the true search direction and constraint violation satisfy $\|\dktrue\|^2 + \|c_k\|_1 \leq (\kappa_{\Psi} + 1) \Psi_k$.
\end{lemma}

\begin{lemma}[{\cite[Lemma 2.12]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}] \label{lem:kappaq}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold. Then, there exists $\kappa_q \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any $\tau \leq \tktritrue$, the true reduction in the merit model satisfies $\Delta q (x_k,\tau,\nabla f(x_k),H_k,\dktrue) \geq \kappa_q \tau \Psi_k$.
\end{lemma}

\blemma[{\cite[Lemma~3.7]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}]\label{lem:phidecrease}
  Let Assumptions \ref{assum:fcsmooth} and \ref{assum:Hk} hold and suppose that the sequence $\{\beta_k\}$ is chosen such that $\beta_k \xi_k \tau_k/(\tau_k L + \Gamma) \in (0,1]$ for all $k \in [\kmax]$.  Then, for all $k \in [\kmax]$, it follows that
  \bequation \label{eq:phidecrease}
    \baligned
      \phi(x_k + \alpha_k d_k, \tau_k) - \phi(x_k, \tau_k)
      &\leq -\alpha_k \Delta q(x_k,\tau_k,\nabla f(x_k),H_k,\dktrue) \\
      &\quad + \thalf \alpha_k \beta_k  \Delta q(x_k,\tau_k,g_k,H_k,d_k) \\
      &\quad + \alpha_k \tau_k \nabla f(x_k)^\top (d_k - \dktrue).
    \ealigned
  \eequation
\elemma

\blemma \label{lem:dexpectation}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in [\kmax]$, it follows that $\E_k[D_k] = \dktrue$, $\E_k[U_k] = \uktrue$, and $\E_k[Y_k] = \yktrue$.  Moreover, there exists $\kappa_d \in \R{}_{>0}$ such that, for all $k \in [\kmax]$, one finds that
  \bequationNN
    \left\|\begin{bmatrix} H_k & J_k^\top \\ J_k & 0 \end{bmatrix}^{-1}\right\| \leq \kappa_d,
  \eequationNN
  from which it follows that
  \bequationNN
    \baligned
      \|\dktrue\| \leq \kappa_d \|\nabla f(x_k)\| &\leq \kappa_d \kappa_g, \\
      \E_k[\|D_k - \dktrue\|] \leq \kappa_d \E_k[\|G_k - \nabla f(x_k)\|] &\leq \kappa_d \sqrt{M},\ \ \text{and} \\
      \E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] &\leq \kappa_d M_\tau.
    \ealigned
  \eequationNN
\elemma
\bproof
  Except for the final inequality, the result follows from \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2021}.  As for the final inequality, observe by the arguments in \cite[Lemma 3.8]{ABerahas_FECurtis_DPRobinson_BZhou_2021} that for any realization of $G_k$ and $D_k$ one finds $\|d_k - \dktrue\| \leq \kappa_d \|g_k - \nabla f(x_k)\|$, so
  \begin{align*}
    &\ \E_k[\|D_k - \dktrue\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \\
    \leq&\ \kappa_d \E_k[\|G_k - \nabla f(x_k)\| | \nabla f(x_k)^\top (D_k - \dktrue) < 0, \Tcal_k < \tau_{k-1}] \leq \kappa_d M_\tau,
  \end{align*}
  as desired. \qed
\eproof


\blemma[{\cite[Lemma~3.9]{ABerahas_FECurtis_DPRobinson_BZhou_2021}}]\label{lem:product_bounds}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for all $k \in [\kmax]$, it follows that
  \bequationNN
    \baligned
      \nabla f(x_k)^\top \dktrue \geq \E_k[G_k^\top D_k] &\geq \nabla f(x_k)^\top \dktrue - \zeta^{-1}M \\
      \text{and}\ \ \E_k[D_k^\top H_k D_k] &\geq (\dktrue)^\top H_k \dktrue.
    \ealigned
  \eequationNN
\elemma

%************
% Subsection
%************
\subsection{Complexity Result} \label{subsec:complexity}

In this section, we present our main complexity results. We derive our results in largely the same manner as the global convergence result in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}, but with two major changes that stem from the need to characterize the behavior of the algorithm in the context of an adaptive merit parameter sequence.  At a high level, the two modifications are as follows:
\begin{enumerate}
    \item We derive, in Lemma~\ref{lem:innerprod}, an upper bound for the last term in~\eqref{eq:phidecrease}, the derivation of which is complicated by the fact that, conditioned on $x_k$ being the $k$th iterate in a run of the algorithm, this term is the product of three correlated random variables: $\Acal_k$, $\Tcal_k$, and $\nabla f(x_k)^\top (D_k - \dktrue)$.  A critical aspect of our derived bound is that we isolate a term for the event when $\nabla f(x_k)^\top (D_k - \dktrue) < 0$ and $\Tcal_k < \tau_{k-1}$, since this happens to be an event that complicates subsequent aspects of our analysis.  In Lemma~\ref{lem:Eksumlsmax}, we prove a high-probability bound on the sum of the probabilities of the occurrences of this event over the entire run of the algorithm.
    \item A critical aspect of the analysis in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021} for the deterministic setting is that one can always tie the reduction in the model of the merit function to a first-order stationarity error measure (with respect to the constrained optimization problem) due to the fact that $\tktritrue \geq \tau_k$ for all $k \in \N{}$.  Unfortunately, however, this inequality is not guaranteed to hold in the stochastic setting, which is problematic for our purposes in this paper.  To account for this issue, we define an auxiliary sequence $\{\hat\Tcal_k\}$ (not generated by the algorithm) such that $\hat{\Tcal}_k := \min\{\Tcal_k, \Tktritrue\}$ for all $k \in [\kmax]$.  In Lemmas~\ref{lem:dqbound} and \ref{lem:hattaudiff}, we analyze behaviors of the algorithm with respect to this auxiliary sequence, and in Lemma~\ref{lem:Ktaulsmax} we provide a high-probability bound on the total number of iterations in which $\Tktritrue < \Tcal_k$ may occur.  (More precisely, Lemma~\ref{lem:Ktaulsmax} considers a superset of the iterations in which this bound may occur, which serves our purposes just as well.)
\end{enumerate}

The first few results in this section consider properties of algorithmic quantities conditioned on the algorithm having generated a certain sequence of stochastic gradient estimates through a given iteration.  In particular, given $k \in [\kmax]$ and $g_{[k-1]}$, values generated by the algorithm have been determined up to the beginning of iteration $k$, including $x_k$, $\dktrue$, and~$\tau_{k-1}$.  Given these quantities, let us define three events:
\bitemize
  \item $\Ek1$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) \geq 0$;
  \item $\Ek2$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} = \tau_{k-1}$; and
  \item $\Ek3$, the event that $\nabla f(x_k)^\top(D_k - \dktrue) < 0$ and $\Tcal_{k} < \tau_{k-1}$.
\eitemize

We now derive an upper bound on the final term in \eqref{eq:phidecrease}.  In the following lemma, we make use, for given $k \in [\kmax]$ and $g_{[k-1]}$, of the stepsize values
\bequation\label{eq.alpha_mins}
  \baligned
    \alpha_{\min,k}^{<} := \frac{\beta_k \xi_{\min} \tau_{\min}}{\tau_{\min}L + \Gamma},\ \ \alpha_{\min,k}^{=} &:= \frac{\beta_k \xi_{\min} \tau_{k-1}}{\tau_{k-1}L + \Gamma}, \\
    \text{and}\ \ \varsigma_{\max,k} &:= \alpha_{\min,k}^{=} + \theta \beta_k^2.
  \ealigned
\eequation
The first two values here represent the smallest stepsizes that may be computed in the event that $\Tcal_k < \tau_{k-1}$ and in the event that $\Tcal_k = \tau_{k-1}$, respectively, for which it is easily verified that $\alpha_{\min,k}^{<} < \alpha_{\min,k}^{=}$.  Hence, $\varsigma_{\max,k}$ represents the largest stepsize that may be computed.

\begin{lemma} \label{lem:innerprod}
  Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold,  and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$, and with the stepsizes $(\alpha_{\min,k}^{<},\alpha_{\min,k}^{=},\varsigma_{\max,k})$ defined as in \eqref{eq.alpha_mins}, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ (\varsigma_{\max,k}\tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta_k^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
  \end{align*}
\end{lemma}
\begin{proof}
  Consider arbitrary $k \in [\kmax]$ and $g_{[k-1]}$, and for ease of exposition, let us denote $\E_{k,j} = \E_k[\nabla f(x_k)^\top(D_k - \dktrue) | E_{k,j}]$ for all $j \in \{1,2,3\}$.  By the Law of Total Expectation, the fact that $0 < \tau_{\min} \leq \Tcal_k \leq \tau_{k-1}$ under $E$, and the definitions of $\alpha_{\min,k}^{<}$, $\alpha_{\min,k}^{=}$, and $\varsigma_{\max,k}$, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    =&\ \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek1] \Prob_k[\Ek1] \\
     &\ + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek2] \Prob_k[\Ek2] \\
     &\ + \E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)|\Ek3] \Prob_k[\Ek3] \\
    \leq&\ \varsigma_{\max,k} \tau_{k-1}  \E_{k,1} \Prob_k[\Ek1] + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,3} \Prob_k[\Ek3].
  \end{align*}
  Using this inequality, the Law of Total Expectation, and Lemma \ref{lem:dexpectation}, one obtains three distinct upper bounds by adding subtracting terms in multiple ways:
  \begin{align*}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \varsigma_{\max,k} \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \varsigma_{\max,k} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \varsigma_{\max,k} \tau_{k-1} \E_{k,3} \Prob_k[\Ek3] + (\alpha_{\min,k}^{<} \tau_{\min} - \varsigma_{\max,k} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \\
    =&\ - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] + (\alpha_{\min,k}^{<} \tau_{\min} - \varsigma_{\max,k} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3]; \\
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \theta \beta_k^2 \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \alpha_{\min,k}^{=} \tau_{k-1} \E_{k,3} \Prob_k[\Ek3] + (\alpha_{\min,k}^{<} \tau_{\min} - \alpha_{\min,k}^{=} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \\
    =&\ \theta \beta_k^2 \tau_{k-1} \E_{k,1} \Prob_k[\Ek1] + (\alpha_{\min,k}^{<} \tau_{\min} - \alpha_{\min,k}^{=} \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3];\ \ \text{and} \\
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \\
    \leq&\ \alpha_{\min,k}^{<} \tau_{\min} \E_{k,1} \Prob_k[\Ek1] + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \\
    &\ + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,2} \Prob_k[\Ek2] + (\alpha_{\min,k}^{=} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2] \\
    &\ + \alpha_{\min,k}^{<} \tau_{\min} \E_{k,3} \Prob_k[\Ek3] \\
    =&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \\
    &\ + (\alpha_{\min,k}^{=} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2].
  \end{align*}
  Averaging these three upper bounds, one obtains
  \begin{align}
    &\E_k[\Acal_k \Tcal_k \nabla f(x_k)^\top(D_k - \dktrue)] \nonumber \\
    \leq&\ \tfrac13 ((\alpha_{\min,k}^{=} + 2\theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\ + \tfrac13 ((\alpha_{\min,k}^{=} - \theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\ + \tfrac13 (2\alpha_{\min,k}^{<} \tau_{\min} - (2\alpha_{\min,k}^{=} + \theta \beta_k^2) \tau_{k-1}) \E_{k,3} \Prob_k[\Ek3] \nonumber \\
    =&\ \tfrac13 ((\alpha_{\min,k}^{=} + 2\theta \beta_k^2) \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\ - \theta \beta_k^2 \tau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\ - \tfrac13 ((2\alpha_{\min,k}^{=} + \theta \beta_k^2) \tau_{k-1} - 2\alpha_{\min,k}^{<} \tau_{\min}) \E_{k,3} \Prob_k[\Ek3]. \label{eq:innerprodproof1}
  \end{align}
  This bound can be rewritten as follows.  By the Law of Total expectation,
  \begin{align}
    &\ \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    =&\ \E_k[\nabla f(x_k)^\top(D_k - \dktrue)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3], \label{eq.new1}
  \end{align}
  and along with Lemma \ref{lem:dexpectation} one finds
  \begin{align}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek2] \Prob_k [\Ek2] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek2] \Prob_k [\Ek2] \nonumber \\
    &= \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \nonumber \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek1]\Prob_k [\Ek1] \nonumber \\
    &\quad - \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\| | \Ek3] \Prob_k [\Ek3] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|] \nonumber \\
    &\leq \kappa_g \E_k[\|D_k - \dktrue\|] \leq \kappa_g \kappa_d \sqrt{M}. \label{eq.new2}
  \end{align}
  In addition, Lemma \ref{lem:dexpectation} also yields that
  \begin{align}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[\nabla f(x_k)^\top(D_k - \dktrue)| \Ek3] \Prob_k[\Ek3] \nonumber \\
    &\leq \E_k[\|\nabla f(x_k)\| \|D_k - \dktrue\|| \Ek3] \Prob_k[\Ek3] \nonumber \\
    &\leq \kappa_g \kappa_d M_{\tau} \Prob_k[\Ek3]. \label{eq.new3}
  \end{align}
  Combining \eqref{eq:innerprodproof1}, \eqref{eq.new1}, \eqref{eq.new2}, and \eqref{eq.new3}, the desired result follows. \qed
\end{proof}

Now, conditioned on given $k \in [\kmax]$ and $g_{[k-1]}$, let us define
\bequation \label{eq:hattaudef}
  \hat{\Tcal}_k := \min\{\Tcal_k, \tktritrue\}.
\eequation

\begin{lemma} \label{lem:dqbound}
  Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$, one finds that
  \begin{align*}
    &\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \\
    \leq&\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)] + \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M \\
    &\ + (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)).
  \end{align*}
\end{lemma}
\begin{proof}
  By the definition of $\Delta q$ in \eqref{eq:deltadef}, one has that
  \begin{align}
    &\ \E_k[\Delta q(x_k, \hat{\Tcal}_k, G_k, H_k, D_k)] \nonumber \\
    =&\ \E_k[-\hat{\Tcal}_k(G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k, 0\}) + \|c_k\|_1] \nonumber \\
    =&\ \E_k[-\hat{\Tcal}_k(G_k^\top D_k - \nabla f(x_k)^\top \dktrue  + \thalf \max\{D_k^\top H_k D_k, 0\} \nonumber \\
    &\qquad - \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\})] \nonumber \\
    &\ + \E_k[-\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\}) + \|c_k\|_1] \nonumber \\
    =&\ \E_k[\hat{\Tcal}_k(\nabla f(x_k)^\top \dktrue - G_k^\top D_k + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} \nonumber \\
    &\ - \thalf \max\{D_k^\top H_k D_k, 0\})] + \E_k[\Delta q(x_k, \hat{\Tcal}_k, \nabla f(x_k), H_k, \dktrue)]. \label{eq:dqbound1}
  \end{align}
  Now, for simplicity of notation, define
  \begin{align*}
    Q_k :=&\ \nabla f(x_k)^\top \dktrue - G_k^\top D_k \\
    &\ + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \max\{D_k^\top H_k D_k, 0\}.
  \end{align*}
  Let $E_Q$ denote the event that $Q_k \geq 0$ and let $E_Q^c$ denote the event that $Q_k < 0$ occurs.  By the Law of Total Expectation, one has that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
      &= \E_k[\hat{\Tcal}_k Q_k | E_Q] \Prob_k[E_Q] + \E_k[\hat{\Tcal}_k Q_k | E_Q^c] \Prob_k[E_Q^c] \\
      &\leq \tau_{k-1} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{\min} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c].
  \end{align*}
  Therefore, by the Law of Total Probability, Lemma \ref{lem:product_bounds}, Jensen's inequality, and convexity of $\max\{\cdot,0\}$, it follows that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
    \leq&\ \tau_{k-1} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{k-1} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    &\ + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    =&\ \tau_{k-1} \E_k[Q_k] + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    =&\ \tau_{k-1} (\nabla f(x_k)^\top \dktrue - \E_k[G_k^\top D_k] \\
    &\ + \thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \E_k[\max\{D_k^\top H_k D_k, 0\}]) \\
    &\ + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    \leq&\ \tau_{k-1} \zeta^{-1} M + (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c],
  \end{align*}
  and by similar reasoning one finds that
  \begin{align*}
    \E_k[\hat{\Tcal}_k Q_k]
    \leq&\ \tau_{\min} \E_k[Q_k | E_Q] \Prob_k[E_Q] + \tau_{\min} \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \\
    &\ + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \\
    =&\ \tau_{\min} \E_k[Q_k] + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \\
    \leq&\ \tau_{\min} \zeta^{-1} M + (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q].
  \end{align*}
  Averaging these two upper bounds, one finds that
  \begin{align}
    \E_k[\hat{\Tcal}_k Q_k] 
    \leq&\ \thalf (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M + \thalf (\tau_{k-1} - \tau_{\min}) \E_k[Q_k | E_Q] \Prob_k[E_Q] \nonumber \\
    &\ + \thalf (\tau_{\min} - \tau_{k-1}) \E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] \label{eq:dqbound2}.
  \end{align}
  Our goal now is to bound the latter two terms in \eqref{eq:dqbound2}.  Toward this end, observe that by the Cauchy-Schwarz inequality, Lemma~\ref{lem:dexpectation}, Assumption~\ref{assum:eventE}, Jensen's inequality, and concavity of the square root over $\R{}_{\geq0}$, one finds that
  \begin{align}
    &\ \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top D_k|] \nonumber \\
    \leq&\ \E_k[|\nabla f(x_k)^\top \dktrue - G_k^\top \dktrue|] +\E_k[|G_k^\top \dktrue - G_k^\top D_k|] \nonumber \\
    \leq&\ \|\dktrue\| \E_k [\|\nabla f(x_k) - G_k\|] + \E_k[\|G_k\|\|\dktrue - D_k\|] \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]} + \kappa_d \E_k[\|G_k\| \|\nabla f(x_k) - G_k\|]  \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{\E_k[\|\nabla f(x_k)-G_k\|^2]}  \nonumber \\
    &\ + \kappa_d \E_k[(\|G_k - \nabla f(x_k)\| + \|\nabla f(x_k)\|) \|\nabla f(x_k) - G_k\|] \nonumber \\
    \leq&\ \kappa_d \kappa_g \sqrt{M} + \kappa_d (M + \kappa_g \sqrt{M}) = \kappa_d \sqrt{M}(2\kappa_g + \sqrt{M}). \label{eq.wednesday1}
  \end{align}
  In addition, by the Cauchy-Schwarz inequality, Lemma~\ref{lem:dexpectation}, and Assumption~\ref{assum:eventE}, and the fact that $\|a\|^2 \leq 2(\|a - b\|^2 + \|b\|^2)$ for any $(a,b) \in \R{n} \times \R{n}$, one finds
  \begin{align}
    &\ \E_k[|\thalf \max\{(\dktrue)^\top H_k \dktrue, 0\} - \thalf \max\{D_k^\top H_k D_k, 0\}|] \nonumber \\
    \leq&\ |\thalf \max\{(\dktrue)^\top H_k \dktrue, 0\}| + \E_k[|\thalf \max\{D_k^\top H_k D_k, 0\}|] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \thalf \|H_k\|\E_k[\|D_k\|^2] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \thalf \kappa_d^2 \|H_k\|\E_k[\|G_k\|^2] \nonumber \\
    \leq&\ \thalf \|H_k\|\|\dktrue\|^2 + \kappa_d^2 \|H_k\|\E_k[\|G_k - \nabla f(x_k)\|^2 + \|\nabla f(x_k)\|^2] \nonumber \\
    \leq&\ \thalf \kappa_H \kappa_d^2 \kappa_g^2 + \kappa_H \kappa_d^2 (M + \kappa_g^2) \nonumber \\
    \leq&\ \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2). \label{eq.wednesday2}
  \end{align}
  By the Law of Total Expectation, \eqref{eq.wednesday1}, and \eqref{eq.wednesday2}, it follows that
  \begin{align*}
    \E_k[Q_k | E_Q] \Prob_k[E_Q] &= \E_k[|Q_k| | E_Q] \Prob_k[E_Q] \\
    &= \E_k[|Q_k|] - \E_k[|Q_k| | E_Q^c] \Prob_k[E_Q^c] \\
    &\leq \kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2),
  \end{align*}
  and by a similar argument, one finds that
  \begin{align*}
    -\E_k[Q_k | E_Q^c] \Prob_k[E_Q^c] &= \E_k[|Q_k| | E_Q^c] \Prob_k[E_Q^c] \\
    &= \E_k[|Q_k|] - \E_k[|Q_k| | E_Q] \Prob_k[E_Q] \\
    \leq&\ \kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2).
  \end{align*}
  The conclusion follows by combining these equations, \eqref{eq:dqbound1}, and \eqref{eq:dqbound2}. \qed
\end{proof}

Our next lemma bounds differences between expected reductions in the model of the merit function that account for cases when $\hat\Tcal_k < \Tcal_k$.

\begin{lemma} \label{lem:hattaudiff}
  Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold and let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}.  Then, for all $k \in [\kmax]$ and $g_{[k-1]}$, with $(\alpha_{\min,k}^{<},\alpha_{\min,k}^{=},\varsigma_{\max,k})$ defined as in \eqref{eq.alpha_mins} and $\hat{\Tcal}_k$ defined in \eqref{eq:hattaudef}, one finds that
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d)
  \end{align*}
  and
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k, \Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d(2 + \kappa_H \kappa_d) (M + \kappa_g^2).
  \end{align*}
\end{lemma}
\begin{proof}
  Under the stated assumptions, it follows from the stated lemma and definitions, along with the definition of $\Delta q$ in \eqref{eq:deltadef}, that
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] - \E_k[\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)] \\
    =&\ \E_k[\Acal_k (\Tcal_k - \hat{\Tcal}_k) (\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue,0\})] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) |\nabla f(x_k)^\top \dktrue + \thalf \max\{(\dktrue)^\top H_k \dktrue,0\}| \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d \kappa_g^2 + \thalf\kappa_H \kappa_d^2 \kappa_g^2),
  \end{align*}
  and, along with $\|a\|^2 \leq 2(\|a - b\|^2 + \|b\|^2)$ for any $(a,b) \in \R{n} \times \R{n}$, one finds
  \begin{align*}
    &\ \E_k[\Acal_k \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] - \E_k[\Acal_k \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k)] \\
    =&\ \E_k[\Acal_k (\hat{\Tcal}_k - \Tcal_k) (G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k,0\})] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \E_k[|G_k^\top D_k + \thalf \max\{D_k^\top H_k D_k,0\}|] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d + \thalf \kappa_d^2 \kappa_H) \E_k[\|G_k\|^2] \\
    \leq&\ (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) (\kappa_d + \thalf \kappa_d^2 \kappa_H) (2(M + \kappa_g^2)),
  \end{align*}
  which together are the desired conclusions. \qed
\end{proof}

Our next two lemmas are critical elements of our analysis.  For both lemmas, we define, for any $s \in \N{}$ and $\delta \in (0,1)$, the quantities
\bequation \label{eq:hatdelta}
    \hdelta := \frac{\delta}{\sum_{j=0}^{\min\{\smax-1,\kmax\}} \binom{\kmax}{j}}
\eequation
and
\bequation \label{eq:lsd}
  \ell(s,\hdelta) := s + \log(1/\hdelta) + \sqrt{\log(1/\hdelta)^2 + 2 s \log(1/\hdelta)}.
\eequation
The first of these lemmas bounds, with high probability, the sum of the probabilities of the occurrences of event $E_{k,3}$ over the run of the algorithm.

\begin{lemma} \label{lem:Eksumlsmax}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:eventE} hold. Then, for any $\delta \in (0,1)$,
  \bequation \label{eq:Ek3lsmax}
    \Prob\left[\sum_{k=0}^{\kmax} \Prob [E_{k,3} | E, \mathcal{F}_k] \leq \ell(\smax,\hdelta) + 1\Bigg | E \right] \geq 1-\delta.
  \eequation
\end{lemma}
\begin{proof}
  This result is proved in Appendix~\ref{app:probbounds}. \qed
\end{proof}

For our next lemma, let us define the random index set
\bequation \label{eq:Ktau}
  \Kcal_{\tau} := \{k \in [\kmax] : \Tktritrue < \Tcal_{k-1}\}.
\eequation
By the manner in which $\{\Tcal_k\}$, $\{\Tktritrue\}$, and $\{\hat{\Tcal}_k\}$ are defined, this set is always a superset of the iterations in which $\hat{\Tcal}_k < \Tcal_k$; hence, by bounding the cardinality of \eqref{eq:Ktau}, one bounds the cardinality of the set of iterations in which $\hat{\Tcal}_k < \Tcal_k$, which is needed for our main theorem.  The reason that we consider the set $\Kcal_\tau$ in \eqref{eq:Ktau} is the fact that, conditioned on the algorithm having generated a particular set of stochastic gradients up to the beginning of iteration $k$, whether or not $\tktritrue < \tau_{k-1}$ holds has already been determined; in other words, the occurrence of this inequality does not depend on $G_k$.  This means that  $G_k$ is conditionally independent of the event $\Tktritrue < \Tcal_{k-1}$ given $g_{[k-1]}$ and $E$, which is a fact that is exploited in the proof of the lemma.

\begin{lemma} \label{lem:Ktaulsmax}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold and let $\Kcal_\tau$ be defined as in \eqref{eq:Ktau}.  Then, for any $\delta \in (0,1)$, it follows that
  \bequation \label{eq:Ktaulsmax}
    \Prob\left[|\mathcal{K}_{\tau}| \leq \left\lceil \frac{\ell(\smax,\hdelta)+1}{p_{\tau}}\right\rceil \Bigg| E\right] \geq 1-\delta.
  \eequation
\end{lemma}
\begin{proof}
  This result is proved in Appendix~\ref{app:probbounds}.
\end{proof}

We are now prepared to prove a convergence rate result.

\begin{theorem} \label{thm:complexity}
  Suppose Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:eventE}, and \ref{assum:ptau} hold, let $\kappa_d \in \R{}_{>0}$ be defined by Lemma~\ref{lem:dexpectation}, define
  \bequationNN
    A_{\min} :=\ \frac{\xi_{\min} \tau_{\min}}{\tau_{\min}L + \Gamma}\ \ \text{and}\ \ A_{\max} := \frac{\xi_{-1} \tau_{-1}}{\tau_{-1}L + \Gamma},
  \eequationNN
  suppose that $\beta_k = \beta$ for all $k \in [\kmax]$ where
  \bequation\label{def.beta}
    \beta := \frac{\gamma}{\sqrt{\kmax+1}}\ \ \text{for some}\ \ \gamma \in \(0,\frac{A_{\min}}{A_{\max} + \theta}\right],
  \eequation
  define
  \bequationNN
    \baligned
      \Mbar :=&\ \tfrac14 (A_{\max} + \theta\beta) (\tau_{-1} + \tau_{\min}) \zeta^{-1} M \\
      &\ + \thalf (A_{\max} + \theta\beta) (\tau_{-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)) \\
      &\ + \theta \tau_{-1} \kappa_g \kappa_d \sqrt{M} \\
      \kappa_{E_3} :=&\ ((A_{\max} + \theta \beta)\tau_{-1} - A_{\min} \tau_{\min}) \kappa_g \kappa_d M_\tau, \\
      \kappa_{\Delta q,1} :=&\ ((A_{\max} + \theta \beta) \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d)\ \ \text{and} \\
      \kappa_{\Delta q,2} :=&\ ((A_{\max} + \theta \beta) \tau_{-1} - A_{\min} \tau_{\min}) \kappa_d (1 + \thalf \kappa_H \kappa_d) (M + \kappa_g^2),
    \ealigned
  \eequationNN
  and, for all $k \in [\kmax]$ and $g_{[k-1]}$, let $\hat{\Tcal}_k$ be defined as in \eqref{eq:hattaudef}.  Then, with $K^*$ having a discrete uniform distribution over $[\kmax]$, one finds that
  \begin{align}
    &\ \E[\Delta q(X_{K^*},\hat{\Tcal}_{K^*},\nabla f(X_{K^*}),H_{K^*},D_{K^*}^{\rm true}) | E] \nonumber \\
    \leq &\ 2\(\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \Mbar \gamma^2 + \kappa_{E_3} \gamma (\ell(\smax,\hdelta/2)+1)/\sqrt{\kmax+1}}{A_{\min} \gamma \sqrt{\kmax+1}}\) \nonumber \\
    &\ + \frac{2(\kappa_{\Delta q,1} \gamma + \kappa_{\Delta q,2} \gamma^2/\sqrt{\kmax+1})}{A_{\min} \gamma (\kmax+1)} \left\lceil\frac{\ell(\smax,\hdelta/2)+1}{p_{\tau}}\right\rceil. \label{eq:complexity}
  \end{align}
\end{theorem}
\begin{proof}
  First, consider arbitrary $k \in [\kmax]$.  By Lemmas~\ref{lem:phidecrease} and \ref{lem:innerprod}, one has that
  \begin{align*}
    &\ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k [\phi(x_k, \Tcal_k)] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) \\
    &\ + \Acal_k \Tcal_k \nabla f(x_k)^\top (D_k - \dktrue)] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue)
    + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k)] \\
    &\ + (\varsigma_{\max,k}\tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M}.
  \end{align*}
  Let $E_{k,\tau}$ be the event that $\Tktritrue \geq \tau_{k-1}$ and let $E_{k,\tau}^c$ be the complementary event that $\Tktritrue < \tau_{k-1}$.  Observe that whether $E_{k,\tau}$ or $E_{k,\tau}^c$ occurs is determined by events leading up to iteration $k$.  Hence, the bounds in Lemmas~\ref{lem:dqbound} and \ref{lem:hattaudiff} hold even if one conditions on the occurence of event $E_{k,\tau}$ or on the occurence of $E_{k,\tau}^c$.  This means that, with the bound above, \eqref{eq:hattaudef}, Lemma~\ref{lem:dqbound}, and \eqref{def.beta} (which additionally ensures that $\beta \in (0,1]$), one finds that
  \begin{align*}
    &\ \E_k [\phi(x_k + \alpha_k D_k, \Tcal_k) | E_{\tau,k}^c] - \E_k [\phi(x_k, \Tcal_k) | E_{\tau,k}^c] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    =&\ \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ -A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \thalf (A_{\max}\beta + \theta\beta^2) \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{\tau,k}^c] \\
    &\ + ((A_{\max}\beta + \theta\beta^2) \tau_{k-1} - A_{\min} \beta \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ -(A_{\min} - \thalf (A_{\max} + \theta\beta) \beta) \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \tfrac14 (A_{\max} + \theta\beta) \beta^2 (\tau_{k-1} + \tau_{\min}) \zeta^{-1} M \\
    &\ + \thalf (A_{\max} + \theta\beta) \beta^2 (\tau_{k-1} - \tau_{\min}) (\kappa_d \sqrt{M} (2\kappa_g + \sqrt{M}) + \kappa_H \kappa_d^2 (M + \tfrac32 \kappa_g^2)) \\
    &\ + ((A_{\max} + \theta\beta) \tau_{k-1} - A_{\min} \tau_{\min}) \beta \kappa_g \kappa_d M_\tau \Prob_k[\Ek3 | E_{\tau,k}^c] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\
    \leq&\ - \thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}^c] \\
    &\ + \kappa_{E_3} \beta \Prob_k[\Ek3 | E_{\tau,k}^c] + \Mbar \beta^2,
  \end{align*}
  and, since $\Tktritrue \geq \tau_{k-1} \geq \Tcal_k$ in~$E_{k,\tau}$, one finds with Lemma~\ref{lem:hattaudiff} that
  \begin{align*}
    &\ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k) | E_{k,\tau}] - \E_k [\phi(x_k, \Tcal_k) | E_{k,\tau}] \\
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    &\ + \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    &\ - \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    &\ + (\varsigma_{\max,k}\tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_g \kappa_d M_\tau \Prob_k[\Ek3] + \theta \beta^2 \tau_{k-1} \kappa_g \kappa_d \sqrt{M} \\ 
    \leq&\ \E_k[-\Acal_k \Delta q(x_k,\Tcal_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\Tcal_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    &\ - \thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}] \\
    &\ - \E_k[-\Acal_k \Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) + \thalf \Acal_k \beta  \Delta q(x_k,\hat{\Tcal}_k,G_k,H_k,D_k) | E_{k,\tau}] \\
    &\ + \kappa_{E_3} \beta \Prob_k[\Ek3 | E_{\tau,k}] + \Mbar \beta^2 \\ 
    \leq&\ -\thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}] \\
    &\ + (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d \kappa_g^2(1 + \thalf \kappa_H \kappa_d) \\
    &\ + \thalf (\varsigma_{\max,k} \tau_{k-1} - \alpha_{\min,k}^{<} \tau_{\min}) \kappa_d(2 + \kappa_H \kappa_d) (M + \kappa_g^2) \beta \\
    &\ + \kappa_{E_3} \beta \Prob_k[E_{k,3} | E_{k,\tau}] + \Mbar \beta^2 \\
    \leq&\ -\thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E_{\tau,k}] \\
    &\ + \kappa_{E_3} \beta \Prob_k[E_{k,3} | E_{k,\tau}] + \Mbar \beta^2 + \kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2.
  \end{align*}
  Hence, by the laws of total probability and expectation, one finds that
  \begin{align*}
    &\ \E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k[\phi(x_k, \Tcal_k)] \\
    =&\ (\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)|E_{k,\tau}] - \E_k[\phi(x_k, \Tcal_k)| E_{k,\tau}]) \Prob_k[E_{k,\tau}] \\
    &\ + (\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)|E_{k,\tau}^c] - \E_k[\phi(x_k, \Tcal_k)| E_{k,\tau}^c]) \Prob_k[E_{k,\tau}^c] \\
    \leq&\ -\thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)] \\
    &\ + \kappa_{E_3} \beta \Prob_k[E_{k,3}] + \Mbar \beta^2 + (\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2) \Prob_k[E_{k,\tau}]
  \end{align*}
  Summing this inequality for all $k \in [\kmax]$ yields
  \begin{align*}
    &\ \sum_{k=0}^{\kmax} (\E_k [\phi(x_k + \Acal_k D_k, \Tcal_k)] - \E_k[\phi(x_k, \Tcal_k)]) \\
    \leq&\ \sum_{k=0}^{\kmax} (-\thalf A_{\min} \beta \E_k[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue)]) \\
    &\ + \sum_{k=0}^{\kmax} (\kappa_{E_3} \beta \Prob_k[E_{k,3}] + (\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2) \Prob_k[E_{k,\tau}]) + (\kmax + 1) \Mbar \beta^2.
  \end{align*}
  
  Let us now turn to analyzing the overall behavior of the algorithm through iterations $k \in [\kmax]$.  Let $f_{G_{[\kmax]}}$ denote the probability density function of $G_{[\kmax]}$ and observe that, for all $k \in [\kmax]$, one finds $\Prob_k[E_{k,\tau}] \in \{0,1\}$ since, when conditioned on $E$ and $\Fcal_k$, the event $E_{k,\tau}$ is independent of $G_k$.  Therefore, by the bound above, the law of total expectation, Lemma \ref{lem:Eksumlsmax}, Lemma \ref{lem:Ktaulsmax}, and the union bound, it follows that, with probability at least $1-\delta$, one finds
  \begin{align}
    &\ \sum_{k=0}^{\kmax} (\E[\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_{k+1}] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_{k+1}]) \nonumber \\
    =&\ \int_{g_{[\kmax]} \in \Fcal_{\kmax+1}} \sum_{k=0}^{\kmax} \E[\phi(x_k + \Acal_k D_k, \Tcal_k) - \phi(x_k,\Tcal_k) | E, G_{[\kmax]} = g_{[\kmax]}] \nonumber \\
    &\hspace{1.3in} \cdot f_{G_{[\kmax]}}(g_{[\kmax]}) \textrm{d}g_{[\kmax]} \nonumber \\
    \leq&\ \int_{g_{[\kmax]} \in \Fcal_{\kmax+1}} \Bigg(-\thalf A_{\min} \beta \sum_{k=0}^{\kmax} \E[\Delta q(x_k,\hat{\Tcal}_k,\nabla f(x_k),H_k,\dktrue) | E, G_{[\kmax]} = g_{[\kmax]}] \nonumber \\
    &\hspace{1.3in} + \kappa_{E_3} \beta \sum_{k=0}^{\kmax} \Prob[\Ek3 | E, G_{[\kmax]} = g_{[\kmax]}] \nonumber \\
    &\hspace{1.3in} + (\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2) \sum_{k=0}^{\kmax} \Prob[E_{k,\tau} | E, G_{[\kmax]} = g_{[\kmax]}] \Bigg) \nonumber \\
    &\hspace{1.3in} \cdot f_{G_{[\kmax]}}(g_{[\kmax]}) \textrm{d}g_{[\kmax]} \nonumber \\
    &\ + (\kmax+1) \Mbar \beta^2 \nonumber \\
    =&\ -\thalf A_{\min} \beta \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue) | E, \Fcal_k] \nonumber \\
    &\ + \kappa_{E_3} \beta \sum_{k=0}^{\kmax} \Prob[\Ek3 | E, \Fcal_k] + (\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2) \E[|\Kcal_\tau| | E] + (\kmax + 1) \Mbar \beta^2 \nonumber \\
    \leq&\ -\thalf A_{\min} \beta \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue) | E, \Fcal_k] \nonumber \\
    &\ + \kappa_{E_3} \beta (\ell(\smax,\hdelta/2)+1) \nonumber \\
    &\ + (\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2) \left\lceil\frac{\ell(\smax,\hdelta/2)+1}{p_{\tau}}\right\rceil + (\kmax+1) \Mbar \beta^2. \label{eq:complexityproof1}
  \end{align}
  The left-hand side of this inequality satisfies
  \begin{align}
    &\ \sum_{k=0}^{\kmax} (\E [\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_{k+1}] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_{k+1}]) \nonumber \\
    =&\ \sum_{k=0}^{\kmax} \Bigg( \E[\Tcal_k (f(X_k + \Acal_k D_k) - f_{\min}) + \|c(X_k + \Acal_k D_k)\|_1 | E,\Fcal_{k+1}] \nonumber \\
    &\hspace{0.45in} - \E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E,\Fcal_{k+1}] \Bigg). \label{eq.newnumb}
  \end{align}
  It follows by the merit parameter updating strategy and the definition of the filtration (which in particular guarantees that $\Tcal_{k-1}$ and $X_k$ are fully determined by $G_{[k-1]}$, and are therefore conditionally independent of $\Fcal_{k+1}$) that, for all $k \in [\kmax]$, one finds
  \bequationNN
    \baligned
      &\ -\E[\Tcal_k (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_{k+1}] \\
      \geq&\ - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_{k+1}] \\
      =&\ - \E[\Tcal_{k-1} (f(X_k) - f_{\min}) + \|c(X_k)\|_1 | E, \Fcal_k],
    \ealigned
  \eequationNN
  Thus, from \eqref{eq.newnumb}, it follows that
  \begin{align*}
    &\ \sum_{k=0}^{\kmax} (\E[\phi(X_k + \Acal_k D_k, \Tcal_k) | E, \Fcal_{k+1}] - \E[\phi(X_k,\Tcal_k) | E, \Fcal_{k+1}]) \\
    \geq&\ \E[\Tcal_{\kmax} (f(X_{\kmax+1}) - f_{\min}) + \|c(X_{\kmax+1})\|_1 | E,\Fcal_{\kmax+1}] - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) - \|c_0\|_1.
  \end{align*}
  Combining this with \eqref{eq:complexityproof1}, one obtains that
  \begin{align*}
    &\ \frac{\beta}{\sum_{k=0}^{\kmax} \beta} \sum_{k=0}^{\kmax} \E[\Delta q(X_k,\hat{\Tcal}_k,\nabla f(X_k),H_k,\Dktrue) | E, \Fcal_k] \\
    \leq &\ 2\(\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (\kmax+1) \Mbar \beta^2 + \kappa_{E_3} \beta (\ell(\smax,\hdelta/2)+1)}{A_{\min} {\sum_{k=0}^{\kmax} \beta}}\) \nonumber \\
    &\ + \frac{2(\kappa_{\Delta q,1} \beta + \kappa_{\Delta q,2} \beta^2)}{A_{\min} {\sum_{k=0}^{\kmax} \beta}} \left\lceil\frac{\ell(\smax,\hdelta/2)+1}{p_{\tau}}\right\rceil.
  \end{align*}
  Hence, by the definitions of $K^*$ and $\beta$, the desired conclusion follows. \qed
\end{proof}

The following corollary translates the result of the preceding theorem to a result pertaining to a stationary measure of \eqref{eq:fdef}; recall \eqref{eq:optconds}.

\begin{corollary} \label{coro:complexity}
  Under the assumptions and conditions of Theorem \ref{thm:complexity}, it holds with probability at least $1-\delta \in (0,1)$ that
  \begin{align*}
    &\ \E\left[\frac{\|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\|^2}{\kappa_H^2} + \|c(X_{K^*})\|_1 \Bigg| E\right] \\
    \leq&\ 2 (\kappa_\Psi + 1) \(\frac{\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \Mbar \gamma^2}{\kappa_q \tau_{\min} A_{\min} \gamma \sqrt{\kmax+1}}\) \\
    &\ + 2(\kappa_\Psi + 1) \(\frac{\kappa_{E_3} \gamma (\ell(\smax,\hdelta/2)+1)}{\kappa_q \tau_{\min} A_{\min} \gamma \sqrt{\kmax+1}}\) \\
    &\ + (\kappa_\Psi + 1) \(\frac{2(\kappa_{\Delta q,1} \gamma + \kappa_{\Delta q,2} \gamma^2/\sqrt{\kmax+1})}{\kappa_q \tau_{\min} A_{\min} \gamma (\kmax+1)}\) \left\lceil\frac{\ell(\smax,\hdelta/2)+1}{p_{\tau}}\right\rceil.
  \end{align*}
  Hence, the worst-case complexity bound described in Section~\ref{sec.preview} holds.
\end{corollary}
\begin{proof}
  The result follows by Lemma \ref{lem:kappapsi}, Lemma \ref{lem:kappaq}, and Theorem \ref{thm:complexity} combined with \eqref{eq:sqpsystemdet}, which implies that
  \bequationNN
    \|\nabla f(X_{K^*}) + J_{K^*}^\top Y_{K^*}^{true}\| = \|H_{k^*} D^{true}_{K^*}\| \leq \kappa_H \|D^{true}_{K^*}\|.
  \eequationNN
  The worst-case complexity bound described in Section~\ref{sec.preview} follows by combining this result with the definitions of $\kappa_{E_3}$, $\kappa_{\Delta q,1}$, $\kappa_{\Delta q,2}$, and Lemma \ref{lem:Orderlsd} in Appendix \ref{app:probbounds}.
  \qed
\end{proof}

Again, we remark that this result, when viewed in terms of the squared norm of the gradient of the Lagrangian, matches the worst-case complexity of the stochastic gradient method for the unconstrained setting~\cite{DDavis_DDrusvyatskiy_2019}.

%************
% Subsection
%************
\subsection{Complexity Result for Symmetric Sub-Gaussian Distributions} \label{subsec:subgauss}

In this section, we show that Assumptions \ref{assum:eventE} and \ref{assum:ptau} occur with high probability when the stochastic gradient $G_k$ follows a symmetric, sub-Gaussian distribution.

Throughout this section, we work with the following assumption.

\begin{assumption} \label{assum:symmsubgauss}
    There exists $M \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, the stochastic gradient $G_k$ satisfies
    \bequation
        \E[G_k | g_{[k-1]}] = \nabla f(x_k),
    \eequation
    \bequation \label{eq:subgauss}
        \E[\exp(\|G_k-\nabla f(x_k)\|^2/M) | g_{[k-1]}] \leq \exp(1),
    \eequation
    and the quantities $G_k - \nabla f(x_k)$ and $\nabla f(x_k) - G_k$ are equivalent in distribution. Finally, for all $k \in [\kmax]$, the ratio parameter $\xi_k$ satisfies $\xi_k = \xi_{\min}$.
\end{assumption}

The above assumption has a number of important implications. The first is that Assumption \ref{assum:ptau} occurs (without conditioning on event $E$) with $p_{\tau} = \frac12$, as we show in the following lemma.

\blemma \label{lem:subgptau}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then,
    \bequationNN
      \baligned
        \Prob[& G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} \geq \\
        & \nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} | g_{[k-1]}] \geq \frac12.
      \ealigned
    \eequationNN
\elemma

\bproof
    Let $Z_k$ be a basis for the null space of $J_k$, which under Assumption \ref{assum:fcsmooth} is a matrix in $\R{n\times(n-m)}$. Then, let $W_k$ be the random variable in $\R{n-m}$ such that $U_k = Z_k W_k$ and $\wktrue$ in $\R{n-m}$ be such that $\uktrue = Z_k \wktrue$. It follows from the first block in \eqref{eq:sqpsystem} that 
    \bequationNN
        H_k (Z_k W_k + v_k) + J_k^\top Y_k = -G_k \Longleftrightarrow Z_k W_k = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (G_k + H_k v_k).
    \eequationNN
    Using this equality and simplifying,
    \bequationNN
        G_k^\top D_k + D_k^\top H_k D_k = v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} G_k + H_k^{1/2} v_k).
    \eequationNN
    In a similar fashion, by \eqref{eq:sqpsystemdet},
    \bequationNN
        Z_k \wktrue = -Z_k (Z_k^\top H_k Z_k)^{-1} Z_k^\top (\nabla f(x_k) + H_k v_k)
    \eequationNN
    so that
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + (\dktrue)^\top H_k \dktrue \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} \nabla f(x_k) + H_k^{1/2} v_k).
    \end{align*}

    Then,
    \begin{align*}
        &G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (G_k -\nabla f(x_k))),
    \end{align*}
    and,
    \begin{align*}
        &\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \\
        &= v_k^\top H_k^{1/2}(I - H_k^{1/2} Z_k(Z_k^\top H_k Z_k)^{-1} Z_k^\top H_k^{1/2})(H_k^{-1/2} (\nabla f(x_k) - G_k)),
    \end{align*}
    which are equivalent in distribution by Assumption \ref{assum:symmsubgauss}. Therefore,
    \begin{align*}
        &\Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &=\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}].
    \end{align*}
    In addition, we have
    \begin{align*}
        1 &= \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \\
        &+\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} \geq 0 | g_{[k-1]}] \\
        &-\Prob[\nabla f(x_k)^\top \dktrue + \max\{(\dktrue)^\top H_k \dktrue,0\} - G_k^\top D_k - \max\{D_k^\top H_k D_k,0\} = 0 | g_{[k-1]}].
    \end{align*}
    Taking these two together, it follows that
    \bequationNN
        \Prob[G_k^\top D_k + \max\{D_k^\top H_k D_k,0\} - \nabla f(x_k)^\top \dktrue - \max\{(\dktrue)^\top H_k \dktrue,0\} \geq 0 | g_{[k-1]}] \geq \frac12,
    \eequationNN
    proving the claim. \qed
\eproof

Next, we repeat a well known property of sub-Gaussian random variables.
\blemma \label{lem:subgboundedrv}
    Suppose Assumption \ref{assum:symmsubgauss} holds. Then, for any $\delta \in (0,1)$,
    \bequation \label{eq:subgboundedrv}
        \Prob\left[\underset{k \in [\kmax]}{\max} \|G_k - \nabla f(X_k)\| \leq \sqrt{M \left(1 + \log \left(\frac{\kmax+1}{\delta}\right)\right)}\right] \geq 1 - \delta.
    \eequation
\elemma

\bproof
    By Markov's inequality,
    \begin{align*}
        &\Prob\left[\underset{k \in [\kmax]}{\max} \|G_k - \nabla f(X_k)\|^2 > M \left(1 + \log \left(\frac{\kmax+1}{\delta}\right)\right)\right] \\
        &= \Prob\left[\exp\left(\underset{k \in [\kmax]}{\max} \|G_k - \nabla f(X_k)\|^2/M\right) > \exp\left(1 + \log\left(\frac{\kmax+1}{\delta}\right)\right)\right] \\
        &\leq \exp\left(-1 - \log \left(\frac{\kmax+1}{\delta}\right)\right)\E\left[\exp\left(\underset{k \in [\kmax]}{\max} \|G_k - \nabla f(X_k)\|^2/M\right)\right] \\
        &= \exp\left(-1 - \log \left(\frac{\kmax+1}{\delta}\right)\right)\E\left[\underset{k \in [\kmax]}{\max} \exp\left(\|G_k - \nabla f(X_k)\|^2/M\right)\right] \\
        &\leq \exp\left(-1 - \log \left(\frac{\kmax+1}{\delta}\right)\right)\sum_{k=0}^{\kmax} \E\left[\exp\left(\|G_k - \nabla f(X_k)\|^2/M\right)\right]
    \end{align*}
    
    Next, let $f_{G_{[\kmax]}}$ denote the probability density function of $G_{[\kmax]}$. Then, by the law of total expectation and Assumption \ref{assum:symmsubgauss},
    \begin{align*}
       &\quad \sum_{k=0}^{\kmax} \E\left[\exp\left(\|G_k - \nabla f(X_k)\|^2/M\right)\right] \\
       &= \int_{g_{[\kmax]} \in \Fcal_{\kmax+1}} \sum_{k=0}^{\kmax} \E\left[\exp\left(\|G_k - \nabla f(X_k)\|^2/M\right) \bigg| G_{[\kmax]} = g_{[\kmax]} \right] \\ &\hspace{1.4in} \cdot f_{G_{[\kmax]}}(g_{[\kmax]}) \textnormal{d}g_{[\kmax]} \\
       &\leq \int_{g_{[\kmax]} \in \Fcal_{\kmax+1}} \sum_{k=0}^{\kmax} \E\left[\exp(1) \right] f_{G_{[\kmax]}}(g_{[\kmax]})  = (\kmax + 1) \exp(1).
    \end{align*}
    Therefore,
    \begin{align*}
        &\Prob\left[\underset{k \in [\kmax]}{\max} \|G_k - \nabla f(X_k)\|^2 > M \left(1 + \log \left(\frac{\kmax+1}{\delta}\right)\right)\right] \\
        &\leq \exp\left(-1 - \log \frac{\kmax+1}{\delta}\right) (\kmax + 1) \exp(1) \\
        &= \exp(-1) \frac{\delta}{\kmax+1} (\kmax+1)\exp(1) = \delta,
    \end{align*}
    
    which proves the result. \qed
\eproof

We conclude this section by showing that under Assumption \ref{assum:symmsubgauss}, event $E$ as defined in Assumption \ref{assum:eventE} occurs with high probability.

\blemma \label{lem:subgeventE}
    Suppose that Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, and \ref{assum:symmsubgauss} hold. Then, there exists a constant $\kappa_{\tau_{\min}}$ such that, with probability at least $1-\delta$, event $E$ of Assumption \ref{assum:eventE} occurs with
    \begin{align*}
        M_\tau &= \sqrt{M \left(1 + \log\left( \frac{\kmax+1}{\delta}\right)\right)} \\
        \tau_{\min} &= \frac{(1-\sigma)(1-\epsilon_\tau)}{\kappa_{\tau_{\min}}}, \\
        \textnormal{and} \ \smax &= \min\left\{\kmax + 1, \left\lceil\frac{\log \left(\frac{\tau_{-1}\kappa_{\tau_{\min}}}{(1-\sigma)(1-\epsilon_\tau)}\right)}{\log\left(\frac{1}{1 - \epsilon_\tau}\right)}\right\rceil\right\},
    \end{align*}
    where
    \begin{align*}
        \kappa_{\tau_{\min}} &= \kappa_v \Bigg(\kappa_g + \sqrt{M \left(1 + \log\left(\frac{\kmax+1}{\delta}\right)\right)} \\
        &\quad+ \frac{\kappa_H}{\zeta} \left(\sqrt{M \left(1 + \log\left(\frac{\kmax+1}{\delta}\right)\right)} + \kappa_g + \zeta + \kappa_H \kappa_v \kappa_c\right)\Bigg),
    \end{align*}
    where $\kappa_v$ defined in \cite[Lemma 2.9]{ABerahas_FECurtis_DPRobinson_BZhou_2021} and $\kappa_c$ is a bound on $\|c\|_2$ that is guaranteed by Assumption \ref{assum:fcsmooth}.
\elemma

\bproof
    We begin the proof by noting that by Jensen's inequality and the convexity of $\exp(\cdot)$,
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2| g_{[k-1]}] \leq M.
    \eequationNN
    The bound on $M_\tau$ follows directly from Lemma \ref{lem:subgboundedrv}. The bound on $\tau_{\min}$ follows by the arguments of \cite[Lemma 2.15 and 2.16]{ABerahas_FECurtis_DPRobinson_BZhou_2021} combined with \eqref{eq:subgboundedrv}. Finally, the bound on $\smax$ follows from combining the bound on $\tau_{\min}$ with \eqref{eq:smaxbound} and the properties of logarithms. \qed
\eproof

\iffalse
\tred{Update 4/20 that I don't know where to put right now.}

We can also get a similar (though looser bound) for the case where we just have bounded variance!

\blemma \label{lem:boundeddiffvariance}
    For all $k \in \{0,\dots,\kmax\}$, let
    \bequationNN
        \E[\|G_k - \nabla f(x_k)\|^2 | \mathcal{F}_k] \leq M.
    \eequationNN
   Then,
    \bequationNN
        \Prob\left[\underset{0 \leq k \leq \kmax}{\max} \|G_k - \nabla f(x_k)\| \leq \sqrt{\frac{(\kmax+1)M}{\delta}}\right] \geq 1-\delta.
    \eequationNN
\elemma

\bproof
    Let $g := \{g_0,\dots,g_{\kmax}\}$ denote any sequence of stochastic gradients that is measurable with respect to the filtration $\mathcal{F}_{\kmax}$. Then, by Markov's inequality, concavity of the square root, Jensen's inequality, and the law of total expectation,
    \begin{align*}
        &\Prob\Bigg[\underset{0 \leq k \leq \kmax}{\max} \|G_{k} - \nabla f(x_k)\|^2 > \frac{(\kmax+1)M}{\delta}\Bigg] \\
        &\leq \E\left[\underset{0 \leq k \leq \kmax}{\max} \|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(\kmax+1)M} \\
        &\leq \sum_{k=0}^{\kmax} \E\left[\|G_{k} - \nabla f(x_k)\|^2\right] \frac{\delta}{(\kmax+1)M} \\
        &= \frac{\delta}{(\kmax+1)M} \sum_{k=0}^{\kmax} \int_{g \in \mathcal{F}_{\kmax}} \E\left[\|G_{k} - \nabla f(x_k)\|^2 | G_{0} = g_{0}, \dots, G_{k-1} = g_{k-1}\right] f_{G} dg \\
        &\leq \frac{\delta}{(\kmax+1)M} (\kmax + 1) M \int_{g \in \mathcal{F}_{\kmax}} f_{G}(g) dg = \delta,
    \end{align*}
    where $f_G(g)$ is the probability density function of the random variable $G$.
\eproof

What does this mean for our results? We can repeat the proof of Lemma \ref{lem:subgeventE} so that with probability at least $1-\delta$,
\bequationNN
    \tau_{\min} = \mathcal{O}\left(\sqrt{\frac{\delta}{\kmax+1}}\right)
\eequationNN
and, for sufficiently large $\kmax$,
\bequationNN
    \smax = \mathcal{O}\left(\log \sqrt{\frac{\kmax+1}{\delta}}\right). 
\eequationNN
Thus,
\bequationNN
    \frac{\smax}{\sqrt{\kmax+1}} = \mathcal{O} \left(\frac{\log \sqrt{\frac{\kmax+1}{\delta}}}{\sqrt{\kmax+1}} \right),
\eequationNN
which means we can always get a useful complexity result, so long as $\kmax$ is sufficently large.

Unfortunately, because the bound from Lemma \ref{lem:boundeddiffvariance} is $\mathcal{O}(\sqrt{\kmax+1})$, we cannot use this approach to directly bound $\ktaudec$ and obtain a meaningful complexity result. Thus, additional assumptions are still needed in this case.
\fi

%************
% Subsection
%************
\subsection{Complexity Result with Decreasing Ratio Parameter} \label{subsec:ratioparam}

In this section, we relax Assumption \ref{assum:eventE} with respect to the random variable $\{\Xi_k\}$ and allow it to be adaptive over the course of the algorithm. Due to the definition of $\{\Xi_k\}$, it satisfies a deterministic lower-bound, $\xi_{\min}$, such that $\xi_k \geq \xi_{\min} > 0$ holds for all $k$ \cite[Lemma 3.5]{ABerahas_FECurtis_DPRobinson_BZhou_2021}. Therefore, it follows that there exists a maximum number of decreases of $\xi$, which we denote by $r_{\max}$, that satisfies
\bequationNN
    r_{\max} \leq \min\left\{\kmax+1, \left\lceil \frac{\log(\xi_{\min}/\xi_{-1})}{\log(1-\epsilon_\xi)} \right\rceil\right\}.
\eequationNN
To formalize our new assumption, we define the event
\bequationNN
    E_{\xi} := E(\kmax,\smax,r_{\max},\tau_{\min},\xi_{\min}),
\eequationNN
which we define as the event such that, in every realization of the algorithm, the merit parameters $\{\tau_k\}^{\kmax}_0$ and ratio parameters $\{\xi_k\}^{\kmax}_{k=0}$ satisfy

\bitemize
  \item $\tau_k \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\tktritrue \geq \tau_{\min} > 0$ for all $k \in [\kmax]$,
  \item $\xi_k \geq \xi_{\min} > 0$ for all $k \in [\kmax]$,
  \item $|\{k \in [\kmax] : \tau_k < \tau_{k-1}\}| \leq \smax$, and
  \item $|\{k \in [\kmax] : \xi_k < \xi_{k-1}\}| \leq r_{\max}$.
\eitemize
We note once again that the conditions on $\xi_k$ hold \textit{deterministically}, so this event is identical to event $E$ defined in \eqref{def:E}, with the exception that $\xi_k$ may be adaptively updated.

For the remainder of this section, let
\bequationNN
    \Prob_k[\cdot] := \Prob[\cdot | E_{\xi}, G_{[k-1]} = g_{[k-1]}] \quad \and \quad \E_k[\cdot] := \Prob[\cdot | E_{\xi}, G_{[k-1]} = g_{[k-1]}]
\eequationNN
Now, we can state our new assumption.

\bassumption\label{assum:eventExi}
  There exists $M \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that
  \bequationNN
    \E_k[G_k] = \nabla f(x_k) \quad \text{and} \quad
     \E_k[\|G_k - \nabla f(x_k)\|_2^2] \leq M.
  \eequationNN
  In addition, there exist $M_1 \in \R{}_{>0}$, $M_2 \in \R{}_{>0}$, and $M_3 \in \R{}_{>0}$ such that, for all $k \in [\kmax]$ and any realization $g_{[k-1]}$ of $G_{[k-1]}$, one finds that\footnote{\textcolor{red}{MON: I didn't change this assumption to add the either $\P = 0$ or $\E \leq M$ that was added to Assumption \ref{assum:eventE} because I didn't feel it was that important and didn't want to add three more lines to the statement of the assumption.}}
  \bequationNN
    \baligned
      \E_k[\|G_k - \nabla f(x_k)\| &|\nabla f(x_k)^\top(D_k - \dktrue)) < 0, \Tcal_k < \tau_{k-1}, \Xi_k = \xi_{k-1}] \leq \kappa_1, \\
      \E_k[\|G_k - \nabla f(x_k)\| &|\nabla f(x_k)^\top(D_k - \dktrue)) < 0, \Tcal_k = \tau_{k-1}, \Xi_k < \xi_{k-1}] \leq \kappa_2, \\
      \E_k[\|G_k - \nabla f(x_k)\| &|\nabla f(x_k)^\top(D_k - \dktrue)) < 0, \Tcal_k < \tau_{k-1}, \Xi_k < \xi_{k-1}] \leq \kappa_3.
    \ealigned
  \eequationNN
\eassumption

This assumption is largely the same as Assumption \ref{assum:eventE}. The major new requirement due to the adaptive $\{\Xi_k\}$ sequence is the addition of two more events under which the norm difference of $G_k$ and $\nabla f(x_k)$ is bounded.

We remark that this assumption holds with high-probability under Assumption \ref{assum:symmsubgauss} (without the condition that $\xi_k = \xi_{\min}$), a result which can easily be derived by simple modification of the techniques used in Section \ref{subsec:subgauss}. We leave this derivation as an exercise for the reader.

The complexity analysis for this case follows by essentially the same arguments as those used to derive a complexity result under Assumption \ref{assum:eventE}. A slight modification of Lemma \ref{lem:innerprod} is needed to include the three events related to $\nabla f(x_k)^\top(D_k-\dktrue)$ that appear in Assumption \ref{assum:eventExi} (as opposed to the one in Assumption \ref{assum:eventE}), which yields a result in terms of the probabilities of these three events. Then, a slightly modified Lemma \ref{lem:Eksumlsmax} and the union bound can be applied two additional times to derive a complexity result. Since the analysis is a relatively straightforward extension of the results in Section \ref{subsec:complexity}, we simply state our complexity result here.
\begin{theorem}
    Let Assumptions \ref{assum:fcsmooth}, \ref{assum:Hk}, \ref{assum:ptau}, and \ref{assum:eventExi} hold. Then, with probability at least $1-\delta$,
    \begin{align*}
        &\E[\|\nabla f(x_{k^*}) + J_{k^*}^\top y_{k^*}^{true}\|^2 + \|c_{k^*}\| |
        E_{\xi}] \\
        &= \mathcal{O}\Bigg(\frac{\tau_{-1}(f_0 - f_{\min}) + \|c_0\|_1 + M}{\sqrt{\kmax+1}} \\
        &\quad+ \frac{(\tau_{-1}\xi_{-1} - \tau_{\min}\xi_{\min})(\log(\kmax)(\smax + r_{\max}) + \log(1/\delta))}{\sqrt{\kmax+1}}\Bigg).
    \end{align*}
\end{theorem}

\bproof
    We leave the proof as an exercise for the reader. \qed
\eproof

%*********
% Section
%*********
\section{Conclusion} \label{sec:conclusion}

In this work, we derived the first worst-case complexity result for an adaptive stochastic algorithm for equality constrained optimization. We developed a stochastic SQP algorithm with an adaptive $\ell$-1 merit function, based on the framework proposed in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2021}. While key to a practical algorithm, the adaptivity in the merit function introduced a number of theoretical challenges to overcome. Under mostly standard assumptions, we prove that, with high probability, the expected value of the norm of the gradient of the Lagrangian decays at a rate of $k^{-4}$ (ignoring log factors), matching the worst-case complexity of the stochastic gradient method. We believe the theoretical tools developed within may be applicable to a broad class of constrained stochastic optimization methods that utilize an adaptive merit function. 

\iffalse
OLD STUFF BELOW:

%************
% Subsection
%************
\subsection{Quick Complexity Highlight}
Quick highlight of the main complexity result for meeting on 3/9/2021:

Let $\mathcal{I} \subseteq \{0,1,\dots,\kmax\}$ denote the index set of ``good" iterations. Overall analysis will lead to a result of the form (with $\beta_k := \beta = \gamma/\sqrt{\kmax+1}$:
\begin{align*}
    &\sum_{k \in \mathcal{I}} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\quad\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &\quad+ C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau}.
\end{align*}
To get the expectation that we want, we need to add and subtract:
\begin{align*}
    &\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)] \\
    &\leq 2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M}) \\
    &+ C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + \sum_{k \in \mathcal{I}^c} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)].
\end{align*}
Then, because the number of ``bad" iterations is bounded by $\ell(\smax,\delta)/p_{\tau}$,
\begin{align*}
    &\frac{\sum_{k=0}^{\kmax} \beta \E_k [\Delta q(x_k, \tau_k, \nabla f(x_k), H_k, \dktrue)]}{\sum_{k=0}^{\kmax} \beta} \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\sum_{k=0}^{\kmax} \beta} \\
    &+ \frac{C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + C_4 \ell(\smax,\delta)/p_{\tau}}{\sum_{k=0}^{\kmax} \beta}.
\end{align*}
So that,
\begin{align*}
    &\E [\Delta q(x^*, \tau^*, \nabla f(x^*), H^*, d^{*,true})] \\
    &\leq 2 \frac{(\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\sqrt{\kmax + 1}} \\
    &+ \frac{C_1 \ell(\smax,\delta)
    + C_2 \ell(r_{\max},\delta) + C_3 \ell(\smax,\delta)/p_{\tau} + C_4 \ell(\smax,\delta)/p_{\tau}}{\sqrt{\kmax+1}}.
\end{align*}

Algorithm \ref{alg:ssqp} generates a random process $\{\bar{G}_k,X_k,\bar{D}_k,\bar{\mathcal{T}}_k,\bar{\Xi}_k,\bar{\mathcal{A}}_k\}$. We will denote all random quantities by capital letters and their realizations by small letters. The random gradient estimate is denoted by $\bar{G}_k$ and its realizations by $\bar{g}_k = \bar{G}_k(\omega)$. Similarly, let the random quantities $x_k = X_k(\omega)$ (iterates), $\bar{d}_k = \bar{D}_k(\omega)$ (search directions), $\btau_k = \bar{\mathcal{T}}_k(\omega)$ (merit parameter), $\bxi_k = \bar{\Xi}_k(\omega)$ (reduction ratio), and $\bar{\alpha}_k = \bar{\mathcal{A}}_k(\omega)$ (step sizes) denote their respective realizations. We will assume that the estimates $\bar{G}_k$ obey some standard properties, conditioned on the past.

To formalize conditioning on the past, let $\mathcal{F}_k$ denote the $\sigma$-algebra generated by the random variables $\bar{G}_0, \dotsc \bar{G}_{k-1}$. For completness, we set $\mathcal{F}_{-1} = \sigma(x_0)$. As a result, we have that $\mathcal{F}_{k}$ for $k \geq -1$ is a filtration.

Let $E_{\tau,low}$ denote the event that the merit parameter sequence eventually remains constant at a sufficiently small positive value.
We will derive our complexity result under the assumption that this event occurs.

\begin{assumption} \label{assum:taulow}
Event $E_{\tau,low}$ occurs in the sense that there exists an iteration
number $\bar{k}_{\tau,\xi} \in \mathbb{N}$ and a merit parameter value
$\btau_{\min} \in \R{}_{>0}$ such that
\begin{equation} \label{eq:taumin}
    \btau_k = \btau_{\min} \leq \btau_k^{trial} \quad and \quad
    \xi_k = \xi_{\min} \quad for \; all \quad k \geq \bar{k}_{\tau,\xi}.
\end{equation}
In addition, the sequence of random gradients $\bar{G}_k$ generated by Algorithm \ref{alg:ssqp} satisfies
\begin{equation*}
    \E_{k,\tau,small}[\bar{G}_k] = g_k \quad and \quad \E_{k,\tau,small}[\|\bar{G}_k - g_k\|^2] \leq M
\end{equation*}
where $\E_{k,\tau,small}$ denotes expectation with respect to the distribution of $\omega$ conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_{k}$.
\end{assumption}

For the rest of this section, let $\Prob_k[\cdot]$ ($\E_k[\cdot]$) denote the probabilty (expectation) conditioned on the event that $E_{\tau,low}$ occurs and the filtration $\mathcal{F}_k$.

Our analysis relies on the following three events. For all $k$, let $\Ek1$ be the event that $g_k^\top(\bd_k - d_k) \geq 0$, let $\Ek2$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} = \btau_{k-1}$, and let $\Ek3$ be the event that $g_k^\top(\bd_k - d_k) < 0$ and $\btau_{k} < \btau_{k-1}$.

We require an additonal assumption to obtain our complexity result:
\begin{assumption} \label{assum:boundedrv}
There exists $\kappa_{\Ek3} > 0$ such that
\begin{equation} \label{eq:boundedrv}
    \E_k [\|\bar{g}_k-g_k\||\Ek3] \leq \kappa_{E_3}.
\end{equation}
\end{assumption}
The above assumption holds under a number of conditions, including when
$\bar{g}_k$ is a bounded random vector.

%NEW
\textcolor{red}{TODO:} Ignoring $\xi_k$ for now. Will probably need additional cases in the proof eventually...

\begin{lemma} \label{lem:innerprodold}
Suppose that Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\kappa_g \in \R{}_{>0}$ be an upper bound for $\{\|g_k\|_2\}$, the existence of which follows under \cite[Assumption 1]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\bxi_k = \bxi_{\min}$ and define
\bequationNN
\balpha_{\min,k} := \frac{\beta_k \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max,k} := \frac{\beta_k \bxi_{\min} \btau_{k-1}}{\btau_{k-1}L + \Gamma}.
\eequationNN

Then, with $\kappa_d \in \R{}_{>0}$ from Lemma 3.6 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} which satisfies
$\|\bar{d}_k-d_k\| \leq \kappa_d \|\bar{g}_k-g_k\|$,
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq  (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we adopt the notation
\begin{align*}
\E_{k,1} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek1] \\
\E_{k,2} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek2] \\
\E_{k,3} &= \E_k[g_k^\top(\bd_k - d_k)|\Ek3].
\end{align*}

Now, by the Law of Total Expectation as well as the definitions of $\btau_{\min}$, $\balpha_{\min,k}$, and $\balpha_{\max,k}$, it follows that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &= \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek1] \Prob_k[\Ek1] + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek2] \\
    &\quad + \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)|\Ek2] \Prob_k[\Ek3] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad+ \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3].
\end{align*}

By Lemma 3.6, this means that
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) \E_{k,3} \Prob_k[\Ek3]
    -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3] \\
    &= -\btau_{k-1} \theta \beta_k^2 \E_{k,2} \Prob[\Ek2]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Similarly, by Lemma 3.6, we have
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{k-1} \balpha_{\max,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{k-1} \balpha_{\max,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{k-1} \balpha_{\max,k} \E_{k,3} \Prob_k[\Ek3]
    +\btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3] \\
    &= \btau_{k-1} \theta \beta_k^2 \E_{k,1} \Prob[\Ek1]
    + (\btau_{\min} \balpha_{\min,k} - \btau_{k-1} \balpha_{\max,k}) \E_{k,3} \Prob_k[\Ek3].
\end{align*}

Using the same approach a third time,
\begin{align*}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \\
    &\leq \btau_{\min} \balpha_{\min,k} \E_{k,1} \Prob_k[\Ek1]
    + \btau_{\min} \balpha_{\min,k} \E_{k,2} \Prob_k[\Ek2] \\
    &\quad + \btau_{\min} \balpha_{\min,k} \E_{k,3} \Prob_k[\Ek3]
    +(\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \\
    &= (\btau_{k-1} (\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob[\Ek1] \\
    &\quad+ (\btau_{k-1} \balpha_{\max,k} - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2].
\end{align*}

Summing these three inequalities yields

\begin{align}
    &\E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)] \nonumber \\
    &\leq \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,1} \Prob_k[\Ek1] \nonumber \\
    &\quad+(\btau_{k-1} (\balpha_{\max,k} - \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad+(2 \btau_{\min} \balpha_{\min,k} - \btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2)) \E_{k,3} \Prob_k[\Ek3]) \nonumber \\
    &= \frac13((\btau_{k-1}(\balpha_{\max,k} + 2\theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) (\E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2]) \nonumber \\
    &\quad -3 \theta \beta_k^2 \btau_{k-1} \E_{k,2} \Prob_k[\Ek2] \nonumber \\
    &\quad-(\btau_{k-1}(2\balpha_{\max,k} + \theta \beta_k^2) - 2 \btau_{\min} \balpha_{\min,k}) \E_{k,3} \Prob_k[\Ek3]). \label{eq:innerprodproof1old}
\end{align}
Now, by Assumption \ref{assum:boundedrv},
\begin{align*}
    -\E_{k,3} \Prob_k[\Ek3]
    &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek3] \Prob_k[\Ek3]  \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \|g_k\| \E_k[\|\bar{d}_k - d_k\|| \Ek3] \Prob_k[\Ek3] \\
    &\leq \kappa_g \kappa_d \E_k[\|\bar{g}_k - g_k\| | \Ek3] \Prob_k[\Ek3]  \\
    &\leq \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3] .
\end{align*}

In addition, by the Law of Total expectation, we have
\bequationNN
    \E_{k,1} \Prob_k[\Ek1] + \E_{k,2} \Prob_k[\Ek2] = \E_k[g_k^\top(\bd_k - d_k)] -\E_{k,3} \Prob_k[\Ek3] = -\E_{k,3} \Prob_k[\Ek3]
\eequationNN
as well as
\begin{align*}
    -\E_{k,2} \Prob_k [\Ek2] &= -\E_k[g_k^\top(\bar{d}_k - d_k)| \Ek2] \Prob_k [\Ek2] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek2] \\
    &= \E_k[\|g_k\| \|\bar{d}_k - d_k\|] - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek1]\Prob_k [\Ek1] \\
    &\quad - \E_k[\|g_k\| \|\bar{d}_k - d_k\| | \Ek3] \Prob_k [\Ek3] \\
    &\leq \E_k[\|g_k\| \|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \E_k[\|\bar{d}_k - d_k\|] \\
    &\leq \kappa_g \kappa_d \sqrt{M},
\end{align*}
where the last inequality follows by Lemma 3.6. Using these three inequalities with
\eqref{eq:innerprodproof1old}, yields
\begin{align*}
    \E_k[\balpha_k \btau_k g_k^\top(\bd_k - d_k)]
    &\leq (\btau_{k-1}(\balpha_{\max,k} + \theta \beta_k^2) - \btau_{\min} \balpha_{\min,k}) \kappa_g \kappa_d \kappa_{E_3} \Prob_k[\Ek3]\\
    &\quad+ \theta \beta_k^2 \btau_{k-1} \kappa_g \kappa_d \sqrt{M}.
\end{align*}
which proves the result.
\end{proof}

The above result provides an upper bound in terms of the probability that the event $\Ek3$ occurs. Due to the assumed lower bound on $\btau_k$, this event can only occur a finite number of times. To obtain our final result, we need an upper bound on the summation of the probability that $\Ek3$ occurs. The first component of this upper bound comes from the Chernoff bound.

\begin{lemma} \label{lem:chernoff}
Let $Z_0, \dotsc, Z_{k}$ be independent Bernoulli random variables and let $s \in \mathbb{N}_{>0}$.
%Let
%\begin{equation} \label{eq:lsd}
%    \ell(s,\delta) := S + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 S \log(1/\delta)}.
%\end{equation}
Then, for any $\delta \in (0, 1)$,%\todo{FEC: I suggest ``Let ... random variables for any $k \in \mathbb{N}_{\geq0}$.  Then, for any $s \in \mathbb{N}_{\geq0}$ and $\delta \in (0,1)$, ....}
\begin{equation}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s\right] \leq \delta,
\end{equation}
whenever
\begin{equation} \label{eq:lsdold}
    \sum_{i=0}^{k} \Prob[Z_i = 1] \geq \ell(s,\delta) \quad where \quad \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
\end{equation}
\end{lemma}

\begin{proof}
Denote $\mu = \sum_{i=0}^{k} \Prob[Z_i = 1]$.%\todo{FEC: In the general form, the definition of $\mu$ is in terms of expected value.  Maybe for clarity we should write $\mu = \sum_{i=0}^k E[Z_i] = \sum_{i=0}^k \Prob[Z_i = 1]$, where the latter is true only because we have Bernoulli random variables.} Then by Chernoff's bound, for any $\rho \in (0,1)$,
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq (1-\rho) \mu \right]
    \leq e^{-\mu \rho^2/2}.
\end{equation*}
Now, setting $\rho = 1 - s/\mu$ (which is in $(0,1)$ by (\ref{eq:lsd})), we have
\begin{equation*}
    \Prob\left[\sum_{i=0}^{k} Z_i \leq s \right]
    \leq e^{-\mu (1-s/\mu)^2/2}.
\end{equation*}
To prove the result, we need to show that%\todo{FEC: In the proof, you start with what we need, then work backwards to show what we want.  I'd prefer if we start with what we have (assumed in the statement) and prove that it gives what we want.  Does that make sense?}
\begin{equation*}
    e^{-\mu (1-s/\mu)^2/2} \leq \delta
\end{equation*}
holds. Therefore, we need
\begin{equation*}
    -\mu(1-s/\mu)^2/2 \leq \log(\delta)
\end{equation*}
to be satisfied. Rearranging this inequality, and using $\log(\delta) = -\log(1/\delta)$,%\todo{FEC: I don't see where the last equation comes from.  Did you scale it by $2\mu$?  I'm not seeing it.}
\begin{equation*}
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta) = \mu^2 - 2\mu (s+\log(1/\delta)) + s^2. 
\end{equation*}
Therefore, using the quadratic equation and taking the positive root,
\begin{align*}
    \mu &\geq s + \log(1/\delta) + \frac12\sqrt{4(s+\log(1/\delta))^2 - 4 s^2} \\
    &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)},
\end{align*}
which proves the result.
\end{proof}

Unfortunately, the events $\Ek3$ are not independent of each other so we can not directly apply Chernoff's bound. However, we can use this result in combination with an observation about the limited nature of the dependency between these events to prove the following result.

%IDEA: Rewrite lemma to prove that $K_stop <= k_{S,\delta}$ w.h.p. when $k_{s,\delta}$ exists. Gets rid of this whole J_i,stop nonsense

%This rewrite sucks, should just do it instance-wise.

%Essential components:
%   Independence when the leave one out sum is less than s.
%   Conclusion: w.h.p K_stop <= k_s,delta (or something similar).

%Crappy parts:
%   Conditioning on k_s,delta being well defined. Any better way to handle it? Yes if we do it instance wise. But then that notation is a bit frustrating
%   Top part is fine, gets rough as soon as we introduce E_s,delta.

\begin{lemma} \label{lem:depbernoulli}
For any $k \in \mathbb{N}_{\geq 0}$, let $Z_0, \dotsc, Z_{k}$ be Bernoulli random variables. Let $s \in \mathbb{N}_{>0}$.%\todo{FEC: Is it right to say that $Z_i$ is Bernoulli upfront?  Or should we be saying that, conditioned on ${\cal F}_i$, the random variable $Z_i$ is Bernoulli?  I guess technically it's Bernoulli in any case, since it's 0--1, but maybe we should say the condition since we always talk about conditional probabilities?}
For any $\hat{k} \in \{0,\dotsc,k\}$ and $i \in \{0,\dotsc,\hat{k}\}$, let $E_{\hat{k},i}$ be the event that $\sum_{j\leq \hat{k},j\neq i} Z_j < s$. We assume the following about the random variable $Z_i$ for each $i \in \{0,\dotsc,k\}$:
\begin{enumerate}
    \item $\Prob[Z_i = 1 | \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}] = \Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\hat{k}}]$.
    \item $\Prob[Z_i = 1| \mathcal{F}_i, E_{\hat{k},i}^c] = 0.$
\end{enumerate}
%Let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_{k}$. %and let $\bar{G}_{i}$ be measurable with respect to $\mathcal{F}_i$ for all $i \in \{-1,\dotsc,\hat{k}-1\}$.
Let $\delta \in (0,1)$ and let $\ell(s,\delta)$ be defined as in (\ref{eq:lsd}). Let $K_{s,\delta}$ be the random variable such that, for any realization of $\bar{G}_0,\dotsc,\bar{G}_{k-1}$ that is measurable with respect to $\mathcal{F}_k$,
\bequationNN
    k_{s,\delta} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta) \right\},
\eequationNN
($k_{s,\delta} = \infty$ for any realization such that $\sum_{i=0}^k \Prob[Z_i=1|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s,\delta)$ does not occur).
In addition, let $K_{stop}$ be the random variable
\bequationNN
K_{stop} := \min_{j \in \{0,\dotsc,k\}} \left\{\sum_{i=0}^{j} Z_i = s\right\},
\eequationNN
($k_{stop} = \infty$ for any realization of $Z$ such that $\sum_{i=0}^{k} z_i < s$).

We define two events:%\todo{FEC: How do these events depend on $k$?  Should we take it that $k$ is ``fixed'' in some sense, but we are considering the events for any $s$?  But shouldn't we be proving the result ``for any $k$'' as well, in which case the events should depend on $k$, too?}
\begin{enumerate}
    \item Let $E_{k,s,\delta}$ be the event that 
    $\sum_{i=0}^k \Prob[Z_i=1|\mathcal{F}_i] \geq \ell(s,\delta)$.
    \item Let $E_{k,s,\delta,stop}$ be the event that $K_{stop} > K_{s,\delta}$.
\end{enumerate}
Then,
\begin{equation*}
    \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
\end{equation*}
%We assume the following:
%\begin{enumerate}
%    \item For any $i \in \{0,\dotsc,\hat{k}\}$, let $J_{i,stop}$ be the event that $i > K_{stop}$ and  
%    \bequationNN
%    \Prob[(Z_i = 1) \cap J_{i,stop} | \mathcal{F}_i] = 0.
%    \eequationNN
%    (high level idea: once a realization of $Z$ has $s$ successes, the probability of $Z_i = 1$ is $0$.)
    %and thus $\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] = \sum_{i=0}^{K_{stop}} \Prob[Z_i = 1 | \mathcal{F}_i]$.
%the minimum integer such that $\sum_{i=0}^{k_{stop}} Z_i = s$ (set $k_{stop} = \infty$ if $\sum_{i=0}^{\hat{k}} Z_i < s$). Let $Y_i = 0$ for all $i > k_{stop}$.
%    \item For any $\bar{k} \in \{0,\dotsc,\hat{k}\}$, let $J_{\bar{k},i}$ be the event that $\sum_{j\leq \bar{k},j\neq i} Z_j < s$. Then, $\Prob[Z_i = 1| \mathcal{F}_i] = \Prob[Z_i = 1| \mathcal{F}_i, J_{\bar{k},i}, Z_0, \dotsc, Z_{i-1}, Z_{i+1}, \dotsc ,Z_{\bar{k}}]$. (high level idea: if the summation leaving out $Z_i$ does not equal $s$, then $Z_i$ is independent of all other $Z_j$.)
%\end{enumerate}

%$\Prob[Z_i = 1|\nu_i] = \Prob[Z_i = 1|\nu_i, Z_0, %\dotsc, Z_{i-1}$.
%let $\Prob[Z_i=1|\nu_i] = \Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}]$ hold unless $\sum_{j=0}^{\bar{k}} Z_j = s$ in which case $\Prob[Z_i=1|\nu_i,Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{\bar{k}}] = 0$ holds for any $i$ such that $\sum_{j\leq \bar{k}, j\neq i} Z_j = s$.
%Then, for any $\delta \in (0,1)$,
%\begin{equation}
%    \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1 | \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \geq 1 - \delta,
%\end{equation}
%where $\ell(s,\delta)$ is defined in (\ref{eq:lsd}).
\end{lemma}

\begin{proof}
    %We work with any fixed sequence $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ satisfying these conditions.
    %Note that by the definition of our filtration, it should be clear that $\Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{k-1}] = \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]$ for any $i \in \{0,\dotsc,k\}$.
    
    %We begin the proof by showing that
    %\begin{equation*}
    %    \Prob\left[ \right] \geq 1 - \delta,
    %\end{equation*}
    %holds for any fixed $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$. To prove this, we assume that $\sum_{i=0}^{\hat{k}} \Prob[Z_i| \bar{g_0}, \dotsc, \bar{g}_{i-1}] \geq \ell(s,\delta)$ (as the result is trivial otherwise).
    
    Let $E_{k,s,\delta}$ and $E_{k,s,\delta,stop}$ both occur. Then, since $E_{k,s,\delta}$ occurs, $k_{s,\delta}$ is finite. In addition, because $E_{k,s,\delta,stop}$ occurs,
    we have that
    \bequationNN
        \sum_{i=0}^{k_{s,\delta}} z_i < s.
    \eequationNN
    Therefore, for all $i \in \{0,\dotsc,k_{s,\delta}\}$, $E_{k_{s,\delta},i}$ occurs. Thus, for all $i,j \in \{0,\dotsc,k_{s,\delta}\}$, $Z_i$ and $Z_j$ were mutually independent.
    
    Due to the independence $Z$ in this case, by Lemma \ref{lem:chernoff},
    \bequationNN
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s\right] \leq \delta,
    \eequationNN
    and thus,
    \bequationNN
        \Prob[E_{k,s,\delta} \cap E_{k,s,\delta,stop} | \mathcal{F}_k] \leq \delta.
    \eequationNN
    
    Now, let $\hat{Z}_0, \dotsc, \hat{Z}_{k}$ be independent Bernoulli random variables such that $\Prob[\hat{Z}_i = 1] = \Prob[Z_i = 1|\mathcal{F}_i]$ for all $i=0,\dotsc,k$. Let $E$ be the event that $\sum_{i=0}^{k_{s,\delta}} Z_i < s$ and let $E_{k,s,\delta}$ occur. Now, for each $i=0,\dotsc,k_{s,\delta}$, it follows that if event $E$ occurs, $E_{k_{s,\delta},i}$ must occur as well, so $Z_i$ is independent of $Z_0,\dotsc,Z_{i-1},Z_{i+1},\dotsc,Z_{k_{s,\delta}}$ conditioned on the event $E$. Thus, whenever $E$ occurs, $Z_0,\dotsc,Z_{k_{s,\delta}}$ are identical in distribution to $\hat{Z}_0,\dotsc,\hat{Z}_{k_{s,\delta}}$. Therefore, by Lemma \ref{lem:chernoff},
    \begin{equation}
        \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = \Prob\left[\sum_{i=0}^{k_{s,\delta}} \hat{Z}_i < s\right] \leq
        \delta.
    \end{equation}
    It follows that
    \begin{equation*}
           \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i \geq s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] = 1 -    \Prob\left[\sum_{i=0}^{k_{s,\delta}} Z_i < s \Bigg| \bar{g_0}, \dotsc, \bar{g}_{k_{s,\delta}-1} \right] \geq 1 - \delta,
    \end{equation*}
    and thus
    \begin{equation*}
        \Prob[k_{stop} \leq k_{S,\delta}] \geq 1 - \delta.
    \end{equation*}
    In addition, by the definition of $k_{stop}$ and $J_{i,stop}$, with probability at least $1-\delta$,
    \begin{align*}
        \sum_{i=0}^{\hat{k}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}]
        &= \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq \sum_{i=0}^{k_{S,\delta}}  \Prob[Z_i = 1|\bar{g_0}, \dotsc, \bar{g}_{i-1}] \\
        &\leq 1 + \ell(s,\delta),
    \end{align*}
    and thus,
    \begin{equation*}
        \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1|\bar{g}_0, \dotsc, \bar{g}_{i-1}] \leq 1 + \ell(s,\delta) \right] \geq 1 - \delta.
    \end{equation*}
    Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i = 1| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_{\hat{k}}} \Prob\left[\sum_{i=0}^{\hat{k}} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{\hat{k}-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\hat{k}-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\hat{k}}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
\end{proof}

This setup applies to $\Ek3$ under Assumption \ref{assum:taulow} due to the definitions of $\btau$ and $\btau_{\min}$. In particular, at each iteration where $\Ek3$ occurs, $\btau_{k} \leq (1-\varepsilon)\btau_{k-1}$ holds. Therefore, if we perform this process $s$ times, until
\begin{equation*}
    \btau_{\min} \geq (1-\varepsilon)^s \btau_{-1},
\end{equation*}
it follows that $\Ek3$ cannot occur again by Assumption \ref{assum:taulow}. Thus, solving this inequality for $s$, we have
\bequation \label{eq:Stmin}
    s_{\btau_{\min}} := \left\lceil\frac{\log(\btau_{\min}/\tau_{-1})}{\log(1-\varepsilon)}\right\rceil
\eequation
which is the maximum number of times $\Ek3$ can occur.

Now we can show how to apply the above lemma to $\Ek3$.

\begin{lemma}
    Let Assumptions \ref{assum:taulow} and \ref{assum:boundedrv} hold as well as \cite[Assumptions 1 and 2]{ABerahas_FECurtis_DPRobinson_BZhou_2020}. Let $\beta_j = \beta$, $L_j = L$, and $\Gamma_j = \Gamma$ for all $j=0,\dotsc, k$. Let 
    \bequationNN
        \balpha_{\min} := \frac{\beta \bxi_{\min} \btau_{\min}}{\btau_{\min}L + \Gamma} \mbox{ and } \balpha_{\max} := \frac{\beta \bxi_{\min} \btau_{-1}}{\btau_{-1}L + \Gamma}.
    \eequationNN
    Let $\delta \in (0,1)$. Then, with probability at least $1-\delta$,
    \begin{align}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top (\bar{d}_j-d_j)]
        &\leq (\btau_{-1} (\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3}(1 + \ell(s_{\btau_{\min}},\delta))\\
    &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}, \nonumber
    \end{align}
    where
    \bequationNN
        \ell(s_{\btau_{\min}},\delta) := s_{\btau_{\min}} + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s_{\btau_{\min}} \log(1/\delta)}.
    \eequationNN
\end{lemma}

\begin{proof}
    By Lemma \ref{lem:innerprod},
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq \sum_{j=0}^k (\btau_{j-1}(\balpha_{\max,j} + \theta \beta_j^2) - \btau_{\min} \balpha_{\min,j}) \kappa_g \kappa_d \kappa_{E_3} \Prob_j[E_{j,3}]\\
        &\quad+ \theta \beta_j^2 \btau_{j-1} \kappa_g \kappa_d \sqrt{M}.
    \end{align*}
    Using our assumption on $\beta$, $L$, and $\Gamma$, we can upper bound this inequality as
    \begin{align} \label{eq:ipproof1}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} \sum_{j=0}^k \Prob_j[E_{j,3}]\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M}. \nonumber
    \end{align}
   
    To show the final result, we need to apply Lemma \ref{lem:depbernoulli}. To do this, let the event that $\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\} = \{\bar{g}_0,\dotsc,\bar{g}_{k-1}\}$ be measurable with respect to the filtration $\mathcal{F}_k$ and for all $i=0,\dotsc,k$, let $Z_i = 1$ if $E_{i,3}$ occurs and let $Z_i = 0$ otherwise. Recall that $\Prob_i[\cdot]$ is conditioned on the event $E_{\tau,low}$ occurring as well as the filtration $\mathcal{F}_i$.
    
    Now, let $s = s_{\btau_{\min}}$, so that $s$ is the maximum number of iterations in which $\Ek3$ can occur by Assumption \ref{assum:taulow}. Then, it is easy to verify that by the definition of our filtration, the probability that $\Ek3$ occurs is independent of the $E_{i,3}$ for all other $i$, whenever $\Ek3$ can occur without contradicting Assumption \ref{assum:taulow}. This holds whenever $E_{\hat{k},i}$ occurs, so that the first property of $Z_i$ in Lemma \ref{lem:depbernoulli} holds. On the other hand, when $E_{\hat{k},i}^c$ occurs it is clear that if $\Ek3$ occurs as well that Assumption \ref{assum:taulow} must be contradicted. Thus, second property of $Z_i$ in Lemma \ref{lem:depbernoulli} is satisfied as well.
    
    Now, presume that $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] \geq \ell(s_{\btau_{\min}},\delta)$. Then, by Lemma \ref{lem:depbernoulli},
    \bequationNN
        \Prob[K_{stop} \leq k_{s_{\btau_{\min}},\delta}] \geq 1 - \delta.
    \eequationNN
    In addition, by the definition of $s_{\btau_{\min}}$ and $K_{stop}$, it follows that whenever $K_{stop}$ is finite,
    \bequationNN
        \sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] =
        \sum_{i=0}^{k_{stop}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}].
    \eequationNN
    Thus, with probability at least $1 - \delta$,
     \bequationNN
        \sum_{i=0}^{k} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq \sum_{i=0}^{k_{s_{\btau_{\min}}}} \Prob[Z_i = 1 | \bar{g}_0,\dotsc,\bar{g}_{i-1}]
        \leq 1 + \ell(s_{\btau_{\min}},\delta).
    \eequationNN
    
    On the other hand, if $\sum_{i=0}^k \Prob_i[E_{i,3}|\bar{g}_0,\dotsc,\bar{g}_{i-1}] < \ell(s_{\btau_{\min}},\delta)$, it is clear that $\sum_{i=0}^{k} \Prob[E_{i,3} | \bar{g}_0,\dotsc,\bar{g}_{i-1}] \leq 1 + \ell(s_{\btau_{\min}},\delta)$. Since $\{\bar{g}_0,\dotsc,\bar{g}_{\hat{k}-1}\}$ was any sequence which was measurable with respect to the filtration $\mathcal{F}_{\hat{k}}$, by the Law of Total Probability,
    \begin{align*}
        &\Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}| \mathcal{F}_i] \leq 1 + \ell(s,\delta)\right] \\
        &=\int_{\bar{g} \in \mathcal{F}_k} \Prob\left[\sum_{i=0}^{k} \Prob[E_{i,3}|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq 1 + \ell(s,\delta) | \left\{\bar{G}_0,\dotsc,\bar{G}_{k-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{k-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
        &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_k} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta),
    \end{align*}
    where $f_{\bar{G}}(\bar{g})$ is the probability density function for $\bar{G}$ evaluated at $\bar{g}$.
    
    Combining this with (\ref{eq:ipproof1}),
    \begin{align*}
        \sum_{j=0}^k \E_j[\balpha_j \btau_j g_j^\top(\bd_j - d_j)]
        &\leq (\btau_{-1}(\balpha_{\max} + \theta \beta^2) - \btau_{\min} \balpha_{\min}) \kappa_g \kappa_d \kappa_{E_3} (1 + \ell(s_{\btau_{\min}},\delta))\\
        &\quad+ (k+1) \theta \beta^2 \btau_{-1} \kappa_g \kappa_d \sqrt{M},
    \end{align*}
    holds with probability at least $1-\delta$.
\end{proof}

\begin{theorem}
Suppose that Assumption 4 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} holds. Define 
\bequationNN
\bar{A}_{\min} := \frac{\bar{\xi}_{\min} \bar{\tau}_{\min}}{\tau_{-1}L + \gamma} \mbox{ and }
\bar{A}_{\max} := \frac{\xi_{-1} \tau_{-1}}{\bar{\tau}_{\min}L + \gamma}
\eequationNN
as well as
\bequationNN
\bar{M} := \tau_{-1} \left(\frac12 (\bar{A}_{\max} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
Let the sequence $\{\beta_k\}$ is chosen such that
\bequationNN
\beta_k = \beta := \frac{\gamma}{\sqrt{K+1}}
\eequationNN
for some
\bequationNN
\gamma \leq \min\left\{\frac{\bar{A}_{\min}}{\bar{A}_{\max} + \theta},
\frac{1}{\bar{A}_{\min}}\right\}.
\eequationNN
Then,
\begin{equation}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + c_0 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation}
\end{theorem}

\begin{proof}
Let
\bequationNN
\bar{A}_k = \frac{\bar{\xi}_{k} \bar{\tau}_{k}}{\bar{\tau_{k}}L + \gamma} \mbox{ and }
\bar{M}_k = \bar{\tau}_{k} \left(\frac12 (\bar{A}_{k} + \theta) \zeta^{-1} M + \theta \kappa_g \kappa_d \sqrt{M}\right).
\eequationNN
It follows that $\bar{A}_k \beta \leq \bar{\alpha}_k \leq (\bar{A}_k + \theta)\beta$. Using  Lemmas 3.2(d), 3.5, 3.8, and 3.9 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} (with the replacement of $\bar{\tau}_{\min}$ by $\bar{\tau}_k$), we have
\begin{align*}
    &\E_k[\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\leq \E_k [-\bar{\alpha}_k \Delta q(x_k, \bar{\tau_k}, g_k, H_k, d_k) + \frac12 \bar{\alpha}_k \beta \Delta q(x_k, \bar{\tau_k}, \bar{g}_k, H_k, \bar{d}_k) + \bar{\alpha}_k \bar{\tau}_k g_k^\top (\bar{d}_k - d_k)] \\
    &\leq -\beta(\bar{A}_k - \frac12(\bar{A}_k + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}_k \\
    &\leq -\beta(\bar{A}_{\min} - \frac12(\bar{A}_{\max} + \theta) \beta) \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M} \\
    &\leq -\frac12 \beta \bar{A}_{\min} \Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k) + \beta^2 \bar{M}
\end{align*}
Summing this inequality from $0$ to $K$,
\begin{align}
&\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \nonumber \\ 
&\leq -\frac12 \bar{A}_{\min} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)] + (K+1) \beta^2 \bar{M}. \label{eq:stochasticproof1old}
\end{align}
Now, we work with the left hand side of this inequality,
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k f(x_k + \bar{\alpha}_k \bar{d}_k) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k f_k + c_k] \\
    &= \sum_{k=0}^K \E_k [\bar{\tau}_k (f(x_k + \bar{\alpha}_k \bar{d}_k) - f_{\min}) + \|c(x_k + \bar{\alpha}_k \bar{d}_k)\|_1] - \E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k].
\end{align*}
Now, conditioned on the algorithm reaching $x_k$, it follows by the monotonicity of $\tau$
that
\bequationNN
-\E_k[\bar{\tau}_k (f_k - f_{\min}) + c_k] \geq - \E_k[\bar{\tau}_{k-1} (f_k - f_{\min}) + c_k].
\eequationNN
Therefore, summing this inequality yields
\begin{align*}
    &\sum_{k=0}^K \E_k [\phi(x_k + \bar{\alpha}_k \bar{d}_k, \bar{\tau}_k)] - \E_k[\phi(x_k,\bar{\tau}_k] \\
    &\geq \E_K [\bar{\tau}_K (f_{K+1} - f_{\min}) + \|c_K\|_1] - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 \\
    &\geq - \tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1.
\end{align*}
Using this lower bound with \eqref{eq:stochasticproof1old}
\begin{equation*}
    \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min}}.
\end{equation*}
Dividing both sides by the summation of $\beta$,
\begin{equation*}
    \frac{1}{\sum_{k=0}^K \beta} \sum_{k=0}^K \beta \E_k [\Delta q(x_k, \bar{\tau}_k, g_k, H_k, d_k)]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Now, by the definition of $x_{k^*}$, the left hand side is simply
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + (K+1) \beta^2 \bar{M})}{\bar{A}_{\min} \sum_{k=0}^K \beta}.
\end{equation*}
Using the definition of $\beta$, this becomes
\begin{equation*}
    \E [\Delta q(x_{k^*}, \bar{\tau}_{k^*}, g_{k^*}, H_{k^*}, d_{k^*})]
    \leq \frac{2 (\tau_{-1} (f_0 - f_{\min}) + \|c_0\|_1 + \gamma^2 \bar{M})}{\gamma \bar{A}_{\min} \sqrt{K+1}}.
\end{equation*}
\end{proof}

\newpage
\appendix

%*********
% Section
%*********
\section{FEC Notes}

Algorithm \ref{alg:ssqp} generates a random process
\bequationNN
  \{(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)\},
\eequationNN
where
\bitemize
  \item $\Xbar_k$ is the algorithm iterate in iteration $k$,
  \item $\Gbar_k$ is the stochastic gradient in iteration $k$,
  \item $\Dbar_k$ is the search direction in iteration $k$,
  \item $\overline\Tcal_k$ is the merit parameter in iteration $k$,
  \item $\Sbar_k$ is the number of merit parameter decreases up to the end of iteration $k$,
  \item $\overline\Xi_k$ is the ratio parameter in iteration $k$, and
  \item $\overline\Acal_k$ is the stepsize in iteration $k$.
\eitemize
A realization of $(\Xbar_k,\Gbar_k,\Dbar_k,\overline\Tcal_k,\Sbar_k,\overline\Xi_k,\overline\Acal_k)$ is denoted as
\bequationNN
  (\xbar_k,\gbar_k,\dbar_k,\bar\tau_k,\sbar_k,\bar\xi_k,\bar\alpha_k).
\eequationNN

Let $\Fcal_k$ denote the $\sigma$-algebra generated by the random variables $\{\Gbar_0,\dots,\Gbar_{k-1}\}$, the realization of which (along with $\Xbar_0 = x_0$) determines the realization of
\bequationNN
  \{\Xbar_j\}_{j=1}^k\ \ \text{and}\ \ \{(\Dbar_j,\overline\Tcal_j,\Sbar_j,\overline\Xi_j,\overline\Acal_j)\}_{j=0}^{k-1}.
\eequationNN
For completeness, let $\Fcal_{-1} = \sigma(x_0)$.  As a result, $\{\Fcal_k\}_{k\geq-1}$ is a filtration.

Let us consider a conditional model under the following assumption.
We introduce the following assumption.

\newpage

\bassumption\label{ass:FEC}
  Conditioned on the event $E := E(\kmax,\smax,\tau_{\min},\xi_{\min})$ that
  \bitemize
    \item the algorithm runs until the $(\kmax+1)$th iterate is determined,
    \item in every realization there are at most $\smax$ decreases of the merit parameter,
    \item in every realization we have $\bar\tau_k \geq \tau_{\min}$ for all $k \in \{0,\dots,\kmax\}$, and
    \item in every realization we have $\bar\xi_k = \bar\xi_{-1} = \bar\xi_{\min}$ for all $k \in \{0,\dots,\kmax\}$,
  \eitemize
  the stochastic gradients satisfy the following for all $k \in \{0,\dots,\kmax\}$:
  \bequationNN
    \baligned
      \E[\Gbar_k &| E, \Fcal_k] = \nabla f(\xbar_k), \\
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2^2 &| E, \Fcal_k] \leq M, \\ \text{and}\ \ 
      \E[\|\Gbar_k - \nabla f(\xbar_k)\|_2 &| E, \Fcal_k, \nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0, \bar\tau_k < \bar\tau_{k-1}] \leq \kappa,
    \ealigned
  \eequationNN
  where $d(\xbar_k,\nabla f(\xbar_k))$ is the step that would be computed at an iterate $\xbar_k$ if the true gradient $\nabla f(\xbar_k)$ were used in the search direction computation.
\eassumption

Going forward, let us define the binary random variable
\bequation %\label{eq:zkdef}
  Z_k = \bcases 1 & \text{if $\nabla f(\xbar_k)^\top(\dbar_k - d(\xbar_k,\nabla f(\xbar_k))) < 0$ and $\bar\tau_k < \bar\tau_{k-1}$} \\ 0 & \text{otherwise.} \ecases
\eequation
Due to the definition of the event $E$, direct consequences of Assumption~\ref{ass:FEC} are
\bequation\label{eq:probz0}
  \baligned
    \P[Z_k = 1 &| E, \Fcal_k, \Sbar_{k-1} = \smax] = 0 \\ \text{and}\ \ 
    \P[Z_k = 1 &| E, \Fcal_k, \Tbar_{k-1}(1 - \epsilon_\tau) < \tau_{\min}] = 0.
  \ealigned
\eequation

\bequationNN
  \P[Z_j = 1 | E, \Fcal_k, \Sbar_{k-1} < \smax, \Tbar_{k-1}(1 - \epsilon_\tau) \geq \tau_{\min}]\ \ \text{for $j \in \{k,\dots,\kmax\}$}
\eequationNN

Our overall goal is to prove an upper bound (in high probability) on
\bequationNN
  \sum_{k=0}^{\kmax} p_k,\ \ \text{where}\ \ p_k := \P[Z_k = 1 | E, \Fcal_k].
\eequationNN
%From total probability and \eqref{temp}:
%\bequationNN
%  \baligned
%    \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k]
%    &= \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{\kmax} < \smax] \cdot \P[\Sbar_{\kmax} < \smax | E, \Fcal_k] \\
%    &+ \sum_{k=0}^{\kmax} \P[Z_k = 1 | E, \Fcal_k, \Sbar_{\kmax} = \smax] \cdot \P[\Sbar_{\kmax} = \smax | E, \Fcal_k]
%  \ealigned
%\eequationNN

As a first step, we prove the following.

\blemma\label{lem:chernoff_new}
  For any $k \in \N{}$, let $\{Y_0,\dots,Y_k\}$ be independent Bernoulli random variables.  Then, for any $s \in \N{}_{>0}$ and $\delta \in (0,1)$, it follows that
  \bequationNN
    \mu := \sum_{j=0}^k \P[Y_j = 1] \geq \ell(s,\delta)\ \ \implies\ \ \P\left[\sum_{j=0}^k Y_j \leq s\right] \leq \delta,
  \eequationNN
  where
  \bequation\label{eq:lsd_new}
    \ell(s,\delta) := s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2 s \log(1/\delta)}.
  \eequation
\elemma
\bproof
  By the multiplicative form of Chernoff's bound, it follows for $\rho := 1 - s/\mu$ (which is in the interval $(0,1)$ by (\ref{eq:lsd_new})) that
  \bequationNN
    \P\left[\sum_{j=0}^{k} Y_j \leq s \right] \leq e^{-\frac{\mu \rho^2}{2}} = e^{-\frac{\mu (1-s/\mu)^2}{2}}.
  \eequationNN
  Hence, to prove the result, all that remains is to show that $e^{-\frac{\mu (1-s/\mu)^2}{2}} \leq \delta$, i.e.,
  \bequationNN
    -\frac{\mu(1-s/\mu)^2}{2} \leq \log(\delta)
  \eequationNN
  Using $\log(\delta) = -\log(1/\delta)$, this inequality is equivalent to
  \bequationNN
    0 \leq \frac{\mu(1-s/\mu)^2}{2} - \log(1/\delta) = \frac{(\mu - s)^2}{2\mu} - \log(1/\delta),
  \eequationNN
  which holds if and only if $\mu^2 - 2\mu (s+\log(1/\delta)) + s^2 \geq 0$.  Viewing the left-hand side of this inequality as a convex quadratic function in $\mu$, one finds that the inequality holds as long as $\mu$ is greater than or equal to the positive root of the quadratic, i.e.,
  \bequationNN
    \baligned
      \mu
        &\geq s + \log(1/\delta) + \sqrt{(s+\log(1/\delta))^2 - s^2} \\
        &= s + \log(1/\delta) + \sqrt{\log(1/\delta)^2 + 2s\log(1/\delta)}.
    \ealigned
  \eequationNN
  Since this holds under assumption in the lemma, the result is proved.
\eproof

Assumption 3.10 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} includes two key components. First, it ensures that $\tau_k = \tau_{\min}$ and $\xi_k = \xi_{\min}$ when $k$ is sufficently large. It also assumes that $\tau_k \leq \tauktri$ at each of these iterations. Assumption \ref{assum:eventE} allows us to control the effects of $\tau_k$ and $\xi_k$ decreasing in the analysis. However, it does not guarantee that $\tau_k \leq \tauktri$ holds. In order to derive a (probabilistic) bound on the number of iterations at which $\tau_k > \tauktri$ occurs, we introduce the following assumption.

\begin{assumption} %\label{assum:ptau}
At every iteration $k$,
\bequation
    \Prob[\bar{g}_k^\top \bar{d}_k + \max\{\bar{d}_k^\top H_k \bar{d}_k,0\} \geq g_k^\top d_k + \max\{d_k^\top H_k d_k,0\} | E, \mathcal{F}_k] \geq p_{\tau}.
\eequation
\end{assumption}
This assumption is satisfied with $p_{\tau}$ when $\bar{g}_k$ is drawn from a Gaussian distrbution \cite[Example 3.14]{ABerahas_FECurtis_DPRobinson_BZhou_2020}.

This assumption is leads to the following lemma.

\blemma \label{lem:Etautrial_old}
    Let Assumptions \ref{ass:FEC} and \ref{assum:ptau} hold. Let $E_{\tauktri}$ be the event that $\tauktri < \bar{\tau}_{k-1}$. Then,
    \bequation
        \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, E_{\tauktri}] \geq p_{\tau}.
    \eequation
\elemma

\bproof
    TODO: Copy proof from my notes.
\eproof

Due to the above lemma and Assumption \ref{ass:FEC}, it follows that
\bequationNN
    \Prob[E_{\tauktri} | \mathcal{F}_k, E, \bar{S}_{k-1} = \smax] = 0.
\eequationNN
In addition, by the definition of $\bar{\tau}_k$,
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, E_{\tau_{k}^{trial}}^c] = 0,
\eequationNN
so 
\bequationNN
    \Prob[\tau_{k}^{trial} < \bar{\tau}_k | \mathcal{F}_k, E, \bar{S}_{k-1} = \smax] = 0.
\eequationNN

Now, by Lemma \ref{lem:Etautrial} and the fact that $E_{\tau_{k}^{trial}}$ is not dependent on $\bar{g}_k$, it follows that
\bequation \label{eq:Etrialtaudec_old}
    \Prob[E_{\tau_{k}^{trial}} | \mathcal{F}_k, E, \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E] < p_{\tau}] = 0.
\eequation

Idea from here: Let $\bar{P}_k = \Prob[\bar{\tau}_k < \bar{\tau}_{k-1} | \mathcal{F}_k, E, \bar{S}_{k-1} < \smax]$ and let $Z_k$ be the indicator of the event that $\bar{\tau}_k < \bar{\tau}_{k-1}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{\kmax} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{\kmax + 1}} \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(\smax,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{\kmax + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}

Then, by \eqref{eq:Etrialtaudec}, with probability $1-\delta$, the number of occurrences of $E_{\tau_{k}^{trial}}$ is bounded by
\bequationNN
    |E_{\tau_{k}^{trial}}| \leq \left\lceil\frac{ \ell(\smax,\delta) + 1 }{p_{\tau}}\right\rceil.
\eequationNN
Thus, by the definition of $\bar{\tau}_k$, it follows that
\bequationNN
    |\tauktri < \bar{\tau}_k|\leq \left\lceil\frac{ \ell(\smax,\delta) + 1 }{p_{\tau}}\right\rceil. 
\eequationNN

\newpage

%*********
% Section
%*********
\section{Mike's Simpler Problem} \label{app:simple}

Let $Y_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:simple1}
  \baligned
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i < \smax\right] &= p_k \\ \text{and}\ \ 
    \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \geq \smax\right] &= 0
  \ealigned
\eequation
for some $\smax \in \{1,\dotsc,\kmax\}$, where $p_k \in [0,1]$ for all $k \in \{0,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$
\bequation \label{eq:simple2}
    \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Y_k = \smax \right].
\eequation

The following lemma proves \eqref{eq:simple2}.
\begin{lemma} \label{lem:simple1}
    Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
    \bequationNN
      \baligned
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax\right] &= p_k \\ \text{and}\ \ 
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq \smax\right] &= 0,
      \ealigned
    \eequationNN
    for some $\smax \in \{1,\dotsc,\kmax\}$, where $p_k \in (0,1]$ for all $k \in \{0,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k = \smax$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} p_k + \sum_{k=j}^{\kmax} 0 = \sum_{k=0}^{j-1} p_k.
    \end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \right] \\
        &= \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} p_k \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
    \end{align*}
    which completes the proof.
\end{proof}

The left side of this equation is similar to our goal for the actual problem, while the right is potentially easier to work with. 
A good starting point would be to try to prove a bound on
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = \smax \right]
\eequationNN
for any $\ell \in \{\smax-1,\dotsc,\kmax\}$.

It clearly follows that
\bequationNN
    \Prob\left[\sum_{k=0}^{\ell} Y_k = \smax \right] = 1 -  \Prob\left[\sum_{k=0}^{\ell} Y_k < \smax \right].
\eequationNN
We can find a lower bound on the right hand side of this equation using the following lemma.
\begin{lemma} \label{lem:simple2}
    Let $\ell \in \{\smax-1,\dotsc,\kmax\}$ and let $\hat{Y}_0,\dotsc,\hat{Y}_{\ell}$ be independent \\Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then,
    \bequationNN
        \Prob\left[\sum_{k=0}^{\ell} Y_k < \smax \right] = \Prob\left[\sum_{k=0}^{\ell} \hat{Y}_k < \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    For all $k \in \{0,\dotsc,\ell\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,\ell\}$, let
    \bequationNN 
        \bar{y}_k := \bcases
        1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < \smax \\
        0 & \textrm{otherwise},
        \ecases
    \eequationNN
    and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    \begin{align*}
        \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < \smax\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq \smax\right] &= 0
    \end{align*}
    
    Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ are equivalent in distribution to $Y_0, \dotsc, Y_{\ell}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{\ell} \hat{Y}_k < \smax$ occurs if and only if the event $\sum_{k=0}^{\ell} \bar{Y}_k < \smax$ occurs as well. Thus,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\ell} \hat{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{\ell} \bar{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{\ell} Y_k < \smax\right],
    \eequationNN
    where the last equality holds because 
    $\bar{Y}_0, \dotsc, \bar{Y}_{\ell}$ and $Y_0, \dotsc, Y_{\ell}$ are equivalent in distribution.
\end{proof}

We can use these lemmas as well as Lemma \ref{lem:chernoff_new} to get our desired bound in high probability.

\begin{lemma} \label{lem:simple3}
    Let $\smax \in \{1,\dotsc,\kmax\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,\kmax\}$, let $Y_k$ be Bernoulli random variables which satisfy \eqref{eq:simple1}, where $p_k \in (0,1]$. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{\kmax} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(\smax,\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(\smax,\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $\sum_{k=0}^{\kmax} p_k \leq \ell(\smax,\delta) + 1$. Then, by the definition of $Y_k$, it is clear that
    \bequationNN
        \sum_{k=0}^{\kmax} \Prob \left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i \right] \leq \ell(\smax,\delta) + 1
    \eequationNN
    holds deterministically, so the result is trivial in this case. Thus, for the remainder of the proof, we assume that $\sum_{k=0}^{\kmax} p_k > \ell(\smax,\delta) + 1$.
    
    Now, let $k_{\smax,\delta}$ be the minimum integer such that
    \bequationNN
        \sum_{k=0}^{k_{\smax,\delta}} p_k \geq \ell(\smax,\delta).
    \eequationNN
    Let $\hat{Y}_0,\dotsc,\hat{Y}_{k_{\smax,\delta}}$ be independent Bernoulli random variables with $\Prob[\hat{Y}_k = 1] = p_k$. Then, by Lemma \ref{lem:simple2} and Lemma \ref{lem:chernoff_new},
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax\right] = \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k < \smax\right] \leq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k \leq \smax\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{\smax,\delta}} p_k \right] &\geq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k = \smax \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{\smax,\delta}} p_k \leq \ell(\smax,\delta) + 1$.
\end{proof}

%Since the $\hat{Y}_k$ variables are independent, we can use this lemma and the CDF of the binomial distribution to get an exact description of the summation of interest. Alternatively, we can derive a bound for it by using a tail bound, such as Hoeffding's inequality or Chernoff's bound. The second option is likely to be more relevant in the more general setting of our actual algorithm.

What I'd hope a final result to look like:
\bequationNN
    \Prob\left[\sum_{k=0}^{\kmax} \Prob\Big[Z_k = 1 \Big| \mathcal{F}_{k}\Big] \leq \ell(\smax,\delta)\right] \geq 1 -\delta.
\eequationNN

Update: 2/8/2021

Let $\bar{P}_k = \Prob[Z_k=1| E, \mathcal{F}_k, \bar{S}_{k-1} < \smax]$ and let $\bar{p}_k \in [0,1]$ for all \\$k \in \{0,\dotsc,\kmax\}$. Then, by \eqref{eq:probz0} and Lemma \ref{lem:simple3}, it follows that
\bequationNN
    \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\}
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] \geq 1-\delta,
\eequationNN
holds for any $\bar{p}$ such that $\Prob\left[\left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\right] \neq 0$.
Therefore, by the law of total probability
\begin{align*}
    &\Prob\left[\sum_{k=0}^{\kmax} \Prob[Z_k = 1| E,\mathcal{F}_k] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{p} \in [0,1]^{\kmax + 1}} \Prob\Bigg[\sum_{k=0}^{\kmax} \Prob[Z_k|E,\mathcal{F}_k] \leq \ell(s,\delta) + 1 \Bigg| \left\{\bar{P}_0, \dotsc, \bar{P}_{\kmax}\right\} 
    = \left\{\bar{p}_0,\dotsc,\bar{p}_{\kmax}\right\}\Bigg] f_{\bar{P}}(\bar{p}) d\bar{p} \\
    &\geq (1 - \delta) \int_{\bar{p} \in [0,1]^{\kmax + 1}} f_{\bar{P}}(\bar{p}) d\bar{p} = (1 - \delta).
\end{align*}


Old idea:

If
\bequation \label{eq:simple3}
    \Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | E, \left\{\bar{G}_0,\dotsc,\bar{G}_{\kmax-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\kmax-1}\right\}\right] \geq 1-\delta
\eequation
holds for any $\bar{g}_0,\dotsc,\bar{g}_{\kmax}$, then we are done because:
\begin{align*}
    &\Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i = 1| \mathcal{F}_i] \leq \ell(s,\delta) + 1\right] \\
    &=\int_{\bar{g} \in \mathcal{F}_{\kmax}} \Prob\left[\sum_{i=0}^{\kmax} \Prob[Z_i|\bar{G}_0, \dotsc,\bar{G}_{i-1}] \leq \ell(s,\delta) + 1 | \left\{\bar{G}_0,\dotsc,\bar{G}_{\kmax-1}\right\} = \left\{\bar{g}_0, \dotsc, \bar{g}_{\kmax-1}\right\}\right] f_{\bar{G}}(\bar{g}) d\bar{g} \\
    &\geq (1 - \delta) \int_{\bar{g} \in \mathcal{F}_{\kmax}} f_{\bar{G}}(\bar{g}) d\bar{g} = (1 - \delta).
\end{align*}
Unfortunately, when conditioning on a realization from the filtration, we fix both the probabilities as well as whether the events occurred. Thus, the probabilities on the left side of \eqref{eq:simple3} is always 0 or 1.

%*********
% Section
%*********
\section{A Different Problem}

Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy
\bequation \label{eq:different1}
  \begin{split}
    &\Prob\Bigg[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0,\dotsc,Z_{k-1}\Bigg] \in [0,1] \\ \text{and}\ \
    &\Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i \geq \smax\right] = 0
  \end{split}
\eequation
for some $\smax \in \{1,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$
\bequation \label{eq:different2}
    \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
\eequation
We prove this inequality in the following lemma.

\begin{lemma} \label{lem:different1}
    Let $Z_k$ for $k \in \{0,\dotsc,\kmax\}$ be Bernoulli random variables which satisfy \eqref{eq:different1}, for some $\smax \in \{1,\dotsc,\kmax\}$. Then, for any $j \in \{\smax, \dotsc, \kmax\}$,
    \bequationNN
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] \right] \geq \Prob\left[\sum_{k=0}^{j-1} Z_k = \smax \right].
    \eequationNN
\end{lemma}

\begin{proof}
    Let $E_j$ be the event that $\sum_{k=0}^{j-1} Z_k \geq \smax$. Then, by the definition of $Z_k$,
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j \right] = 0, \text{ for all $k \geq j$}.
    \eequationNN
    Therefore,
    \begin{align*}
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right]
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] + \sum_{k=j}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j\right] \\
        &\leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] + \sum_{k=j}^{\kmax} 0 \\
        &= \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right].
    \end{align*}
    
    %Now, letting $E_j^c$ denote the complement of $E_j$, the definition of $Z_k$ yields
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c \right] = \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \textrm{ for all $k \leq j$.}
    %\eequationNN
    %Thus,
    %\begin{align*}
    %    \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right]
    %    &\geq \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, E_j^c\right] \\
    %    &= \sum_{k=0}^{j} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right].
    %\end{align*}
    
    Then, by the law of total probability,
    \begin{align*}
        &\Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \right] \\
        &= \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \Bigg| E_j \right] \Prob[E_j] \\
        &\quad+ \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i\right] \leq \sum_{k=0}^{j-1} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax \right] \Bigg| E_j^c \right] \Prob[E_j^c] \\
        &\geq 1 \Prob[E_j] = \Prob[E_j],
\end{align*}
which completes the proof.
\end{proof}

Next, we would like to derive an analog to Lemma \ref{lem:simple2}.
\begin{lemma} \label{lem:different2}
    Let $p \in \{\smax-1,\dotsc,\kmax\}$. Then, there exist independent Bernoulli random variables $\hat{Z}_0, \dotsc, \hat{Z}_p$ which satisfy
    \begin{align*}
        &\Prob\left[\sum_{k=0}^{p} Z_k < \smax \right] = \Prob\left[\sum_{k=0}^{p} \hat{Z}_k < \smax \right] \\
        \textrm{and } &\sum_{k=0}^p \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] = \sum_{k=0}^p \Prob\left[ \hat{Z}_k = 1\right].
    \end{align*}
\end{lemma}

\begin{proof}
    General idea: For any sequence of $\Prob\left[Z_k = 1 \Big| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right]$, there exists a fixed sequence of independent random variables that could generate this sequence in the same way that $\bar{Y}_k$ was generated in Lemma \ref{lem:simple2}. If we can get to that point, believe we can verbatim copy the rest of the proof.
    
    %To begin, note that for all $Z_0,\dotsc,Z_{\kmax}$ satisfying \eqref{eq:different1}, there exists a set of independent Bernoulli random variables 
    %$\hat{Z}_0, \dotsc, \hat{Z}_p$ such that
    %\bequationNN
    %    \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right].
    %\eequationNN

    %For all $k \in \{0,\dotsc,p\}$, let $\hat{y}_k$ be a realization of the random variable $\hat{Y}_k$. Then, for all $k \in \{0,\dotsc,p\}$, let
    %\bequationNN 
    %    \bar{y}_k := \bcases
    %    1 & \textrm{when } \hat{y}_k = 1 \textrm{ and } \sum_{i=0}^{k-1} \bar{y}_i < \smax \\
    %    0 & \textrm{otherwise},
    %    \ecases
    %\eequationNN
    %and let $\bar{Y}_k$ denote the Bernoulli random variable of which $\bar{y}_k$ is a realization. By the definition of $\hat{Y}_k$ %\todo{Not only the independence of the $\Yhat_k$ variables, but the fact that they are Bernoulli, yes?}
    %and the definition of $\bar{Y}_k$, it follows that%\todo{Like I did for the previous lemma, I would write this as a pair of conditional probabilities, not using ``cases'' that depend on a random inequality.}
    %\begin{align*}
    %    \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i < \smax\right] &= p_k \\
    %    \textrm{and } \Prob\left[\bar{Y}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Y}_i \geq \smax\right] &= 0
    %\end{align*}
    
    %Therefore, by \eqref{eq:simple1}, $\bar{Y}_0, \dotsc, \bar{Y}_{p}$ are equivalent in distribution to $Y_0, \dotsc, Y_{p}$. Now, by the definition of $\bar{Y}_k$, the event $\sum_{k=0}^{p} \hat{Y}_k < \smax$ occurs if and only if the event $\sum_{k=0}^{p} \bar{Y}_k < \smax$ occurs as well. Thus,
    %\bequationNN
    %    \Prob\left[ \sum_{k=0}^{p} \hat{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{p} \bar{Y}_k < \smax\right] = \Prob\left[ \sum_{k=0}^{p} Y_k < \smax\right],
    %\eequationNN
    %where the last equality holds because 
    %$\bar{Y}_0, \dotsc, \bar{Y}_{p}$ and $Y_0, \dotsc, Y_{p}$ are equivalent in distribution.
\end{proof}

\begin{lemma}
    Let $\smax \in \{1,\dotsc,\kmax\}$ and $\delta \in (0,1)$.
    For all $k \in \{0,\dotsc,\kmax\}$, let $Z_k$ be Bernoulli random variables which satisfy \eqref{eq:different1}. Then,
    \bequation
        \Prob\left[\sum_{k=0}^{\kmax} \Prob \left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1} \right] \leq \ell(\smax,\delta) + 1\right] \geq 1 - \delta,
    \eequation
    where $\ell(\smax,\delta)$ is defined in \eqref{eq:lsd_new}.
\end{lemma}

\begin{proof}
    Let $E$ be the event that 
    \bequationNN
        \sum_{k=0}^{\kmax} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}\right] > \ell(\smax,\delta).
    \eequationNN
    
    Then, let $K_{\smax,\delta}$ be the random variable whose realization $k_{\smax,\delta}$ is the minimum integer that satisfies
    \bequationNN
        \sum_{k=0}^{k_{\smax,\delta}} \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i, Z_0, \dotsc, Z_{k-1}, E\right] \geq \ell(\smax,\delta).
    \eequationNN

    Now, for any $Z_0,\dotsc, Z_p$ which satisfies \eqref{eq:different1} and $E$, there exist independent Bernoulli random variables $\hat{Z}_0,\dotsc,\hat{Z}_{k_{\smax},\delta}$ such that
    \bequationNN
        \Prob\left[Z_k = 1 \Bigg| \sum_{i=0}^{k-1} Z_i < \smax, E, Z_0, \dotsc, Z_{k-1}\right] = \Prob\left[\hat{Z}_k = 1\right] \textrm{ for all } k \in \{0,\dotsc,k_{\smax,\delta}\}.
    \eequationNN

    Then, let $\bar{Z}_0,\dotsc,\bar{Z}_{k_{\smax,\delta}}$ be Bernoulli random variables such that
    \begin{align*}
        \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i < \smax\right] &= p_k \\
        \textrm{and } \Prob\left[\bar{Z}_k = 1 \Bigg| \sum_{i=0}^{k-1} \bar{Z}_i \geq \smax\right] &= 0
    \end{align*}
    
    
    \bequationNN
        \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax\right] = \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k < \smax\right] \leq \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} \hat{Y}_k \leq \smax\right] \leq \delta.
    \eequationNN
    Finally, by Lemma \ref{lem:simple1},
    \begin{align*}
        \Prob\left[ \sum_{k=0}^{\kmax} \Prob\left[Y_k = 1 \Bigg| \sum_{i=0}^{k-1} Y_i\right] \leq \sum_{k=0}^{k_{\smax,\delta}} p_k \right] &= \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k = \smax \right] \\
        &= 1 - \Prob\left[\sum_{k=0}^{k_{\smax,\delta}} Y_k < \smax \right] \\
        &\geq 1 - \delta.
    \end{align*}
    The result follows by noting that $\sum_{k=0}^{k_{\smax,\delta}} p_k \leq \ell(\smax,\delta) + 1$.
\end{proof}


%DETERMINISTIC ANALYSIS BELOW
Given an objective function $f : \R{n} \rightarrow \R{}$ and a
constraint function $c : \R{n} \rightarrow \R{m}$, consider the optimization problem
\begin{equation} \label{eq:fdef}
    \underset{x \in \R{n}}{\min} \enspace f(x) \; \mbox{ s.t. } c(x)=0.
\end{equation}
Defining the Lagrangian $\ell : \R{n} \times \R{m} \rightarrow \R{}$ corresponding to \eqref{eq:fdef} by $\ell(x,y) = f(x) + c(x)^\top y$, the first-order stationarity conditions
for \eqref{eq:fdef} are given by
\begin{equation} \label{eq:1on}
    0 = \left[
    \begin{matrix}
    \nabla_x \ell(x,y) \\ \nabla_y \ell(x,y)
    \end{matrix}
    \right]
    = \left[
    \begin{matrix}
    \nabla f(x) + J(x)^T y \\ c(x)
    \end{matrix}
    \right].
\end{equation}
Letting $f_k := f(x_k)$, $g_k := \nabla f(x_k)$, $c_k := c(x_k)$, and $J_k := J(x_k) := \nabla c(x_k)^\top$ for all $k \in \mathbb{N}$ and given a sequence $\{H_k\}$ satisfying a standard type of sufficiency condition for equality constrained optimization, the SQP subproblem is given by
\begin{equation} \label{eq:sqpsubproblem}
    \underset{d \in \R{n}}{\min} f_k + g_k^\top d + \frac12 d^\top H_k d \; \mbox{ s.t. } c_k + J_k d = 0.
\end{equation}
The optimal solution $d_k$ of this subproblem, and an associated Lagrange multiplier $y_k \in \R{m}$, can be obtained by solving the linear system of equations
\begin{equation} \label{eq:sqpsystem}
    \left[
    \begin{matrix}
    H_k & J_k^\top \\
    J_k & 0
    \end{matrix}
    \right]
    \left[
    \begin{matrix}
    d_k \\ y_k
    \end{matrix}
    \right]
    = -\left[
    \begin{matrix}
    g_k \\ c_k
    \end{matrix}
    \right].
\end{equation}
At each iteration, the algorithm uses a merit function with the $\ell_1$-norm penalty function $\phi : \R{n} \times \R{}_+ \rightarrow \R{}$ defined by
\begin{equation} \label{eq:phidef}
    \phi(x,\tau) = \tau f(x) + \|c(x)\|_1
\end{equation}
where $\tau \in \R{}_+$ is a merit parameter that is updated at each iteration of the algorithm. We use a local model of the merit function $q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    q(x,\tau,\nabla f(x), H, d) = \tau (f(x) + \nabla f(x)^\top d + \frac12 \max\left\{d^\top H d,0\right\}) + \|c(x) + J(x) d\|_1.
\end{equation}
A useful quantity is the reduction in is model for a given $d \in \R{n}$ with $c(x) + J(x) d = 0$, i.e., $\delta q : \R{n} \times \R{}_+ \times \R{n} \times \mathbb{S}^n \times \R{n} \rightarrow \R{}$ defined by
\begin{equation}
    \begin{split}
    \Delta q(x,\tau,\nabla f(x), H, d) &:= q(x,\tau,\nabla f(x), H, 0) - q(x,\tau, \nabla f(x), H, d) \\
    &= -\tau (\nabla f(x)^\top d + \frac12\max\left\{d^\top H d,0\right\}) + \|c(x)\|_1.
    \end{split}
\end{equation}

For the purposes of this note, we will declare $x_k$ an approximate solution of (\ref{eq:fdef}) when
\begin{equation} \label{eq:eps1on}
    \|g_k + J_k^\top y_k\| \leq \varepsilon  \quad \mbox{ and } \quad \|c_k\| \leq \varepsilon,
\end{equation}
both hold for some $k \in \mathbb{N}$. We will derive a worst-case complexity result
in terms of the maximum number of iterations required to find a point statisfying \eqref{eq:eps1on}. We refer the reader to \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} for the
full definition of the algorithms. To prove our complexity result, we will use the following results which were proven in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}:
\begin{itemize}
    \item The merit parameter $\tau_k$ has an upper and lower bound given by $\tau_{-1} \geq \tau_k \geq \tau_{\min}$ (Lemma 2.14).
    \item The stepsize $\alpha_k$ is lower bounded by $\alpha_{\min}$ (Lemma 2.15).
    \item Let $d_k = u_k + v_k$ where $u_k \in \mbox{Null}(J_k)$ and $v_k \in \mbox{Range}(J_k^\top)$ for all $k \in \mathbb{N}$. Then, by Lemma 2.7,
    \begin{equation} \label{eq:vltc}
        \max\left\{\|v_k\|,\|v_k\|^2\right\} \leq \kappa_v \|c_k\|,
    \end{equation}
    for some $\kappa_v > 0$.
    \item Let $\kappa_{uv}$ and $\zeta$ be strictly positive scalars. Then, by Lemma 2.8,
    \begin{equation} \label{eq:dposcurve}
        \|u_k\|^2 \geq \kappa_{uv} \|v_k\|^2 \implies d_k^\top H_k d_k \geq \frac14 \zeta \|u_k\|^2.
    \end{equation}
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:deltabound}
        \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \frac12 \tau_k \max\{d_k^\top H_k d_k, 0\} + \sigma\|c_k\|_1,
    \end{equation}
    (equation 2.9 in \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020}).
    \item For all $k \in \mathbb{N}$,
    \begin{equation} \label{eq:meritdecrease}
        \phi(x_k + \alpha_k d_k, \tau_k) \leq \phi(x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k),
    \end{equation}
    (Lemma 2.12).
\end{itemize}

Armed with these results, we will prove the following lemma about sufficient decrease in the merit function whenever \eqref{eq:eps1on} does not hold.
\begin{lemma} \label{lem:suffdecrease}
Define
\begin{equation} \label{eq:kappahat}
    \hat{\kappa} := \frac{1}{\sqrt{1+\kappa_{uv}}\max\{\kappa_J,\kappa_H\}\kappa_v}
\end{equation}
and
\begin{equation} \label{eq:kappadec}
    \kappadec := \min\left\{\sigma \hat{\kappa},
    \frac18 \tau_{\min}\zeta\kappa_{uv}\kappa_v^2 \hat{\kappa}^2\right\}.
\end{equation}
Let $\varepsilon < 1$ and let at least one of $\|g_k + J_k^\top y_k\| > \varepsilon$ and/or $\|c_k\| > \varepsilon$ hold. Then,
\begin{equation} \label{eq:suffdecrease}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \varepsilon^2.
\end{equation}
\end{lemma}

\begin{proof}
To begin, assume for contradiction that
\bequationNN
\|d_k\| \leq \frac{\varepsilon}{\max\{\kappa_J,\kappa_H\}}.
\eequationNN
Then, by the definitions of $d_k$ and $y_k$ as well as $\|H_k\| \leq \kappa_H$,
\bequationNN
\|g_k + J_k^\top y_k\| = \|H_k d_k\| \leq \kappa_H \|d_k\| \leq \frac{\varepsilon \kappa_H}{\max\{\kappa_J,\kappa_H\}} \leq \varepsilon.
\eequationNN
In addition, by the definition of $d_k$ and $\|J_k\| \leq \kappa_J$,
\bequationNN
\|c_k\| = \|J_k d_k\| \leq \kappa_J \|d_k\| \leq \frac{\varepsilon \kappa_J}{\max\{\kappa_J,\kappa_H\}} \leq \varepsilon.
\eequationNN
Therefore, \eqref{eq:eps1on} holds at $k$, which is a contradiction and we must
have
\begin{equation} \label{eq:dlength}
\|d_k\| > \frac{\varepsilon}{\max\{\kappa_J,\kappa_H\}}.
\end{equation}

We consider two cases in the rest of the proof. First, let $\|c_k\| \leq \hat{\kappa} \varepsilon$. Then, by \eqref{eq:vltc} and $\|c_k\| \leq \hat{\kappa} \varepsilon$,
\bequationNN
\|v_k\|^2 \leq \kappa_v^2 \|c_k\|^2 \leq \kappa_v^2 \hat{\kappa}^2 \varepsilon^2.
\eequationNN
On the other hand, by \eqref{eq:dlength},
\begin{align*}
    \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} &< \|d_k\|^2 \\
    &= \|u_k\|^2 + \|v_k\|^2 \\
    &\leq \|u_k\|^2 + \kappa_v^2 \hat{\kappa}^2 \varepsilon^2,
\end{align*}
which implies
\begin{align*} \label{eq:ulb}
    \|u_k\|^2 &\geq \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \kappa_v^2 \hat{\kappa}^2 \varepsilon^2 \\
    &= \frac{\varepsilon^2}{\max\{\kappa_J^2,\kappa_H^2\}} - \frac{ \varepsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \frac{\kappa_{uv}\varepsilon^2}{(1+\kappa_{uv})\max\{\kappa_J^2,\kappa_H^2\}} \\
    &= \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2 \\
    &\geq \kappa_{uv} \|v_k\|^2.
\end{align*}
Thus, by \eqref{eq:dposcurve}, we have
\bequationNN
d_k^\top H_k d_k \geq \frac14 \zeta\|u_k\|^2 \geq \frac14 \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2.
\eequationNN
Therefore,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} \\
    &\geq \frac18 \tau_{\min} \zeta \kappa_{uv} \kappa_v^2 \hat{\kappa}^2 \varepsilon^2,
\end{align*}
which implies \eqref{eq:suffdecrease} in this case.

Now, presume that $\|c_k\| > \hat{\kappa} \varepsilon$ holds. Then, by \eqref{eq:deltabound} and $\varepsilon < 1$,
\begin{align*}
    \Delta q(x_k, \tau_k, g_k, H_k, d_k) &\geq \frac12 \tau_k \max\left\{ d_k^\top H_k d_k 0\right\} + \sigma \|c_k\|_1 \\
    &\geq \sigma \|c_k\|_1 \\
    &\geq \sigma \hat{\kappa} \varepsilon^2.
\end{align*}
Thus, (\ref{eq:suffdecrease}) holds in this case as well.
\end{proof}

We can use this lemma to prove the following complexity result.

\begin{theorem}
Let
\begin{equation} \label{eq:kbar}
    \bK := \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec} \varepsilon^{-2},
\end{equation}
where $\kappadec$ is defined in \eqref{eq:kappadec}.
Presume Assumptions 1 and 2 of \cite{ABerahas_FECurtis_DPRobinson_BZhou_2020} hold.
Then, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in no more than $\bK$ iterations (a similar result holds for Algorithm 2.2 with a revised definition of $\alpha_{\min}$).
\end{theorem}

\begin{proof}
Assume for contradiction that for all iterations $k = 0,1, \dotsc, \bK$, \eqref{eq:eps1on}
does not hold. Then, by Lemma \ref{lem:suffdecrease}, we have
\bequationNN
\Delta q(x_k, \tau_k, g_k, H_k, d_k) \geq \kappadec \varepsilon^2.
\eequationNN
Then, at each iteration, by \eqref{eq:meritdecrease},
\begin{align*}
    \phi (x_k + \alpha_k d_k, \tau_k) &\leq \phi (x_k, \tau_k) - \eta \alpha_k \Delta q(x_k, \tau_k, g_k, H_k, d_k) \\
    &\leq \phi(x_k, \tau_k) - \eta \alpha_{\min} \kappadec \varepsilon^2.
\end{align*}
Using the definition of $\phi$ in \eqref{eq:phidef} as well as $x_{k+1} = x_k + \alpha_k d_k$, the above inequality becomes,
\bequationNN
\tau_k f_{k+1} + \|c_{k+1}\|_1 \leq \tau_k f_k + \|c_k\|_1 - \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Summing this inequality for all iterations $k = 0,1, \dotsc, \bK$, we have
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \sum_{k=0}^{\bK} \tau_k (f_{k+1}-f_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Now, by removing the first and last term of the summation, this inequality can be rewritten
as
\bequationNN
\|c_{\bK+1}\|_1 - \|c_0\|_1 + \tau_{\bK}f_{\bK+1} - \tau_0 f_0
+ \sum_{k=1}^{\bK} f_k (\tau_{k-1} - \tau_k) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
By definition, $\tau_k$ is a decreasing sequence. Therefore, we have $\tau_{k-1} - \tau_k \geq 0$
for all $k$. Then, since $\|c_{\bK+1}\|_1 \geq 0$ and $f_k \geq \flow$ holds for all $k$, we have
\bequationNN
- \|c_0\|_1 + \tau_{\bK}\flow - \tau_0 f_0
+ \flow (\tau_{0} - \tau_{\bK}) \leq
- (\bK+1) \eta \alpha_{\min} \kappadec \varepsilon^2.
\eequationNN
Rearranging this inequality, we have
\bequationNN
\bK+1 \leq \frac{\tau_0 (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \varepsilon^2}
\leq \frac{\tau_{-1} (f_0 - \flow) + \|c_0\|_1}{\eta \alpha_{\min} \kappadec \varepsilon^2}
= \bK,
\eequationNN
which is a contradiction. Therefore, Algorithm 2.1 finds a point satisfying \eqref{eq:eps1on} in
at most $\bK$ iterations.
\end{proof}
\fi


